Elasticity Detection: A Building Block for Internet Congestion Control

This paper introduces Nimbus, a robust technique to detect whether the cross traffic competing with a flow is "elastic", and shows that this elasticity detector improves congestion control. If cross traffic is inelastic, then a sender can control queueing delays while achieving high throughput, but in the presence of elastic traffic, it may lose throughput if it attempts to control packet delay. To estimate elasticity, Nimbus modulates the flow's sending rate with sinusoidal pulses that create small traffic fluctuations at the bottleneck link, and measures the frequency response of the rate of the cross traffic. Our results on emulated and real-world paths show that congestion control using elasticity detection achieves throughput comparable to Cubic, but with delays that are 50-70 ms lower when cross traffic is inelastic. Nimbus detects the nature of the cross traffic more accurately than Copa, and is usable as a building block by other end-to-end algorithms.

==> Makefile <==
# Copyright 2004 Chris Monson (shiblon@gmail.com)
# Latest version available at http://www.bouncingchairs.net/oss
#
#    This file is part of ``Chris Monson's Free Software''.
#
#    ``Chris Monson's Free Software'' is free software; you can redistribute it
#    and/or modify it under the terms of the GNU General Public License as
#    published by the Free Software Foundation, Version 2.
#
#    ``Chris Monson's Free Software'' is distributed in the hope that it will
#    be useful, but WITHOUT ANY WARRANTY; without even the implied warranty of
#    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
#    Public License for more details.
#
#    You should have received a copy of the GNU General Public License along
#    with ``Chris Monson's Free Software''; if not, write to the Free Software
#    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA
#
#    It is also available on the web at http://www.gnu.org/copyleft/gpl.html
#
#    Note that using this makefile to build your documents does NOT place them
#    under the GPL unless you, the author, specifically do so.  In other words,
#    I, Chris Monson, the copyright holder and author of this makefile,
#    consider it impossible to ``link'' to this makefile in any way covered by
#    the GPL.
#
#
# TO OBTAIN INSTRUCTIONS FOR USING THIS FILE, RUN:
#    make help
#
fileinfo	:= LaTeX Makefile
author		:= Chris Monson
version		:= 2.2.0
#
.DEFAULT_GOAL	:= all
# Note that the user-global version is imported *after* the source directory,
# so that you can use stuff like ?= to get proper override behavior.
.PHONY: Makefile GNUmakefile Makefile.ini $(HOME)/.latex-makefile/Makefile.ini
-include Makefile.ini
-include $(HOME)/.latex-makefile/Makefile.ini
# Better names for these things
.PHONY: Variables.ini $(HOME)/.latex-makefile/Variables.ini
-include Variables.ini
-include $(HOME)/.latex-makefile/Variables.ini
#
# This can be pdflatex or latex - you can change this by adding the following line to your Makefile.ini:
# BUILD_STRATEGY := latex
BUILD_STRATEGY		?= pdflatex
#
# Sets LC_ALL=C, by default, so that the locale-aware tools, like sort, be
# # immune to changes to the locale in the user environment.
export LC_ALL		?= C
#
#
# If you specify sources here, all other files with the same suffix
# will be treated as if they were _include_ files.
#onlysources.tex	?= main.tex
#onlysources.tex.sh	?=
#onlysources.tex.pl	?=
#onlysources.tex.py	?=
#onlysources.rst	?=
#onlysources.fig	?=
#onlysources.gpi	?=
#onlysources.dot	?=
#onlysources.xvg	?=
#onlysources.svg	?=
#onlysources.eps.gz	?=
#onlysources.eps	?=
#
# If you list files here, they will be treated as _include_ files
#includes.tex		?= file1.tex file2.tex
#includes.tex.sh	?=
#includes.tex.pl	?=
#includes.tex.py	?=
#includes.rst		?=
#includes.fig		?=
#includes.gpi		?=
#includes.dot		?=
#includes.xvg		?=
#includes.svg		?=
#includes.eps.gz	?=
#includes.eps		?=
#
# If you list files or wildcards here, they will *not* be cleaned - default is
# to allow everything to be cleaned.
#neverclean		?= *.pdf
#
# Alternatively (recommended), you can add those lines to a Makefile.ini file
# and it will get picked up automatically without your having to edit this
# Makefile.
#
# KNOWN ISSUES:
# * The following occurs:
#   file with: \usepackage{named}\bibliographystyle{named}
#   Compile
#   change to: \usepackage{apalike}\bibliographystyle{apalike}
#   Compile again -- BARF!
#
#   The workaround: make clean-nographics; make
#
#   Note that we may not be able to fix this.  LaTeX itself barfs
#   on this, not the makefile.  The very first invocation of LaTeX
#   (when something like this has happened) reads the existing .aux
#   file and discovers invalid commands like \citeauthoryear that
#   are only valid in the package that was just removed.  It then
#   tries to parse them and explodes.  It's not at all clear to me
#   how to fix this.  I tried removing the .aux files on the first
#   run of LaTeX, but that necessarily requires more subsequent
#   rebuilds on common edits.  There does not appear to be a
#   graceful solution to this issue.
#
#
# CHANGES:
# Chris Monson (2011-05-20):
# * Bumped version to 2.2.0 (release!)
# Chris Monson (2011-05-19):
# * Bumped version to 2.2.0-rc15
# * Issue 125: infinite recursion with nomenclature files
# * Issue 125: removed .d as a target for .nls in get-log-index
# * Cleaned up invocation of run-makeindex to take an optional .ist instead of flags.
# Chris Monson (2011-04-06):
# * Bumped version to 2.2.0-rc14
# * Issue 121: Added Targets.ini and corresponding help text for it.
# * Issue 121: Added Variables.ini (Makefile.ini still works, though).
# * Issue 121: Added .DEFAULT_GOAL optional setting.
# * Issue 120: xindy compatibility
# Chris Monson (2011-03-16):
# * Bumped version to 2.2.0-rc13
# * Fixed a bug in kspewhich invocation - random characters and a missing pipe.
# * Added font embedding to gnuplot output.
# Chris Monson (2011-03-15):
# * Bumped version to 2.2.0-rc12
# * Issue 119: Annoying warning from which if Gnuplot not installed.
# * Fixed catchall error output to show more info from the log.  Cutting off the
#     first line is too jarring.
# * Issue 118: Better glossary support
# Chris Monson (2011-03-03):
# * Bumped version to 2.2.0-rc11
# * Issue 112: Fixed regression introduced by use of cygpath (ugly warnings)
# Chris Monson (2011-02-03):
# * Bumped version to 2.2.0-rc10
# * Issue 112: Added path normalization for cygwin systems
# * Fixed a bug in get-missing-inputs where we weren't specifying target files
# Chris Monson (2011-01-24):
# * Issue 111: Added .jpeg as a possible image extension
# Chris Monson (2011-01-21):
# * Issue 110: Long filenames not produced correctly in .d file
# * Fixed problem with unknown control sequence error parsing
# * Fixed problem with \r in fatal output (was interpreted as LF by echo)
# * Removed a spurious "hi"
# Chris Monson (2011-01-14):
# * Bumped version to 2.2.0-rc8
# * Issue 107: Removed comment with embedded newline, fixing MinGW on Windows 7.
# Chris Monson (2011-01-07):
# * Emit an error if .gpi.d files have dependencies with : in the name
# Chris Monson (2011-01-05):
# * Bumped version to 2.2.0-rc7
# * Issue 106: existing graphic dependencies not generated correctly
# Chris Monson (2011-01-04):
# * Issue 106: not cleaning eps log files properly
# * Issue 106: not rebuilding after creating .pdf graphics from .eps
# * Issue 94: svg going unnecessarily through eps (can't reproduce)
# Chris Monson (2010-12-31):
# * Issue 100: make hanging because of faulty graphics detection (sed bug)
# * Issue 108: do not ignore fatal errors from pdftex
# Chris Monson (2010-12-23):
# * Added gpi_global to gnuplot dependencies so that changes are detected
# Chris Monson (2010-12-20):
# * Updated build file to be smarter about Python version detection
# * Created a bunch of test files and supporting scripts
# * Issue 72: added apacite capaability (thanks to matkarat)
# Chris Monson (2010-11-23):
# * Changed to multi-part makefile build (split out sed scripts)
# * Added build script and supporting infrastructure
# * Updated test directory format
# * Added notes about needed test cases
# * Changed to use -file-line-error and fixed multiple inclusion/error bugs
# * Added run_sed.py to allow easy testing of sed scripts outside of make
# Chris Monson (2010-11-11):
# * Bumped version to 2.2.0-rc7
# * issue 92: broken hyperref driver detection fixed
# * issue 101: Broken inkscape conversion
# * issue 102: Broken specification of font size for gnuplot pdfcairo
# * Added KEEP_TEMP so that we can avoid deleting useful temporaries for debugging
# * Restructured gnuplot code to be easier to follow
# * Fixed a bug in convert-gpi where we were using $< instead of $1
# Chris Monson (2010-11-03):
# * Bumped version to 2.2.0-rc6
# * issue 96: Fix sed errors when using make variables in substitutions
# Chris Monson (2010-07-28):
# * Bumped version to 2.2.0-rc5 (rc4 is broken)
# * Bail out when we find the use of the import.sty package
# * Issue 90: Add -z to dvips invocation
# * Issue 67: Add xelatex support (thanks to Nikolai Prokoschenko for the patch!)
# * Issue 85: Add warning about make 3.80
# Chris Monson (2010-06-20):
# * Bumped version to 2.2.0-rc3
# * Attempt to fix bug with ! error detection (issue 88)
# * Added svg->pdf direct support (issue 89)
# Chris Monson (2010-04-28):
# * Bumped version to 2.2.0-rc2
# * Fixed %._show target
# Chris Monson (2010-04-08):
# * Bumped version to 2.2.0-rc1
# * Added back in the rst_style_file stuff that got broken when switching
#     rst -> tex to use the script mechanism
# Chris Monson (2010-03-23):
# * Bumped version to 2.2.0-beta8
# * Work on issue 76: bad backtick escape for some sed versions, failure
#     to clear out the hold buffer when outputting MISSING comment.
#     - Backed out 2>&1 to &> (doesn't work in sh)
#     - Backed out using . to source variables
# Chris Monson (2010-03-22):
# * Bumped version to 2.2.0-beta7
# * Issue 72: Fix latex/bibtex invocation order for annotated bib styles
# * Fixed informational output to reflect which LaTeX run we're on
# * Fixed graphic detection to include graphics that are already there in
#     .d files
# * Tightened up the .d file output to only make .d depend on graphic
#     *source* files.  This means that building foo.d no longer
#     builds all of the graphics files on which foo.tex depends.
#     Had to use .SECONDEXPANSION trickery to make it work.
# * Changed get-graphics to only accept a stem.
# * Fixed build-once logic for scripted .tex to work better
# * Made get-inputs sed script more maintainable.
# * Moved Makefile.ini import up higher.
# * Changed bare stems to not recursively invoke make
# * Updated diff output to be more silent everywhere
# * Added a MISSING comment to the .d file if stuff isn't found - forces
#     removal of .1st.make file, which often forces it to try again.
# * Fixed broken graphics-target function
# * Added sleep to .d file generation when stuff is missing - if it
#     builds too fast, make doesn't realize it needs to be reloaded,
#     and thus never discovers some deeper dependencies (especially
#     evident when graphics are included from scripted include
#     files).
# Chris Monson (2010-03-17):
# * Bumped version to 2.2.0-beta6
# * Fixed bareword builds to actually work (requires static patterns)
# * Fixed colorization to work with new paragraph stuff
# Chris Monson (2010-03-17):
# * Bumped version to 2.2.0-beta5
# * Fixed graphic detection to be much more focused - splits log file
#     into paragraphs before doing pattern matching.
# * Fixed make foo to work properly (recursively calls make foo.pdf)
# * Fixed gpi -> pdf generation to not waste time building .eps *after*
#     the pdf already exists.
# * Changed log copies to include MAKE_RESTARTS as part of the name.
# * Fixed missing include file detection (also makes use of the paragraph
#     stuff) to detect missing scripted include files.
# Chris Monson (2010-03-16):
# * Bumped version to 2.2.0-beta4
# * issue 70: .pdf not moved out of the way properly on first
#     compilation, resulting in early error detection failure.
# * issue 74: fixed broken error on missing .aux files: the
#     implementation was masking real errors.
# Chris Monson (2010-03-15):
# * Bumped version to 2.2.0-beta3
# * issue 71: Made the tput dependency optional
# * issue 73: Made .tex targets not pull in .d files (building them from
#     scripts should not require a .d)
# * issue 74: Output a much saner error when a .aux file is not produced
#     (e.g., when you are typing "make" without arguments in a
#     directory with included .tex files that are not named with
#     ._include_.)
# Chris Monson (2010-03-11):
# * Bumped version to 2.2.0-beta2
# * Fixed clean-graphics to get rid of intermediate .eps files that may
#     be hanging around
# * Added an automatic setting to use eps terminals in pdflatex mode for
#     gnuplot if it doesn't understand pdf.
# * issue 66: Removed grayscale generation via magic suffix.  Grayscale
#     generation is now only available via GRAY=1
# * issue 68: Added explicit handling of LC_ALL for locale-aware tools
#     like "sort"
# Chris Monson (2010-03-10):
# * Bumped version to 2.2.0-beta1
# * Fixed success message to handle output message in different places
# * Added name of produced file to success message
# Chris Monson (2010-03-10):
# * Bumped version to 2.2.0-alpha3
# * Added meaningful error message for wrong hyperref options
# * Added meaningful error message for incorrect graphics extensions
# Chris Monson (2010-03-09):
# * Bumped version to 2.2.0-alpha2
# * Updated graphics handling (gnuplot and fig generate pdf natively)
# * Changed xmgrace to output monochrome natively
# Chris Monson (2010-03-09):
# * Bumped version to 2.2.0-alpha1 - major change!
# * Support pdflatex natively and by default (issue 6 - a long time coming)
# * Add ability to have a single $HOME/.latex-makefile/Makefile.ini for
#     all invocations
# * Reworked graphic inclusion detection so that extensions need not be
#     specified for either build strategy (e.g.,
#     \includegraphics{test1.eps} -> \includegrahpics{test1})
# * Changed log format to include filenames and line numbers
# Chris Monson (2010-02-04):
# * Bumped version to 2.1.43
# * All of the following are for issue 63 (thanks to mojoh81):
# * Added documentation about fixing Makefile.ini default target
# * Added perl and python script targets
# * Fixed run logic to allow included .tex files to be scripted (the
#     run-again logic now detects missing .tex files, and the MV
#     command has been switched out for a command that only invokes
#     MV if the files exist)
# * Changed scripted generation to only run once per make invocation
# * Added dependency on expr
# Chris Monson (2010-01-19):
# * Bumped version to 2.1.42
# * issue 62: Added .brf extension to cleanable files (backrefs)
# Chris Monson (2010-01-07):
# * Bumped version to 2.1.41
# * issue 60: bad makeindex runs now error out on subsequent tries
# Chris Monson (2009-12-01):
# * Bumped version to 2.1.40
# * issue 36: build all indices (for e.g., splitidx usage)
# * issue 59: clean up all generated files (including indices)
# Chris Monson (2009-11-23):
# * Bumped version to 2.1.39
# * issue 57: change ps2pdf invocations to just use gs directly
# Chris Monson (2009-11-19):
# * Bumped version to 2.1.38
# * issue 57: Added some limited support for Cygwin (spaces in filenames)
# Chris Monson (2009-11-15):
# * Bumped version to 2.1.37
# * Removed svninfo, since this is now managed by mercurial
# * Fixed typo in changelist
# * Issue 52: added jpg->eps conversion (thanks to brubakee)
# * Issue 54: fix missing Overfull colorization due to lack of a blank
#     line preceding the first error.
# * Issue 51: remove head.tmp and body.tmp in make clean invocation
# * Issue 56: maintain multiple versions of log files (for debugging)
# Chris Monson (2009-11-14):
# * Bumped version to 2.1.36
# * Issues 53 and 49: added .brf, .mtc, and .maf to the cleanables
# Chris Monson (2009-11-05):
# * Bumped version to 2.1.35
# * Added nomenclature support (see issue 48)
# Chris Monson (2009-10-29):
# * Bumped version to 2.1.34
# * Fixed _out_ creation bug introduced in 2.1.33 (it was always created)
# * Fixed erroneous help output for $HOME in BINARY_TARGET_DIR
# * Changed contact email address - bring on the spam!
# Chris Monson (2009-10-21):
# * Bumped version to 2.1.33
# * Fixed issue 46, adding support for dot2tex (thanks to fdemesmay)
# * Made all_files.* settable in Makefile.ini (using ?= instead of :=)
# * Fixed issue 47, thanks to fdemesmay: add binary copy directory, copy
#     dvi, pdf, and ps if it exists
# Chris Monson (2009-09-25):
# * Bumped version to 2.1.32
# * Fixed so that a changed lol file will cause a rebuild
# * Added .lol files to the cleanable list
# Chris Monson (2009-09-08):
# * Bumped version to 2.1.31
# * Closed issue 43: evince doesn't notice pdf change w/out touch
# Chris Monson (2009-08-28):
# * Bumped version to 2.1.30
# * Closed issue 39: Capture multi-line log warnings/errors to output
# Chris Monson (2009-08-26):
# * Bumped version to 2.1.29
# * Closed issue 42: add svg support using inkscape
# Chris Monson (2009-08-17):
# * Bumped version to 2.1.28
# * Patch from paul.biggar for issue 38: package warnings are overlooked
# Chris Monson (2009-08-07):
# * Bumped version to 2.1.27
# * Included patch for issue 37 - removes pdf/ps files before copying,
#     allowing some broken viewers to see changes properly.
# Chris Monson (2009-05-15):
# * Bumped version to 2.1.26
# * Included patch for issue 9 from favonia - detects .fig changes for
#     pstex files during regular compilation, so long as the pstex
#     has been built at least once with make all-pstex.
# Chris Monson (2009-03-27):
# * Bumped version to 2.1.25
# * Cleaned up a bunch of variable setting stuff - more stuff is now
#     settable from Makefile.ini
# * Cleaned up documentation for various features, especially settable
#     variables.
# * issue 28: support for png -> eps conversion (it even looks good!)
# * issue 29: support for "neverclean" files in Makefile.ini
# * issue 30: make ps2pdf14 the default - fall back when not there
# Chris Monson (2009-03-09):
# * Bumped version to 2.1.24
# * issue 27: xmgrace support (thanks to rolandschulzhd)
# Chris Monson (2008-10-23):
# * Bumped version to 2.1.23
# * issue 23: fixed _check_programs to not use bash string subs
# Chris Monson (2008-09-02):
# * Bumped version to 2.1.22
# * Appled patch from Holger <yllohy@googlemail.com> to add include
#     sources and some documentation updates.
# * Updated backup_patterns to be a bit more aggressive (also thanks to
#     Holger)
# Chris Monson (2008-08-30):
# * Bumped version to 2.1.21
# * Added ability to specify onlysources.* variables to indicate the only
#     files that should *not* be considered includes.  Thanks to Holger
#     <yllohy@googlemail.com> for this patch.
# * Added an automatic include of Makefile.ini if it exists.  Allows
#     settings to be made outside of this makefile.
# Chris Monson (2008-05-21):
# * Bumped version to 2.1.20
# * Added manual pstex compilation support (run make all-pstex first)
# * Removed all automatic pstex support.  It was totally breaking
#     everything and is very hard to incorporate into the makefile
#     concept because it requires LaTeX to *fail* before it can
#     determine that it needs the files.
# Chris Monson (2008-04-17):
# * Bumped version to 2.1.19
# * Changed the pstex build hack to be on by default
# Chris Monson (2008-04-09):
# * Bumped version to 2.1.18
# * issue 16: fixed pstex build problems, seems nondeterministic.  Added
#     gratuitious hack for testing: set PSTEX_BUILD_ALL_HACK=1.
# Chris Monson (2008-04-09):
# * Bumped version to 2.1.17
# * issue 20: fixed accumulation of <pid>*.make files - wildcard was
#     refusing to work on files that are very recently created.
# Chris Monson (2008-04-02):
# * Bumped version to 2.1.16
# * issue 19: Removed the use of "type" to fix broken "echo" settings
# Chris Monson (2008-03-27):
# * Bumped version to 2.1.15
# * issue 18: Favors binary echo over builtin, as binary understands -n
# * issue 16: Fixed handling of missing pstex_t files in the log
# * issue 9: Added .SECONDARY target for .pstex files
# Chris Monson (2008-03-21):
# * Bumped version to 2.1.14
# * Fixed broken aux file flattening, which caused included bibs to be
#     missed.
# Chris Monson (2008-03-20):
# * Bumped version to 2.1.13
# * Changed error output colorization to show errors for missing files
#     that are not graphics files.
# Chris Monson (2008-03-20):
# * Bumped version to 2.1.12
# * Fixed a regression introduced in r28 that makes bibtex fail when
#     there is no index file present
# Chris Monson (2008-03-03):
# * Bumped version to 2.1.11
# * Fixed issue 11 (handle index files, reported by abachn)
# * Cleaned up some comments and help text
# Chris Monson (2008-01-24):
# * Bumped version to 2.1.10
# * Fixed to work when 'sh' is a POSIX shell like 'dash'
# Chris Monson (2007-12-12):
# * Bumped version to 2.1.9
# * Fixed documentation and dependency graph for pstex files
# Chris Monson (2007-12-12):
# * Bumped version to 2.1.8
# * Added basic pstex_t support for fig files (Issue 9 by favonia)
#     I still suggest that psfrag be used instead.
# Chris Monson (2007-10-16):
# * Bumped version to 2.1.7
# * Removed todo item: allow other comment directives for rst conversion
# * Added ability to use global rst style file _rststyle_._include_.tex
# * Added help text to that effect
# Chris Monson (2007-05-20):
# * Bumped version to 2.1.6
# * Changed default paper size for rst files
# * Added todo item: fix paper size for rst files
# * Added todo item: allow other comment directives for rst conversion
# Chris Monson (2007-04-02):
# * Bumped version to 2.1.5
# * Addressed Issue 7, incorrect .gpi.d generation in subdirectories
# Chris Monson (2007-03-28):
# * Bumped version to 2.1.4
# * Fixed syntax error in dot output
# Chris Monson (2007-03-01):
# * Bumped version to 2.1.3
# * Added reST to the included documentation
# * Fixed graphics and script generation to be settable in the
#     environment.
# Chris Monson (2007-02-23):
# * Bumped version to 2.1.2
# * Added the ability to generate .tex files from .rst files
# Chris Monson (2006-10-17):
# * Bumped version to 2.1.1
# * Fixed includes from subdirectories (sed-to-sed slash escape problem)
# Chris Monson (2006-10-05):
# * Bumped version to 2.1.0 (pretty serious new feature added)
# * New feature: bib files can now be anywhere on the BIBINPUTS path
# * New programs: kpsewhich (with tetex) and xargs (BSD)
# Chris Monson (2006-09-28):
# * Bumped version to 2.0.9
# * Added ability to parse more than one bibliography
# Chris Monson (2006-06-01):
# * Bumped version to 2.0.8
# * Added .vrb to the list of cleaned files
# Chris Monson (2006-04-26):
# * Bumped version to 2.0.7
# * Fixed so that clean-nographics does not remove .gpi.d files
# * Removed jpg -> eps hack (not working properly -- just pre-convert)
# * Fixed so that postscript grayscale can be done with BSD sed
# Chris Monson (2006-04-25):
# * Bumped version to 2.0.6
# * Fixed so that changed toc, lot, lof, or out causes a rebuild
# Chris Monson (2006-04-17):
# * Bumped version to 2.0.5
# * Added jpg -> eps conversion target
# Chris Monson (2006-04-12):
# * Bumped version to 2.0.4
# * Fixed BSD sed invocation to not use \| as a branch delimiter
# * Added a comment section on what is and is not allowed in BSD sed
# * Made paper size handling more robust while I was at it
# * Fixed postscript RGB grayscale to use a weighted average
# * Fixed postscript HSB grayscale to convert to RGB first
# * Fixed a problem with rebuilding .bbl files
# Chris Monson (2006-04-11):
# * Bumped version to 2.0.3
# * Fixed some BSD sed problems: can't use \n in substitutions
# Chris Monson (2006-04-10):
# * Bumped version to 2.0.2
# * Once again removed ability to create .tex files from scripts
# * \includeonly works again
# Chris Monson (2006-04-09):
# * Bumped version to 2.0.1
# * Fixed grayscale postscript handling to be more robust
# * Added ability to generate ._gray_. files from eps and eps.gz
# * Added ability to clean ._gray_.eps files created from .eps files
# Chris Monson (2006-04-07):
# * Bumped version to 2.0.0
# * Removed clunky ability to create included .tex files from scripts
# * Added note in the help about included tex scripting not working
# * Fixed the .eps generation to delete %.gpihead.make when finished
# * Abandoned designs to use shell variables to create sed scripts
# * Abandoned __default__.tex.sh idea: it causes recursion with %: .
# * Removed web page to-do.  All items are now complete.
# * Added better grayscale conversion for dot figures (direct ps fixup).
# * Include files can now be scripted (at the expense of \includeonly).
# * Updated dependency graph to contain better node names.
# Chris Monson (2006-04-06):
# * Bumped version to 2.0b3
# * Top level includes now fail if there is no rule to build them
# * A helpful message is printed when they do fail
# * Grayscale has been changed to be ._gray_, other phonies use _ now, too
# * Grayscale handling has been completed
# * Changed _include_stems target to _includes target.
# * Fixed _includes target to be useful by itself.
# * Removed the ability to specify clean and build targets at once
# * Verified that epsfig works fine with current code
# * Fixed included scripts so that they are added to the dep files
# * Fixed so that graphics includes don't happen if they aren't for gpi
# * Fixed dot output to allow grayscale.
# Chris Monson (2006-04-05):
# * Bumped version to 2.0b2
# * Removed automatic -gray output.  It needs fixing in a bad way.
# * Revamped dependency creation completely.
# * Fixed conditional inclusion to actually work (test.nobuild.d, test.d).
# * Fixed clean target to remove log targets
# * Added the 'monochrome' word for gray gpi output
# * Added a _check_gpi_files target that checks for common problems
# * Changed the _version target into the version target (no _)
# * Added better handling of grayscale files.  Use the .gray.pdf target.
# * Fixed testing for rebuilds
# Chris Monson (2006-04-04):
# * Bumped version to 2.0b1
# * Changed colorization of output
# * Made .auxbbl and .auxtex .make files secondary targets
# * Shortened and simplified the final latex invocation loop
# * Added version-specific output ($$i vs. $$$$i) in latex loop
# * Added a build message for the first .dvi run (Building .dvi (0))
# * Removed some build messages that most people don't care about.
# * Simplified procedure for user-set colors -- simple text specification
# * Fixed diff output to...not output.
# * Fixed rerun bug -- detect not only when preceded with LaTeX Warning
# * Sped up gpi plotting
# * Added error handling and colorized output for gpi failure
# * Documented color changing stuff.
# * Now sort the flattened aux file to avoid false recompilation needs
# * Added clean-nographics target
# * Don't remove self.dvi file if self.aux is missing in the log
# * Clarified some code.  Did some very minor adjusting.
# Chris Monson (2006-04-03):
# * Bumped version to 2.0a7
# * Added .dvi and .ps files as secondary files.
# * Fixed handling of multiple run detection when includeonly is in use.
# * Added code to flatten .aux files.
# * Added more files as .SECONDARY prerequisites to avoid recompilation.
# * Fixed the inputs generation to be much simpler and to use pipes.
# * Added the dependency graph directly into the makefile.
# * Changed flatten-aux to remove \@writefile \relax \newlabel, etc.
# * Undid pipe changes with sed usage (BSD sed doesn't know -f-).
# * Added a _check_programs target that tells you what your system has.
# * Fixed an error in colorization that made unnecessary errors appear
# * Added view targets.
# * Updated help text.
# * Augmented cookies so that .aux can trigger .bbl and .dvi rebuilds
# * Added more informative error handling for dvips and ps2pdf
# Chris Monson (2006-04-02):
# * Bumped version to 2.0a6
# * Added indirection to .bbl dependencies to avoid rebuilding .bbl files
# * Streamlined the diff invocation to eliminate an existence test
# * Removed special shell quote escape variables
# * Moved includes to a more prominent location
# * Fixed .inputs.make to not contain .aux files
# * Fixed embedding to use a file instead of always grepping.
# * Added *.make.temp to the list of cleanable files
# * Fixed Ruby.  It should now be supported properly.
# * Now differentiate between all, default, and buildable files.
# * Fixed to bail out on serious errors.
# * Revised the handling of includable files.  Still working on it.
# Chris Monson (2006-03-31):
# * Bumped version to 2.0a5
# * Fixed a bug with LaTeX error detection (there can be spaces)
# * Added .bbl support, simplifying everything and making it more correct
# * Refactored some tests that muddy the code
# * Did a little cleanup of some shell loops that can safely be make loops
# * Added support for graphviz .dot files
# * Made _all_programs output easier to read
# * Added the ruby support that has long been advertised
# * Font embedding was screwed up for PostScript -- now implicit
# * Changed the generation of -gray.gpi files to a single command
# * Changed any make-generated file that is not included from .d to .make
# Chris Monson (2006-03-30):
# * Bumped version to 2.0a4
# * Fixed a bug with very long graphics file names
# * Added a todo entry for epsfig support
# * Fixed a bug paper size bug: sometimes more than one entry appears
# * Fixed DVI build echoing to display the number instead of process ID
# * DVI files are now removed on first invocation if ANY file is missing
# * Added a simple grayscale approach: if a file ends with -gray.gpi, it
#     is created from the corresponding .gpi file with a special
#     comment ##GRAY in its header, which causes coloring to be
#     turned off.
# * Fixed a bug in the handling of .tex.sh files.  For some reason I had
#     neglected to define file stems for scripted output.
# * Removed a trailing ; from the %.graphics dependencies
# * Added dvips embedding (I think it works, anyway)
# Chris Monson (2006-03-29):
# * Bumped version to 2.0a3
# * Fixed error in make 3.79 with MAKEFILE_LIST usage
# * Added the presumed filename to the _version output
# * Added a vim macro for converting sed scripts to make commands
# * Added gpi dependency support (plotting external files and loading gpi)
# * Allow .gpi files to be ignored if called .include.gpi or .nobuild.gpi
# * Fixed sed invocations where \+ was used.  BSD sed uses \{1,\}.
# Chris Monson (2006-03-28):
# * Bumped version to 2.0a2
# * Added SHELL_DEBUG and VERBOSE options
# * Changed the default shell back to /bin/sh (unset, in other words)
# * Moved .PHONY declarations closer to their targets
# * Moved help text into its own define block to obtain better formatting
# * Removed need for double-entry when adding a new program invocation
# * Moved .SECONDARY declaration closer to its relevant occurrence
# * Commented things more heavily
# * Added help text about setting terminal and output in gnuplot
# * Created more fine-grained clean targets
# * Added a %.graphics target that generates all of %'s graphics
# * Killed backward-compatible graphics generation (e.g., eps.gpi=gpi.eps)
# * For now, we're just GPL 2, not 3.  Maybe it will change later
# * Made the version and svninfo into variables
# Chris Monson (2006-03-27):
# * Bumped version to 2.0a1
# * Huge, sweeping changes -- automatic dependencies
#

# IMPORTANT!
#
# When adding to the following list, do not introduce any blank lines.  The
# list is extracted for documentation using sed and is terminated by a blank
# line.
#
# EXTERNAL PROGRAMS:
# = ESSENTIAL PROGRAMS =
# == Basic Shell Utilities ==
CAT		?= cat
CP		?= cp -f
DIFF		?= diff
ECHO		?= echo
EGREP		?= egrep
ENV		?= env
EXPR		?= expr
MV		?= mv -f
SED		?= sed
SORT		?= sort
TOUCH		?= touch
UNIQ		?= uniq
WHICH		?= which
XARGS		?= xargs
SLEEP		?= sleep
# == LaTeX (tetex-provided) ==
BIBTEX		?= bibtex
DVIPS		?= dvips
LATEX		?= latex
PDFLATEX	?= pdflatex
XELATEX		?= xelatex
EPSTOPDF	?= epstopdf
MAKEINDEX	?= makeindex
XINDY		?= xindy
KPSEWHICH	?= kpsewhich
GS		?= gs
# = OPTIONAL PROGRAMS =
# == For MikTex under Cygwin, to get path names right
CYGPATH		?= cygpath
# == Makefile Color Output ==
TPUT		?= tput
# == TeX Generation ==
PERL		?= perl
PYTHON		?= python
RST2LATEX	?= rst2latex.py
# == EPS Generation ==
CONVERT		?= convert	# ImageMagick
DOT		?= dot		# GraphViz
DOT2TEX		?= dot2tex	# dot2tex - add options (not -o) as needed
FIG2DEV		?= fig2dev	# XFig
GNUPLOT		?= gnuplot	# GNUplot
INKSCAPE	?= inkscape	# Inkscape (svg support)
XMGRACE		?= xmgrace	# XMgrace
PNGTOPNM	?= pngtopnm	# From NetPBM - step 1 for png -> eps
PPMTOPGM	?= ppmtopgm	# From NetPBM - (gray) step 2 for png -> eps
PNMTOPS		?= pnmtops	# From NetPBM - step 3 for png -> eps
GUNZIP		?= gunzip	# GZipped EPS
# == Beamer Enlarged Output ==
PSNUP		?= psnup
# == Viewing Stuff ==
VIEW_POSTSCRIPT	?= gv
VIEW_PDF	?= xpdf
VIEW_GRAPHICS	?= display

# Xindy glossaries
XINDYLANG	?= english
XINDYENC	?= utf8

# If cygpath is present, then we create a path-norm function that uses it,
# otherwise the function is just a no-op.  Issue 112 has details.
USE_CYGPATH := $(if $(shell $(WHICH) $(CYGPATH) 2>/dev/null),yes,)

# $(call get-cygpath,<path>)
define get-cygpath
$(shell $(CYGPATH) -u "$(shell $(CYGPATH) -s -w $1)")
endef

define path-norm
$(if $(USE_CYGPATH),$(call get-cygpath,$1),$1)
endef

# Command options for embedding fonts and postscript->pdf conversion
PS_EMBED_OPTIONS	?= -dPDFSETTINGS=/printer -dEmbedAllFonts=true -dSubsetFonts=true -dMaxSubsetPct=100
PS_COMPATIBILITY	?= 1.4

# If set to something, will cause temporary files to not be deleted immediately
KEEP_TEMP	?=

# Defaults for GPI
DEFAULT_GPI_EPS_FONTSIZE	?= 22
DEFAULT_GPI_PDF_FONTSIZE	?= 12

# Style file for ReST
RST_STYLE_FILE			?= $(wildcard _rststyle_._include_.tex)

# This ensures that even when echo is a shell builtin, we still use the binary
# (the builtin doesn't always understand -n)
FIXED_ECHO	:= $(if $(findstring -n,$(shell $(ECHO) -n)),$(shell which echo),$(ECHO))
ECHO		:= $(if $(FIXED_ECHO),$(FIXED_ECHO),$(ECHO))

define determine-gnuplot-output-extension
$(if $(shell $(WHICH) $(GNUPLOT) 2>/dev/null),
     $(if $(findstring unknown or ambiguous, $(shell $(GNUPLOT) -e "set terminal pdf" 2>&1)),
	  eps, pdf),
     none)
endef

GNUPLOT_OUTPUT_EXTENSION	?= $(strip $(call determine-gnuplot-output-extension))

# Internal code should use this because of :=.  This means that the potentially
# expensive script invocation used to determine whether pdf is available will
# only be run once.
GPI_OUTPUT_EXTENSION := $(strip $(GNUPLOT_OUTPUT_EXTENSION))

# Note, if the terminal *does* understand fsize, then we expect this call to
# create a specific error here: "fsize: expecting font size".  Otherwise, we
# assume that fsize is not understood.
GPI_FSIZE_SYNTAX := $(strip \
$(if \
  $(filter pdf,$(GPI_OUTPUT_EXTENSION)),\
  $(if \
    $(findstring fsize: expecting font size,$(shell $(GNUPLOT) -e "set terminal pdf fsize" 2>&1)),\
    fsize FONTSIZE,\
    font ",FONTSIZE"),\
  FONTSIZE))

# Directory into which we place "binaries" if it exists.
# Note that this can be changed on the commandline or in Makefile.ini:
#
# Command line:
#   make BINARY_TARGET_DIR=$HOME/pdfs myfile.pdf
#
# Also, you can specify a relative directory (relative to the Makefile):
#   make BINARY_TARGET_DIR=pdfs myfile.pdf
#
# Or, you can use Makefile.ini:
#
#   BINARY_TARGET_DIR := $(HOME)/bin_out
#
BINARY_TARGET_DIR	?= _out_

RESTARTS		:= $(if $(MAKE_RESTARTS),$(MAKE_RESTARTS),0)
# SH NOTES
#
# On some systems, /bin/sh, which is the default shell, is not linked to
# /bin/bash.  While bash is supposed to be sh-compatible when invoked as sh, it
# just isn't.  This section details some of the things you have to stay away
# from to remain sh-compatible.
#
#	* File pattern expansion does not work for {}
#	* [ "$x" = "$y" ] has to be [ x"$x" x"$y" ]
#	* &> for stderr redirection doesn't work, use 2>&1 instead
#
# BSD SED NOTES
#
# BSD SED is not very nice compared to GNU sed, but it is the most
# commonly-invoked sed on Macs (being based on BSD), so we have to cater to
# it or require people to install GNU sed.  It seems like the GNU
# requirement isn't too bad since this makefile is really a GNU makefile,
# but apparently GNU sed is much less common than GNU make in general, so
# I'm supporting it here.
#
# Sad experience has taught me the following about BSD sed:
#
# 	* \+ is not understood to mean \{1,\}
# 	* \| is meaningless (does not branch)
# 	* \n cannot be used as a substitution character
# 	* ? does not mean \{0,1\}, but is literal
# 	* a\ works, but only reliably for a single line if subsequent lines
# 		have forward slashes in them (as is the case in postscript)
#
# For more info (on the Mac) you can consult
#
# man -M /usr/share/man re_format
#
# And look for the word "Obsolete" near the bottom.

#
# EXTERNAL PROGRAM DOCUMENTATION SCRIPT
#

# $(call output-all-programs,[<output file>])
define output-all-programs
	[ -f '$(this_file)' ] && \
	$(SED) \
		-e '/^[[:space:]]*#[[:space:]]*EXTERNAL PROGRAMS:/,/^$$/!d' \
		-e '/EXTERNAL PROGRAMS/d' \
		-e '/^$$/d' \
		-e '/^[[:space:]]*#/i\ '\
		-e 's/^[[:space:]]*#[[:space:]][^=]*//' \
		$(this_file) $(if $1,> '$1',) || \
	$(ECHO) "Cannot determine the name of this makefile."
endef

# If they misspell gray, it should still work.
GRAY	?= $(call get-default,$(GREY),)

#
# Utility Functions and Definitions
#

# Don't call this directly - it is here to avoid calling wildcard more than
# once in remove-files.
remove-files-helper	= $(if $1,$(RM) $1,$(sh_true))

# $(call remove-files,file1 file2)
remove-files		= $(call remove-files-helper,$(wildcard $1))

# Removes all cleanable files in the given list
# $(call clean-files,file1 file2 file3 ...)
# Works exactly like remove-files, but filters out files in $(neverclean)
clean-files		= \
	$(call remove-files-helper,$(call cleanable-files,$(wildcard $1)))

# Outputs all generated files to STDOUT, along with some others that are
# created by these (e.g., .idx files end up producing .ilg and .ind files).
# Discovered by reading *.fls OUTPUT lines and producing corresponding .ind
# filenames as needed.
#
# $(call get-generated-names,<source recorder file (*.fls)>)
define get-generated-names
[ -f '$1' ] && \
$(SED) \
	-e '/^OUTPUT /{' \
	-e '  s///' \
	-e '  p' \
	-e '  s/\.idx/\.ind/p' \
	-e '  s/\.ind/\.ilg/p' \
	-e '}' \
	-e 'd' \
	'$1' \
| $(SORT) | $(UNIQ)
endef

# This removes files without checking whether they are there or not.  This
# sometimes has to be used when the file is created by a series of shell
# commands, but there ends up being a race condition: make doesn't know about
# the file generation as quickly as the system does, so $(wildcard ...) doesn't
# work right.  Blech.
# $(call remove-temporary-files,filenames)
remove-temporary-files	= $(if $(KEEP_TEMP),:,$(if $1,$(RM) $1,:))

# Create an identifier from a file name
# $(call cleanse-filename,filename)
cleanse-filename	= $(subst .,_,$(subst /,__,$1))

# Escape dots
# $(call escape-fname-regex,str)
escape-fname-regex	= $(subst /,\\/,$(subst .,\\.,$1))

# Test that a file exists
# $(call test-exists,file)
test-exists		= [ -e '$1' ]

# $(call move-files,source,destination)
move-if-exists		= $(call test-exists,$1) && $(MV) '$1' '$2'

# Copy file1 to file2 only if file2 doesn't exist or they are different
# $(call copy-if-different,sfile,dfile)
copy-if-different	= $(call test-different,$1,$2) && $(CP) '$1' '$2'
copy-if-exists		= $(call test-exists,$1) && $(CP) '$1' '$2'
move-if-different	= $(call test-different,$1,$2) && $(MV) '$1' '$2'
replace-if-different-and-remove	= \
	$(call test-different,$1,$2) \
	&& $(MV) '$1' '$2' \
	|| $(call remove-files,'$1')

# Note that $(DIFF) returns success when the files are the SAME....
# $(call test-different,sfile,dfile)
test-different		= ! $(DIFF) -q '$1' '$2' >/dev/null 2>&1
test-exists-and-different	= \
	$(call test-exists,$2) && $(call test-different,$1,$2)

# Return value 1, or value 2 if value 1 is empty
# $(call get-default,<possibly empty arg>,<default value if empty>)
get-default	= $(if $1,$1,$2)

# Copy a file and log what's going on
# $(call copy-with-logging,<source>,<target>)
define copy-with-logging
if [ -d '$2/' ]; then \
	if $(CP) '$1' '$2/'; then \
		$(ECHO) "$(C_INFO)Copied '$1' to '$2/'$(C_RESET)"; \
	else \
		$(ECHO) "$(C_ERROR)Failed to copy '$1' to '$2/'$(C_RESET)"; \
	fi; \
fi
endef

# Gives a reassuring message about the failure to find include files
# $(call include-message,<list of include files>)
define include-message
$(strip \
$(if $(filter-out $(wildcard $1),$1),\
	$(shell $(ECHO) \
	"$(C_INFO)NOTE: You may ignore warnings about the"\
	"following files:" >&2;\
	$(ECHO) >&2; \
	$(foreach s,$(filter-out $(wildcard $1),$1),$(ECHO) '     $s' >&2;)\
	$(ECHO) "$(C_RESET)" >&2)
))
endef
# Characters that are hard to specify in certain places
space		:= $(empty) $(empty)
colon		:= \:
comma		:= ,

# Useful shell definitions
sh_true		:= :
sh_false	:= ! :

# Clear out the standard interfering make suffixes
.SUFFIXES:

# Turn off forceful rm (RM is usually mapped to rm -f)
ifdef SAFE_RM
RM	:= rm
endif

# Turn command echoing back on with VERBOSE=1
ifndef VERBOSE
QUIET	:= @
endif

# Turn on shell debugging with SHELL_DEBUG=1
# (EVERYTHING is echoed, even $(shell ...) invocations)
ifdef SHELL_DEBUG
SHELL	+= -x
endif

# Get the name of this makefile (always right in 3.80, often right in 3.79)
# This is only really used for documentation, so it isn't too serious.
ifdef MAKEFILE_LIST
this_file	:= $(word $(words $(MAKEFILE_LIST)),$(MAKEFILE_LIST))
else
this_file	:= $(wildcard GNUmakefile makefile Makefile)
endif

# Terminal color definitions

REAL_TPUT 	:= $(if $(NO_COLOR),,$(shell $(WHICH) $(TPUT)))

# $(call get-term-code,codeinfo)
# e.g.,
# $(call get-term-code,setaf 0)
get-term-code = $(if $(REAL_TPUT),$(shell $(REAL_TPUT) $1),)

black	:= $(call get-term-code,setaf 0)
red	:= $(call get-term-code,setaf 1)
green	:= $(call get-term-code,setaf 2)
yellow	:= $(call get-term-code,setaf 3)
blue	:= $(call get-term-code,setaf 4)
magenta	:= $(call get-term-code,setaf 5)
cyan	:= $(call get-term-code,setaf 6)
white	:= $(call get-term-code,setaf 7)
bold	:= $(call get-term-code,bold)
uline	:= $(call get-term-code,smul)
reset	:= $(call get-term-code,sgr0)

#
# User-settable definitions
#
LATEX_COLOR_WARNING	?= magenta
LATEX_COLOR_ERROR	?= red
LATEX_COLOR_INFO	?= green
LATEX_COLOR_UNDERFULL	?= magenta
LATEX_COLOR_OVERFULL	?= red bold
LATEX_COLOR_PAGES	?= bold
LATEX_COLOR_BUILD	?= cyan
LATEX_COLOR_GRAPHIC	?= yellow
LATEX_COLOR_DEP		?= green
LATEX_COLOR_SUCCESS	?= green bold
LATEX_COLOR_FAILURE	?= red bold

# Gets the real color from a simple textual definition like those above
# $(call get-color,ALL_CAPS_COLOR_NAME)
# e.g., $(call get-color,WARNING)
get-color	= $(subst $(space),,$(foreach c,$(LATEX_COLOR_$1),$($c)))

#
# STANDARD COLORS
#
C_WARNING	:= $(call get-color,WARNING)
C_ERROR		:= $(call get-color,ERROR)
C_INFO		:= $(call get-color,INFO)
C_UNDERFULL	:= $(call get-color,UNDERFULL)
C_OVERFULL	:= $(call get-color,OVERFULL)
C_PAGES		:= $(call get-color,PAGES)
C_BUILD		:= $(call get-color,BUILD)
C_GRAPHIC	:= $(call get-color,GRAPHIC)
C_DEP		:= $(call get-color,DEP)
C_SUCCESS	:= $(call get-color,SUCCESS)
C_FAILURE	:= $(call get-color,FAILURE)
C_RESET		:= $(reset)

#
# PRE-BUILD TESTS
#

# Check that clean targets are not combined with other targets (weird things
# happen, and it's not easy to fix them)
hascleangoals	:= $(if $(sort $(filter clean clean-%,$(MAKECMDGOALS))),1)
hasbuildgoals	:= $(if $(sort $(filter-out clean clean-%,$(MAKECMDGOALS))),1)
ifneq "$(hasbuildgoals)" ""
ifneq "$(hascleangoals)" ""
$(error $(C_ERROR)Clean and build targets specified together$(C_RESET)))
endif
endif

#
# VARIABLE DECLARATIONS
#

# Names of sed scripts that morph gnuplot files -- only the first found is used
GNUPLOT_SED	:= global-gpi.sed gnuplot.sed
GNUPLOT_GLOBAL	:= global._include_.gpi gnuplot.global

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
default_graphic_extension	?= eps
latex_build_program		?= $(LATEX)
build_target_extension		?= dvi
hyperref_driver_pattern		?= hdvips
hyperref_driver_error		?= Using dvips: specify ps2pdf in the hyperref options.
endif

ifeq "$(strip $(BUILD_STRATEGY))" "pdflatex"
default_graphic_extension	?= pdf
latex_build_program		?= $(PDFLATEX)
build_target_extension		?= pdf
hyperref_driver_pattern		?= hpdf.*
hyperref_driver_error		?= Using pdflatex: specify pdftex in the hyperref options (or leave it blank).
endif

ifeq "$(strip $(BUILD_STRATEGY))" "xelatex"
default_graphic_extension	?= pdf
latex_build_program		?= $(XELATEX)
build_target_extension		?= pdf
hyperref_driver_pattern		?= hdvipdf.*
hyperref_driver_error		?= Using pdflatex: specify pdftex in the hyperref options (or leave it blank).
endif

# Files of interest
all_files.tex		?= $(wildcard *.tex)
all_files.tex.sh	?= $(wildcard *.tex.sh)
all_files.tex.pl	?= $(wildcard *.tex.pl)
all_files.tex.py	?= $(wildcard *.tex.py)
all_files.rst		?= $(wildcard *.rst)
all_files.fig		?= $(wildcard *.fig)
all_files.gpi		?= $(wildcard *.gpi)
all_files.dot		?= $(wildcard *.dot)
all_files.xvg		?= $(wildcard *.xvg)
all_files.svg		?= $(wildcard *.svg)
all_files.png		?= $(wildcard *.png)
all_files.jpg		?= $(wildcard *.jpg)
all_files.jpeg		?= $(wildcard *.jpeg)
all_files.eps.gz	?= $(wildcard *.eps.gz)
all_files.eps		?= $(wildcard *.eps)

# Utility function for obtaining all files not specified in $(neverclean)
# $(call cleanable-files,file1 file2 file3 ...)
# Returns the list of files that is not in $(wildcard $(neverclean))
cleanable-files = $(filter-out $(wildcard $(neverclean)), $1)

# Utility function for getting all .$1 files that are to be ignored
#  * files listed in $(includes.$1)
#  * files not listed in $(onlysources.$1) if it is defined
ignore_files = \
  $(includes.$1) \
  $(if $(onlysources.$1),$(filter-out $(onlysources.$1), $(all_files.$1)))

# Patterns to never be allowed as source targets
ignore_patterns	:= %._include_

# Patterns allowed as source targets but not included in 'all' builds
nodefault_patterns := %._nobuild_ $(ignore_patterns)

# Utility function for getting targets suitable building
# $(call filter-buildable,suffix)
filter-buildable	= \
	$(filter-out $(call ignore_files,$1) \
		$(addsuffix .$1,$(ignore_patterns)),$(all_files.$1))

# Utility function for getting targets suitable for 'all' builds
# $(call filter-default,suffix)
filter-default		= \
	$(filter-out $(call ignore_files,$1) \
		$(addsuffix .$1,$(nodefault_patterns)),$(all_files.$1))

# Top level sources that can be built even when they are not by default
files.tex	:= $(call filter-buildable,tex)
files.tex.sh	:= $(call filter-buildable,tex.sh)
files.tex.pl	:= $(call filter-buildable,tex.pl)
files.tex.py	:= $(call filter-buildable,tex.py)
files.rst	:= $(call filter-buildable,rst)
files.gpi	:= $(call filter-buildable,gpi)
files.dot	:= $(call filter-buildable,dot)
files.fig	:= $(call filter-buildable,fig)
files.xvg	:= $(call filter-buildable,xvg)
files.svg	:= $(call filter-buildable,svg)
files.png	:= $(call filter-buildable,png)
files.jpg	:= $(call filter-buildable,jpg)
files.jpeg	:= $(call filter-buildable,jpeg)
files.eps.gz	:= $(call filter-buildable,eps.gz)
files.eps	:= $(call filter-buildable,eps)

# Make all pstex targets secondary.  The pstex_t target requires the pstex
# target, and nothing else really depends on it, so it often gets deleted.
# This avoids that by allowing *all* fig files to be pstex targets, which is
# perfectly valid and causes no problems even if they're going to become eps
# files in the end.
.SECONDARY:	$(patsubst %.fig,%.pstex,$(files.fig))

# Top level sources that are built by default targets
default_files.tex	:= $(call filter-default,tex)
default_files.tex.sh	:= $(call filter-default,tex.sh)
default_files.tex.pl	:= $(call filter-default,tex.pl)
default_files.tex.py	:= $(call filter-default,tex.py)
default_files.rst	:= $(call filter-default,rst)
default_files.gpi	:= $(call filter-default,gpi)
default_files.dot	:= $(call filter-default,dot)
default_files.fig	:= $(call filter-default,fig)
default_files.xvg	:= $(call filter-default,xvg)
default_files.svg	:= $(call filter-default,svg)
default_files.png	:= $(call filter-default,png)
default_files.jpg	:= $(call filter-default,jpg)
default_files.jpeg	:= $(call filter-default,jpeg)
default_files.eps.gz	:= $(call filter-default,eps.gz)
default_files.eps	:= $(call filter-default,eps)

# Utility function for creating larger lists of files
# $(call concat-files,suffixes,[prefix])
concat-files	= $(foreach s,$1,$($(if $2,$2_,)files.$s))

# Useful file groupings
all_files_source	:= $(call concat-files,tex,all)
all_files_scripts	:= $(call concat-files,tex.sh tex.pl tex.py rst,all)

.PHONY: $(all_files_scripts)

default_files_source	:= $(call concat-files,tex,default)
default_files_scripts	:= $(call concat-files,tex.sh tex.pl tex.py rst,default)

files_source	:= $(call concat-files,tex)
files_scripts	:= $(call concat-files,tex.sh tex.pl tex.py rst)

# Utility function for obtaining stems
# $(call get-stems,suffix,[prefix])
get-stems	= $(sort $($(if $2,$2_,)files.$1:%.$1=%))

# List of all stems (including ._include_ and ._nobuild_ file stems)
all_stems.tex		:= $(call get-stems,tex,all)
all_stems.tex.sh	:= $(call get-stems,tex.sh,all)
all_stems.tex.pl	:= $(call get-stems,tex.pl,all)
all_stems.tex.py	:= $(call get-stems,tex.py,all)
all_stems.rst		:= $(call get-stems,rst,all)
all_stems.fig		:= $(call get-stems,fig,all)
all_stems.gpi		:= $(call get-stems,gpi,all)
all_stems.dot		:= $(call get-stems,dot,all)
all_stems.xvg		:= $(call get-stems,xvg,all)
all_stems.svg		:= $(call get-stems,svg,all)
all_stems.png		:= $(call get-stems,png,all)
all_stems.jpg		:= $(call get-stems,jpg,all)
all_stems.jpeg		:= $(call get-stems,jpeg,all)
all_stems.eps.gz	:= $(call get-stems,eps.gz,all)
all_stems.eps		:= $(call get-stems,eps,all)

# List of all default stems (all default PDF targets):
default_stems.tex		:= $(call get-stems,tex,default)
default_stems.tex.sh		:= $(call get-stems,tex.sh,default)
default_stems.tex.pl		:= $(call get-stems,tex.pl,default)
default_stems.tex.py		:= $(call get-stems,tex.py,default)
default_stems.rst		:= $(call get-stems,rst,default)
default_stems.fig		:= $(call get-stems,fig,default)
default_stems.gpi		:= $(call get-stems,gpi,default)
default_stems.dot		:= $(call get-stems,dot,default)
default_stems.xvg		:= $(call get-stems,xvg,default)
default_stems.svg		:= $(call get-stems,svg,default)
default_stems.png		:= $(call get-stems,png,default)
default_stems.jpg		:= $(call get-stems,jpg,default)
default_stems.jpeg		:= $(call get-stems,jpeg,default)
default_stems.eps.gz		:= $(call get-stems,eps.gz,default)
default_stems.eps		:= $(call get-stems,eps,default)

# List of all stems (all possible bare PDF targets created here):
stems.tex		:= $(call get-stems,tex)
stems.tex.sh		:= $(call get-stems,tex.sh)
stems.tex.pl		:= $(call get-stems,tex.pl)
stems.tex.py		:= $(call get-stems,tex.py)
stems.rst		:= $(call get-stems,rst)
stems.fig		:= $(call get-stems,fig)
stems.gpi		:= $(call get-stems,gpi)
stems.dot		:= $(call get-stems,dot)
stems.xvg		:= $(call get-stems,xvg)
stems.svg		:= $(call get-stems,svg)
stems.png		:= $(call get-stems,png)
stems.jpg		:= $(call get-stems,jpg)
stems.jpeg		:= $(call get-stems,jpeg)
stems.eps.gz		:= $(call get-stems,eps.gz)
stems.eps		:= $(call get-stems,eps)

# Utility function for creating larger lists of stems
# $(call concat-stems,suffixes,[prefix])
concat-stems	= $(sort $(foreach s,$1,$($(if $2,$2_,)stems.$s)))

# The most likely to be source but not finished product go first
graphic_source_extensions	:= fig \
				   gpi \
				   xvg \
				   svg \
				   dot \
				   eps.gz

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
graphic_source_extensions	+= png jpg jpeg
graphic_target_extensions	:= eps ps
endif

ifeq "$(strip $(BUILD_STRATEGY))" "pdflatex"
graphic_source_extensions	+= eps
graphic_target_extensions	:= pdf png jpg jpeg mps tif
endif

ifeq "$(strip $(BUILD_STRATEGY))" "xelatex"
graphic_source_extensions	+= eps
graphic_target_extensions	:= pdf png jpg jpeg mps tif
endif

all_stems_source	:= $(call concat-stems,tex,all)
all_stems_script	:= $(call concat-stems,tex.sh tex.pl tex.py rst,all)
all_stems_graphic	:= $(call concat-stems,$(graphic_source_extensions),all)
all_stems_ss		:= $(sort $(all_stems_source) $(all_stems_script))
all_stems_sg		:= $(sort $(all_stems_script))
all_stems_ssg		:= $(sort $(all_stems_ss))

default_stems_source	:= $(call concat-stems,tex,default)
default_stems_script	:= $(call concat-stems,tex.sh tex.pl tex.py rst,default)
default_stems_ss	:= $(sort $(default_stems_source) $(default_stems_script))
default_stems_sg	:= $(sort $(default_stems_script))
default_stems_ssg	:= $(sort $(default_stems_ss))

stems_source		:= $(call concat-stems,tex)
stems_script		:= $(call concat-stems,tex.sh tex.pl tex.py rst)
stems_graphic		:= $(call concat-stems,$(graphic_source_extensions))
stems_gg		:= $(sort $(stems_graphic))
stems_ss		:= $(sort $(stems_source) $(stems_script))
stems_sg		:= $(sort $(stems_script))
stems_ssg		:= $(sort $(stems_ss))

# Calculate names that can generate the need for an include file.  We can't
# really do this with patterns because it's too easy to screw up, so we create
# an exhaustive list.
allowed_source_suffixes	:= \
	pdf \
	ps \
	dvi \
	ind \
	nls \
	bbl \
	aux \
	aux.make \
	d \
	auxbbl.make \
	_graphics \
	_show
allowed_source_patterns		:= $(addprefix %.,$(allowed_source_suffixes))

allowed_graphic_suffixes	:= \
	pdf \
	eps \
	gpihead.make \
	gpi.d
allowed_graphic_patterns	:= $(addprefix %.,$(allowed_graphic_suffixes))

# All targets allowed to build documents
allowed_source_targets	:= \
	$(foreach suff,$(allowed_source_suffixes),\
	$(addsuffix .$(suff),$(stems_ssg)))

# All targets allowed to build graphics
allowed_graphic_targets	:= \
	$(foreach suff,$(allowed_graphic_suffixes),\
	$(addsuffix .$(suff),$(stems_gg)))

# All targets that build multiple documents (like 'all')
allowed_batch_source_targets	:= \
	all \
	all-pdf \
	all-ps \
	all-dvi \
	all-bbl \
	all-ind \
	all-gls \
	all-nls \
	show

# All targets that build multiple graphics (independent of document)
allowed_batch_graphic_targets	:= \
	all-graphics \
	all-pstex \
	all-dot2tex \
	show-graphics

# Now we figure out which stuff is available as a make target for THIS RUN.
real_goals	:= $(call get-default,$(filter-out _includes,$(MAKECMDGOALS)),\
			all)

specified_source_targets	:= $(strip \
	$(filter $(allowed_source_targets) $(stems_ssg),$(real_goals)) \
	)

specified_batch_source_targets	:= $(strip \
	$(filter $(allowed_batch_source_targets),$(real_goals)) \
	)

specified_graphic_targets	:= $(strip \
	$(filter $(allowed_graphic_targets),$(real_goals)) \
	)

specified_batch_graphic_targets	:= $(strip \
	$(filter $(allowed_batch_graphic_targets),$(real_goals)) \
	)

specified_gpi_targets	:= $(patsubst %.gpi,%.$(default_graphic_extension),\
	$(filter $(patsubst %.$(default_graphic_extension),%.gpi,$(specified_graphic_targets)),\
		$(all_files.gpi)) \
	)

# Determine which .d files need including from the information gained above.
# This is done by first checking whether a batch target exists.  If it does,
# then all *default* stems are used to create possible includes (nobuild need
# not apply for batch status).  If no batch targets exist, then the individual
# targets are considered and appropriate includes are taken from them.
source_stems_to_include	:= \
	$(sort\
	$(if $(specified_batch_source_targets),\
		$(default_stems_ss),\
		$(foreach t,$(specified_source_targets),\
		$(foreach p,$(allowed_source_patterns),\
			$(patsubst $p,%,$(filter $p $(stems_ssg),$t)) \
		)) \
	))

# Determine which .gpi.d files are needed using the above information.  We
# first check whether a batch target is specified, then check individual
# graphics that may have been specified.
graphic_stems_to_include	:= \
	$(sort\
	$(if $(specified_batch_graphic_targets),\
		$(default_stems.gpi),\
		$(foreach t,$(specified_gpi_targets),\
		$(foreach p,$(allowed_graphic_patterns),\
			$(patsubst $p,%,$(filter $p,$t)) \
		)) \
	))

# All dependencies for the 'all' targets
all_pdf_targets		:= $(addsuffix .pdf,$(stems_ssg))
all_ps_targets		:= $(addsuffix .ps,$(stems_ssg))
all_dvi_targets		:= $(addsuffix .dvi,$(stems_ssg))
all_tex_targets		:= $(addsuffix .tex,$(stems_sg))
all_d_targets		:= $(addsuffix .d,$(stems_ssg))
all_graphics_targets	:= $(addsuffix .$(default_graphic_extension),$(stems_gg))
all_pstex_targets	:= $(addsuffix .pstex_t,$(stems.fig))
all_dot2tex_targets	:= $(addsuffix .dot_t,$(stems.dot))

all_known_graphics	:= $(sort $(all_graphics_targets) $(wildcard *.$(default_graphic_extension)))

default_pdf_targets	:= $(addsuffix .pdf,$(default_stems_ss))

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
default_ps_targets	:= $(addsuffix .ps,$(default_stems_ss))
default_dvi_targets	:= $(addsuffix .dvi,$(default_stems_ss))
pre_pdf_extensions	:= dvi ps
endif

# Extensions generated by LaTeX invocation that can be removed when complete
rm_ext		:= \
	log *.log aux $(pre_pdf_extensions) pdf blg bbl out nav snm toc lof lot lol pfg \
	fls vrb idx ind ilg glg glo gls lox nls nlo nlg brf mtc maf brf ist
backup_patterns	:= *~ *.bak *.backup body.tmp head.tmp

graph_stem	:= _graph

# All LaTeX-generated files that can be safely removed

rm_tex := \
	$(foreach e,$(rm_ext),$(addsuffix .$e,$(all_stems_source))) \
	$(foreach e,$(rm_ext) tex,$(addsuffix .$e,$(all_stems_sg))) \
	$(addsuffix .log,$(all_ps_targets) $(all_pdf_targets)) \
	$(addsuffix .*.log,$(stems_graphic))

# These are the files that will affect .gpi transformation for all .gpi files.
#
# Use only the first one found.  Backward compatible values are at the end.
# Note that we use foreach, even though wildcard also returns a list, to ensure
# that the order in the uppercase variables is preserved.  Directory listings
# provide no such guarantee, so we avoid relying on them.
gpi_sed		:= $(strip \
	$(firstword $(foreach f,$(GNUPLOT_SED),$(wildcard $f))))
gpi_global	:= $(strip \
	$(firstword $(foreach f,$(GNUPLOT_GLOBAL),$(wildcard $f))))

#
# Functions used in generating output
#

# Outputs all source dependencies to stdout.  The first argument is the file to
# be parsed, the second is a list of files that will show up as dependencies in
# the new .d file created here.
#
# $(call get-inputs,<parsed file>,<target files>)
define get-inputs
$(SED) \
-e '/^INPUT/!d' \
-e 's!^INPUT \(\./\)\{0,1\}!!' \
-e 's/[[:space:]]/\\ /g' \
-e 's/\(.*\)\.aux$$/\1.tex/' \
-e '/\.tex$$/b addtargets' \
-e '/\.cls$$/b addtargets' \
-e '/\.sty$$/b addtargets' \
-e '/\.pstex_t$$/b addtargets' \
-e '/\.dot_t$$/b addtargets' \
-e 'd' \
-e ':addtargets' \
-e 's!.*!$2: $$(call path-norm,&)!' \
'$1' | $(SORT) | $(UNIQ)
endef

# $(call get-missing-inputs,<log file>,<target files>)
define get-missing-inputs
$(SED) \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\(\n\)\(.*\)/\2\1/' \
-e '}' \
-e '/^::P\(P\{1,\}\)::/{' \
-e '  s//::\1::/' \
-e '  G' \
-e '  h' \
-e '  d' \
-e '}' \
-e '/^::P::/{' \
-e '  s//::0::/' \
-e '  G' \
-e '}' \
-e 'b start' \
-e ':needonemore' \
-e 's/^/::P::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needtwomore' \
-e 's/^/::PP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needthreemore' \
-e 's/^/::PPP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':start' \
-e '/^! LaTeX Error: File `/{' \
-e '  b needtwomore' \
-e '}' \
-e '/^::0::\(.*\)/{' \
-e '  s//\1/' \
-e '  /Default extension: /!d' \
-e '  s/.*File `\([^'"'"']*\)'"'"' not found.*/\1/' \
-e '  s/[[:cntrl:]]//' \
-e '  /\.tex/!s/$$/.tex/' \
-e '  s/[[:space:]]/\\ /g' \
-e '  h' \
-e '  s/.*/# MISSING input "&" - (presence of comment affects build)/' \
-e '  p' \
-e '  s/.*//' \
-e '  x' \
-e '  s!^.*!$2: $$(call path-norm,&)!' \
-e '  p' \
-e '}' \
-e 'd' \
'$1' | $(SORT) | $(UNIQ)
endef

# Get source file for specified graphics stem.
#
# $(call graphics-source,<stem>)
define graphics-source
$(strip $(firstword \
	$(wildcard \
		$(addprefix $1.,\
			$(graphic_source_extensions))) \
	$1 \
))
endef

# Get the target file for the specified graphics file/stem
#
# $(call graphics-target,<stem>)
define graphics-target
$(strip $(if 	$(filter $(addprefix %.,$(graphic_target_extensions)),$1), $1,
	$(firstword $(patsubst $(addprefix %.,$(graphic_source_extensions) $(graphic_target_extensions)), %, $1).$(default_graphic_extension) $1.$(default_graphic_extension))))
endef

# Outputs all of the graphical dependencies to stdout.  The first argument is
# the stem of the source file being built, the second is a list of suffixes
# that will show up as dependencies in the generated .d file.
#
# Note that we try to escape spaces in filenames where possible.  We have to do
# it with three backslashes so that as the name percolates through the makefile
# it eventually ends up with the proper escaping when the build rule is found.
# Ugly, but it appears to work.  Note that graphicx doesn't allow filenames
# with spaces, so this could in many ways be moot unless you're using something
# like grffile.
#
# For pdflatex, we really need the missing file to be specified without an
# extension, otherwise compilation barfs on the first missing file.  Truly
# annoying, but there you have it.
#
# It turns out that the graphics errors, although they have lines with empty
# space, are only made of two paragraphs.  So, we just use some sed magic to
# get everything into paragraphs, detect when it's a paragraph that interests
# us, and double it up.  Then we get the filename only if we're missing
# extensions (a sign that it's graphicx complaining).
#
# $(call get-graphics,<target file stem>)
#.log,$(addprefix $*.,d $(build_target_extension) _graphics)
define get-graphics
$(SED) \
-e '/^File: \(.*\) Graphic file (type [^)]*)/{' \
-e '  s//\1/' \
-e '  b addtargets' \
-e '}' \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\(\n\)\(.*\)/\2\1/' \
-e '}' \
-e '/^::P\(P\{1,\}\)::/{' \
-e '  s//::\1::/' \
-e '  G' \
-e '  h' \
-e '  d' \
-e '}' \
-e '/^::P::/{' \
-e '  s//::0::/' \
-e '  G' \
-e '}' \
-e 'b start' \
-e ':needonemore' \
-e 's/^/::P::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needtwomore' \
-e 's/^/::PP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needthreemore' \
-e 's/^/::PPP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':start' \
-e '/^[^[:cntrl:]:]*:[[:digit:]]\{1,\}: LaTeX Error: File `/{' \
-e '  s/\n//g' \
-e '  b needonemore' \
-e '}' \
-e '/^::0::.*: LaTeX Error: File `/{' \
-e '  /\n\n$$/{' \
-e '    s/^::0:://' \
-e '    b needonemore' \
-e '  }' \
-e '  s/\n\{1,\}/ /g' \
-e '  s/[[:space:]]\{1,\}/ /g' \
-e '  s/^.*File `//' \
-e '  s/'"'"' not found\..*extensions: \([^[:space:]]*\).*/::::\1/' \
-e '  h' \
-e '  s/\(.*\)::::\(.*\)/# MISSING stem "\1" - allowed extensions are "\2" - leave comment here - it affects the build/' \
-e '  p' \
-e '  g' \
-e '  s/::::.*//' \
-e '  b addtargets' \
-e '}' \
-e 'd' \
-e ':addtargets' \
-e 's/[[:space:]]/\\\\\\&/g' \
-e 'h' \
-e 's/.*/-include &.gpi.d/' \
-e 'p' \
-e 'g' \
-e 's!.*!$1.d: $$$$(call graphics-source,&)!' \
-e 'p' \
-e 's/.*//' \
-e 'x' \
-e 's!.*!$1.$(build_target_extension) $1._graphics: $$$$(call graphics-target,&)!' \
-e 'p' \
-e 'd' \
$1.log
endef

# Checks for build failure due to pstex inclusion, and gives instructions.
#
# $(call die-on-pstexs,<parsed file>)
define die-on-pstexs
if $(EGREP) -q '^! LaTeX Error: File .*\.pstex.* not found' $1; then \
	$(ECHO) "$(C_ERROR)Missing pstex_t file(s)$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)Please run$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)  make all-pstex$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)before proceeding.$(C_RESET)"; \
	exit 1; \
fi
endef

# Checks for the use of import.sty and bails - we don't support subdirectories
#
# $(call die-on-import-sty,<log file>)
define die-on-import-sty
if $(EGREP) -s '/import.sty\)' '$1'; then \
	$(ECHO) "$(C_ERROR)import.sty is not supported - included files must"; \
	$(ECHO) "$(C_ERROR)be in the same directory as the primary document$(C_RESET)"; \
	exit 1; \
fi
endef

# Checks for build failure due to dot2tex, and gives instructions.
#
# $(call die-on-dot2tex,<parsed file>)
define die-on-dot2tex
if $(EGREP) -q ' LaTeX Error: File .*\.dot_t.* not found' $1; then \
	$(ECHO) "$(C_ERROR)Missing dot_t file(s)$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)Please run$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)  make all-dot2tex$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)before proceeding.$(C_RESET)"; \
	exit 1; \
fi
endef

# Checks for the existence of a .aux file, and dies with an error message if it
# isn't there.  Note that we pass the file stem in, not the full filename,
# e.g., to check for foo.aux, we call it thus: $(call die-on-no-aux,foo)
#
# $(call die-on-no-aux,<aux stem>)
define die-on-no-aux
if [ ! -e '$1.aux' ]; then \
	$(call colorize-latex-errors,$1.log); \
	$(ECHO) "$(C_ERROR)Error: failed to create $1.aux$(C_RESET)"; \
	exit 1; \
fi
endef

# Outputs all index files to stdout.  Arg 1 is the source file stem, arg 2 is
# the list of targets for the discovered dependency.
#
# $(call get-log-index,<log file stem>,<target files>)
define get-log-index
$(SED) \
-e 's/^No file \(.*\.ind\)\.$$/TARGETS=\1/' \
-e 's/^No file \(.*\.[gn]ls\)\.$$/TARGETS=\1/' \
-e 's/[[:space:]]/\\&/g' \
-e '/^TARGETS=/{' \
-e '  h' \
-e '  s!^TARGETS=!$2: !p' \
-e '  g' \
-e '  s!^TARGETS=\(.*\)!\1: $1.tex!p' \
-e '}' \
-e 'd' \
'$1.log' | $(SORT) | $(UNIQ)
endef


# Outputs all bibliography files to stdout.  Arg 1 is the source stem, arg 2 is
# a list of targets for each dependency found.
#
# The script kills all lines that do not contain bibdata.  Remaining lines have
# the \bibdata macro and delimiters removed to create a dependency list.  A
# trailing comma is added, then all adjacent commas are collapsed into a single
# comma.  Then commas are replaced with the string .bib[space], and the
# trailing space is killed off.  Finally, all filename spaces are escaped.
# This produces a list of space-delimited .bib filenames, which is what the
# make dep file expects to see.
#
# Note that we give kpsewhich a bogus argument so that a failure of sed to
# produce output will not cause an error.
#
# $(call get-bibs,<aux file>,<targets>)
define get-bibs
$(SED) \
-e '/^\\bibdata/!d' \
-e 's/\\bibdata{\([^}]*\)}/\1,/' \
-e 's/,\{2,\}/,/g' \
-e 's/[[:space:]]/\\&/g' \
-e 's/,/.bib /g' \
-e 's/ \{1,\}$$//' \
$1 | $(XARGS) $(KPSEWHICH) '#######' | \
$(SED) \
-e 's!^!$2: !' | \
$(SORT) | $(UNIQ)
endef

# Makes a an aux file that only has stuff relevant to the target in it
# $(call make-auxtarget-file,<flattened-aux>,<new-aux>)
define make-auxtarget-file
$(SED) \
-e '/^\\newlabel/!d' \
$1 > $2
endef

# Makes an aux file that only has stuff relevant to the bbl in it
# $(call make-auxbbl-file,<flattened-aux>,<new-aux>)
define make-auxbbl-file
$(SED) \
-e '/^\\newlabel/d' \
$1 > $2
endef

# Makes a .gpi.d file from a .gpi file
# $(call make-gpi-d,<.gpi>,<.gpi.d>)
define make-gpi-d
$(ECHO) '# vim: ft=make' > $2; \
$(ECHO) 'ifndef INCLUDED_$(call cleanse-filename,$2)' >> $2; \
$(ECHO) 'INCLUDED_$(call cleanse-filename,$2) := 1' >> $2; \
$(call get-gpi-deps,$1,$(addprefix $(2:%.gpi.d=%).,$(GPI_OUTPUT_EXTENSION) gpi.d)) >> $2; \
$(ECHO) 'endif' >> $2;
endef

# Parse .gpi files for data and loaded dependencies, output to stdout
#
# The sed script here tries to be clever about obtaining valid
# filenames from the gpi file.  It assumes that the plot command starts its own
# line, which is not too difficult a constraint to satisfy.
#
# This command script also generates 'include' directives for every 'load'
# command in the .gpi file.  The load command must appear on a line by itself
# and the file it loads must have the suffix .gpi.  If you don't want it to be
# compiled when running make graphics, then give it a suffix of ._include_.gpi.
#
# $(call get-gpi-deps,<gpi file>,<targets>)
define get-gpi-deps
$(SED) \
-e '/^[[:space:]]*s\{0,1\}plot/,/[^\\]$$/{' \
-e ' H' \
-e ' /[^\\]$$/{' \
-e '  s/.*//' \
-e '  x' \
-e '  s/\\\{0,1\}\n//g' \
-e '  s/^[[:space:]]*s\{0,1\}plot[[:space:]]*\(\[[^]]*\][[:space:]]*\)*/,/' \
-e '  s/[[:space:]]*\(['"'"'\'"'"''"'"'"][^'"'"'\'"'"''"'"'"]*['"'"'\'"'"''"'"'"]\)\{0,1\}[^,]*/\1/g' \
-e '  s/,['"'"'\'"'"''"'"'"]-\{0,1\}['"'"'\'"'"''"'"'"]//g' \
-e '  s/[,'"'"'\'"'"''"'"'"]\{1,\}/ /g' \
-e '  s/.*:.*/$$(error Error: Filenames with colons are not allowed: &)/' \
-e '  s!.*!$2: &!' \
-e '  p' \
-e ' }' \
-e ' d' \
-e '}' \
-e 's/^[[:space:]]*load[[:space:]]*['"'"'\'"'"''"'"'"]\([^'"'"'\'"'"''"'"'"]*\.gpi\)['"'"'\'"'"''"'"'"].*$$/-include \1.d/p' \
-e 'd' \
'$1'
endef

# Colorizes real, honest-to-goodness LaTeX errors that can't be overcome with
# recompilation.
#
# Note that we only ignore file not found errors for things that we know how to
# build, like graphics files.
#
# Also note that the output of this is piped through sed again to escape any
# backslashes that might have made it through.  This is to avoid sending things
# like "\right" to echo, which interprets \r as LF.  In bash, we could just do
# ${var//\\/\\\\}, but in other popular sh variants (like dash), this doesn't
# work.
#
# $(call colorize-latex-errors,<log file>)
define colorize-latex-errors
$(SED) \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\(\n\)\(.*\)/\2\1/' \
-e '}' \
-e '/^::P\(P\{1,\}\)::/{' \
-e '  s//::\1::/' \
-e '  G' \
-e '  h' \
-e '  d' \
-e '}' \
-e '/^::P::/{' \
-e '  s//::0::/' \
-e '  G' \
-e '}' \
-e 'b start' \
-e ':needonemore' \
-e 's/^/::P::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needtwomore' \
-e 's/^/::PP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needthreemore' \
-e 's/^/::PPP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':start' \
-e '/^! LaTeX Error: File /{' \
-e '  s/\n//g' \
-e '  b needtwomore' \
-e '}' \
-e 's/^[^[:cntrl:]:]*:[[:digit:]]\{1,\}:/!!! &/' \
-e 's/^\(.*\n\)\([^[:cntrl:]:]*:[[:digit:]]\{1,\}: .*\)/\1!!! \2/' \
-e '/^!!! .* LaTeX Error: File /{' \
-e '  s/\n//g' \
-e '  b needonemore' \
-e '}' \
-e '/^::0::! LaTeX Error: File .*/{' \
-e '  /\n\n$$/{' \
-e '    s/^::0:://' \
-e '    b needonemore' \
-e '  }' \
-e '  s/^::0::! //' \
-e '  s/^\(.*not found.\).*Enter file name:.*\n\(.*[[:digit:]]\{1,\}\): Emergency stop.*/\2: \1/' \
-e '  b error' \
-e '}' \
-e '/^::0::!!! .*LaTeX Error: File .*/{' \
-e '  /\n\n$$/{' \
-e '    s/^::0:://' \
-e '    b needonemore' \
-e '  }' \
-e '  s/::0::!!! //' \
-e '  /could not locate.*any of these extensions:/{' \
-e '    d' \
-e '  }' \
-e '  s/\(not found\.\).*/\1/' \
-e '  b error' \
-e '}' \
-e '/^\(.* LaTeX Error: Missing .begin.document.\.\).*/{' \
-e '  s//\1 --- Are you trying to build an include file?/' \
-e '  b error' \
-e '}' \
-e '/.*\(!!! .*Undefined control sequence\)[^[:cntrl:]]*\(.*\)/{' \
-e '  s//\1: \2/' \
-e '  s/\nl\.[[:digit:]][^[:cntrl:]]*\(\\[^\\[:cntrl:]]*\).*/\1/' \
-e '  b error' \
-e '}' \
-e '/^\(!pdfTeX error:.*\)s*/{' \
-e '  b error' \
-e '}' \
-e '/.*\(!!! .*\)/{' \
-e '  s//\1/' \
-e '  s/[[:cntrl:]]//' \
-e '  s/[[:cntrl:]]$$//' \
-e '  b error' \
-e '}' \
-e 'd' \
-e ':error' \
-e 's/^!\(!! \)\{0,1\}\(.*\)/$(C_ERROR)\2$(C_RESET)/' \
-e 'p' \
-e 'd' \
'$1' | $(SED) -e 's/\\\\/\\\\\\\\/g'
endef

# Colorize Makeindex errors
define colorize-makeindex-errors
$(SED) \
-e '/^!! /{' \
-e '  N' \
-e '  s/^.*$$/$(C_ERROR)&$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
'$1'
endef

# Colorize xindy errors
# $(call colorize-xindy-errors,<log file>)
define colorize-xindy-errors
$(SED) \
-e 's/^xindy:.*/$(C_ERROR)&$(C_RESET)/p' \
-e 'd' \
'$1'
endef

# Colorize epstopdf errors
#
# $(call colorize-epstopdf-errors,<log file>)
define colorize-epstopdf-errors
$(SED) \
-e '/^Error:/,/^Execution stack:/{' \
-e '  /^Execution stack:/d' \
-e '  s/.*/$(C_ERROR)&$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
'$1'
endef

# Colorize GNUplot errors
#
# $(call colorize-gnuplot-errors,<log file>)
define colorize-gnuplot-errors
$(SED) \
-e '/, line [0-9]*:/!{' \
-e '  H' \
-e '  x' \
-e '  s/.*\n\(.*\n.*\)$$/\1/' \
-e '  x' \
-e '}' \
-e '/, line [0-9]*:/{' \
-e '  H' \
-e '  /unknown.*terminal type/{' \
-e '    s/.*/--- Try changing the GNUPLOT_OUTPUT_EXTENSION variable to '"'"'eps'"'"'./' \
-e '    H' \
-e '  }' \
-e '  /gpihead/{' \
-e '    s/.*/--- This could be a Makefile bug - contact the maintainer./' \
-e '    H' \
-e '  }' \
-e '  g' \
-e '  s/.*/$(C_ERROR)&$(C_RESET)/' \
-e '  p' \
-e '}' \
-e '/^gnuplot>/,/^$$/{' \
-e '  s/^gnuplot.*/$(C_ERROR)&/' \
-e '  s/^$$/$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
$1
endef

# Colorize GraphViz errors
#
# $(call colorize-dot-errors,<log file>)
define colorize-dot-errors
$(SED) \
-e 's/.*not found.*/$(C_ERROR)&$(C_RESET)/p' \
-e '/^Error:/,/context:/s/.*/$(C_ERROR)&$(C_RESET)/p' \
-e 's/^Warning:.*/$(C_WARNING)&$(C_RESET)/p' \
-e 'd' \
'$1'
endef

# Get all important .aux files from the top-level .aux file and merges them all
# into a single file, which it outputs to stdout.
#
# $(call flatten-aux,<toplevel aux>,<output file>)
define flatten-aux
$(SED) \
-e '/\\@input{\(.*\)}/{' \
-e     's//\1/' \
-e     's![.:]!\\&!g' \
-e     'h' \
-e     's!.*!\\:\\\\@input{&}:{!' \
-e     'p' \
-e     'x' \
-e     's/\\././g' \
-e     's/.*/r &/p' \
-e     's/.*/d/p' \
-e     's/.*/}/p' \
-e     'd' \
-e '}' \
-e 'd' \
'$1' > "$1.$$$$.sed.make"; \
$(SED) -f "$1.$$$$.sed.make" '$1' > "$1.$$$$.make"; \
$(SED) \
-e '/^\\relax/d' \
-e '/^\\bibcite/d' \
-e 's/^\(\\newlabel{[^}]\{1,\}}\).*/\1/' \
"$1.$$$$.make" | $(SORT) > '$2'; \
$(call remove-temporary-files,$1.$$$$.make $1.$$$$.sed.make)
endef

# Generate pdf from postscript
#
# Note that we don't just call ps2pdf, since there are so many versions of that
# script on various systems.  Instead, we call the postscript interpreter
# directly.
#
# $(call ps2pdf,infile,outfile,[embed fonts])
define ps2pdf
	$(GS) \
		-dSAFER -dCompatibilityLevel=$(PS_COMPATIBILITY) \
		$(if $3,$(PS_EMBED_OPTIONS)) \
		-q -dNOPAUSE -dBATCH \
		-sDEVICE=pdfwrite -sstdout=%stderr \
		'-sOutputFile=$2' \
		-dSAFER -dCompatibilityLevel=$(PS_COMPATIBILITY) \
		$(if $3,$(PS_EMBED_OPTIONS)) \
		-c .setpdfwrite \
		-f '$1'
endef

# Colorize LaTeX output.
color_tex := \
$(SED) \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\n//' \
-e '  /Output written on /{' \
-e '    s/.*Output written on \([^(]*\) (\([^)]\{1,\}\)).*/Success!  Wrote \2 to \1/' \
-e '    s/[[:digit:]]\{1,\}/$(C_PAGES)&$(C_RESET)/g' \
-e '    s/Success!/$(C_SUCCESS)&$(C_RESET)/g' \
-e '    s/to \(.*\)$$/to $(C_SUCCESS)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  / *LaTeX Error:.*/{' \
-e '    s/.*\( *LaTeX Error:.*\)/$(C_ERROR)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  /.*Warning:.*/{' \
-e '    s//$(C_WARNING)&$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  /Underfull.*/{' \
-e '    s/.*\(Underfull.*\)/$(C_UNDERFULL)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  /Overfull.*/{' \
-e '    s/.*\(Overfull.*\)/$(C_OVERFULL)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  d' \
-e '  :end' \
-e '  G' \
-e '}'

# Colorize BibTeX output.
color_bib := \
$(SED) \
-e 's/^Warning--.*/$(C_WARNING)&$(C_RESET)/' \
-e 't' \
-e '/---/,/^.[^:]/{' \
-e '  H' \
-e '  /^.[^:]/{' \
-e '    x' \
-e '    s/\n\(.*\)/$(C_ERROR)\1$(C_RESET)/' \
-e '    p' \
-e '    s/.*//' \
-e '    h' \
-e '    d' \
-e '  }' \
-e '  d' \
-e '}' \
-e '/(.*error.*)/s//$(C_ERROR)&$(C_RESET)/' \
-e 'd'

# Make beamer output big enough to print on a full page.  Landscape doesn't
# seem to work correctly.
enlarge_beamer	= $(PSNUP) -l -1 -W128mm -H96mm -pletter

# $(call test-run-again,<source stem>)
test-run-again	= $(EGREP) -q '^(.*Rerun .*|No file $1\.[^.]+\.)$$' $1.log

# This tests whether the build target commands should be run at all, from
# viewing the log file.
# $(call test-log-for-need-to-run,<source stem>)
define test-log-for-need-to-run
$(SED) \
-e '/^No file $(call escape-fname-regex,$1)\.aux\./d' \
$1.log \
| $(EGREP) -q '^(.*Rerun .*|No file $1\.[^.]+\.|No file .+\.tex\.|LaTeX Warning: File.*)$$'
endef

# LaTeX invocations
#
# $(call latex,<tex file>,[<extra LaTeX args>])
run-latex	= $(latex_build_program) -interaction=batchmode -file-line-error $(if $2,$2,) $1 > /dev/null

# $(call latex-color-log,<LaTeX stem>)
latex-color-log	= $(color_tex) $1.log

# $(call run-makeindex,<input>,<output>,<log>,[.ist style file])
define run-makeindex
success=1; \
if ! $(MAKEINDEX) -q $1 -t $3 -o $2 $(if $4,-s $4,) > /dev/null || $(EGREP) -q '^!!' $3; \
then \
	$(call colorize-makeindex-errors,$3); \
	$(RM) -f '$2'; \
	success=0; \
fi; \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef


# $(call run-xindy,<input>,<output>,<module>,<log>)
define run-xindy
success=1; \
if ! $(XINDY) -q -o $2 -L $(XINDYLANG) -C $(XINDYENC) -I xindy -M $3 -t $4 $1 > /dev/null || $(EGREP) -q '^xindy:' $4; then \
	$(call colorize-xindy-errors,$4); \
	$(RM) -f '$2'; \
	success=0; \
fi; \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef

# This runs the given script to generate output, and it uses MAKE_RESTARTS to
# ensure that it never runs it more than once for a particular root make
# invocation.
#
# $(call run-script,<interpreter>,<input>,<output>)
define run-script
[ ! -e '$2.cookie' ] && $(ECHO) "restarts=$(RESTARTS)" > $2.cookie && $(ECHO) "level=$(MAKELEVEL)" >> $2.cookie; \
restarts=`$(SED) -n -e 's/^restarts=//p' $2.cookie`; \
level=`$(SED) -n -e 's/^level=//p' $2.cookie`; \
if $(EXPR) $(MAKELEVEL) '<=' $$level '&' $(RESTARTS) '<=' $$restarts >/dev/null; then \
	$(call echo-build,$2,$3,$(RESTARTS)-$(MAKELEVEL)); \
	$1 '$2' '$3'; \
	$(ECHO) "restarts=$(RESTARTS)" > '$2.cookie'; \
	$(ECHO) "level=$(MAKELEVEL)" >> '$2.cookie'; \
fi
endef

# BibTeX invocations
#
# $(call run-bibtex,<tex stem>)
run-bibtex	= $(BIBTEX) $1 | $(color_bib)


# $(call convert-eps-to-pdf,<eps file>,<pdf file>,[gray])
# Note that we don't use the --filter flag because it has trouble with bounding boxes that way.
define convert-eps-to-pdf
$(if $3,$(CAT) '$1' | $(call kill-ps-color) > '$1.cookie',$(CP) '$1' '$1.cookie'); \
$(EPSTOPDF) '$1.cookie' --outfile='$2' > $1.log; \
$(call colorize-epstopdf-errors,$1.log);
endef

# $(call default-gpi-fontsize,<output file>)
#
# Find the default fontsize given the *output* file (it is based on the output extension)
#
default-gpi-fontsize = $(if $(filter %.pdf,$1),$(DEFAULT_GPI_PDF_FONTSIZE),$(DEFAULT_GPI_EPS_FONTSIZE))

# $(call gpi-fontsize,<gpi file>,<output file>)
#
# Find out what the gnuplot fontsize should be.  Tries, in this order:
# - ##FONTSIZE comment in gpi file
# - ##FONTSIZE comment in global gpi file
# - default fontsize based on output type
define gpi-fontsize
$(strip $(firstword \
	$(shell $(SED) -e 's/^\#\#FONTSIZE=\([[:digit:]]\{1,\}\)/\1/p' -e 'd' $1 $(strip $(gpi_global))) \
	$(call default-gpi-fontsize,$2)))
endef

# $(call gpi-monochrome,<gpi file>,[gray])
define gpi-monochrome
$(strip $(if $2,monochrome,$(if $(shell $(EGREP) '^\#\#[[:space:]]*GRAY[[:space:]]*$$' $1 $(gpi_global)),monochrome,color)))
endef

# $(call gpi-font-entry,<output file>,<fontsize>)
#
# Get the font entry given the output file (type) and the font size.  For PDF
# it uses fsize or font, for eps it just uses the bare number.
gpi-font-entry = $(if $(filter %.pdf,$1),$(subst FONTSIZE,$2,$(GPI_FSIZE_SYNTAX)),$2)

# $(call gpi-terminal,<gpi file><output file>,[gray])
#
# Get the terminal settings for a given gpi and its intended output file
define gpi-terminal
$(if $(filter %.pdf,$2),pdf enhanced,postscript enhanced eps) \
$(call gpi-font-entry,$2,$(call gpi-fontsize,$1,$2)) \
$(call gpi-monochrome,$1,$3)
endef

# $(call gpi-embed-pdf-fonts,<input file>,<output file>)
#
define gpi-embed-pdf-fonts
$(GS) \
	-q \
	-dSAFER \
	-dNOPAUSE \
	-dBATCH \
	-sDEVICE=$(if $(filter pdf,$(GPI_OUTPUT_EXTENSION)),pdfwrite,pswrite) \
	-sOutputFile='$2' \
	-sstdout=%stderr \
	-dCompatibilityLevel=1.5 \
	-dPDFSETTINGS=/prepress \
	-c .setpdfwrite \
	-f '$1'
endef

# $(call convert-gpi,<gpi file>,<output file>,[gray])
#
define convert-gpi
$(ECHO) 'set terminal $(call gpi-terminal,$1,$2,$3)' > $1head.make; \
$(ECHO) 'set output "$2"' >> $1head.make; \
$(if $(gpi_global),$(CAT) $(gpi_global) >> $1head.make;,) \
fnames='$1head.make $1';\
$(if $(gpi_sed),\
	$(SED) -f '$(gpi_sed)' $$fnames > $1.temp.make; \
	fnames=$1.temp.make;,\
) \
success=1; \
if ! $(GNUPLOT) $$fnames 2>$1.log; then \
	$(call colorize-gnuplot-errors,$1.log); \
	success=0; \
else \
	if ! $(call gpi-embed-pdf-fonts,$2,$2.embed.make); then \
		success = 0; \
	else \
		$(call move-if-exists,$2.embed.make,$2); \
	fi; \
fi; \
$(if $(gpi_sed),$(call remove-temporary-files,$1.temp.make);,) \
$(call remove-temporary-files,$1head.make); \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef

# Creation of .eps files from .png files
#
# The intermediate step of PNM (using NetPBM) produces much nicer output than
# ImageMagick's "convert" binary.  I couldn't get the right combination of
# flags to make it look nice, anyway.
#
# To handle gray scale conversion, we pipe things through ppmtopgm in the
# middle.
#
# $(call convert-png,<png file>,<eps file>)
define convert-png
$(PNGTOPNM) "$1" \
	$(if $3,| $(PPMTOPGM),) \
	| $(PNMTOPS) -noturn \
	> "$2"
endef

# Creation of .eps files from .jpg/.jpeg files
#
# Thanks to brubakee for this solution.
#
# Uses Postscript level 2 to avoid file size bloat
# $(call convert-jpg,<jpg file>,<eps file>)
define convert-jpg
$(CONVERT) $(if $3,-type Grayscale,) '$1' eps2:'$2'
endef

# Creation of .eps files from .fig files
# $(call convert-fig,<fig file>,<output file>,[gray])
convert-fig	= $(FIG2DEV) -L $(if $(filter %.pdf,$2),pdf,eps) $(if $3,-N,) $1 $2

# Creation of .pstex files from .fig files
# $(call convert-fig-pstex,<fig file>,<pstex file>)
convert-fig-pstex	= $(FIG2DEV) -L pstex $1 $2 > /dev/null 2>&1

# Creation of .pstex_t files from .fig files
# $(call convert-fig-pstex-t,<fig file>,<pstex file>,<pstex_t file>)
convert-fig-pstex-t	= $(FIG2DEV) -L pstex_t -p $3 $1 $2 > /dev/null 2>&1

# Creation of .dot_t files from .dot files
# #(call convert-dot-tex,<dot file>,<dot_t file>)
convert-dot-tex		= $(DOT2TEX) '$1' > '$2'

# Converts svg files into .eps files
#
# $(call convert-svg,<svg file>,<eps/pdf file>,[gray])
convert-svg	= $(INKSCAPE) --without-gui $(if $(filter %.pdf,$2),--export-pdf,--export-eps)='$2' '$1'

# Converts xvg files into .eps files
#
# $(call convert-xvg,<xvg file>,<eps file>,[gray])
convert-xvg	= $(XMGRACE) '$1' -printfile - -hardcopy -hdevice $(if $3,-mono,) EPS > '$2'

# Converts .eps.gz files into .eps files
#
# $(call convert-epsgz,<eps.gz file>,<eps file>,[gray])
convert-epsgz	= $(GUNZIP) -c '$1' $(if $3,| $(call kill-ps-color)) > '$2'

# Converts .eps files into .eps files (usually a no-op, but can make grayscale)
#
# $(call convert-eps,<in file>,<out file>,[gray])
convert-eps	= $(if $3,$(call kill-ps-color) $1 > $2)

# The name of the file containing special postscript commands for grayscale
gray_eps_file	:= gray.eps.make

# Changes sethsbcolor and setrgbcolor calls in postscript to always produce
# grayscale.  In general, this is accomplished by writing new versions of those
# functions into the user dictionary space, which is looked up before the
# global or system dictionaries (userdict is one of the permanent dictionaries
# in postscript and is not read-only like systemdict).
#
# For setrgbcolor, the weighted average of the triple is computed and the
# triple is replaced with three copies of that average before the original
# procedure is called: .299R + .587G + .114B
#
# For sethsbcolor, the color is first converted to RGB, then to grayscale by
# the new setrgbcolor operator as described above.  Why is this done?
# Because simply using the value component will tend to make pure colors
# white, a very undesirable thing.  Pure blue should not translate to white,
# but to some level of gray.  Conversion to RGB does the right thing.  It's
# messy, but it works.
#
# From
# http://en.wikipedia.org/wiki/HSV_color_space#Transformation_from_HSV_to_RGB,
# HSB = HSV (Value = Brightness), and the formula used to convert to RGB is
# as follows:
#
# Hi = int(floor(6 * H)) mod 6
# f = 6 * H - Hi
# p = V(1-S)
# q = V(1-fS)
# t = V(1-(1-f)S)
# if Hi = 0: R G B <-- V t p
# if Hi = 1: R G B <-- q V p
# if Hi = 2: R G B <-- p V t
# if Hi = 3: R G B <-- p q V
# if Hi = 4: R G B <-- t p V
# if Hi = 5: R G B <-- V p q
#
# The messy stack-based implementation is below
# $(call create-gray-eps-file,filename)
define create-gray-eps-file
$(ECHO) -n -e '\
/OLDRGB /setrgbcolor load def\n\
/setrgbcolor {\n\
    .114 mul exch\n\
    .587 mul add exch\n\
    .299 mul add\n\
    dup dup\n\
    OLDRGB\n\
} bind def\n\
/OLDHSB /sethsbcolor load def\n\
/sethsbcolor {\n\
    2 index                     % H V S H\n\
    6 mul floor cvi 6 mod       % Hi V S H\n\
    3 index                     % H Hi V S H\n\
    6 mul                       % 6H Hi V S H\n\
    1 index                     % Hi 6H Hi V S H\n\
    sub                         % f Hi V S H\n\
    2 index 1                   % 1 V f Hi V S H\n\
    4 index                     % S 1 V f Hi V S H\n\
    sub mul                     % p f Hi V S H\n\
    3 index 1                   % 1 V p f Hi V S H\n\
    6 index                     % S 1 V p f Hi V S H\n\
    4 index                     % f S 1 V p f Hi V S H\n\
    mul sub mul                 % q p f Hi V S H\n\
    4 index 1 1                 % 1 1 V q p f Hi V S H\n\
    5 index                     % f 1 1 V q p f Hi V S H\n\
    sub                         % (1-f) 1 V q p f Hi V S H\n\
    8 index                     % S (1-f) 1 V q p f Hi V S H\n\
    mul sub mul                 % t q p f Hi V S H\n\
    4 -1 roll pop               % t q p Hi V S H\n\
    7 -2 roll pop pop           % t q p Hi V\n\
    5 -2 roll                   % Hi V t q p\n\
    dup 0 eq\n\
    {1 index 3 index 6 index}\n\
    {\n\
        dup 1 eq\n\
        {3 index 2 index 6 index}\n\
        {\n\
            dup 2 eq\n\
            {4 index 2 index 4 index}\n\
            {\n\
                dup 3 eq\n\
                {4 index 4 index 3 index}\n\
                {\n\
                    dup 4 eq\n\
                    {2 index 5 index 3 index}\n\
                    {\n\
                        dup 5 eq\n\
                        {1 index 5 index 5 index}\n\
                        {0 0 0}\n\
                        ifelse\n\
                    }\n\
                    ifelse\n\
                }\n\
                ifelse\n\
            }\n\
            ifelse\n\
        }\n\
        ifelse\n\
    }\n\
    ifelse                      % B G R Hi V t q p\n\
    setrgbcolor\n\
    5 {pop} repeat\n\
} bind def\n'\
> $1
endef

# This actually inserts the color-killing code into a postscript file
# $(call kill-ps-color)
define kill-ps-color
$(SED) -e '/%%EndComments/r $(gray_eps_file)'
endef

# Converts graphviz .dot files into .eps files
# Grayscale is not directly supported by dot, so we pipe it through fig2dev in
# that case.
# $(call convert-dot,<dot file>,<eps file>,<log file>,[gray])
define convert-dot
$(DOT) -Tps '$1' 2>'$3' $(if $4,| $(call kill-ps-color)) > $2; \
$(call colorize-dot-errors,$3)
endef

# Convert DVI to Postscript
# $(call make-ps,<dvi file>,<ps file>,<log file>,[<paper size>])
make-ps		= \
	$(DVIPS) -z -o '$2' $(if $(filter-out BEAMER,$4),-t$(firstword $4),) '$1' \
		$(if $(filter BEAMER,$4),| $(enlarge_beamer)) > $3 2>&1

# Convert Postscript to PDF
# $(call make-pdf,<ps file>,<pdf file>,<log file>,<embed file>)
make-pdf	= \
	$(call ps2pdf,$1,$2,$(filter 1,$(shell $(CAT) '$4'))) > '$3' 2>&1

# Display information about what is being done
# $(call echo-build,<input file>,<output file>,[<run number>])
echo-build	= $(ECHO) "$(C_BUILD)= $1 --> $2$(if $3, ($3),) =$(C_RESET)"
echo-graphic	= $(ECHO) "$(C_GRAPHIC)= $1 --> $2 =$(C_RESET)"
echo-dep	= $(ECHO) "$(C_DEP)= $1 --> $2 =$(C_RESET)"

# Display a list of something
# $(call echo-list,<values>)
echo-list	= for x in $1; do $(ECHO) "$$x"; done

#
# DEFAULT TARGET
#

.PHONY: all
all: $(default_pdf_targets) ;

.PHONY: all-pdf
all-pdf: $(default_pdf_targets) ;

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.PHONY: all-ps
all-ps: $(default_ps_targets) ;

.PHONY: all-dvi
all-dvi: $(default_dvi_targets) ;
endif

#
# VIEWING TARGET
#
.PHONY: show
show: all
	$(QUIET)for x in $(default_pdf_targets); do \
		[ -e "$$x" ] && $(VIEW_PDF) $$x & \
	done

#
# INCLUDES
#
source_includes	:= $(addsuffix .d,$(source_stems_to_include))
graphic_includes := $(addsuffix .gpi.d,$(graphic_stems_to_include))

# Check the version of the makefile
ifneq "" "$(filter 3.79 3.80,$(MAKE_VERSION))"
$(warning $(C_WARNING)Your version of make is too old.  Please upgrade.$(C_RESET))
endif

# Include only the dependencies used
ifneq "" "$(source_includes)"
include $(source_includes)$(call include-message,$(source_includes))
endif
ifneq "" "$(graphic_includes)"
include $(graphic_includes)$(call include-message,$(graphic_includes))
endif

#
# MAIN TARGETS
#

# Note that we don't just say %: %.pdf here - this can tend to mess up our
# includes, which detect what kind of file we are asking for.  For example,
# asking to build foo.pdf is much different than asking to build foo when
# foo.gpi exists, because we look through all of the goals for *.pdf that
# matches *.gpi, then use that to determine which include files we need to
# build.
#
# Thus, we invoke make recursively with better arugments instead, restarting
# all of the appropriate machinery.
.PHONY: $(default_stems_ss)
$(default_stems_ss): %: %.pdf ;

# This builds and displays the wanted file.
.PHONY: $(addsuffix ._show,$(stems_ssg))
$(addsuffix ._show,$(stems_ssg)): %._show: %.pdf
	$(QUIET)$(VIEW_PDF) $< &

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.SECONDARY: $(all_pdf_targets)
%.pdf: %.ps %.embed.make
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-pdf,$<,$@.temp,$@.log,$*.embed.make); \
	if [ x"$$?" = x"0" ]; then \
	    $(if $(VERBOSE),$(CAT) $@.log,:); \
	    $(RM) -f '$@'; \
	    $(MV) '$@.temp' '$@'; \
	    $(TOUCH) '$@'; \
	    $(call copy-with-logging,$@,$(BINARY_TARGET_DIR)); \
	else \
	    $(CAT) $@.log; \
	    $(call remove-temporary-files,'$@.temp'); \
	    $(sh_false); \
	fi

.SECONDARY: $(all_ps_targets)
%.ps: %.dvi %.paper.make
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-ps,$<,$@.temp,$@.log,\
			$(firstword $(shell $(CAT) $*.paper.make))); \
	if [ x"$$?" = x"0" ]; then \
	    $(if $(VERBOSE),$(CAT) $@.log,:); \
	    $(RM) -f '$@'; \
	    $(MV) '$@.temp' '$@'; \
	    $(TOUCH) '$@'; \
	    $(call copy-with-logging,$@,$(BINARY_TARGET_DIR)); \
	else \
	    $(CAT) $@.log; \
	    $(call remove-temporary-files,'$@.temp'); \
	    $(sh_false); \
	fi
endif

# Build the final target (dvi or pdf) file.  This is a very tricky rule because
# of the way that latex runs multiple times, needs graphics after the first run
# (or maybe already has them), and relies on bibliographies or indices that may
# not exist.
#
#	Check the log for fatal errors.  If they exist, colorize and bail.
#
#	Create the .auxtarget.cookie file.  (Needed for next time if not present)
#
#	If any of the following are true, we must rebuild at least one time:
#
#	* the .bbl was recently rebuilt
#
#		check a cookie, then delete it
#
#	* any of several output files was created or changed:
#
#		check $*.run.cookie, then delete it
#
#	* the .aux file changed in a way that necessitates attention
#
#		Note that if the .auxtarget.make file doesn't exist, this means
#		that we are doing a clean build, so it doesn't figure into the
#		test for running again.
#
#		compare against .auxtarget.make
#
#		move if different, remove if not
#
#	* the .log file has errors or warnings requiring at least one more run
#
#	We use a loop over a single item to simplify the process of breaking
#	out when we find one of the conditions to be true.
#
#	If we do NOT need to run latex here, then we move the $@.1st.make file
#	over to $@ because the target file has already been built by the first
#	dependency run and is valid.
#
#	If we do, we delete that cookie file and do the normal multiple-runs
#	routine.
#
ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.SECONDARY: $(all_dvi_targets)
endif
%.$(build_target_extension): %.bbl %.aux %.$(build_target_extension).1st.make
	$(QUIET)\
	fatal=`$(call colorize-latex-errors,$*.log)`; \
	if [ x"$$fatal" != x"" ]; then \
		$(ECHO) "$$fatal"; \
		exit 1; \
	fi; \
	$(call make-auxtarget-file,$*.aux.make,$*.auxtarget.cookie); \
	run=0; \
	for i in 1; do \
		if $(call test-exists,$*.bbl.cookie); then \
			run=1; \
			break; \
		fi; \
		if $(call test-exists,$*.run.cookie); then \
			run=1; \
		    	break; \
		fi; \
		if $(call \
		test-exists-and-different,$*.auxtarget.cookie,$*.auxtarget.make);\
		then \
			run=1; \
			break; \
		fi; \
		if $(call test-log-for-need-to-run,$*); then \
			run=1; \
			break; \
		fi; \
		if [ ! -e $*.1st.*.make ]; then \
			run=1; \
			break; \
		fi; \
	done; \
	$(call remove-temporary-files,$*.bbl.cookie $*.run.cookie); \
	$(MV) $*.auxtarget.cookie $*.auxtarget.make; \
	if [ x"$$run" = x"1" ]; then \
		$(call remove-files,$@.1st.make); \
		for i in 2 3 4 5; do \
			$(if $(findstring 3.79,$(MAKE_VERSION)),\
				$(call echo-build,$*.tex,$@,$(RESTARTS)-$$$$i),\
				$(call echo-build,$*.tex,$@,$(RESTARTS)-$$i)\
			); \
			$(call run-latex,$*); \
			$(CP) '$*.log' '$*.'$(RESTARTS)-$$i'.log'; \
			$(call test-run-again,$*) || break; \
		done; \
	else \
		$(MV) '$@.1st.make' '$@'; \
	fi; \
	$(call copy-with-logging,$@,$(BINARY_TARGET_DIR)); \
	$(call latex-color-log,$*)

# Build the .bbl file.  When dependencies are included, this will (or will
# not!) depend on something.bib, which we detect, acting accordingly.  The
# dependency creation also produces the %.auxbbl.make file.  BibTeX is a bit
# finicky about what you call the actual files, but we can rest assured that if
# a .auxbbl.make file exists, then the .aux file does, as well.  The
# .auxbbl.make file is a cookie indicating whether the .bbl needs to be
# rewritten.  It only changes if the .aux file changes in ways relevant to .bbl
# creation.
#
# Note that we do NOT touch the .bbl file if there is no need to
# create/recreate it.  We would like to leave existing files alone if they
# don't need to be changed, thus possibly avoiding a rebuild trigger.
%.bbl: %.auxbbl.make
	$(QUIET)\
	$(if $(filter %.bib,$^),\
		$(call echo-build,$(filter %.bib,$?) $*.aux,$@); \
		$(call run-bibtex,$*); \
		$(TOUCH) $@.cookie; \
	) \
	if $(EGREP) -q 'bibstyle.(apacite|apacann|chcagoa|[^}]*annot)' '$*.aux'; then \
		$(call echo-build,** annotated extra latex **,output ignored,$(RESTARTS)-1); \
		$(call run-latex,$*); \
		$(CP) '$*.log' '$*.$(RESTARTS)-annotated.log'; \
		$(if $(filter %.bib,$^),\
			$(call echo-build,** annotated extra bibtex ** $(filter %.bib,$?) $*.aux,$@); \
			$(call run-bibtex,$*); \
			$(TOUCH) $@.cookie; \
		) \
		$(call echo-build,** annotated extra latex **,output ignored,$(RESTARTS)-2); \
		$(call run-latex,$*); \
	fi

# Create the index file - note that we do *not* depend on %.tex here, since
# that unnecessarily restricts the kinds of indices that we can build to those
# with exactly the same stem as the source file.  Things like splitidx create
# idx files with other names.
#
# Therefore, we add the .tex dependency in the sourcestem.d file in the call to
# get index file dependencies from the logs.
%.ind:	%.idx
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.ilg)

# Create a glossary file from a .ist file
%.gls:	%.glo %.tex %.ist
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.glg,$*.ist)

# Create a glossary file from a glossary input formatted for xindy
%.gls:	%.glo %.tex %.xdy
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-xindy,$<,$@,$*,$*.glg)

# Create the glossary file from a nomenclature file
%.gls:	%.glo %.tex nomencl.ist
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.glg,nomencl.ist)

# Create the nomenclature file
%.nls:	%.nlo %.tex nomencl.ist
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.nlg,nomencl.ist)

# SCRIPTED LaTeX TARGETS
#
# Keep the generated .tex files around for debugging if needed.
.SECONDARY: $(all_tex_targets)

%.tex::	%.tex.sh
	$(QUIET)$(call run-script,$(SHELL),$<,$@)

%.tex::	%.tex.py
	$(QUIET)$(call run-script,$(PYTHON),$<,$@)

%.tex::	%.tex.pl
	$(QUIET)$(call run-script,$(PERL),$<,$@)

%.tex::	%.rst $(RST_STYLE_FILE)
	$(QUIET)\
	$(call run-script,$(RST2LATEX)\
		--documentoptions=letterpaper\
		$(if $(RST_STYLE_FILE),--stylesheet=$(RST_STYLE_FILE),),$<,$@)

#
# GRAPHICS TARGETS
#
.PHONY: all-graphics
all-graphics:	$(all_graphics_targets);

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.PHONY: all-pstex
all-pstex:	$(all_pstex_targets);
endif

.PHONY: all-dot2tex
all-dot2tex:	$(all_dot2tex_targets);

.PHONY: show-graphics
show-graphics: all-graphics
	$(VIEW_GRAPHICS) $(all_known_graphics)

$(gray_eps_file):
	$(QUIET)$(call echo-build,$^,$@)
	$(QUIET)$(call create-gray-eps-file,$@)

ifeq "$(strip $(BUILD_STRATEGY))" "pdflatex"
%.pdf: %.eps $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-eps-to-pdf,$<,$@,$(GRAY))

ifeq "$(strip $(GPI_OUTPUT_EXTENSION))" "pdf"
%.pdf:	%.gpi %.gpi.d $(gpi_sed) $(gpi_global)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,$(GRAY))
endif

%.pdf:	%.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,$(GRAY))

%.pdf:	%.svg
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-svg,$<,$@,$(GRAY))
endif

ifeq "$(strip $(BUILD_STRATEGY))" "xelatex"
%.pdf: %.eps $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-eps-to-pdf,$<,$@,$(GRAY))

ifeq "$(strip $(GPI_OUTPUT_EXTENSION))" "pdf"
%.pdf:	%.gpi %.gpi.d $(gpi_sed) $(gpi_global)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,$(GRAY))
endif

%.pdf:	%.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,$(GRAY))

endif


%.eps:	%.gpi %.gpi.d $(gpi_sed) $(gpi_global)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,$(GRAY))

%.eps: %.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,$(GRAY))

%.eps: %.dot $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-dot,$<,$@,$<.log,$(GRAY))

%.eps: %.xvg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-xvg,$<,$@,$(GRAY))

ifneq "$(default_graphic_extension)" "pdf"
# We have a perfectly good build rule for svg to pdf, so we eliminate this to
# avoid confusing make (it sometimes chooses to go svg -> eps -> pdf).
%.eps: %.svg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-svg,$<,$@,$(GRAY))

# Similarly for these, we don't need eps if we have supported extensions
# already.
%.eps: %.jpg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-jpg,$<,$@,$(GRAY))

%.eps: %.jpeg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-jpg,$<,$@,$(GRAY))

%.eps: %.png $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-png,$<,$@,$(GRAY))
endif

%.eps: %.eps.gz $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-epsgz,$<,$@,$(GRAY))

%.pstex: %.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex,$<,$@,$(GRAY))

%.pstex_t: %.fig %.pstex
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex-t,$<,$@,$*.pstex,$(GRAY))

%.dot_t: %.dot
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-dot-tex,$<,$@)

#
# DEPENDENCY-RELATED TARGETS.
#

# Generate all of the information needed to get dependencies
# As a side effect, this creates a .dvi or .pdf file (depending on the build
# strategy).  We need to be sure to remove it if there are errors.  Errors can
# take several forms and all of them are found within the log file:
#	* There was a LaTeX error
#	* A needed file was not found
#	* Cross references need adjustment
#
# Behavior:
#	This rule is responsible for generating the following:
#	%.aux
#	%.d
#	%.aux.make
#	%.(pdf|dvi).1st.make (the .pdf or .dvi output file, moved)
#
#	Steps:
#
#	Run latex
#	Move .pdf or .dvi somewhere else (make no judgements about success)
#	Flatten the .aux file into another file
#	Add source dependencies
#	Add graphic dependencies
#	Add bib dependencies
#
#	Create cookies for various suffixes that may represent files that
#	need to be read by LaTeX in order for it to function properly.
#
#	Note that if some of the dependencies are discovered because they turn
#	up missing in the log file, we really need the .d file to be reloaded.
#	Adding a sleep command helps with this.  Otherwise make is extremely
#	nondeterministic, sometimes working, sometimes not.
#
#	Usually we can force this by simply removing the generated pdf file and
#	not creating a .1st.make file..
#
%.$(build_target_extension).1st.make %.d %.aux %.aux.make %.fls: %.tex
	$(QUIET)$(call echo-build,$<,$*.d $*.$(build_target_extension).1st.make,$(RESTARTS)-1)
	$(QUIET)\
	$(call run-latex,$<,-recorder) || $(sh_true); \
	$(CP) '$*.log' '$*.$(RESTARTS)-1.log'; \
	$(call die-on-import-sty,$*.log); \
	$(call die-on-dot2tex,$*.log); \
	$(call die-on-no-aux,$*); \
	$(call flatten-aux,$*.aux,$*.aux.make); \
	$(ECHO) "# vim: ft=make" > $*.d; \
	$(ECHO) ".PHONY: $*._graphics" >> $*.d; \
	$(call get-inputs,$*.fls,$(addprefix $*.,aux aux.make d $(build_target_extension))) >> $*.d; \
	$(call get-missing-inputs,$*.log,$(addprefix $*.,aux aux.make d $(build_target_extension))) >> $*.d; \
	$(ECHO) ".SECONDEXPANSION:" >> $*.d; \
	$(call get-graphics,$*) >> $*.d; \
	$(call get-log-index,$*,$(addprefix $*.,aux aux.make)) >> $*.d; \
	$(call get-bibs,$*.aux.make,$(addprefix $*.,bbl aux aux.make)) >> $*.d; \
	$(EGREP) -q "# MISSING" $*.d && $(SLEEP) 1 && $(RM) $*.pdf; \
	$(call move-if-exists,$*.$(build_target_extension),$*.$(build_target_extension).1st.make); \
	for s in toc out lot lof lol nav; do \
		if [ -e "$*.$$s" ]; then \
			if ! $(DIFF) -q $*.$$s $*.$$s.make >/dev/null 2>&1; then \
				$(TOUCH) $*.run.cookie; \
			fi; \
			$(CP) $*.$$s $*.$$s.make; \
		fi; \
	done

# This is a cookie that is updated if the flattened aux file has changed in a
# way that affects the bibliography generation.
.SECONDARY: $(addsuffix .auxbbl.make,$(stems_ssg))
%.auxbbl.make: %.aux.make
	$(QUIET)\
	$(call make-auxbbl-file,$<,$@.temp); \
	$(call replace-if-different-and-remove,$@.temp,$@)

# Build a dependency file for .gpi files.  These often plot data files that
# also reside in the directory, so if a data file changes, it's nice to know
# about it.  This also handles loaded .gpi files, whose filename should have
# _include_. in it.
%.gpi.d: %.gpi
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-gpi-d,$<,$@)

# Store the paper size for this document -- note that if beamer is used we set
# it to the special BEAMER paper size.  We only do this, however, if the
# special comment exists, in which case we enlarge the output with psnup.
#
#	The paper size is extracted from a documentclass attribute.
%.paper.make: %.tex
	$(QUIET)$(SED) \
	-e '/\\documentclass/,/}/{' \
	-e '  s/%.*//' \
	-e '  H' \
	-e '  /}/{' \
	-e '    s/.*//' \
	-e '    x' \
	-e '    /\\documentclass/!d' \
	-e '    s/[\n[:space:]]*//g' \
	-e '    s/\([,{[]\)\([[:alnum:]]\{1,\}\)paper\([],}]\)/\1%-\2-%\3/g' \
	-e '    s/\([,{[]\)\(landscape\)\([],}]\)/\1%-\2-%\3/g' \
	-e '    s/^[^%]*%-//' \
	-e '    s/-%[^%]*$$//' \
	-e '    s/-%[^%]%-/ /g' \
	-e '    p' \
	-e '  }' \
	-e '  d' \
	-e '}' \
	-e 'd' \
	$< > $@; \
	$(EGREP) -q '^[^%]*\\documentclass[^{]*{beamer}' $< && \
	(\
		$(EGREP) -q '^%%[[:space:]]*BEAMER[[:space:]]*LARGE$$' $< && \
		$(ECHO) "BEAMER" > $@ || \
		: > $@ \
	) || $(sh_true)

# Store embedding instructions for this document using a special comment
%.embed.make: %.tex
	$(QUIET)$(EGREP) '^%%[[:space:]]*NO[[:space:]]*EMBED[[:space:]]*$$' $< \
		&& $(ECHO) '' > $@ \
		|| $(ECHO) '1' > $@;

#
# HELPFUL PHONY TARGETS
#

.PHONY: _all_programs
_all_programs:
	$(QUIET)$(ECHO) "== All External Programs Used =="
	$(QUIET)$(call output-all-programs)

.PHONY: _check_programs
_check_programs:
	$(QUIET)$(ECHO) "== Checking Makefile Dependencies =="; $(ECHO)
	$(QUIET) \
	allprogs=`\
	 ($(call output-all-programs)) | \
	 $(SED) \
	 -e 's/^[[:space:]]*//' \
	 -e '/^#/d' \
	 -e 's/[[:space:]]*#.*//' \
	 -e '/^=/s/[[:space:]]/_/g' \
	 -e '/^[[:space:]]*$$/d' \
	 -e 's/^[^=].*=[[:space:]]*\([^[:space:]]\{1,\}\).*$$/\\1/' \
	 `; \
	spaces='                             '; \
	for p in $${allprogs}; do \
	case $$p in \
		=*) $(ECHO); $(ECHO) "$$p";; \
		*) \
			$(ECHO) -n "$$p:$$spaces" | $(SED) -e 's/^\(.\{0,20\}\).*$$/\1/'; \
			loc=`$(WHICH) $$p`; \
			if [ x"$$?" = x"0" ]; then \
				$(ECHO) "$(C_SUCCESS)Found:$(C_RESET) $$loc"; \
			else \
				$(ECHO) "$(C_FAILURE)Not Found$(C_RESET)"; \
			fi; \
			;; \
	esac; \
	done

.PHONY: _check_gpi_files
_check_gpi_files:
	$(QUIET)$(ECHO) "== Checking all .gpi files for common errors =="; \
	$(ECHO); \
	for f in $(files.gpi); do \
	result=`$(EGREP) '^([^#]*set terminal |set output )' $$f`; \
	$(ECHO) -n "$$f: "; \
	if [ x"$$result" = x"" ]; then \
		$(ECHO) "$(C_SUCCESS)Okay$(C_RESET)"; \
	else \
		$(ECHO) "$(C_FAILURE)Warning: Problematic commands:$(C_RESET)";\
		$(ECHO) "$(C_ERROR)$$result$(C_RESET)"; \
	fi; \
	done; \
	$(ECHO)

.PHONY: _all_stems
_all_stems:
	$(QUIET)$(ECHO) "== All Stems =="
	$(QUIET)$(call echo-list,$(sort $(default_stems_ss)))

.PHONY: _includes
_includes:
	$(QUIET)$(ECHO) "== Include Stems =="
	$(QUIET)$(ECHO) "=== Sources ==="
	$(QUIET)$(call echo-list,$(sort $(source_includes)))
	$(QUIET)$(ECHO) "=== Graphics ==="
	$(QUIET)$(call echo-list,$(sort $(graphic_includes)))

.PHONY: _all_sources
_all_sources:
	$(QUIET)$(ECHO) "== All Sources =="
	$(QUIET)$(call echo-list,$(sort $(all_files.tex)))

.PHONY: _dependency_graph
_dependency_graph:
	$(QUIET)$(ECHO) "/* LaTeX Dependency Graph */"
	$(QUIET)$(call output-dependency-graph)

.PHONY: _show_dependency_graph
_show_dependency_graph:
	$(QUIET)$(call output-dependency-graph,$(graph_stem).dot)
	$(QUIET)$(DOT) -Tps -o $(graph_stem).eps $(graph_stem).dot
	$(QUIET)$(VIEW_POSTSCRIPT) $(graph_stem).eps
	$(QUIET)$(call remove-temporary-files,$(graph_stem).*)

.PHONY: _sources
_sources:
	$(QUIET)$(ECHO) "== Sources =="
	$(QUIET)$(call echo-list,$(sort $(files.tex)))

.PHONY: _scripts
_scripts:
	$(QUIET)$(ECHO) "== Scripts =="
	$(QUIET)$(call echo-list,$(sort $(files_scripts)))

.PHONY: _graphic_outputs
_graphic_outputs:
	$(QUIET)$(ECHO) "== Graphic Outputs =="
	$(QUIET)$(call echo-list,$(sort $(all_graphics_targets)))

.PHONY: _env
_env:
ifdef .VARIABLES
	$(QUIET)$(ECHO) "== MAKE VARIABLES =="
	$(QUIET)$(call echo-list,$(foreach var,$(sort $(.VARIABLES)),'$(var)'))
endif
	$(QUIET)$(ECHO) "== ENVIRONMENT =="
	$(QUIET)$(ENV)

#
# CLEAN TARGETS
#
# clean-generated is somewhat unique - it relies on the .fls file being
# properly built so that it can determine which of the files was generated, and
# which was not.  Expect it to silently fail if the .fls file is missing.
#
# This is used to, e.g., clean up index files that are generated by the LaTeX.
.PHONY: clean-generated
clean-generated:
	$(QUIET)$(call clean-files,$(foreach e,$(addsuffix .fls,$(all_stems_source)),\
						$(shell $(call get-generated-names,$e))))

.PHONY: clean-deps
clean-deps:
	$(QUIET)$(call clean-files,$(all_d_targets) *.make *.make.temp *.cookie)

.PHONY: clean-tex
clean-tex: clean-deps
	$(QUIET)$(call clean-files,$(rm_tex))

.PHONY: clean-graphics
# TODO: This *always* deletes pstex files, even if they were not generated by
# anything....  In other words, if you create a pstex and pstex_t pair by hand
# an drop them in here without the generating fig file, they will be deleted
# and you won't get them back.  It's a hack put in here because I'm not sure we
# even want to keep pstex functionality, so my motivation is not terribly high
# for doing it right.
clean-graphics:
	$(QUIET)$(call clean-files,$(all_graphics_targets) *.gpi.d *.pstex *.pstex_t *.dot_t)

.PHONY: clean-backups
clean-backups:
	$(QUIET)$(call clean-files,$(backup_patterns) *.temp)

.PHONY: clean-auxiliary
clean-auxiliary:
	$(QUIET)$(call clean-files,$(graph_stem).*)

.PHONY: clean-nographics
clean-nographics: clean-tex clean-deps clean-backups clean-auxiliary ;

.PHONY: clean
clean: clean-generated clean-tex clean-graphics clean-deps clean-backups clean-auxiliary ;

#
# HELP TARGETS
#

.PHONY: help
help:
	$(help_text)

.PHONY: version
version:
	$(QUIET)\
	$(ECHO) "$(fileinfo) Version $(version)"; \
	$(ECHO) "by $(author)"; \

#
# HELP TEXT
#

define help_text
# $(fileinfo) Version $(version)
#
# by $(author)
#
# Generates a number of possible output files from a LaTeX document and its
# various dependencies.  Handles .bib files, \include and \input, and .eps
# graphics.  All dependencies are handled automatically by running LaTeX over
# the source.
#
# USAGE:
#
#    make [GRAY=1] [VERBOSE=1] [SHELL_DEBUG=1] <target(s)>
#
# STANDARD OPTIONS:
#    GRAY:
#        Setting this variable forces all recompiled graphics to be grayscale.
#        It is useful when creating a document for printing.  The default is
#        to allow colors.  Note that it only changes graphics that need to be
#        rebuilt!  It is usually a good idea to do a 'make clean' first.
#
#    VERBOSE:
#        This turns off all @ prefixes for commands invoked by make.  Thus,
#        you get to see all of the gory details of what is going on.
#
#    SHELL_DEBUG:
#        This enables the -x option for sh, meaning that everything it does is
#        echoed to stderr.  This is particularly useful for debugging
#        what is going on in $$(shell ...) invocations.  One of my favorite
#        debugging tricks is to do this:
#
#        make -d SHELL_DEBUG=1 VERBOSE=1 2>&1 | less
#
#    KEEP_TEMP:
#        When set, this allows .make and other temporary files to stick around
#        long enough to do some debugging.  This can be useful when trying to
#        figure out why gnuplot is not doing the right things, for example
#        (e.g., look for *head.make).
#
# STANDARD AUXILIARY FILES:
#
#      Variables.ini (formerly Makefile.ini, which still works)
#
#          This file can contain variable declarations that override various
#          aspects of the makefile.  For example, one might specify
#
#          neverclean := *.pdf *.ps
#          onlysources.tex := main.tex
#          LATEX_COLOR_WARNING := 'bold red uline'
#
#          And this would override the neverclean setting to ensure that pdf
#          and ps files always remain behind, set the makefile to treat all
#          .tex files that are not "main.tex" as includes (and therefore not
#          default targets).  It also changes the LaTeX warning output to be
#          red, bold, and underlined.
#
#          There are numerous variables in this file that can be overridden in
#          this way.  Search for '?=' to find them all.
#
#          The Variables.ini is imported before *anything else* is done, so go
#          wild with your ideas for changes to this makefile in there.  It
#          makes it easy to test them before submitting patches.
#
#          If you're adding rules or targets, however, see Targets.ini below.
#
#      Targets.ini
#
#          This is included much later in the makefile, after all variables and
#          targets are defined.  This is where you would put new make rules,
#          e.g.,
#
#          generated.tex: generating_script.weird_lang depA depB
#             ./generating_script.weird_lang > $$@
#
#          In this file, you have access to all of the variables that the
#          makefile creates, like $(onlysources.tex).  While accessing those can
#          be somewhat brittle (they are implementation details and may change),
#          it is a great way to test your ideas when submitting feature requests.
#
# STANDARD ENVIRONMENT VARIABLES:
#
#      LATEX_COLOR_WARNING        '$(LATEX_COLOR_WARNING)'
#      LATEX_COLOR_ERROR          '$(LATEX_COLOR_ERROR)'
#      LATEX_COLOR_UNDERFULL      '$(LATEX_COLOR_UNDERFULL)'
#      LATEX_COLOR_OVERFULL       '$(LATEX_COLOR_OVERFULL)'
#      LATEX_COLOR_PAGES          '$(LATEX_COLOR_PAGES)'
#      LATEX_COLOR_BUILD          '$(LATEX_COLOR_BUILD)'
#      LATEX_COLOR_GRAPHIC        '$(LATEX_COLOR_GRAPHIC)'
#      LATEX_COLOR_DEP            '$(LATEX_COLOR_DEP)'
#      LATEX_COLOR_SUCCESS        '$(LATEX_COLOR_SUCCESS)'
#      LATEX_COLOR_FAILURE        '$(LATEX_COLOR_FAILURE)'
#
#   These may be redefined in your environment to be any of the following:
#
#      black
#      red
#      green
#      yellow
#      blue
#      magenta
#      cyan
#      white
#
#   Bold or underline may be used, as well, either alone or in combination
#   with colors:
#
#      bold
#      uline
#
#   Order is not important.  You may want, for example, to specify:
#
#   export LATEX_COLOR_SUCCESS='bold blue uline'
#
#   in your .bashrc file.  I don't know why, but you may want to.
#
# STANDARD TARGETS:
#
#    all:
#        Make all possible documents in this directory.  The documents are
#        determined by scanning for .tex and .tex.sh (described in more detail
#        later) and omitting any file that ends in ._include_.tex or
#        ._nobuild_.tex.  The output is a set of .pdf files.
#
#        If you wish to omit files without naming them with the special
#        underscore names, set the following near the top of the Makefile,
#        or (this is recommended) within a Makefile.ini in the same directory:
#
#         includes.tex := file1.tex file2.tex
#
#        This will cause the files listed to be considered as include files.
#
#        If you have only few source files, you can set
#
#         onlysources.tex := main.tex
#
#        This will cause only the source files listed to be considered in
#        dependency detection.  All other .tex files will be considered as
#        include files.  Note that these options work for *any* source type,
#        so you could do something similar with includes.gpi, for example.
#        Note that this works for *any valid source* target.  All of the
#        onlysources.* variables are commented out in the shipping version of
#        this file, so it does the right thing when they simply don't exist.
#        The comments are purely documentation.  If you know, for example, that
#        file.mycoolformat is supported by this Makefile, but don't see the
#        "onlysources.mycoolformat" declared in the comments, that doesn't mean
#        you can't use it.  Go ahead and set "onlysources.mycoolformat" and it
#        should do the right thing.
#
#    show:
#        Builds and displays all documents in this directory.  It uses the
#        environment-overridable value of VIEW_PDF (currently $(VIEW_PDF)) to
#        do its work.
#
#    all-graphics:
#        Make all of the graphics in this directory.
#
#    all-pstex (only for BUILD_STRATEGY=latex):
#        Build all fig files into pstex and pstex_t files.  Gray DOES NOT WORK.
#
#    all-gray-pstex (only for BUILD_STRATEGY=latex):
#          Build all fig files into grayscale pstex and pstex_t files.
#
#    all-dot2tex:
#          Build all dot files into tex files.
#
#    show-graphics:
#        Builds and displays all graphics in this directory.  Uses the
#        environment-overridable value of VIEW_GRAPHICS (currently
#        $(VIEW_GRAPHICS)) to do its work.
#
#    clean:
#        Remove ALL generated files, leaving only source intact.
#        This will *always* skip files mentioned in the "neverclean" variable,
#        either in this file or specified in Makefile.ini:
#
#         neverclean := *.pdf *.ps
#
#       The neverclean variable works on all "clean" targets below, as well.
#
#    clean-graphics:
#        Remove all generated graphics files.
#
#    clean-backups:
#        Remove all backup files: $(backup_patterns)
#        (XFig and other editors have a nasty habit of leaving them around)
#        Also removes Makefile-generated .temp files
#
#    clean-tex:
#        Remove all files generated from LaTeX invocations except dependency
#        information.  Leaves graphics alone.
#
#    clean-deps:
#        Removes all auto-generated dependency information.
#
#    clean-auxiliary:
#        Removes extra files created by various targets (like the dependency
#        graph output).
#
#    clean-nographics:
#        Cleans everything *except* the graphics files.
#
#    help:
#        This help text.
#
#    version:
#        Version information about this LaTeX makefile.
#
# DEBUG TARGETS:
#
#    _all_programs:
#        A list of the programs used by this makefile.
#
#    _check_programs:
#        Checks your system for the needed software and reports what it finds.
#
#    _check_gpi_files:
#        Checks the .gpi files in the current directory for common errors, such
#        as specification of the terminal or output file inside of the gpi file
#        itself.
#
#    _dependency_graph:
#        Outputs a .dot file to stdout that represents a graph of LaTeX
#        dependencies.  To see it, use the _show_dependency_graph target or
#        direct the output to a file, run dot on it, and view the output, e.g.:
#
#        make _dependency_graph > graph.dot
#        dot -T ps -o graph.eps graph.dot
#        gv graph.eps
#
#    _show_dependency_graph:
#        Makes viewing the graph simple: extracts, builds and displays the
#        dependency graph given in the _dependency_graph target using the value
#        of the environment-overridable VIEW_POSTSCRIPT variable (currently set
#        to $(VIEW_POSTSCRIPT)).  The postscript viewer is used because it
#        makes it easier to zoom in on the graph, a critical ability for
#        something so dense and mysterious.
#
#    _all_sources:
#        List all .tex files in this directory.
#
#    _sources:
#        Print out a list of all compilable sources in this directory.  This is
#        useful for determining what make thinks it will be using as the
#        primary source for 'make all'.
#
#    _scripts:
#        Print out a list of scripts that make knows can be used to generate
#        .tex files (described later).
#
#    _all_stems:
#        Print a list of stems.  These represent bare targets that can be
#        executed.  Listing <stem> as a bare target will produce <stem>.pdf.
#
#    _includes:
#        A list of .d files that would be included in this run if _includes
#        weren't specified.  This target may be used alone or in conjunction
#        with other targets.
#
#    _graphic_outputs:
#        A list of all generated .eps files
#
#    _env:
#        A list of environment variables and their values.  If supported by
#        your version of make, also a list of variables known to make.
#
# FILE TARGETS:
#
#    %, %.pdf:
#        Build a PDF file from the corresponding %.tex file.
#
#        If BUILD_STRATEGY=pdflatex, then this builds the pdf directly.
#        Otherwise, it uses this old-school but effective approach:
#
#            latex -> dvips -> ps2pdf
#
#        The BUILD_STRATEGY can be overridden in Makefile.ini in the same
#        directory.  The default is pdflatex.
#
#        Reasons for using latex -> dvips include the "psfrag" package, and the
#        generation of postscript instead of PDF.  Arguments for using pdflatex
#        include "new and shiny" and "better supported."  I can't argue with
#        either of those, and supporting them both didn't turn out to be that
#        difficult, so there you have it.  Choices.
#
#    %._show:
#        A phony target that builds the pdf file and then displays it using the
#        environment-overridable value of VIEW_PDF ($(VIEW_PDF)).
#
#    %._graphics:
#        A phony target that generates all graphics on which %.pdf (or %.dvi)
#        depends.
#
#    %.ps (only for BUILD_STRATEGY=latex):
#        Build a Postscript file from the corresponding %.tex file.
#        This is done using dvips.  Paper size is automatically
#        extracted from the declaration
#
#        \documentclass[<something>paper]
#
#        or it is the system default.
#
#        If using beamer (an excellent presentation class), the paper
#        size is ignored.  More on this later.
#
#    %.dvi (only for BUILD_STRATEGY=latex):
#        Build the DVI file from the corresponding %.tex file.
#
#    %.ind:
#        Build the index for this %.tex file.
#
#    %.gls:
#        Build the nomenclature glossary for this %.tex file.
#
#    %.nls:
#        Build the (newer) nomenclature file for this %.tex file.
#
#    %.eps:
#        Build an eps file from one of the following file types:
#
#       .dot    : graphviz
#       .gpi    : gnuplot
#       .fig    : xfig
#       .xvg    : xmgrace
#       .svg    : scalable vector graphics (goes through inkscape)
#       .png    : png (goes through NetPBM)
#       .jpg      : jpeg (goes through ImageMagick)
#       .eps.gz : gzipped eps
#
#       The behavior of this makefile with each type is described in
#       its own section below.
#
#    %.pstex{,_t} (only for BUILD_STRATEGY=latex):
#       Build a .pstex_t file from a .fig file.
#
# FEATURES:
#
#    Optional Binary Directory:
#        If you create the _out_ directory in the same place as the makefile,
#        it will automatically be used as a dumping ground for .pdf (or .dvi,
#        .ps, and .pdf) output files.
#
#        Alternatively, you can set the BINARY_TARGET_DIR variable, either as a
#        make argument or in Makefile.ini, to point to your directory of
#        choice.  Note that no pathname wildcard expansion is done in the
#        makefile, so make sure that the path is complete before going in
#        there.  E.g., if you want to specify something in your home directory,
#        use $$HOME/ instead of ~/ so that the shell expands it before it gets
#        to the makefile.
#
#    External Program Dependencies:
#        Every external program used by the makefile is represented by an
#        ALLCAPS variable at the top of this file.  This should allow you to
#        make judgments about whether your system supports the use of this
#        makefile.  The list is available in the ALL_PROGRAMS variable and,
#        provided that you are using GNU make 3.80 or later (or you haven't
#        renamed this file to something weird like "mylatexmakefile" and like
#        invoking it with make -f) can be viewed using
#
#        make _all_programs
#
#        Additionally, the availability of these programs can be checked
#        automatically for you by running
#
#        make _check_programs
#
#        The programs are categorized according to how important they are and
#        what function they perform to help you decide which ones you really
#        need.
#
#    Colorized Output:
#        The output of commands is colorized to highlight things that are often
#        important to developers.  This includes {underfull,overfull}
#        {h,v}boxes, general LaTeX Errors, each stage of document building, and
#        the number of pages in the final document.  The colors are obtained
#        using 'tput', so colorization should work pretty well on any terminal.
#
#        The colors can be customized very simply by setting any of the
#        LATEX_COLOR_<CONTEXT> variables in your environment (see above).
#
#    Predecessors to TeX Files:
#        Given a target <target>, if no <target>.tex file exists but a
#        corresponding script or predecessor file exists, then appropriate
#        action will be taken to generate the tex file.
#
#        Currently supported script or predecessor languages are:
#
#        sh:     %.tex.sh
#        perl:   %.tex.pl
#        python: %.tex.py
#
#           Calls the script using the appropriate interpreter, assuming that
#           its output is a .tex file.
#
#           The script is called thus:
#
#              <interpreter> <script file name> <target tex file>
#
#           and therefore sees exactly one parameter: the name of the .tex
#           file that it is to create.
#
#           Why does this feature exist?  I ran into this while working on
#           my paper dissertation.  I wrote a huge bash script that used a
#           lot of sed to bring together existing papers in LaTeX.  It
#           would have been nice had I had something like this to make my
#           life easier, since as it stands I have to run the script and
#           then build the document with make.  This feature provides hooks
#           for complicated stuff that you may want to do, but that I have
#           not considered.  It should work fine with included dependencies,
#           too.
#
#           Scripts are run every time make is invoked.  Some trickery is
#           employed to make sure that multiple restarts of make don't cause
#           them to be run again.
#
#        reST: %.rst
#
#           Runs the reST to LaTeX converter to generate a .tex file
#           If it finds a file names _rststyle_._include_.tex, uses it as
#           the "stylesheet" option to rst2latex.
#
#           Note that this does not track sub-dependencies in rst files.  It
#           assumes that the top-level rst file will change if you want a
#           rebuild.
#
#    Dependencies:
#
#        In general, dependencies are extracted directly from LaTeX output on
#        your document.  This includes
#
#        *    Bibliography information
#        *    \include or \input files (honoring \includeonly, too)
#        *    Graphics files inserted by the graphicx package
#
#        Where possible, all of these are built correctly and automatically.
#        In the case of graphics files, these are generated from the following
#        file types:
#
#        GraphViz:      .dot
#        GNUPlot:       .gpi
#        XFig:          .fig
#        XMgrace:       .xvg
#        SVG:           .svg
#        PNG:           .png
#        JPEG:          .jpg
#        GZipped EPS:   .eps.gz
#
#        If the file exists as a .eps already, it is merely used (and will not
#        be deleted by 'clean'!).
#
#        LaTeX and BibTeX are invoked correctly and the "Rerun to get
#        cross-references right" warning is heeded a reasonable number of
#        times.  In my experience this is enough for even the most troublesome
#        documents, but it can be easily changed (if LaTeX has to be run after
#        BibTeX more than three times, it is likely that something is moving
#        back and forth between pages, and no amount of LaTeXing will fix
#        that).
#
#        \includeonly is honored by this system, so files that are not
#        specified there will not trigger a rebuild when changed.
#
#    Beamer:
#        A special TeX source comment is recognized by this makefile (only when
#        BUILD_STRATEGY=latex, since this invokes psnup):
#
#        %%[[:space:]]*BEAMER[[:space:]]*LARGE
#
#        The presence of this comment forces the output of dvips through psnup
#        to enlarge beamer slides to take up an entire letter-sized page.  This
#        is particularly useful when printing transparencies or paper versions
#        of the slides.  For some reason landscape orientation doesn't appear
#        to work, though.
#
#        If you want to put multiple slides on a page, use this option and then
#        print using mpage, a2ps, or psnup to consolidate slides.  My personal
#        favorite is a2ps, but your mileage may vary.
#
#        When beamer is the document class, dvips does NOT receive a paper size
#        command line attribute, since beamer does special things with sizes.
#
#    GNUPlot Graphics:
#        When creating a .gpi file, DO NOT INCLUDE the "set terminal" or "set
#        output" commands!  The makefile will include terminal information for
#        you.  Besides being unnecessary and potentially harmful, including the
#        terminal definition in the .gpi file makes it harder for you, the one
#        writing the document, to preview your graphics, e.g., with
#
#           gnuplot -persist myfile.gpi
#
#        so don't do specify a terminal or an output file in your .gpi files.
#
#        When building a gpi file into an eps file, there are several features
#        available to the document designer:
#
#        Global Header:
#            The makefile searches for the files in the variable GNUPLOT_GLOBAL
#            in order:
#
#            ($(GNUPLOT_GLOBAL))
#
#            Only the first found is used.  All .gpi files in the directory are
#            treated as though the contents of GNUPLOT_GLOBAL were directly
#            included at the top of the file.
#
#            NOTE: This includes special comments! (see below)
#
#        Font Size:
#            A special comment in a .gpi file (or a globally included file) of
#            the form
#
#            ## FONTSIZE=<number>
#
#            will change the font size of the GPI output.  If font size is
#            specified in both the global file and the GPI file, the
#            specification in the individual GPI file is used.
#
#        Grayscale Output:
#            GNUplot files also support a special comment to force them to be
#            output in grayscale *no matter what*:
#
#            ## GRAY
#
#            This is not generally advisable, since you can always create a
#            grayscale document using the forms mentioned above.  But, if your
#            plot simply must be grayscale even in a document that allows
#            colors, this is how you do it.
#
#    XFig Graphics:
#            No special handling is done with XFig, except when a global
#            grayscale method is used, e.g.
#
#                make GRAY=1 document
#
#            In these cases the .eps files is created using the -N switch to
#            fig2dev to turn off color output.  (Only works with eps, not pstex
#            output)
#
#    GraphVis Graphics:
#            Color settings are simply ignored here.  The 'dot' program is used
#            to transform a .dot file into a .eps file.
#
#            If you want, you can use the dot2tex program to convert dot files
#            to tex graphics.  The default is to just call dot2tex with no
#            arguments, but you can change the DOT2TEX definition to include
#            options as needed (in your Makefile.ini).
#
#            Note that, as with pstex, the makefile cannot use latex's own
#            output to discover all missing dot_t (output) files, since anytime
#            TeX includes TeX, it has to bail when it can't find the include
#            file.  It can therefore only stop on the first missing file it
#            discovers, and we can't get a large list of them out easily.
#
#            So, the makefile errors out if it's missing an included dot_t
#            file, then prompts the user to run this command manually:
#
#                make all-dot2tex
#
#    GZipped EPS Graphics:
#
#        A .eps.gz file is sometimes a nice thing to have.  EPS files can get
#        very large, especially when created from bitmaps (don't do this if you
#        don't have to).  This makefile will unzip them (not in place) to
#        create the appropriate EPS file.
#
#
endef

#
# DEPENDENCY CHART:
#
# digraph "g" {
#     rankdir=TB
#     size="9,9"
#     edge [fontsize=12 weight=10]
#     node [shape=box fontsize=14 style=rounded]
#
#     eps [
#         shape=Mrecord
#         label="{{<gpi> GNUplot|<epsgz> GZip|<dot> Dot|<fig> XFig}|<eps> eps}"
#         ]
#     pstex [label="%.pstex"]
#     pstex_t [label="%.pstex_t"]
#     tex_outputs [shape=point]
#     extra_tex_files [shape=point]
#     gpi_data [label="<data>"]
#     gpi_includes [label="_include_.gpi"]
#     aux [label="%.aux"]
#     fls [label="%.fls"]
#     idx [label="%.idx"]
#     glo [label="%.glo"]
#     ind [label="%.ind"]
#     log [label="%.log"]
#     tex_sh [label="%.tex.sh"]
#     rst [label="%.rst"]
#     tex [
#         shape=record
#         label="<tex> %.tex|<include> _include_.tex"
#         ]
#     include_aux [label="_include_.aux"]
#     file_bib [label=".bib"]
#     bbl [label="%.bbl"]
#     dvi [label="%.dvi"]
#     ps [label="%.ps"]
#     pdf [label="%.pdf"]
#     fig [label=".fig"]
#     dot [label=".dot"]
#     gpi [label=".gpi"]
#     eps_gz [label=".eps.gz"]
#
#     gpi_files [shape=point]
#
#     rst -> tex:tex [label="reST"]
#     tex_sh -> tex:tex [label="sh"]
#     tex_pl -> tex:tex [label="perl"]
#     tex_py -> tex:tex [label="python"]
#     tex -> tex_outputs [label="latex"]
#     tex_outputs -> dvi
#     tex_outputs -> aux
#     tex_outputs -> log
#     tex_outputs -> fls
#     tex_outputs -> idx
#     tex_outputs -> include_aux
#     aux -> bbl [label="bibtex"]
#     file_bib -> bbl [label="bibtex"]
#     idx -> ind [label="makeindex"]
#     glo -> gls [label="makeindex"]
#     nlo -> nls [label="makeindex"]
#     gls -> extra_tex_files
#     nls -> extra_tex_files
#     ind -> extra_tex_files
#     bbl -> extra_tex_files
#     eps -> extra_tex_files
#     extra_tex_files -> dvi [label="latex"]
#     gpi_files -> eps:gpi [label="gnuplot"]
#     gpi -> gpi_files
#     gpi_data -> gpi_files
#     gpi_includes -> gpi_files
#     eps_gz -> eps:epsgz [label="gunzip"]
#     fig -> eps:fig [label="fig2dev"]
#     fig -> pstex [label="fig2dev"]
#     fig -> pstex_t [label="fig2dev"]
#     pstex -> pstex_t [label="fig2dev"]
#     dot -> eps:dot [label="dot"]
#     dvi -> ps [label="dvips"]
#     include_aux -> bbl [label="bibtex"]
#     ps -> pdf [label="ps2pdf"]
#
#     edge [ color=blue label="" style=dotted weight=1 fontcolor=blue]
#     fls -> tex:include [label="INPUT: *.tex"]
#     fls -> file_bib [label="INPUT: *.aux"]
#     aux -> file_bib [label="\\bibdata{...}"]
#     include_aux -> file_bib [label="\\bibdata{...}"]
#     log -> gpi [label="Graphic file"]
#     log -> fig [label="Graphic file"]
#     log -> eps_gz [label="Graphic file"]
#     log -> dot [label="Graphic file"]
#     log -> idx [label="No file *.ind"]
#     log -> glo [label="No file *.gls"]
#     log -> nlo [label="No file *.nls"]
#     gpi -> gpi_data [label="plot '...'"]
#     gpi -> gpi_includes [label="load '...'"]
#     tex:tex -> ps [label="paper"]
#     tex:tex -> pdf [label="embedding"]
# }
#

#
# DEPENDENCY CHART SCRIPT
#
# $(call output_dependency_graph,[<output file>])
define output-dependency-graph
	if [ -f '$(this_file)' ]; then \
	$(SED) \
		-e '/^[[:space:]]*#[[:space:]]*DEPENDENCY CHART:/,/^$$/!d' \
		-e '/DEPENDENCY CHART/d' \
		-e '/^$$/d' \
		-e 's/^[[:space:]]*#//' \
		$(this_file) $(if $1,> '$1',); \
	else \
		$(ECHO) "Cannot determine the name of this makefile."; \
	fi
endef
#
.PHONY: Targets.ini $(HOME)/.latex-makefile/Targets.ini
-include Targets.ini
-include $(HOME)/.latex-makefile/Targets.ini
#
# vim: noet sts=0 sw=8 ts=8



==> abstract.tex <==
%\subsection*{Abstract}
%\begin{abstract}
%\abstract
%\pg{Needs to be changed. Should be lesser than 200 words as per guidelines.}

This paper introduces Nimbus, a robust technique to detect whether the cross traffic competing with a flow is ``elastic'', and shows that this elasticity detector improves congestion control. If cross traffic is inelastic, then the sender can control queueing delays while achieving high throughput, but otherwise it should not attempt to control packet delay. Nimbus modulates the flow's rate with sinusoidal pulses that create small traffic fluctuations at the bottleneck link, and it estimates elasticity from the frequency response (FFT) of the rate of the cross traffic.  Our results on emulated and real-world paths show that congestion control using elasticity detection  achieves throughput comparable to or better than Cubic, but with delays that are much lower when cross traffic is inelastic (50--70 ms lower in our experiments on average). Compared to Copa, \name detects the nature of the cross traffic more accurately (as a result, in a typical experiment, it achieves 45\% higher throughput at similar delay); and unlike Copa, Nimbus can be used as a building block by other end-to-end algorithms.

%This paper develops a techniqhat ue to detect whether the cross traffic competing with a flow is elastic or not, and shows how to use the elasticity detector to improve congestion control. If the cross traffic is elastic, i.e., made up of flows like Cubic or NewReno that increase their rate to fill up all available bandwidth, then one should use a scheme that competes well with such traffic. Such a scheme will not be able to control delays because the cross traffic will not cooperate to maintain low delays. If, however, cross traffic is inelastic, then one can use a suitable delay-controlled algorithm.

%Our elasticity detector uses an asymmetric sinusoidal pulse pattern and estimates elasticity by computing the frequency response (FFT) of the cross traffic estimate; we have measured its accuracy to be over 90\%. We present the design and evaluation of \name, a congestion control protocol that uses the elasticity detector to switch between delay-control and TCP-competitive modes. Our results on emulated and real-world paths show that Nimbus achieves throughput comparable to or better than Cubic always, but with delays that are much lower when cross traffic is inelastic. Unlike BBR, \name is fair to Cubic, and has significantly lower delay by 40-50 ms. Compared to Copa, which also switches between a delay-controlling and a TCP-competitive mode, \name is more robust at correctly detecting the nature of cross traffic, and unlike Copa, it is usable by a variety of delay-based and TCP-competitive methods.

==> concl.tex <==
\newcommand{\conclsec}{Conclusion}
\section{\conclsec}
\label{s:concl}
This paper showed a method for detecting the elasticity of cross traffic and showed that it is a useful building block for congestion control. The detection technique uses a carefully constructed asymmetric sinusoidal pulse and observes the frequency response of cross traffic rates at a sender. We presented several controlled experiments to demonstrate its robustness and accuracy. Elasticity detection enables protocols to combine the best aspects of delay-control methods with TCP-competitiveness. We found that our proposed methods are beneficial not only on a variety of emulated conditions that model realistic workloads, but also on a collection of 25 real-world Internet paths.

\textbf{This work does not raise any ethical issues.}\\
\if 0

using two distinct modes in end-to-end congestion control for traffic aggregates. By taking advantage of the persistence of traffic in a bundle, we showed how to estimate the volume and the elasticity of cross traffic. These estimators allow \name to pick the best mode in which to operate: with inelastic traffic, the delay-control rule achieves high throughput while maintaining delays near a specified threshold, and with elastic cross traffic, the TCP-competitive mode emulates the behavior of a specified number of elastic long-running flows.

%To our knowledge, \name is the first scheme that achieves low delays whenever possible and throughput competitive with buffer-filling TCPs.

There are important directions for future work. First, how should \name be modified to allow multiple concurrent bundles to share bandwidth equitably with each other and with other competing traffic? Second, how best to detect elasticity for non-ACK-clocked traffic (e.g., BBR)? Third, how high must the access link rate be compared to the bottleneck rate for the methods we have proposed to be effective? Fourth, are there other ways to modulate transmissions on pulses to detect cross traffic that can handle access rates that are lower than 25\% of the bottleneck link rate. And last but not least, how to improve performance on paths with rate policers that drop packets (some of our experiments are on such paths) and on paths with active queue management schemes?

\fi



==> cover.tex <==
% -*-latex-*-
% 
% For questions, comments, concerns or complaints:
% thesis@mit.edu
% 
%
% $Log: cover.tex,v $
% Revision 1.8  2008/05/13 15:02:15  jdreed
% Degree month is June, not May.  Added note about prevdegrees.
% Arthur Smith's title updated
%
% Revision 1.7  2001/02/08 18:53:16  boojum
% changed some \newpages to \cleardoublepages
%
% Revision 1.6  1999/10/21 14:49:31  boojum
% changed comment referring to documentstyle
%
% Revision 1.5  1999/10/21 14:39:04  boojum
% *** empty log message ***
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.3  93/05/17  17:06:29  starflt
% Added acknowledgements section (suggested by tompalka)
% 
% Revision 1.2  92/04/22  13:13:13  epeisach
% Fixes for 1991 course 6 requirements
% Phrase "and to grant others the right to do so" has been added to 
% permission clause
% Second copy of abstract is not counted as separate pages so numbering works
% out
% 
% Revision 1.1  92/04/22  13:08:20  epeisach

% NOTE:
% These templates make an effort to conform to the MIT Thesis specifications,
% however the specifications can change.  We recommend that you verify the
% layout of your title page with your thesis advisor and/or the MIT 
% Libraries before printing your final copy.
\title{Elasticity Detection: A Building Block for  Delay-Sensitive Congestion Control}

\author{Prateesh Goyal}
% If you wish to list your previous degrees on the cover page, use the 
% previous degrees command:
%       \prevdegrees{A.A., Harvard University (1985)}
% You can use the \\ command to list multiple previous degrees
%       \prevdegrees{B.S., University of California (1978) \\
%                    S.M., Massachusetts Institute of Technology (1981)}
\department{Department of Electrical Engineering and Computer Science}

% If the thesis is for two degrees simultaneously, list them both
% separated by \and like this:
% \degree{Doctor of Philosophy \and Master of Science}
\degree{Master of Science in Computer Science and Engineering}

% As of the 2007-08 academic year, valid degree months are September, 
% February, or June.  The default is June.
\degreemonth{June}
\degreeyear{2018}
\thesisdate{May 22, 2018}

%% By default, the thesis will be copyrighted to MIT.  If you need to copyright
%% the thesis to yourself, just specify the `vi' documentclass option.  If for
%% some reason you want to exactly specify the copyright notice text, you can
%% use the \copyrightnoticetext command.  
%\copyrightnoticetext{\copyright IBM, 1990.  Do not open till Xmas.}

% If there is more than one supervisor, use the \supervisor command
% once for each.
\supervisor{Hari Balakrishnan}{Fujitsu Chair Professor}
\supervisor{Mohammad Alizadeh}{Assistant Professor}

% This is the department committee chairman, not the thesis committee
% chairman.  You should replace this with your Department's Committee
% Chairman.
\chairman{Professor Leslie A. Kolodziejski}{Chair, Department Committee on Graduate Theses}

% Make the titlepage based on the above information.  If you need
% something special and can't use the standard form, you can specify
% the exact text of the titlepage yourself.  Put it in a titlepage
% environment and leave blank lines where you want vertical space.
% The spaces will be adjusted to fill the entire page.  The dotted
% lines for the signatures are made with the \signature command.
\maketitle

% The abstractpage environment sets up everything on the page except
% the text itself.  The title and other header material are put at the
% top of the page, and the supervisors are listed at the bottom.  A
% new page is begun both before and after.  Of course, an abstract may
% be more than one page itself.  If you need more control over the
% format of the page, you can use the abstract environment, which puts
% the word "Abstract" at the beginning and single spaces its text.

%% You can either \input (*not* \include) your abstract file, or you can put
%% the text of the abstract directly between the \begin{abstractpage} and
%% \end{abstractpage} commands.

% First copy: start a new page, and save the page number.
\cleardoublepage
% Uncomment the next line if you do NOT want a page number on your
% abstract and acknowledgments pages.
% \pagestyle{empty}
\setcounter{savepage}{\thepage}
\begin{abstractpage}
\input{abstract}
\end{abstractpage}

% Additional copy: start a new page, and reset the page number.  This way,
% the second copy of the abstract is not counted as separate pages.
% Uncomment the next 6 lines if you need two copies of the abstract
% page.
% \setcounter{page}{\thesavepage}
% \begin{abstractpage}
% \input{abstract}
% \end{abstractpage}

%\cleardoublepage

%\section*{Acknowledgments}

%This is the acknowledgements section.  You should replace this with your
%own acknowledgements.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -*-latex-*-


==> delay_control_law.tex <==
\vspace{-5pt}
\newcommand{\delayrulesec}{Delay-Control Mode}
\section{\delayrulesec}
\label{s:delaymode}\label{s:delay-control}
\vspace{-5pt}

\begin{figure}[t]
	\includegraphics[width=\columnwidth]{images/delay_control}
    \caption{\small{{\bf Achieving low delays---}all algorithms achieve close to the spare capacity in throughput, while Nimbus and Vegas achieve low delays as well. The delay axis (vertical) is inverted; better performance is up and to the right.
    Nimbus can be configured for even lower delays at the expense of slightly reduced throughput.
    }}
	\label{fig:delaymode-inelastic}
\end{figure}

The goal of the delay-control rule is to 
achieve high throughput while 
maintaining a specified threshold queueing delay, $d_t >0$. We target such a delay because it allows \name to achieve high utilization and also helps estimate the cross traffic, $z(t)$, accurately. For ease of explanation,
we assume that the path from sender to receiver has only one bottleneck link; the scheme works even otherwise.
%and that this bottleneck is also has the smallest link rate 
%\footnote{In general, the bottleneck link, which is the link where queues are non-zero on the path, need not be the %one with minimum link capacity. \name{} does not, but we do not evaluate this experimentally.} along the path.
%We relax this restriction later.
%Denote the capacity of the bottleneck link by $\mu$. 
In general, the bottleneck link rate $\mu$ could change with time (e.g., a wireless link),
but we assume here that it is constant (i.e., a typical wired link). 

The delay-control rule has two terms. The first term uses the estimate of $z(t)$ to infer the {\em spare capacity} and transmits at a rate proportional to this quantity. The second term adjusts the transmission rate in proportion to the difference between the measured delay and the specified delay threshold.

\Para{Spare capacity term.} The sender, currently sending at rate $R(t)$, estimates the spare capacity as
\begin{equation}
s(t) = 
    \mu 
    - z(t) 
    - R(t) 
= \mu \left(1 - \frac{R(t)}{\Routt}\right)
\label{eq:s}
\end{equation}
Then, the first term in the delay-control rule is a rate update at time $t+\delta$, where $\delta \geq \mbox{RTT}$:
\begin{equation}
  R(t + \delta) = R(t) + \alpha s(t),
\label{eq:spare}
\end{equation}
where $\alpha$ is a step parameter that determines the swiftness with which to move toward $s(t)$.
%

\if 0
A high $\alpha$ can destabilize the system, a low $\alpha$ means slower
convergence.  Since our measurement estimates are delayed by at
least 1 round-trip time (RTT), $\delta > \mbox{RTT}$.
\fi

An equivalent interpretation of the update rule in Eq.~(\ref{eq:spare}) is 
as an exponentially weighted moving average (EWMA) filter because it may be rewritten as 
\begin{equation}
R(t + \delta) = (1 - \alpha) R(t) + \alpha (\mu - z(t)).
\label{eq:ewmaspare}
\end{equation}
The intuition is that we would like $R(t)$ to converge toward $\mu - z$. 
An EWMA is a standard approach used in many similar network estimation problems, and is a natural method in our context.

\Para{Threshold delay term.} Eq.~(\ref{eq:ewmaspare}) is insufficient because with stochastic traffic, a sender pushing the total offered load to $\mu$ would cause buffers to fill. Moreover, if the measured delays are lower than the threshold, the cross-traffic estimator may not produce correct results. In both cases, a term that forces the delay toward the threshold addresses the problems. 

%rule whose goal is to trigger a rate reduction when the queueing delay exceeds a {\em threshold delay}, $d_t$.

Denoting the minimum RTT by $x_p$ and the current RTT by $x_t$, the simplest such term is proportional to $d_t +x_p - x(t)$. This gives the \name{} delay-control rule:
\begin{equation}
R(t+\delta) = 
    R(t) 
    + \alpha s(t)
    + \beta\frac{\mu}{\delta}
        (d_t + x_p - x(t)).
\label{eq:delayrule1}
\end{equation}
The second term with the $\beta$ factor is scaled by $\delta$ to make it unitless.
%and move the bound for stability closer to $1$. 
%While we don't provide a proof for the stability of this control rule, 
Previous work (XCP~\cite{xcp} and RCP~\cite{rcpstable}) has established stability bounds on $\alpha$ and $\beta$ for nearly identical control laws.

Note that this scheme provides a good estimate of $s(t)$ only when the
bottleneck queue is non-empty, so a non-zero threshold delay is important
for high utilization. 
%Setting the threshold to strictly 0 would not work
%well, as we demonstrate in our evaluation. 
This delay-control rule causes the RTT ($x(t)$) to hover around 
$d_t+x_p$. Because $d_t > 0$, this rule ensures high
bottleneck link utilization.

\Fig{delaymode-inelastic} shows this method's ability to hold delays across three cross-traffic rates on a 96 Mbit/s path with 50 ms RTT and a bottleneck buffer of twice the bandwidth-delay product (BDP). 
We show \name with two different target queueing delay settings, $d_{t}$ = 5 ms and $d_{t}$ = 12.5 ms, with cross traffic occupying 25\%, 50\%, and 75\% of the bottleneck rate. Nimbus and Vegas outperform the other protocols in these experiments.

BBR kept the queue size between 1 and 1.5 BDP throughout the experiment; we believe that with cross traffic, BBR over-estimated the available capacity and BDP, which caused it to build up queues. We observed that with no cross traffic, BBR did not have this problem, a similar finding to a recent study~\cite{hockexperimental}.


\cut{For this delay-control rule to work the sender need not have a precise
estimate of $\mu$. An imprecise estimate $\hat \mu$ is equivalent to
scaling down the $\alpha$ and $\beta$ factors by $\frac{\hat
  \mu}{\mu}$. We can estimate $\hat \mu$ by using the packet train
method~\cite{packettrain} or even by crudely using $\hat \mu = R(t)$.
}

\cut{
\subsection{Estimating \textit{x}}

We present here a simple new method to estimate $x$ (or more
precisely, $x_p - x$), required by Eq. (\ref{eq:delayrule}).  All prior
techniques used in protocols that require the one-way delay end up
using the {\em round-trip time}, because they cannot assume that the
sender and receiver clocks are synchronized on the
Internet. Unfortunately, using the RTT implies that the protocol is
now sensitive to traffic or congestion on the reverse path. Similarly, calculating $R_{out}$ based on received time of packets at the sender makes our estimation sensitive to congestion on the reverse paths.

Suppose that the sender and receiver clocks are not synchronized and
the clock times differ by $\eta$ seconds. The sender includes a
timestamp $s_{i}$ whenever a packet is sent, and the receiver echoes
this timestamp to the sender in its ACK for packet $i$. The receiver
also adds its own timestamp, $r_{i}$, to the ACK corresponding the
received packet. Let $\hat{x}_{i}$ be the calculated one-way delay of packet $i$, i.e.,
\begin{equation}
\hat{x}_{i}
\label{eq:x} = r_{i} - s_{i}
\end{equation}

Note that $x_p$ is estimated as $\min_{i} \hat {x}_i$. Hence, both the
estimate of $x_p$ and our estimate of $x$ are off by the same constant
amount, $\eta$, which implies that $d_t + x_p - x$ may be correctly
estimated using $\hat{x}$ using Eq. (\ref{eq:x}).
}

==> elasticity.tex <==
\newcommand{\switchsec}{Cross-Traffic Estimation}
\section{\switchsec}
\label{s:switching}

%Nimbus estimates both the volume and elasticity of cross traffic. It uses the volume in two places: first, to determine the time-series of cross traffic $z(t)$ to use in the mode-switching algorithm, and second, to use in the delay-control algorithm. 
%In addition, Nimbus introduces an estimator to infer whether elastic flows are a significant contributor to the cross traffic and to decide whether to run in delay-control or TCP-competitive mode.

%In addition, Nimbus introduces an estimator to infer whether elastic flows are a significant contributor to the cross traffic and to decide whether to run in delay-control or TCP-competitive mode.

We present a simple method to estimate the total rate of cross traffic (\S\ref{s:zrate}) at the sender. Then, we show how to detect whether the cross traffic contains {\em any} ACK-clocked elastic flows, describing the key principles (\S\ref{s:zelasticity}) and a practical method (\S\ref{sec:pracelas}). 

Figure~\ref{fig:sysmod} shows our network model and introduces some notation. A sender communicates with a receiver over a single bottleneck link of rate $\mu$. The bottleneck link is shared with cross traffic, consisting of an unknown number of flows, each of which is either elastic or inelastic. $S(t)$ and $R(t)$ denote the time-varying sending and receiving rates, respectively, while $z(t)$ is the total rate of the cross traffic. We assume that the sender knows $\mu$, and can use prior work to estimate it ($\S$\ref{s:implementation}).

%Our cross traffic estimation technique requires some degree of traffic persistence. The sender must be able to create sufficient traffic variations  %(e.g., burst at 20\% of the bottleneck capacity for a short period)
%and observe the impact on cross traffic over a period of time. Hence it is best suited for control of large flows, such as large file downloads, data backups to the cloud, etc. Fortunately, it is precisely for such transfers that delay-controlling schemes can provide the most benefit, since short flows are unlikely to cause bufferbloat~\cite{bufferbloat}. 


%A flow is elastic if three conditions hold: (i) its rate is limited by the TCP congestion window, (ii) its transmissions are ACK-clocked, and (iii) the congestion window increases on each ACK or every RTT as long as there is no indication of congestion. Otherwise, it is inelastic. 


%The sender can estimate $\mu$ using prior techniques~\cite{packettrain, dovrolis2001packet, downey1999using, lai2000measuring, jacobson1997pathchar, lai2001nettimer, mar2000pchar}.

%Our  which it can estimate using prior techniques~\cite{}. 

%but we describe how to estimate $\mu$ using a small modification to prior techniques in \S\ref{s:implementation}.

%\vspace{-5pt}
\subsection{Estimating the Rate of Cross Traffic}
\label{s:zrate}

%We estimate $z(t)$ using the estimator
%\vspace{5pt}
%\abovedisplayskip
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/sys_model2.pdf}
    \vspace{-2mm}
    \caption{\small{{\bf Network model.} 
    The time-varying total rate of cross traffic is $z(t)$. The bottleneck link rate is $\mu$. The sender's transmission rate is $S(t)$, and the rate of traffic received by the receiver is $R(t)$.}}
    \label{fig:sysmod}
    \vspace{-4.5mm}
\end{figure}

%\vspace{-3mm}
See \Fig{sysmod}. The total traffic into the bottleneck queue is $S(t) + z(t)$, of which the receiver sees $R(t)$. As long as the bottleneck link is busy (\ie its queue is not empty), and the router treats all traffic the same way, the ratio of $R(t)$ to $\mu$ must be equal to the ratio of $S(t)$ and the total incoming traffic, $S(t)+z(t)$. Using this property, we propose a new estimator for $z(t)$:
\begin{align} \label{eq:zfromR}
\hat{z}(t) &= \mu \frac{S(t)}{R(t)} - S(t).
\end{align}
%\belowdisplayskip
%\vspace{5pt}

%Thus, any protocol that keeps the bottleneck link always busy can estimate $z(t)$ using Eq.~\eqref{eq:zfromR}. 

%As we will see, both the delay-control and TCP-competitive modes in \name attempt to keep the bottleneck busy. 

%, the ratio of $\Rout$ to $\mu$ must be equal to the ratio of $R(t)$ and the total traffic.

We estimate $S(t)$ and $R(t)$ by considering $n$ packets at a time:
%\abovedisplayskip
%\vspace{-3mm}
\begin{equation} 
\centering
S_{i,i+n} = \frac{n_{bytes}} {s_{i+n} - s_i}, \qquad R_{i,i+n} = \frac{n_{bytes}} {r_{i+n} - r_i},
\label{eq:SR}
%\vspace{-1.5mm}
\end{equation}
%\belowdisplayskip
where $n_{bytes}$ is the number of bytes in the $n$ packets, $s_k$ is the time at which the sender sends packet $k$, $r_k$ is the time at which the sender receives the ACK for packet $k$, and the units of the rates are bytes per second. Note that $S(t)$ and $R(t)$ must be measured over the {\em same} $n$ packets.
%

\if 0
Using ACKs to calculate $r_{k}$ makes the $R(t)$ calculation sensitive to ACK compression. To mitigate this effect, we can use receiver timestamps to define $r_k$ as the time at which the receiver received packet $k$. This method is more accurate but requires that the receiver communicate $R(t)$ to the sender in ACKs. In our TCP-based implementation, we use ACK timestamps to avoid receiver modifications.
\fi

% Similarly,  $$R_{out(i,i+n)} = \frac{n} {r_{i+n} - r_i},$$
% where $r_k$ is the time at which the receiver receives packet $k$. \pg{Not sure if we should include this statement}We use receiver timestamps to calculate $\Rout$ to eliminate the effects of queueing and congestion on the reverse path.

We have conducted several tests with various patterns of cross traffic to evaluate the effectiveness of this $z(t)$ estimator. The overall error is small: the 50th and 95th percentiles of the relative error are 1.3\% and 7.5\%, respectively.
Unlike prior work on estimating cross-traffic rate~\cite{strauss2003measurement,jain2002pathload,hu2003evaluation}, our method is in-band and does not use any probe packets; it relies on the property that the sender is persistently backlogged.
%\ma{I think we can cut this.}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/cross_tfk_est.pdf}
%     \caption{\small{ \textbf{Cross traffic rate estimator.} $\hat{z}$ juxtaposed against ground truth ($z$). Our cross traffic estimate tracks the ground truth closely. The $50^{\text{th}}$ and $95^{\text{th}}$ percentiles of the relative error are only $1.3$\% and $7.5$\%, respectively. The cross traffic was  generated using a CAIDA trace~\cite{caida-dataset}. (See \S\ref{s:eval} for details.)}}
%     \label{fig:zestimateworks}
% \end{figure}


%\vspace{-10pt}
\subsection{Elasticity Detection: Principles}
\label{s:zelasticity}
\if 0
The problem of elasticity detection is to distinguish long-lived cross-traffic
flows (termed {\em elastic}), which compete aggressively for link bandwidth,
from short-lived flows (termed {\em inelastic}) that arrive and depart very
quickly with a small burst of packets. Nimbus should compete for its fair share
of bandwidth with elastic flows, but let the inelastic flows pass through
unharmed. 
\fi

We now turn to designing an online estimator for a sender to determine if the cross traffic includes {\em any} elastic flows.\footnote{Receiver participation will improve accuracy by avoiding the need to estimate $R(t)$ from ACKs at the sender, but would be a little harder to deploy.} A strawman approach might attempt to detect elastic flows by estimating the contribution of the cross traffic to queueing delay. For example, the sender can estimate its own contribution to the queueing delay---\ie the ``self-inflicted'' delay---and if the total delay is significantly higher than the self-inflicted delay, conclude that the cross traffic is elastic. 

 \begin{figure}[t]
     \centering
    \includegraphics[width=1.0\columnwidth]{images/overview-cubic2-sigcomm19.pdf}
    \vspace{-9mm}
     \caption{\small Instantaneous delay measurements do not reveal elasticity. The bottom plot shows the total queueing delay (orange) and the self-inflicted delay (green). \an{The experiment contains one background Cubic flow in the elastic region (30--90 s) and CBR cross traffic in the inelastic region (90--150 s).} \cut{The experiment is the same as \Fig{overview:cubic}. \pg{?????????}} }
     \label{fig:si-delay}
%     \vspace{-6mm}
 \end{figure}

% Added recently for arxiv submission

This scheme does not work. To see why, consider the experiment in Figure~\ref{fig:si-delay}, where a Cubic flow shares a link with elastic and inelastic  traffic in two separate time periods. The self-inflicted queueing delay for the Cubic flow (green, bottom figure) looks the same in the elastic and inelastic phases. The reason is that a flow's share of the queue occupancy is proportional to its throughput, which is roughly the same in the two phases (top figure). Because the Cubic flow gets 50\% of the bottleneck link, its self-inflicted delay is roughly half of the total queueing delay always (orange, bottom figure). This example suggests that instantaneous measurements cannot be used to distinguish between elastic and inelastic cross traffic. 
%This example suggests that no measurement at a single point in time can be used to reliably distinguish between elastic and inelastic cross traffic. 



\smallskip
\noindent{\bf To detect elasticity, tickle the cross traffic!} 
Our method detects elasticity by monitoring how the cross traffic responds to induced traffic variations at the bottleneck link over a period of time. The key observation is that elastic flows react in a predictable way to rate fluctuations at the bottleneck. Consider, for example, long-running Cubic or Reno flows, which are ACK-clocked. For these flows, if an ACK is delayed by a time duration $\delta$, then the next packet transmission will also be delayed by $\delta$. Therefore changes in the rate of packet arrivals at the receiver cause similar changes in the sending rate after one RTT via the ACKs. By contrast, the sending rate of inelastic flows does not depend on the receive rate.

%if the mean inter-arrival time between ACKs is $d$, adding an extra delay of $\delta$ on each ACK would reduce the flow's sending rate from $1/d$ to $1/(d+\delta)$ packets per second. 

We induce changes in the inter-packet spacing of cross traffic at the bottleneck link by sending packets in {\em pulses}. We take the desired sending rate, $S(t)$, and alternate between sending at rates higher and rates lower than $S(t)$, ensuring that the mean rate is $S(t)$. Sending in such pulses (e.g., modulated on a sinusoid) changes the inter-packet spacing of the cross traffic departing the bottleneck link in a controlled manner. If the cross traffic contains elastic flows, then because of the induced changes in the ACK clocks of those flows, their rates will react to our pulses. When we increase our rate, the elastic cross traffic will reduce its rate in the next RTT, and conversely. If enough of the cross traffic is elastic, then our sender can measure and detect these fluctuations in the cross traffic rate. 

%If enough of the cross-traffic flows are elastic, then because of the explicitly induced changes in the ACK clocks of those flows, they will react to the changed inter-packet time. In particular, when we increase our rate and transmit a burst, the elastic cross traffic will reduce its rate in the next RTT; the opposite will happen when we decrease our rate.

\Fig{ts:elastic} and \Fig{ts:inelastic} compare the responses of elastic (Cubic) and inelastic (constant bit rate) cross traffic when the sender transmits packets in sinusoisal pulses at frequency $f_p=5$~Hz. $S(t)$ is the sender's rate and $z(t)$ is the estimated cross traffic rate computed using Eq.~\eqref{eq:zfromR}. The path has a minimum RTT of 50 ms and a buffer size of 100 ms (2$\times$ the bandwidth-delay product). The elastic flow's sending rate after one RTT is inversely correlated with the pulses in the sending rate, while the inelastic flow's sending rate is unaffected.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=\columnwidth]{images/TimeSeries_TCP}
        \vspace{-6.5mm}
        \caption{\small Elastic cross traffic}
        \label{fig:ts:elastic}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=\columnwidth]{images/TimeSeries_Poisson}
        \vspace{-6.5mm}
        \caption{\small Inelastic cross traffic}
        \label{fig:ts:inelastic}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small{{\bf Cross traffic's reaction to pulses.} The pulses change the inter packet spacing for cross traffic. Elastic traffic reacts to these changes after a RTT. Inelastic cross traffic is agnostic to these changes.} }
    \label{fig:ts}
    \vspace{-6.5mm}
\end{figure}


%The problem, then, is to detect the presence of elastic cross traffic, $z$, by observing how cross traffic reacts to changes in Nimbus's sending rate. 

\subsection{Elasticity Detection: Practice}
\label{sec:pracelas}
\label{s:pracelas}

To produce a practical method to detect cross traffic using this idea, we must address three challenges:
\begin{CompactEnumerate}
\item Pulses in the sending rate must induce a measurable change in $z$, but not congest the bottleneck link.
\item Because there is natural variation in cross traffic, and noise in $\hat z$, it is not easy to perform a robust comparison between the predicted change in $z$ and the measured $z$. 
\item Because the sender does not know the RTTs of cross-traffic flows, it does not know when to look for the predicted response in the cross-traffic rate.
\end{CompactEnumerate}

The first method we developed to solve these problems measured the {\em cross-correlation} between $S(t)$ and $z(t)$.  A cross-correlation near zero would be considered inelastic cross traffic, whereas a significant non-zero value would indicate elastic cross traffic. 
We found that this approach works well (with square-wave pulses) if the cross traffic is substantially elastic and has a similar RTT to the flow trying to detect elasticity, but not otherwise. The trouble is that because elastic cross traffic will react after {\em its} RTT, $S(t)$ and $z(t)$ must be aligned using the cross traffic's RTT, which is not easy to infer. Moreover, the elastic flows in the cross traffic may have different RTTs, making the alignment even more challenging. % and rendering the method impractical.

\smallskip
\noindent {\bf From time to frequency domain.} We have developed a method that overcomes the three challenges stated above. It uses two ideas. First, the sender modulates its packet transmissions using {\em sinusoidal pulses} at a known frequency $f_p$, with amplitude equal to a modest fraction (e.g., 25\%) of the bottleneck link rate. 
These pulses induce a noticeable change in inter-packet times at the link without causing congestion, because the queues created in one part of the pulse are drained in the subsequent part, and the period of the pulses is short (e.g., $f_p = 5$~Hz). By using short pulses, we ensure that the total burst of data sent in a pulse is a small fraction of the typical bottleneck queue size. 

Second, the sender looks for periodicity in the cross traffic rate at frequency $f_p$, using a frequency domain representation of the cross-traffic rates. We use the Fast Fourier Transform (FFT) of the time series of the cross traffic estimate $\hat z(t)$ over a short time interval (\eg 5 seconds). Detecting periodicity in the frequency domain is more robust than the time-domain, for the same reason that frequency modulation provides better signal-to-noise ratio than amplitude modulation~\cite{rappaport1996wireless}: it is less affected by variations in the cross traffic rate and measurement noise. 
Further, observing the cross traffic's response at a known frequency, $f_p$, yields a method that is robust to the presence of multiple ACK-clocked flows with different RTTs. All the elastic flows in the cross traffic, irrespective of their RTTs and congestion control protocol, will exhibit rate oscillations at the frequency $f_p$. As a result, there will be an overall response at frequency $f_p$ in the cross traffic, equal to superposition of the responses of the individual elastic flows at frequency $f_p$.\footnote{In theory, the response of flows with different RTTs may cancel each other out, but this is very unlikely since it requires specific combinations of RTTs. We have not seen this problem occur in our experiments (\S\ref{s:robustness-synthetic}).} 
%\pg{Should we also highligh robustness to presence of inelastic cross traffic and why is it so?}

%spanning a short interval of time(Snapshot Length, 5 s in our experiments).
%, and turns out to be more robust than using any single cross-traffic rate estimate.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/FFT2}
    \vspace{-10mm}
    \caption{\small{{\bf Cross traffic FFT for elastic and inelastic traffic.} Only the FFT for elastic traffic has a pronounced peak at $f_p$ (5 Hz).}}
    \label{fig:fft}
    \vspace{-6mm}
\end{figure}

\Fig{fft} shows the FFT of the $\hat z(t)$ time-series produced using Eq.~(\ref{eq:zfromR}) for examples of elastic and inelastic cross traffic, respectively. Elastic cross traffic exhibits a pronounced peak at $f_p$ compared to the neighboring frequencies, while for inelastic traffic the FFT magnitude is spread across many frequencies. The magnitude of the peak depends on how much of the cross traffic is elastic; the more elastic the cross traffic, the sharper the peak at $f_p$. Therefore, rather than compare the peak at $f_p$ to a pre-determined threshold, we compare it to the magnitude of the nearby frequencies. 

We define the {\em elasticity metric}, $\eta$, as follows:
\if 0 
\begin{equation} 
\centering
\eta = \frac{|FFT_{z}(f_{p})|}{\max_{f_{p} < f < 2f_{p}} |FFT_{z}(f)|}.
\label{eq:elasticity}
\end{equation}
\fi
%\abovedisplayskip
%\vspace{-3mm}
\begin{equation} 
\centering
\eta = \frac{|FFT_{z}(f_{p})|}{\max_{f \in (f_p,2f_{p})} |FFT_{z}(f)|}
\label{eq:elasticity}
%\vspace{-1mm}
\end{equation}
%\belowdisplayskip

Eq.~\eqref{eq:elasticity} compares the magnitude of the FFT at frequency $f_{p}$ to the peak magnitude in the range from just above $f_{p}$ to just below $2f_{p}$. 
%We use a hard-decision rule for elasticity detection: 
If $\eta$ is less than a threshold $\eta_{thresh} (\geq 1$), then the cross traffic is deemed inelastic; otherwise, it is elastic.

%In \Fig{fft}, $\eta$ for elastic traffic is 10, whereas for inelastic traffic it is close to 1. \pg{We propose a hard-decision rule: if $\eta$ is lesser than a threshold $\eta_{thresh} (\geq 1$), then the cross traffic is considered inelastic; otherwise, it is elastic.}

%In scenarios with a mix of elastic and inelastic cross traffic, we want our elasticity indicator to detect the presence of {\em any} elastic cross traffic. 



%We set the threshold for \name's mode switching rule (\S\ref{s:nimbus-protocol}) using this controlled test: if $\eta \leq 2$, then use the delay-control rule (cross traffic is largely inelastic); otherwise, use the TCP-competitive mode.

\subsection{Setting Parameters for Elasticity Detection}\label{s:elasticity:parameter_tuning}

\noindent{\bf Detection threshold.} In practice, cross traffic is likely to be a mix of elastic and inelastic flows. In such scenarios, we want our detector to be sensitive to the presence of any elastic flows, since even one elastic flow can eventually grab all the link bandwidth from a delay-controlling flow. A large value of $\eta_{thresh}$ will ensure that purely inelastic traffic will always be classified correctly, but cross traffic with small elastic components will be misclassified. \Fig{elasticity:cdf} shows the CDF of elasticity ($\eta$) as the fraction of bytes belonging to elastic flows in the cross traffic varies. The median values range from $\eta = 1$ for purely inelastic traffic to $ \eta = 10$ for purely elastic traffic. We choose a fixed threshold $\eta_{thresh} = 2$, which corresponds to classifying 25\% elastic cross traffic correctly 75\% of the time.
%% Since there isn't be a peak at $f_p$ in FFT for inelastic cross traffic, $\eta$ is close to 1. For cross traffic with any elastic flows, the elastic component reacts to pulses and there is a prominent peak at $f_p$ and $\eta$ is greater than 1. The value of $\eta$ in such situations depends on the fraction of elastic traffic in the cross traffic; decreasing this fraction decreases $\eta$.  Based on this data, we use $\eta_{thresh} = 2$ in our experiments. With this threshold, in the experiment above, the elasticity detector will classify cross traffic as elastic if the elastic component in it is greater than 25\%. Increasing $\eta_{thresh}$ increases the accuracy of classification for inelastic cross traffic but also increases the misclassifications for cross traffic with relatively small elastic component.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/CDF}
    \vspace{-10mm}
    \caption{ \small{Distribution of elasticity with varying elastic fraction of cross traffic. The cross traffic consists of an elastic Cubic flow and inelastic Poisson-distributed traffic with different  rates. Completely inelastic cross traffic has $\eta$ close to zero, while completely elastic cross traffic exhibits $\eta$. Cross traffic with some elastic fraction also exhibits high elasticity ($\eta>2$).}}
    \label{fig:elasticity:cdf}
    \vspace{-2mm}
\end{figure}


\smallskip
\noindent{\bf FFT duration.} Computing FFTs over a small duration allows quick responses to changes in cross traffic, but it increases errors due to noise. Variations in the inelastic cross traffic over small periods can cause false peaks at $f_p$ in the FFT, causing that traffic to be incorrectly classified. We choose an FFT duration of 5 seconds to balance these concerns.

%% \pg{\noindent{\bf FFT Duration.} The duration of time series of cross traffic estimate used for generating the FFT affects classification accuracy. For inelastic cross traffic, decreasing the FFT duration can lead to random peaks at various frequencies in FFT because of variations in rate of cross traffic. Presence of suck peaks at $f_p$ can lead to misclassification as elastic traffic. \Fig{elasticity:FFTDuration}  demonstrates effect of FFT duration on classification accuracy. Increasing FFT duration increase accuracy, however, increasing FFT duration also increases time taken to correctly classify when the cross traffic changes elasticity. Keeping this trade-off in mind, we chose 5 seconds as the FFT duration.}

%\footnote{Majority of the elastic flows will be video streaming (70\% of total traffic on internet \cite{ciscovideo}). Most of these videos are much longer than the FFT duration of 5 seconds (on average youtube videos are about about 4 minutes long ~\cite{youtubestat}), as a result missclassification due to length of FFT duration is not critical.}

\if 0
%% NG: Image for FFT duration. Cut out totally for now.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/FFTDuration.pdf}
    \vspace{-9mm}
    \caption{ \small{Classification accuracy increases on increasing the FFT Duration.}}
    \label{fig:elasticity:FFTDuration}
    \vspace{-4mm}
\end{figure}
\fi

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/Semi-sine-2.png}
    \vspace{-3mm}
    \caption{ \small{{\bf Asymmetric sinusoidal pulse.} The pulse has period $T=1/f_p$. The positive half-sine lasts for $T/4$ with amplitude $\mu/4$, and the negative half-sine lasts for the remaining duration, with amplitude $\mu/12$. The two half-sines cancel out each other over one period.}}
    \label{fig:semi-sine}
    \vspace{-6mm}
\end{figure}

\smallskip
\noindent {\bf Pulse shaping.} Rather than a pure sinusoid, we use an {\em asymmetric} sinusoidal pulse, as shown in \Fig{semi-sine}. In the first one-quarter of the pulse cycle, the sender adds a half-sine of a certain amplitude (e.g., $\mu/4$) to $S(t)$; in the remaining three-quarters of the cycle, it subtracts a half-sine with one-third of the amplitude used in the first quarter of the cycle (e.g., $\mu/12$). The reason for this asymmetric pulse is that it enables senders with low sending rates, $S(t)$, to generate pulses. For example, for a peak amplitude of $\mu/4$, a sender with $S(t)$ as low as $\mu/12$ can generate the asymmetric pulse shown in \Fig{semi-sine}; a symmetric pulse with the same peak rate would require $S(t) > \mu/4$. 
%A peak pulse rate of $\mu/4$ causes a noticeable change to inter-packet times by transmitting a fraction of the bandwidth-delay-product (BDP) worth of packets over a short time period (less than an RTT). 

%; that isn't possible unless we burst out at least a fraction of BDP worth of packets. 

Our pulses produce an observable pattern in the FFT when the cross traffic is elastic. Using asymmetric sinusoidal pulses creates harmonics at multiples of the pulse frequency $f_p$. However, these harmonics do not affect $\eta$ (see Eq.~\eqref{eq:elasticity}), which only uses the FFT in the frequency band $[f_p, 2f_p)$.

\smallskip
\noindent {\bf Pulse duration.}
What should the duration, $T$, of the pulse be? The answer depends on two factors: first, the interval over which $S$ and $R$ are measured (with which the sender computes $\hat z$), and second, the amount of data we are able to send in excess of the mean rate without causing congestion. If $T$ were smaller than the measurement interval of $S$ and $R$, the perturbation to the cross traffic rate during one part of the pulse will be averaged out during the rest of the pulse, resulting in no impact on $\hat z(t)$.
% \pg{then the measurable effect of pulse might reduce}, because the excess in the high part and low part could cancel out over the measurement interval. 
But $T$ cannot be too large because the sender transmits in excess of the mean rate $S(t)$ for $T/4$. 
In particular, the size of the burst sent in a pulse is $\frac{2}{\pi}\frac{\mu}{4}\frac{T}{4} = \frac{T\mu}{8\pi} \approx 0.04 \mu T $. If $T$ is equal to the RTT, this is 4\% of the bandwidth-delay product (BDP).

We set $T$ to a large RTT value observed on the Internet, for example $T = 200$ ms, with the rationale that router buffers are typically provisioned to avoid packet losses for one such RTT, and because our implementation measures $S$ and $R$ over one RTT. We measure rates over one RTT because sub-RTT measurements are confounded by burstiness in packet transmissions (e.g., caused by ACK compression~\cite{jiang2003source}). 

If the cross traffic reacts slower than the pulse duration, our elasticity detector might misclassify those flows. A longer pulse duration, corresponding to the response timescale of the elastic traffic, could detect such flows. 
However, longer pulses would also send more traffic into the network and might cause congestion. 
We evaluate this alternative for detecting PCC-Vivace, a rate-based scheme (not ACK-clocked), in \App{slow-react}.
%Since most of the elastic flows in the WAN are ACK-clocked, and react at RTT timescales, we use the aforementioned value for $T$.
%\pg{\name might misclassify certain elastic rate-based flows (e.g., PCC-Vivace) that don't react to variations in the available bandwidth at the same timescale as the pulse duration. For such flows, the pulse duration would have to be adjusted based on the response timescale, and if the reaction times are too slow, the pulses would last longer, causing congestion. Since most of the elastic flows in the WAN are ACK-clocked, and react at RTT timescales, we use the aforementioned value for $T$.}
%\ma{we could potentially comment on detecting rate-based schemes here. the point is that we can detect them if they react to bandwidth changes quickly, at the timescale of a few RTTs. The pulse amplitude and duration would need to be adjusted based on the response timescale, and if it is too slow, the pulses would become too big, causing congestion.}

%Note that sub-RTT measurements are confounded by burstiness in packet transmissions (e.g., caused by ACK compression~\cite{jiang2003source}). 

%Therefore we should set $T$ to be on the order of a few RTTs. 


%Based on these considerations, $T$ should of the order of tail of observed RTT on internet paths (150 ms). In \S\ref{s:multinimbus} we provide the global preset values of $T$ and $f_p$ used by \name senders in accordance with these constraints.

%Based on these considerations, we set $T$ so that $T/4$ is on the order of the current RTT or a little less than that to avoid packet losses (e.g., $T/4$ could be the minimum observed RTT), and measure $S$ and $R$ (and hence, $z$) using Eq. (\ref{eq:SR}) over the duration of the current RTT (i.e., over exactly one window's worth of packets). As a concrete example, a flow with minimum RTT 50 ms would use $T/4 = 50$ ms, giving a pulse frequency of $1/0.2 = 5$ Hz.


\if 0

\pg{\subsection{Robustness of Elasticity Detector}
\label{s:elasticity:properties}
Going from time to frequency domain allows \name's elasticity detection  mechanism to accurately classify cross traffic under a variety of network (bandwidth delay product, buffer size, RTT, etc.) and cross traffic conditions (RTT and protocol used by elastic cross traffic flows, etc.).} 

\fi


\if 0

The duration of the sinusoidal pulse, $T$, must be at least as long as the current RTT. The reason is that $S(t)$ and $R(t)$ are estimated over the duration of the current RTT (see Eq. (\ref{eq:SR}). If $T$ were smaller than the current RTT, we will not be able to observe the effect of the pulses on cross traffic. For observing the impact of pulses, the duration of a pulse must be greater than time interval over which $S$ and $R$ are calculated. This implies $(1/f_p) > RTT$, hence we choose a frequency of $f_{p}=5$ Hz.
\fi

%\pg{Not sure if we need to make the first statement again} 
%In contrast to BBR, 

\if 0
Rather than a pure sinusoid, we use an {\em asymmetric} sinusoidal pulse, as shown in \Fig{semi-sine}. In the first one-quarter of the pulse cycle, the sender adds a half-sine of a certain amplitude (e.g., $\mu/4$) to $S(t)$; in the remaining three-quarters of the cycle, it subtracts a half-sine with one-third of the amplitude used in the first quarter of the cycle (e.g., $\mu/12$). The reason for this asymmetric sinusoidal pulse is that it enables senders with low sending rates ($S(t)$) to generate pulses. For example, for a peak amplitude of $\mu/4$, a sender with $S(t)$ as low as $\mu/12$ can generate the asymmetric pulse shown in \Fig{semi-sine}; a symmetric pulse with the same peak rate would require $S(t) > \mu/4$. The reason why we need a peak pulse rate of $\mu/4$ is because we need to cause a noticeable change to inter-packet times over a short time period (less than an RTT); that isn't possible unless we burst out at least a fraction of BDP worth of packets. In \S\ref{s:related}, we contrast our pulses with BBR's, which transmits rectangular pulses at 1.25 and 0.75 times the maximum receive rate (this rate may be thought of as a proxy for the bottleneck link rate, $\mu$).
\fi

\if 0

Using asymmetric pulses has two advantages. First, compressing the first half of the pulse (the positive part) over a shorter time period enables the sender to transmit a more concentrated burst of packets without increasing its peak sending rate. This concentrated burst creates a larger disruption to the ACK clock of the elastic flows compared to a symmetric pulse, making them easier to detect. Second, the asymmetric pulse enables senders with low sending rates ($S(t)$) to generate pulses. For example, for a peak amplitude of $\mu/4$, a sender with $S(t)$ as low as $\mu/12$ can generate the asymmetric pulse shown in \Fig{semi-sine}; a symmetric pulse with the same peak rate would require $S(t) > \mu/4$. 

\fi


%\ngs{How do we address the distortion this causes in the FFTs? We must justify why it doesn't affect the FFT much either in principle or in our experiments.}


% \smallskip
% \noindent{\bf Creating pulses when R(t) is small.} The method described above requires that Nimbus's aggregate rate be at least one-quarter of the bottleneck capacity ($\mu$). To relax this requirement, Nimbus uses {\em asymmetric} pulses made up of two half-sine components, as shown in \Fig{semi-sine}. In the first one-quarter of the pulse cycle, Nimbus adds a half-sine of amplitude $\mu/4$ to $S(t)$. In the remaining three-quarters of the cycle, it subtracts a half-sine of amplitude $\mu/12$. Using this approach, Nimbus{} can generate pulses for $S(t)$ as low as $\mu/12$. If the rate of the aggregate falls below this value, Nimbus disables pulses and simply switches to the competitive mode. The idea behind this decision is that if Nimbus controls such a small fraction of the bottleneck capacity, it is unlikely to cause a large queue buildup. If Nimbus's rate grows, pulses will commence again and Nimbus can run its cross traffic estimation algorithm.





% rather than fully-sinusoidal pulses, with each cycle made up of two half-sine pulses. The first half-sine pulse increases the rate and finishes in the first quarter of the cycle with amplitude X, while the second half-sine pulse slows down the rate and lasts for the remaining three quarters of the cycle with amplitude X/3. \hb{XXX show figure?}
% More precisely
% let phase=fraction($t*f_p$)
% if phase$<$0.25
% $$R(t) = R(t) + \frac{\mu}{4} * sin(2*\pi*2*f_p*phase)$$
% else
% $$R(t) = R(t) - \frac{\mu}{12} * sin(2*\pi*(\frac{2}{3})*f_p*(phase-0.25))$$





==> est-bottleneck-bandwidth.tex <==
\vspace{-5pt}
\subsection{Estimating bottleneck bandwidth}
\label{s:btl-bw-est-tech}
\vspace{-5pt}

%Instead of using methods like packet trains, which don't work well in presence of cross traffic, \ma{it may be better to not say this} 

We show how Eq.~(\ref{eq:zfromR}) can be used to estimate $\mu$. This equation has two unknowns: $\mu$ (which we assume for simplicity doesn't change with time) and $z(t)$. If we assume that the cross traffic does not change much in a small time interval $\Delta t$, then $z(t) \approx z(t+\Delta t)$, from which we can estimate $\mu$:

\begin{equation} 
\mu \approx \frac{R(t) - R(t + \Delta t)}{\frac{R(t)}{R_{out}(t)} - \frac{R(t + \Delta t)}{R_{out}(t + \Delta t)}}
\label{eq:muest}
\end{equation}

However, there is one challenge to using Eq.~(\ref{eq:muest}):  
the assumption that $z(t) \approx z(t+\Delta t)$ might not hold when \name continuously generates pulses. Recall that  elastic cross traffic may react to these pulses, creating fluctuations in $z(t)$ over short timescales, which can throw Eq.~(\ref{eq:muest}) off.

To solve this problem, we introduce a separate {\em bandwidth estimation phase} in \name to estimate $\mu$. In this phase, which runs periodically (e.g., every 60 seconds), \name stops transmitting sinusoidal pulses and waits one RTT for fluctuations in $z(t)$ from previous pulses to settle. It then transmits a single square pulse at time $t=t_0$, and samples $z(t)$ at $t=t_0$ and $t=t_0 + \Delta t$. If $\Delta t <$ RTT, the cross traffic will not yet have reacted to this pulse, and hence $z(t_0) \approx z(t_0+\Delta t)$ while $R(t_0) \neq R(t_0 + \Delta t)$. Therefore, we can use Eq.~(\ref{eq:muest}) to estimate $\mu$. We use $\Delta t = 0.5$RTT in our implementation. 

% Because cross traffic will take atleast 1 RTT to react to this pulse, if $\Delta t <$ RTT, then $z(t) \approx z(t+\Delta t)$ and $R(t) \neq R(t + \Delta t)$. Therefore, we can use equation \ref{eq:muest} to estimate $\mu$.

% where there are no pulses in $R$. This approach poses a limitation though. Since there are no pulses, $R(t) \approx R(t+\Delta t)$ and the numerator in equation \ref{eq:muest} might actually be very close to zero, leading to incorrect estimates for $\mu$.

\input{eval-bw-estimate}

% Note that $z(t) \approx z(t + \Delta t)$ is not always true and cross traffic might be changing on its own. A more accurate statement is $E(z(t) - z(t+\Delta t)) = 0$ (i.e., the expected values are equal), and we can use this observation to btain
% an equivalent of Eq.(\ref{eq:muest}). Instead of creating a single pulse, we can create $N > 1$ such pulses. Each of these pulses have to be separated by a non-pulsing duration, such that any given pulse does not affect the background traffic measurements during the next pulse. Following the $N$ pulses, it solves for $\mu$ in $\sum_{i=1}^{N}(z(t_{i}) - z(t_{i}+\Delta t)) \approx 0$

% \hb{HOW WELL DOES THIS WORK? Why is it better than packet trains, e.g.?}

%% \begin{figure}
%%     \centering
%%     \includegraphics[width=\columnwidth]{images/bw_est_varying_load}
%%     \caption{CDF for estimated bandwidth under various traffic load confitions.}
%%     \label{fig:bw_est}
%% \end{figure}


==> eval-bundle-benefits.tex <==
\label{s:foreground-fct}
\vspace{-10pt}
\subsection{Benefits to Bundled Flows} 
In \Sec{other-bundle-transports}, we presented the overall throughput and delay benefits of running a \name bundle.
Here, we show that \name also benefits the component flows.

We measure the impact of \bundling on flows using the metric of flow completion time (FCT). 
Without \bundling, the bottleneck queue's scheduling discipline (\eg FIFO) and TCP sending rates would together determine an inflexible ordering of flows.
If some flows pushed too many packets into the bottleneck queue (\eg because of a high congestion window), they might increase the completion time for short flows. 
Indeed, \bundling can help achieve smaller FCT by intelligently scheduling the packets of the \possbundle flows.
%% Improvements in FCT by scheduling are in addition to improvements in FCTs from better rates (for long flows), lower delays (for short flows), and larger sending rates when a \bundled flow first starts up (for medium-sized flows). We compare the benefits of different \bundle congestion control algorithms to the FCTs of the \bundled flows, as well as the impact of on the cross-flows.

\Para{Experiment setup.} We set up a realistic WAN cross-traffic workload over an emulated \mahimahi bottleneck link similar to the one in \Sec{other-bundle-transports}. Crucially, to measure FCT benefits for the \bundle, we generate {\em non-backlogged} flows within the \bundle using the same flow size distribution as the cross-traffic. The \bundle contributes an average load of 60 Mbit/s, while the cross-traffic contributes 20 Mbit/s.
%
First, we measure the throughput (over 10 ms intervals) and delays (per-packet samples) obtained by the \bundle using a canonical scheduling discipline, namely FIFO (over flow arrivals).
%
We also record the arrival time and demand of each flow.

Unfortunately, a FIFO schedule results in high tail FCT for short flows, since the WAN flow size distribution is heavy-tailed.
%
Our \bundle implementation currently only supports FIFO scheduling.
Therefore, to understand the potential benefit of employing other scheduling disciplines 
\footnote{We believe that implementing simple scheduling disciplines (\eg round robin) for high-rate \bundles is feasible.}
within the \bundle, we \emph{simulate} the scheduling disciplines over the rate and delay traces that we collect.
To verify the fidelity of our simulator, in Appendix~\ref{app:simulator-correct} we successfully compare a simulated FIFO policy to FIFO FCT achieved in emulation.
%
While the \possbundle scheduling discipline affects the ordering of packet transmissions within the \bundle, replacing FIFO with any other {\em work-conserving} scheduling discipline affects neither the overall rate nor the delays obtained in emulations by either the \bundle or the cross-traffic.
%
%% The throughput, delay, and flow arrival time series that we measure from the emulation provide an ``open-loop'' trace that helps evaluate multiple scheduling disciplines for the \bundled flows.


In the experiments below, we measure FCTs of the \bundled flows and the cross-flows under different scenarios.
%
Unless specified otherwise, the \bundle implements per-packet round-robin scheduling (RR) across flows, with \bundle congestion control algorithms \name, Cubic, Vegas, and BBR.
%
We compare the benefits of \bundling to the scenario when both the \bundled flows and the cross-traffic transmit independently using Cubic, as is the norm in the Internet today.
%
We call this baseline {\em \fctbaseline.}

We choose the \bundle parameters to avoid negatively impacting the cross-traffic.
%
%% For \name and for the compared TCPs, we choose the number of emulated long-lived \bundle flows ($N$) according to our belief about the total number of elastic flows at the bottleneck link.
%
As an approximation, for a link load $\rho$ (as a fraction of link rate),  we use the average number of jobs in a processor-sharing~\cite{processor-sharing} queue, 
$\frac{\rho}{1-\rho}$, as an estimate of the total number of active long-lived flows (\bundle and cross-traffic).
%
We then choose $n_b$, the number of long-lived \bundle flows, proportionally to the load offered to the link by the \bundle. 
%
In our experiments, the link utilization is $\frac{80}{96}$, and the \bundle offers a fraction $\frac{60}{60+20}$ of that link load. 
%
We thus choose $N = \frac{80}{16}\times\frac{60}{80} \approx 4$.
%
%% \name uses a queueing delay threshold of 12.5 ms.

\Para{FCT benefits for \bundled flows.} 
%%\Fig{emp:fct:fg} compares the FCTs of \bundled flows across different \bundle congestion control algorithms. 
%
\Fig{emp:fct:fg} shows the median (bar) and 95th percentile (whisker) FCT for \bundled flows across the different \bundle congestion control algorithms, normalized by the median FCT from \fctbaseline in each flow size range.
%
\name consistently improves on \fctbaseline, achieving between 30--75\% of the median FCT across flow sizes ($\approx$70\% for 15 KB and 150 MB flows). 
Short flows benefit from \possname reduction of packet delays.
%
BBR and Cubic have higher median FCT for short flows (15 KB and 150 KB) relative to \name, but their high throughput leads to median FCT comparable to \name for longer flows (1.5 MB and beyond).
%
For \name, BBR, and Cubic, \bundling provides a high initial sending rate for medium to long flows (150 KB--150 MB), resulting in their lower FCT.
%
%
Running a Vegas \bundle generally decreases the median FCT relative to \fctbaseline, but the tail FCT is much higher: when Vegas backs off in the presence of elastic cross-traffic, flows in the \bundle suffer from lower throughput and much higher FCT.
%
%% \Fig{emp:fct:mean:fg} shows the average FCTs across algorithms, normalized by the average FCT for \fctbaseline in each flow size range.
%
%%\possname tail FCT is comparable to \fctbaseline, since 
We find that \name, Cubic, and BBR have tail FCTs comparable to \fctbaseline for short flows, since they achieve similar delays in the tail.
%%As expected, Vegas suffers from higher average FCT than \fctbaseline.

\begin{figure}[t]
%\vspace{-15pt}
    \centering
    \begin{subfigure}[t]{0.9\columnwidth}
        \includegraphics[width=\columnwidth]{images/emp-rr-20-60-fgrnd-median}
        \caption{FCT of \emph{\bundle} flows}
        \label{fig:emp:fct:fg}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.9\columnwidth}
        \includegraphics[width=\columnwidth]{images/emp-rr-20-60-bgrnd-median}
        \caption{FCT of \emph{cross-flows}}
        \label{fig:emp:fct:bg}
    \end{subfigure}
    \caption{\small{\textbf{Comparison of FCT---} Nimbus improves bundle FCT without affecting the FCTs of cross-traffic flows on a non-backlogged Web workload.}}
    \label{fig:emp:fct}
\end{figure}

\label{s:background-fct}
\Para{Impact on cross-traffic FCT.} \Bundling improves FCT for the \bundled flows, but does the improvement come at the cost of higher FCT for the cross-traffic?

\Fig{emp:fct:bg} shows the FCT of cross-traffic with different \bundle congestion control algorithms. \name and Vegas actually {\em improve} both the median and tail FCT of short (15 KB) and long (150 MB) cross-flows, by reducing the overall delays experienced by all traffic at the bottleneck.
%
Cubic is closest to the cross-traffic (both run TCP Cubic).
%
In contrast, BBR's aggressive bandwidth-probing significantly increases the median and tail FCT for cross-traffic across all flow sizes.
%
The average FCT of \name and Cubic are comparable to \fctbaseline, while Vegas provides 50--60\% and BBR between 1.2--2.4$\times$ the average FCT of \fctbaseline.

\label{s:scheduling}
\Para{FCT benefits with advanced scheduling disciplines.} Using scheduling disciplines better than RR can improve the FCTs compared to the results above.
%
In \Fig{bundle:foreground}, we show the median FCT (bar) and $95^{th}$ percentile (whisker) of \name (relative to \fctbaseline) when using shortest remaining processing time (SRPT) scheduling.
%
Though it requires knowledge of flow sizes ahead of time, SRPT achieves a median FCT between 20--70\% of \fctbaseline, and improves on RR across flow sizes.
%
SRPT also improves the $95^{th}$ percentile FCT over \fctbaseline for all but the longest flows.
%
The improvements over RR in tail FCT are most significant for medium-sized flows (150 KB--15 MB) which last sufficiently long to benefit from scheduling decisions, gaining at the expense of the longest flows.
%
The choice of a good \bundle scheduling policy is crucial: FIFO scheduling (not shown) results in median FCTs higher than \fctbaseline by 5--35$\times$.

\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{images/emp-scheduling-20-60-fgrnd-2.pdf}
    \caption{\small{\textbf{Scheduling flows within bundles---}
    Across flow sizes, \name improves median FCT compared to not \bundling; using SRPT scheduling instead of round-robin provides additional improvement.
    }}
    \label{fig:bundle:foreground}
\end{figure}




In summary, \name, with its explicit mode switching, is the only congestion control algorithm that simultaneously improves the \possbundle FCT while not impacting the cross-traffic flows' FCT. 
Furthermore, \name enables advanced scheduling disciplines for the \bundle to further improve FCT.

%%% END OF USEFUL MATERIAL IN THIS FILE %%%
%%%%%%%%%%
%
%% More advanced scheduling disciplines (\eg SRPT) may be approximated by moving flows between queues of different priorities using the size of the flow seen so far (similar to a multi-level feedback queue).

%% We evaluated three bundle scheduling disciplines: FIFO (over flow arrival times), round-robin (RR), and shortest remaining processing time (SRPT). Scheduling decisions are made per-packet for RR and SRPT.
%
%%\Fig{bundle:foreground} compares the average FCT across flows of many size ranges, normalized by a baseline which is the average FCT of the corresponding flow size without any bundling, \ie flows competing as independent TCP Cubic connections.
%
%% We do not show the curve for the FIFO scheduling discipline---it has a much higher average FCT for the shorter flows (factor of 5--35) until the 15 MB flow size range, beyond which sizes it is comparable to the baseline.
%
%% However, as expected, the RR and SRPT scheduling disciplines provide consistently low average FCTs for flows in the size range 15 MBytes or smaller, lying between 20--60\% of the baseline FCTs.
%
%%RR has a slightly higher average FCT than the baseline for the largest flow sizes, but the increase is to be expected: the improvement in the FCT of short flows comes at the expense of the larger ones. Similarly, SRPT also approaches the baseline for the largest flow sizes.

%% These results highlight not only the benefits of bundling for FCTs, but also the importance of picking the right scheduling discipline within the bundle.
%
%% Using a naive scheduling discipline (\eg FIFO) may actually lead to poorer performance compared to not bundling, although it is possible to do much better (\eg reduce average FCTs by 2--5$\times$) with the right choice of scheduling discipline (\eg RR or SRPT).


%% \begin{figure*}
%%    \centering
%%    \begin{subfigure}[b]{0.4\textwidth}
%%        \includegraphics[width=\textwidth]{images/emp-sim-em-20-60-fgrnd.pdf}
%%        \caption{FCTs from simulation and emulation match.}
%%        \label{fig:bundle:verify}
%%    \end{subfigure}
%%    \begin{subfigure}[b]{0.4\textwidth}
%%        \includegraphics[width=\textwidth]{images/emp-scheduling-20-60-fgrnd.pdf}
%%        \caption{FCTs for flows scheduled with bundling, compared to not bundling.}
%%        \label{fig:bundle:foreground}
%%    \end{subfigure}
%%    \label{fig:bundle}
%% \end{figure*}

%% \Fig{bundle:background} shows that we can pick bundle parameters that actually {\em improve} FCTs for flows running outside the bundle (we discuss later how running a bundle with the same parameters is beneficial for the bundled flows as well). Specifically, we choose a delay threshold of 0.25 $\times$ {\ct min\_rtt} in delay-mode and an equivalent TCP flow count of $N=4$ in competitive-mode. \ngs{Prateesh, please verify previous statement.} \pg{Changed the numbers. I am not sure of the math below.} With this configuration, the average FCT of background flows reduces by up to 25\% across flow sizes ranging from 15 KBytes to 150 MBytes.
%% We leave the robust estimation of bundle parameters that ensure fairness to future work.

\if 0
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{images/emp-40-40-total-bgrnd.pdf}
    \caption{FCTs for background traffic with and without bundling.}
    \label{fig:bundle:background}
\end{figure}
\fi




==> eval-bw-estimate.tex <==
%\label{s:btl-bw-est-eval}
We evaluate \possname bandwidth estimator using \mahimahi~\cite{mahimahi}. 
%In the above experiment \name estimates the bottleneck link rate every 10 RTTs until it collects 100 observations.
\Fig{bw_est} shows the CDFs of the estimated $\mu$ with empirical cross-traffic loads for $\mu = 48$ and $96$ Mbit/s. For each load setting the cross traffic was generated dynamically using a CAIDA trace.
We find not only that the median error is always close to 0\footnote{For a more robust $\mu$ estimate, one can run the above estimator multiple times and take the median.}, but that \name estimates $\mu$ to within 10 Mbit/s over 80\% of the time even when the cross-traffic occupies 75\% of the link. 
%Increasing the cross-traffic load increases the variance in our estimator; however, the mean and the median stay close to the correct value.

\if 0

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.5\columnwidth}
        \includegraphics[width=\textwidth]{images/bw_est_varying_load_48.pdf}
        \caption{$\mu$=48 Mbit/s.}
        \label{fig:bw_est_48}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{images/bw_est_varying_load_96.pdf}
        \caption{$\mu$=96 Mbit/s.}
        \label{fig:bw_est_96}
    \end{subfigure}
    \caption{\small{\textbf{Bandwidth estimation---}Across varying link load and bottleneck rate, we compare the CDF of \possname bandwidth estimates to the ground truth, indicated by the vertical line.
    \possname estimates are close to the ground truth.
    }}
    \label{fig:bw_est}
\end{figure}

\fi



==> eval-copa-compare-cross-traffic-rtt.tex <==

\Para{Comparison with Copa.} In an experiment with synthetic cross-traffic, a backlogged \name or Copa flow competes against a backlogged NewReno flow, and we vary the RTT of the NewReno flow between $1-4\times$ the RTT of the \name/Copa flow. \Fig{copa-compare} (right) shows that Copa's accuracy degrades as the RTT of the cross traffic increases; \name's accuracy is much higher, dropping only slightly when the cross traffic RTT is $4\times$ larger than \name. Copa's approach of detecting a drained queue in a short period (5 RTTs of the Copa flow) is problematic since an elastic cross-flow with a large RTT increases its rate slowly enough to evade detection by Copa. Therefore, Copa drains the queue as it expects and concludes that there isn't any non-Copa cross-traffic. We find that this behavior continues until the cross-flow has grown to offer a load close to the link rate, when it starts interfering with Copa's queue draining. By contrast, \name's elasticity detection is more robust since it is based on the time series of variations of the queueing delay. Appendix~\ref{app:copa-compare} provides examples of the throughput and queueing delay dynamics of Copa and \name. %\ma{combine this with other paragraph on Copa. Also, rephrase the point in the related work section about Copa to mention lack of robustness to increasing RTT instead of ``increasing rate slowly''}



==> eval-copa-compare.tex <==
%% \subsection{Is Nimbus More Accurate than Copa?}
%% \subsection{Robustness of Elasticity Detection}


\smallskip
\noindent\textbf{Comparison with Copa.}
\label{s:copa-compare} % real-world workload
%% The experiment in $\S$\ref{s:big-experiment} showed that \name makes fewer mistakes in selecting its mode compared to Copa. 
%
\cut{In an experiment with synthetic cross-traffic,} We now compare the classification accuracy of our elasticity detector with Copa. 
%
First, we generate inelastic cross traffic at different rates and measure the accuracy.%fraction of the time a \name and Copa flow operate in the correct mode.
%
We use a 96 Mbit/s bottleneck link with a 50 ms propagation delay and a 100 ms drop-tail buffer (2 BDP). We consider both constant-bit-rate (CBR) and Poisson cross traffic. \cut{(generated as described in $\S$\ref{s:big-experiment}).}

\Fig{copa-compare} (left) shows that the elasticity detector (shown as \name) has high accuracy in all cases, but Copa's accuracy drops sharply when the cross traffic occupies over 80\% of the link. 
%
This result highlights a pitfall of Copa's approach: setting an operating mode based on the absolute value of queueing delays is problematic.
%
With a high inelastic cross-traffic load, Copa is unable to drain the queue quickly enough (\ie every 5 RTTs), which throws off its detector.
%
In contrast, the elasticity detector estimates elasticity through delay variations caused by its pulses, and is more robust.

Next, we ran a backlogged \name or Copa flow competing against a backlogged NewReno flow. We vary the RTT of the NewReno flow between $1-4\times$ the RTT of the \name/Copa flow. \Fig{copa-compare} (right) shows that Copa's accuracy degrades as the RTT of the cross traffic increases; our elasticity detector's accuracy is much higher, dropping only slightly when the cross traffic RTT is $4\times$ larger than \name. 
%Copa's approach of detecting a drained queue in a short period (5 RTTs of the Copa flow) is problematic\cut{ since }. 
An elastic cross-flow with a large RTT increases its rate slowly enough to evade detection by Copa. Therefore, Copa drains the queue as it expects and concludes the absence of non-Copa cross-traffic. This behavior continues until the cross-flow has grown to offer a load close to the link rate, when it starts interfering with Copa's queue draining. 
By contrast, our elasticity detection is more robust since it is based on the time series of variations of the cross traffic rate\cut{queueing delay}. Moreover, even when the classification acuuracy for Copa is higher, it makes frequent mode-switches and is suspectible to lose throughput against elastic traffic. \App{copa-compare} shows the throughput and queueing delay dynamics of Copa and \name.


%
%% These two results highlight the probems with Copa's approach of setting the operating mode using an expected pattern of queuing delays. We investigated the reasons for Copa's errors in these experiments. In the first case with  inelastic cross traffic, Copa is unable to drain the queue quickly enough (every 5 RTTs); this throws off Copa's detection rule and it switches to competitive mode. In the second case, because a NewReno cross traffic flow with a high RTT increases its rate slowly, it has a small impact on the queuing delay during Copa's 5 RTT period. Therefore, Copa can drain the queue as it expects and it concludes that there isn't any non-Copa cross traffic. This error continues until the rate of the cross traffic gets large enough to interfere with Copa's expected queuing delay behavior. 

==> eval-cross-traffic-impact.tex <==
\subsection{Does Mode Switching Help Cross-Traffic?}
\label{s:cross-traffic-impact}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.43\textwidth]{images/fct3.pdf}
    \caption{\small{Using \name reduces the p95 FCT of cross-flows relative to BBR at all flow sizes, and relative to Cubic for short flows. Vegas provides low cross-flow FCT, but its own rate is low.}}
    \label{fig:emp:fct}
\end{figure}

Using the same setup as \Sec{rw-wl}, we measure the flow completion time (FCT) of cross-flows.
%
\Fig{emp:fct} compares the 95th percentile (p95) cross-flow FCT for cross-flows of different sizes. The FCTs are normalized by the corresponding value for \name at each flow size.

BBR exhibits much higher cross-flow FCT at all sizes compared to all the other protocols, consistent with the observation of unfairness ($\S$\ref{s:big-experiment}). 

%
For small cross-flows ($\leq$ 15 KB), the p95 FCT with \name and Copa are comparable to Vegas and lower than Cubic.
%
%For large cross-flows (150 MB or more), \name shares throughput fairly, giving tail FCT much smaller than BBR, which aggressively utilizes the link capacity.
%
With \name p95 FCT of cross traffic at higher flow sizes are slightly lower than Cubic because of small delays in switching to TCP-competitive-mode.
%
At all flow sizes, Vegas provides the best cross-flow FCTs, but its own flow rate is dismal; Copa is more aggressive than Vegas but less than Nimbus, but at the expense of its own throughput  (\Sec{rw-wl}).



==> eval-delay-control.tex <==
\section{Delay-Control Deep-Dive}  
\label{s:delay-control-eval}
%


%%Loss based schemes like cubic and reno filled up the buffers and incurred high queing delays in doing so. BBR was able to maintain lower delays than cubic and reno but performed worse than \name and Vegas. 

%% %% \ng{We already talk about BBR's high-sending-rate tendencies in the big experiment}



==> eval-empirical-elasticity.tex <==
\if 0
\smallskip
\noindent\textbf{Elasticity metric $\eta$ \vs the ``true'' elasticity of cross-traffic.}
\label{s:elasticity-in-real-cross-traffic}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/emp-switch3}
    \vspace{-5.5mm}
    \caption{\small{The elasticity metric, and hence \possname mode, closely tracks the prevalence of elastic cross-traffic (ground truth measured independently using the volume of ACK-clocked flows). Green-shaded regions indicate inelastic periods.}}
    \label{fig:emp:switch}
    \vspace{-4mm}
\end{figure}

How well does the detector's decision correlate with the true proportion of elastic traffic?
We illustrate the efficacy of elasticity detection for a single experiment over time using our WAN traffic trace (same setup as \Fig{emp}). 

We classify a cross-flow in the trace as elastic if it is guaranteed to have ACK-clocked packet transmissions over its lifetime, \ie flows with sizes higher than the initial congestion window of 10 packets (in Linux 4.10).

The top chart in \Fig{emp:switch} shows the fraction of bytes belonging to elastic flows as a function of time. The bottom chart shows the output of the elasticity detector with the dashed threshold line at $\eta=2$. The green shading corresponds to periods when \name is in delay-control mode. Green regions correlate well with the periods when the true fraction of elastic traffic is low (\eg $<0.3$), while white regions correlate well with periods when the elastic fraction is high. The overall accuracy of our elasticity detector is over 90\%.
\fi

==> eval-multiple-nimbus.tex <==
\subsection{Fairness With Elasticity Detection}
\label{s:multiple-nimbus-fair-sharing}

% Does mode switching permit low delays in the presence of multiple mode switching flows (and possibly other cross-traffic)? 
%
Can multiple flows run elasticity detection and share a bottleneck link fairly with each other and with cross-traffic?

We run \name with Vegas as its delay-control algorithm and supply it with the correct link rate. %\pg{(We use Vegas because the new delay control rule proposed is not fair to other flows with the same rule.)}
%
\Fig{mul_staircase} demonstrates how \name flows react as other \name flows arrive and leave (there is no other cross-traffic). Four flows arrive at a link with rate 96 Mbit/s and \rtt 50 ms. Each flow begins 120 s after the last one began, and lasts for 480 s. The top half shows the rates achieved by the four flows over time. Each new flow begins as a watcher. If the new flow detects a pulser ($t = 120, 240, 360$ s), it remains a watcher. If the pulser goes away or a new flow fails to detect a pulser, one of the watchers becomes a pulser ($t = 480, 720$ s). The pulser can be identified visually by its rate variations.

The flows share the link rate equally. The bottom half of the figure shows the achieved delays with red background shading to indicate when one of the flows is (incorrectly) in competitive-mode. The flows maintain low RTTs and stay in delay-mode for most of the time.

% \Fig{mul_staircase} demonstrates the ``Pulser''/``Watcher'' election in multiple \name setting. 4 \name flows arrive one by one with an inter-arrival time of 120s, each flow lasts for 480s. The figure shows rate and RTT for all the 4 flows. \name flows are able to maintain low delays and achieve fairshare of rate. In the figure, Pulser flow can be visually identified by looking for presence of pulses in its rate. The RTT graphs also show periods(in red) when any of the flows were in competitive(in this case incorrect) mode, which was rare.

% All the \name flows begin as Watchers. Flow 1 starts and realizes that there are no Pulsers and switches to being a Pulser (the pulses can be seen in the rates). Flow 2, 3 and 4 join at t=120s, 240s and 360s respectively. After joining, these flows(2, 3 and 4) infer the presence of a Pulser and choose to be Watchers. After Flow 1 leaves at t=480s, there are no pulsers. Now, all the watcher flows(2, 3 and 4) try switching to Pulser mode, Flow 3 switches first and assumes the role of Pulser, remaining flows continue as Watchers. When Flow 3 ends at t=720s, the process repeats and the only remaining flow, flow 4 assumes the role of Pulser.


\Fig{mul_nimbus_switching} demonstrates multiple \name flows switching in the presence of cross-traffic. We run three \name flows on an emulated 192 Mbit/s link with a propagation delay of 50 ms. The cross-traffic is synthetic. In the first 90 s, the cross-traffic is elastic (three Cubic flows), and for the rest of the experiment, the cross-traffic is inelastic (96 Mbit/s constant bit-rate). The top graph shows the total rate of the three \name flows, along with a reference line for the fair-share rate of the aggregate. The graph at the bottom shows the measured queuing delays. 
%
\name shares the link fairly with other cross-traffic, and achieves low delays by staying in the delay mode in the absence of elastic cross-traffic.
% in \Fig{overview} but with 3 \name flows. Elastic traffic is 3 Cubic flows, inelastic traffic is 96Mbps of CBR traffic. The top graph shows the aggregate throughput of the 3 \name flows. \name flows are able to switch correctly, and achieve fair share of rate, while maintaining low queuing delays in absence of elastic cross traffic.



==> eval-overall-perf.tex <==
\section{Visualizing Nimbus}
\label{s:switching-illustration}

\label{s:big-experiment}


We illustrate \name on a synthetic workload with time-varying cross traffic. We emulate a bottleneck link in \mahimahi~\cite{mahimahi}, a link emulator. The network has a bottleneck rate of 96 Mbit/s, a minimum RTT of 50 ms, and 100 ms (2 BDP) of buffering. We compare two mode-switching protocols, \name (Cubic+BasicDelay) and \name (Cubic+Copa), with Cubic, BBR, Vegas, and PCC-Vivace (all from Linux), Copa (from Copa's authors), and Compound atop CCP (written by us).

The cross-traffic varies over time between elastic, inelastic, and a mix of the two. 
We generate inelastic cross-traffic using Poisson packet arrivals at the specified mean rate.
Elastic cross-traffic uses Cubic, via {\ct iperf}~\cite{iperf}.

\Fig{big} shows the throughput and queuing delays for the various protocols, as well as the correct fair-share rate. Table ~\ref{tab:big-exp} summarizes the deviation from fair-share throughput in the elastic (20--120 s) and inelastic (0--20 and 120--180 s) regions, and the mean queuing delay in the inelastic region. The delay in the elastic region is similar for all schemes.

Throughout the experiment, both Nimbus variants achieve throughput close to the fair-share rate and low ($\leq 15$ ms) queuing delays in the presence of inelastic cross traffic. 
With elastic cross traffic, both variants switch to TCP-competitive mode within 5 s and achieve close to their fair-share rate. The delays during this period approach the buffer size because the competing traffic is buffer-filling; the delays return to their previous low value (15 ms) within 5 s after the elastic cross-flows complete. \name stays in the correct mode throughout the experiment, except for one interval in the competitive period. The deviation from fair-share in the elastic region is because Cubic is not perfectly fair to itself over short time periods.

\begin{figure}[t]
    \centering
		\includegraphics[width=\linewidth]{images_sigcomm20/big-exp-sigcomm20.pdf}
		\vspace{-7mm}
        \caption{\small Performance on a 96 Mbit/s \mahimahi link with 50 ms delay and 2 BDP of buffering while varying the rate and type of cross traffic as denoted at the top of the graph.
        $x$M denotes $x$ Mbit/s of inelastic Poisson cross-traffic. $y$T denotes $y$ long-running Cubic cross-flows.
        The solid black line indicates the correct time-varying fair-share rate that the protocol should achieve given the cross-traffic. For each scheme, the solid line shows throughput and the dotted line shows queuing delay. \pg{The cross-traffic contains elastic flows from 20 s to 120 s}. For \name and Copa, the red shaded regions indicate times spent in the wrong mode (\eg TCP-competitive mode in the absence of elastic cross traffic).}
        \vspace{-6mm}
    \label{fig:big}
\end{figure}


\begin{table}
\small
\begin{center}
\begin{tabular}{cccc}
%\begin{tabular}{c{2cm}|c{2cm}|c{2cm}|c{1.5cm}}
 Scheme & Throughput $\Delta$ & Throughput $\Delta$ & QDelay\\ & Elastic & Inelastic & Inelastic\\ 
 \hline
  \hline
%Ideal fairshare & 1.0 (30.5 Mbps) & 1.0 (68 Mbps) \\
%  \hline
Nimbus & $-0.10$ & $0.0$ & $12$ \\
Cubic+BasicDelay & & & \\
  \hline
Nimbus & $-0.15$ &  $-0.01$ & $14$ \\
Cubic+Copa & & &\\
  \hline
 Cubic & $+0.12$ & $0.0$ & {\color{red}$78$} \\
 \hline
 BBR & {\color{red}$+0.61$} & $-0.02$ & {\color{red}$56$}\\
  \hline
 Vegas & {\color{red}$-0.79$} & {\color{orange}$-0.15$}  & 3\\
  \hline
 Compound &{\color{orange}$-0.25$} & $0.0$ & {\color{orange}$45$}\\
  \hline
 Copa & {\color{red}$-0.54$} & {\color{orange}$-0.19$} & $18$\\
  \hline
 PCC-Vivace & {\color{red}$+0.61$} & $-0.02$ &  {\color{orange}$27$}\\
\end{tabular}
\end{center}
\vspace{-1mm}
\caption{\small{Average queuing delay (in ms) in the inelastic region, and deviation from fairshare throughput in elastic and inelastic regions from \Fig{big}. \name{} is the only scheme to achieve close to fair-share throughput and low delays.}}
\label{tab:big-exp}
\vspace{-9mm}
\end{table}

Cubic achieves it's fair-share rate but experiences high delays (80 ms) throughout. BBR's throughput is often much higher than its fair share with high delays even against inelastic cross-traffic, which prior work has also observed~\cite{copa,bbr-evaluation}. 

Vegas suffers from low throughput in the presence of elastic cross-traffic as it reacts to packet delays. Compound ramps up its rate quickly when it detects low delays, but behaves like TCP Reno otherwise. Hence, it attains slightly lower than its fair-share rate in the presence of Cubic flows, and suffers from high delays even with inelastic cross-traffic. 
Unlike our elasticity detector, Copa uses instantaneous measurements for mode-switching, and the accuracy is vulnerable to the variations in cross traffic. As a result, while Copa generally uses the correct mode it frequently switches mode unnecessarily. \pg{Copa incorrectly switches mode 28 times in the elastic region, while \name{} only switches once.} \an{Copa makes 28 switching errors in the elastic region, while \name{} only switches once.}
In the elastic period, Copa's frequent mode switches lower its throughput (14 Mbit/s) compared to \name (27.5 Mbit/s) and fair-share rate (\eg see 20--40 s). 
Further, by draining queues periodically, Copa incurs minor underutilization against inelastic traffic (\eg 120--140 s).

Vivace competes unfairly with elastic traffic. At times, Vivace fails to maintain low delays against inelastic cross traffic and  incurs heavy packet loss (\eg 160--180s). 


==> eval-real-world.tex <==


\subsection{Performance on Internet Paths}
\label{s:realworld}

%\pg{say something about why we don't have copa, maybe because it requires custom copa receiver?}

We ran \name on Internet paths on 25 paths between five senders and five receivers. The servers were Amazon EC2 instances located in California, London, Frankfurt, Ireland, and Paris, all with 10 Gbit/s links. The receivers were five residential hosts in different autonomous systems. We verified that the bottleneck in each case was not the server's Internet link.

To understand the nature of cross traffic on these paths, we ran experiments with \possname delay-control algorithm (without mode-switching) and Cubic each performing bulk transfers over a three-day period. The results showed that scenarios where cross traffic is predominantly inelastic are common. 
This indicates that delay-control algorithms can be effective on the Internet (see \App{delay-control-motivation} for details).

%shows an example result from one of the paths.
%Figure~\ref{fig:dsmotivation} shows results from one of these paths. The plot shows the average throughput and average delay for Cubic and a \dcc scheme (described in \S\ref{s:nimbus-protocol}) for 100 experiments with each protocol over a three-day period. Each experiment ran for 60 seconds. The \dcc scheme generally achieves much lower delays than Cubic, with similar throughput. This shows that there is an opportunity to significantly improve delays using \dcc algorithms, provided we can detect buffer-filling TCPs and compete with them fairly when needed. 


%
Next, on each path, we initiated bulk data transfers using \name, Cubic, BBR, and Vegas.
%
We ran one minute experiments over five hours on each path, and measured the achieved average throughput and mean delay.
%
\Fig{realworld} shows throughput and delays over three of the paths. The $x$ (delay) axis is inverted; better performance is up and to the right. We find that \name achieves high throughput comparable to BBR in all cases, at noticeably lower delays. 
%
Cubic attains high throughput on paths with deep buffers (\Fig{realworld:1} and \Fig{realworld:2}), but not on paths with packet drops or policers (\Fig{realworld:3}).
%
Vegas attains poor throughput on these paths due to its inability to compete with elastic cross-traffic.
%
These trends illustrate the utility of elasticity detection on Internet paths: it is possible to achieve high throughput and low delays over the Internet using delay-control algorithms with the ability to switch to a different competitive mode when required. 

\Fig{rw_cdf} summarizes the results on the paths with queueing. \name's throughput is similar to Cubic and $10$\% lower than BBR but at much lower delay ($40$--$50$ ms lower than BBR).



\if 0

\cut{Overall, our results, sampled in \Fig{realworld}, highlight the variability of Internet paths. 
There were instances where \name achieved the best throughput and delay among the tested algorithms (5/18), instances where all algorithms performed well (8/18), and instances where another algorithm outperformed \name (5/18).
For example, in Figure~\ref{fig:realworld:2}, we found that on this large-BDP link \name suffered due to its choice of NewReno as the TCP-competitive rate increase rule.
Cubic has a more aggressive update and achieved higher throughput as a result.
%Investigating the causes of good or poor performance is challenging due to the lack of ground truth, but we believe that \name achieves performance sufficiently good to be useful for a public Internet deployment.
Results from the other 15 paths are in Appendix~\ref{app:realworld}.

We observed that \name is predominantly in delay-mode on some paths, and in competitive-mode on some others. 
Further, \name performs similarly to BBR and Cubic on some paths, and similarly to Vegas (albeit invariably with higher throughput) on others.
%Further, there are paths where the throughput-delay metrics of \name are split between the metrics of delay-mode and competitive-mode. 
This suggests that mode-switching occurs on real Internet paths.}

\fi

==> eval-realistic-cross-traffic.tex <==
%%\subsection{Video Cross Traffic}
\label{s:videocross}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images_sigcomm20/video.pdf}
    \vspace{-4.3mm}
    \caption{\small{{\bf Video Cross Traffic.} Throughput and mean delay with video cross-traffic. \name achieves similar throughput as Cubic but reduces delays and performs better than all other schemes. Copa and Vegas achieve low throughput.}}
    \label{fig:vc}
%    \vspace{-6mm}
\end{figure}

\if 0
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/video_1.pdf}
        \vspace{-6mm}
        \caption{\small{4k Video}}
        \label{fig:vc:1}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/video_2.pdf}
        \vspace{-6mm}
        \caption{\small{1080p Video}}
        \label{fig:vc:2}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small{{\bf Video Cross Traffic.} Throughput and mean delay with video cross-traffic. 4K video ramps up aggressively and acts as elastic cross-traffic, while the 1080p video is application-limited and acts as inelastic cross-traffic. \name achieves similar throughput as Cubic but reduces delays. Copa and Vegas achieve low throughput.}}
    \label{fig:vc}
%    \vspace{-4mm}
\end{figure}
\fi
\smallskip
\noindent\textbf{How is video traffic classified?} 
A large fraction of Internet traffic is video streaming~\cite{ciscovideo};
video streams can be application- (inelastic) or network-limited (elastic) at different points in their lifetime. 
We evaluate the performance of transport algorithms in the presence of cross-traffic consisting of a DASH~\cite{dash} based video stream using Cubic. The experiment uses a 4k video as cross-traffic, and a 48 Mbit/s link with 50 ms propagation delay.
%
\Fig{vc} summarizes the throughout and delay of the various schemes. 
Because of effective mode switching, \name achieves similar throughput as Cubic while reducing delays. 
\cut{
Both Copa and Vegas don't compete well with the video stream and achieve close to zero throughput. 
BBR and PCC-Vivace achieve lower throughput and higher delay than \name.
}
%In our experiment the video stream is network-limited (elastic) for the majority of the time, given the bottleneck rate. Indeed, we find that \name is in the TCP-competitive mode majority of the time.


\if 0
%
A DASH video stream can be application- or network-limited at different points in its lifetime; however, we find that the 1080p video stream is largely application-limited (inelastic) and that the 4K stream is network-limited (elastic), given the bottleneck rate. Indeed, we find that \name stays in delay mode and TCP-competitive mode respectively in the two cases.
%
With 1080p video cross-traffic, all schemes achieve similar throughput but the delay-controlling schemes enjoy significantly lower delays. In particular, \name has a throughput similar to Cubic with a 50 ms smaller mean delay.
%
With the 4K video, \name achieves similar throughput and delay as Cubic, but both Copa and Vegas cannot compete with the aggressive video cross-flow and achieve \emph{close to zero throughput}. BBR and PCC-Vivace achieve lower throughput and higher delay than \name.
\fi


==> eval-robustness-parameter-sweep.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{images/mul_rate.pdf}\vspace{-2mm}
    \includegraphics[width=0.9\columnwidth]{images/mul_rtt.pdf}
    \vspace{-5mm}
    \caption{\small {{\bf Multiple competing \name flows.} Multiple \name flows achieve fair sharing of a bottleneck link (top graph). There is at most one \pulser flow at any time; \cut{which can be} identified by its rate variations. Together, the flows achieve low delays by staying in delay mode for most of the duration (bottom graph). The red background shading shows when a \name flow was (incorrectly) in competitive mode.}}
    \label{fig:mul_staircase}
    \vspace{-2mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{images/overview-nimbus-mul-sigcomm19.pdf}
    \vspace{-5mm}
    \caption{\small{{\bf Multiple \name flows  and other cross-traffic.} There are 3 \name flows throughout. Cross traffic in duration 30-90~s is elastic and made up of three Cubic flows. Cross traffic in duration 90-150~s is inelastic and made up of a 96 Mbit/s constant bit-rate stream. Multiple \name flows achieve their fair share rate (top) while maintaining low delays in the absence of elastic cross traffic (bottom).}}
    \label{fig:mul_nimbus_switching}
    \vspace{-5mm}
\end{figure}


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/california-harihome2.pdf}
        \vspace{-6mm}
        \caption{\small{EC2 California to Host A}}
        \label{fig:realworld:1}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/ireland-nghome2.pdf}
        \vspace{-6mm}
        \caption{\small{EC2 Ireland to Host B}}
        \label{fig:realworld:2}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/london-shaileshh2.pdf}
        \vspace{-6mm}
        \caption{\small{EC2 Frankfurt to Host C}}
        \label{fig:realworld:3}
    \end{subfigure}
    \vspace{-6mm}
    \caption{\small {{\bf Performance on three example Internet paths.} The $x$ axis is inverted; better performance is up and to the right. On paths with buffering and no drops, ((a) and (b)), \name achieves the same throughput as BBR and Cubic but reduces delays significantly. On paths with significant packet drops (c), Cubic suffers but \name achieves high throughput.}}
    \label{fig:realworld}
    \vspace{-5mm}
\end{figure*}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/real_delay.pdf}
        %\caption{RTT}
        \label{fig:rw_cdf:delay}
    \end{subfigure}
%%    \begin{subfigure}[b]{0.3\textwidth}
%%        \includegraphics[width=\textwidth]{images/overview-nimbus-cubic-vegas.pdf}
%%        \caption{Cubic Competitive - Vegas DS}
%%        \label{fig:vs:vegas}
%%    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/real_rate.pdf}
        %\caption{Rate}
        \label{fig:rw_cdf:rate}
    \end{subfigure}
    \vspace{-7mm}
    \caption{\small {{\bf Paths with queuing.} \name{} reduces the RTT compared to Cubic and BBR (40-50 ms lower), at similar throughput.}}
    \label{fig:rw_cdf}
    \vspace{-5mm}
\end{figure}

%\Para{


\smallskip
\noindent\textbf{Pulse size, link rate, and offered cross-traffic load.}
\label{s:multifactor-robustness-first-half}
%
%% We now evaluate the robustness of our elasticity detection method to \pg{elastic fraction of cross-traffic,} cross-traffic and \possname RTTs, \pg{differences in \RTT of cross-traffic flows}, bottleneck link rate, the share of the bottleneck controlled by \name, bottleneck buffer size, and \possname pulse size.
%
We perform a multi-factor experiment varying the elasticity detector's pulse size from $1/16$ to $1/2$ the link rate, \possname fair share of the bottleneck link rate from 12.5\%---75\% (by varying the cross-traffic load), bottleneck link rates set to 96, 192, and 384 Mbit/s.%, with three different traffic mixes: (1) purely elastic, (2) purely inelastic, and (3) a 50-50 mix of elastic and inelastic cross-traffic.
%
%\App{robustness-multifactor} provides detailed results and descriptions; we summarize our results here.
%
The accuracy for purely elastic cross-traffic is always higher than 95\%.
%
while the average accuracy over all the points for the other two traffic mixes is more than 90\%.
%
%In general, increasing pulse sizes improves accuracy (\name can create more easily observable change in cross-traffic); increasing link rates improves accuracy (variance of inelastic cross-traffic reduces, resulting in smaller false peaks in the FFT); and decreasing \possname share of the link rate improves accuracy (same reason as the last).
\Fig{heatmap} shows the average detection accuracy over the other two categories of cross-traffic (mix + purely inelastic).
%
%\name achieves an accuracy of more than 90\% averaged over all the points.
%
The classification accuracy is not sensitive to cross traffic load. The elasticity detector's \emph{use of asymmetric pulses} enables a sender to create fluctuations in the cross traffic even when the sending rate is low. As a result, the detection accuracy remains high under high cross-traffic load. 

In general, increasing the pulse sizes improves accuracy because the elasticity detector can create a more easily observable change in the cross-traffic sending rates.
%
An increase in the link rate results in higher accuracy for a given pulse size and \name link share because the variance in the rates of inelastic Poisson cross-traffic reduces with increasing cross-traffic sending rate, reducing the number of false peaks in the cross-traffic FFT.
%
%For the same reason, decreasing \possname share of the link also results in higher accuracy in general.
%
However, at low link rates, the elasticity detector has low accuracy ($\sim$60\%) when it uses high pulse sizes and controls a low fraction of the link rate. We believe that this is due to a quirk in the way the Linux networking stack reports round-trip time measurements under sudden sending rate changes.

\smallskip
\noindent\textbf{Errors in link rate estimation.}
We explicitly supply an incorrect link rate estimate to \name. We vary the error in the link rate estimate from $-50$\% to $+50$\% of the real link rate value. The classification accuracy is high (> 80\%) for all traffic classes when the error is low ($\leq$ 12.5\%). When the error rate is higher, all traffic is classified as elastic. 

To understand why, define $\hat{z}(t)$ as the estimate of the cross traffic rate, $z^{*}(t)$ as the real cross traffic rate, $\hat{\mu}$ as the estimate of the link rate and $\mu^{*}$ as the real link rate. Then, from Equation ~\ref{eq:zfromR}:
\begin{equation}
    \hat{z}(t) = \hat{\mu} \frac{S(t)}{R(t)} - S(t),\qquad
      z^{*}(t) = \mu^{*} \frac{S(t)}{R(t)} - S(t) 
\vspace{-1mm}
\end{equation}
Combining the equations above, we get
\vspace{-2mm}
\begin{equation}
    \hat{z}(t) = \frac{\hat{\mu}}{\mu^{*}} z^{*}(t) + \big(\frac{\hat{\mu}}{\mu^{*}} - 1 \big) S(t) 
\end{equation}
\vspace{-4mm}

When the link estimate is inaccurate, the cross traffic estimate is a linear combination of the real cross traffic rate and the sending rate. As the error increases, the contribution of the sending rate to the cross traffic estimate increases. Since the sending rate oscillates at the pulse frequency, the cross traffic estimate also oscillates, and all cross traffic (regardless of its nature) is classified as elastic.

%The implication is, Nimbus uses the TCP-competetive mode against inelastic cross traffic, and loses the benefits of the delay-controlling algorithm. However, by always running in TCP-competetive mode, Nimbus doesn't lose throughput due to inaccuracies in the link rate estimate. Thus, Nimbus is still safe under such inaccuracies. See \App{robustness:bad-mu} for further explanation.
%We evaluate the impact of inaccuracies in link rate estimation on the classification accuracy. We vary the link rate estimate from -50\% to +50\% of the real link rate value. \Fig{bandwidth_error} shows the misclassification rate for different error rates. The classification accuracy is high for all traffic classes when the error is less than equal to 12.5\%. When the error rate is higher (>= 25\%), all cross traffic is classified as elastic. 

For \name{}, this implies that when the error in link rate estimate is high, it always uses the TCP-competitive mode, and against inelastic cross traffic, \name loses the benefits of delay-controlling mode. \an{reword?} However, by always running in TCP-competitive mode, Nimbus doesn't lose throughput due to inaccuracies in link rate estimation. Thus, running Nimbus is safe under such inaccuracies.

\smallskip
\noindent\textbf{Buffer size, \RTT{}, and Active Queue Management(AQM).} 
\label{s:multifactor-robustness-second-half}
The elasticity detector is robust to these settings (\App{robustness:bufsize-rtt-aqm}).
\cut{
We vary the bottleneck buffer size (drop-tail) from 0.25 BDP to 4 BDP for three categories of cross traffic as in the earlier experiments, with propagation delays of 25 ms, 50 ms, and 75 ms. We also measured classification accuracy when the bottleneck link implements the PIE AQM scheme at two target delays (0.25 BDP and 1 BDP) with a propagation delay of 50 ms.
%

\App{robustness:bufsize-rtt-aqm} provides detailed results.
%
In summary, with purely elastic or inelastic traffic, the elasticity detector has an average accuracy (across 5 runs) of 98\% or more in all cases but two, while with mixed traffic, the accuracy is always 85\% or more.
%
In all cases (including low accuracy ones), \name achieves its fair-share throughput and low delays.
}

==> eval-switching-synthetic.tex <==
%% \subsection{How Robust is Elasticity Detection?}
\label{s:robustness-synthetic}
We evaluate the robustness of the elasticity detector under a variety of network and traffic conditions.
%
Unless specified otherwise, we run \name as a backlogged flow on a 96 Mbit/s bottleneck link with a $50$ ms propagation delay and a $100$ ms drop-tail buffer (2 BDP).
%
We supply \name with the correct link rate for \pg{the experiments in this subsection.}%these experiments. 
%% allowing us to study the robustness of elasticity detection with respect to the properties mentioned above.
%
We consider three categories of synthetic cross-traffic sharing the link with \name: (i) fully inelastic traffic (Poisson); (ii) fully elastic traffic (backlogged NewReno flows); and (iii) an equal mix of inelastic and elastic. The duration of each experiment is 120 seconds. The main performance metric is {\em accuracy}: the fraction of time that the elasticity detector correctly detects the presence of elastic cross-traffic. For each experiment, we report the average accuracy of the detector across 5 runs. \cut{The key take-aways are:

\noindent\textbf{1) Cross-traffic RTT:} The elasticity detector observes the fluctuation in cross-traffic rate in the frequency domain, and thus doesn't need to know the cross-traffic RTT. In particular the cross-traffic RTT changes the phase but not the amplitude of the peak in the FFT.

\noindent\textbf{2) Mix of RTTs in the cross-traffic:} When the cross-traffic contains a mix of elastic flows with different RTTs, all elastic flows, regardless of the RTT, react to the elasticity detector's pulses, the superposition of their rates also oscillates, and the traffic is correctly classified as elastic.

\noindent\textbf{3) High cross-traffic load:} Using asymmetric pulses, a sender is able to create and observe fluctuations in the cross-traffic even when the sending rate is a small fraction of the link capacity.

\noindent\textbf{4) Comparison with Copa:} Compared to our elasticity detector, Copa mis-classifies cross-traffic when the inelastic traffic rate is high, or when elastic flows have high RTTs.}

%\pg{Do we need to add an experiment on versatility, i.e., show Nimbus with different protocols in the competitive and delay mode here?}

\cut{Now we study how sensitive elasticity detection is to the \RTT of the cross-traffic. }
%% We now evaluate the robustness of our elasticity detection method to \pg{elastic fraction of cross-traffic,} cross-traffic and \possname RTTs, \pg{differences in \RTT of cross-traffic flows}, bottleneck link rate, the share of the bottleneck controlled by \name, bottleneck buffer size, and \possname pulse size.
%
\begin{figure}
    \includegraphics[width=\columnwidth]{images/cross_accuracy.pdf}
    \vspace{-9mm}
    \caption{\small The elasticity detector classifies purely elastic and inelastic traffic with accuracy greater than $98$\%. For a mix of elastic and inelastic traffic, the average accuracy is greater than $85$\% in all cases.}
    \label{fig:cross_rtt}
    \vspace{-5mm}
\end{figure}

\begin{figure}
    \includegraphics[width=\columnwidth]{images/heat_map.pdf}
    \vspace{-6mm}
    \caption{\small The elasticity detector is robust to variations in link bandwidth and fraction of traffic controlled by it. The accuracy is high even when the fraction of traffic under control is small. Increasing pulse size increases robustness.}
    \label{fig:heatmap}
    \vspace{-4mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/copa-comparison-combined.pdf}
    \vspace{-6mm}
    \caption{\small{The elasticity detector's classification accuracy is better \cut{has achieves higher classification accuracy}than Copa when (i) inelastic cross traffic occupies a large fraction of the link (left); (ii) elastic cross traffic has higher RTT than the flow's RTT (right).}}
    \vspace{-4mm}
    \label{fig:copa-compare}
\end{figure}

%
%% \ngs{Ignoring PG's comment on persistence. Persistence of nimbus doesn't imply that we'll get the mu right; consider what happens when we have persistent elastic cross-traffic?}
\smallskip
\noindent\textbf{Impact of cross-traffic \RTT.}
We vary the cross-traffic's base RTT from $10$ ms ($0.2\times$ that of \name) to $200$ ms ($4\times$ that of \name).
\Fig{cross_rtt} shows the mean accuracy of each of the three classes of cross-traffic. We find that varying cross-traffic \RTT does not impact detection accuracy. Regardless of the cross-traffic \RTT, the elastic flows respond to fluctuations created by the elasticity detector, generating a peak in the cross-traffic FFT at the oscillation frequency. The cross traffic's \RTT \emph{only affects the phase but not the amplitude} of the peak in the FFT.

%Recall an earlier version of the elasticity detector used cross-correlation between sending rate and the cross-traffic rate (\Sec{pracelas}), however the trouble is that cross-traffic reacts after its \RTT, and we must align the two rates based on the cross-traffic \RTT. 
%In the frequency domain, such differences affect only phase, not amplitude. 
For purely inelastic and purely elastic traffic, the accuracy is more than $98$\% in all cases, while for mixed traffic, the accuracy is more than $85$\% in all cases (a random guess would have only achieved 50\%). 
The accuracy for mixed traffic is lower because \cut{compared to purely elastic as with mixed traffic} only half of the cross traffic oscillates, and the peak in the cross-traffic FFT is thus smaller.

\smallskip
\noindent\textbf{A mix of \RTT{}s in the cross-traffic.} We vary the number of elastic cross traffic flows from $1$ to $5$, where the \RTT of $n^{\text{th}}$ flow in $20 \cdot n$ ms. In case the cross-traffic contains elastic flows, all the elastic flows oscillate at the elasticity detector's pulse frequency. 
As a result, the sum of the rates of these elastic flows also oscillates,\footnote{\an{cut: Note that} \an{S}ince the \RTT{}s are different, the elastic flows' oscillations will differ in phase and the oscillations could in theory cancel each other out leading to mis-classification, but this is unlikely.} and the traffic is correctly classified as elastic. 
For purely elastic and inelastic traffic, the elasticity detector achieves an average accuracy of $98$\% across 5 runs, while for mixed traffic, the mean accuracy is greater than $90$\% in all cases. In other words, heterogeneity in \RTT{}s of cross-flows does not degrade the accuracy of elasticity detection. 

==> eval-switching-wan-traces.tex <==
% \subsection{Throughput \& Delay Benefits With Varying Shares of Bottleneck Link Rate}
%\subsection{Should \possname Link Share Be Large?}

\noindent\textbf{Impact of offered traffic load as a fraction of link rate.}
\label{s:robustness-wan-traces}
\begin{figure}
    \begin{center}
        \begin{subfigure}[b]{0.8\columnwidth}
            \includegraphics[width=\columnwidth]{images/pulse_load_30_2.pdf}\vspace{-26mm}
            \includegraphics[width=\columnwidth]{images/pulse_load_50_2.pdf}
            \label{fig:pulse_load:50}
            \vspace{-7mm}
            
            \subcaption{Cross-Traffic Load: 50\%}
        \end{subfigure}
        \if 0
        \begin{subfigure}[b]{0.8\columnwidth}
            \includegraphics[width=\columnwidth]{images/pulse_load_50_2.pdf}
            \label{fig:pulse_load:50}
            \vspace{-6.5mm}
            \subcaption{Cross-Traffic Load: 50\%}
        \end{subfigure}
        \fi 
        \begin{subfigure}[b]{0.8\columnwidth}
            \includegraphics[width=\columnwidth]{images/pulse_load90_2.pdf}
            \label{fig:pulse_load:90}
            \vspace{-6.5mm}
            \subcaption{Cross-Traffic Load: 90\%}
        \end{subfigure}
        \vspace{-3mm}
        \caption{\small At low cross-traffic loads, \possname queueing delay approaches that of Vegas while its throughput approaches that of Cubic. At high loads, \name behaves like Cubic. Increasing pulse size improves switching accuracy and performance.}
        \label{fig:pulse_load}
    \end{center}
    \vspace{-7mm}
\end{figure}
\cut{
\begin{figure}
    \begin{center}
        \begin{subfigure}[b]{0.8\columnwidth}
            \includegraphics[width=\columnwidth]{images/pulse_load_30_2.pdf}
            \label{fig:pulse_load:30}
            \vspace{-7mm}
            \subcaption{Cross-Traffic Load: 30\%}
        \end{subfigure}
        \if 0
        \begin{subfigure}[b]{0.8\columnwidth}
            \includegraphics[width=\columnwidth]{images/pulse_load_50_2.pdf}
            \label{fig:pulse_load:50}
            \vspace{-7mm}
            \subcaption{Cross-Traffic Load: 50\%}
        \end{subfigure}
        \fi 
        \begin{subfigure}[b]{0.8\columnwidth}
            \includegraphics[width=\columnwidth]{images/pulse_load90_2.pdf}
            \label{fig:pulse_load:90}
            \vspace{-5mm}
            \subcaption{Cross-Traffic Load: 90\%}
        \end{subfigure}
        \vspace{-2mm}
        \caption{\small At low cross-traffic loads, \possname queueing delay approaches that of Vegas while its throughput approaches that of Cubic. At high loads, \name behaves like Cubic. Increasing pulse size improves switching accuracy and performance.}
        \label{fig:pulse_load}
    \end{center}
    \vspace{-5mm}
\end{figure}
}
Is elasticity detection effective solely when a flow controls a large fraction of the link rate?
%
We measure \possname throughput and delay relative to other algorithms when the cross-traffic (from our WAN traffic trace) offers varying traffic loads as fractions of the link rate.
%
%Cross-traffic is derived from our WAN traffic trace (described in \Sec{other-bundle-transports}).
%
We set the cross-traffic's offered load at 50\% and 90\% of the link rate, and measure throughput and delay for two pulse sizes: $0.125\mu$ and $0.25\mu$.
%As before, the flow corresponding to \name and the compared algorithms in each experiment is backlogged. We evaluate \name with three different sizes of the pulses used for elasticity  detection (\Sec{pracelas}), corresponding to 0.125$\times$, 0.25$\times$, and 0.375$\times$ the link rate.

\Fig{pulse_load} shows our findings. In all cases, \name lowers delay without hurting throughput. The delay benefits are most pronounced when cross traffic is low, but \possname throughput-delay benefits persist even when the cross-traffic uses a large fraction (90\%) of the link rate. 
As cross traffic increases, \possname delay improvements decrease, because it must stay in TCP-competitive mode more often. 
Third, \possname behavior is better at the larger pulse size, but it retains benefits even at $0.125\mu$.

%At low cross-traffic loads (30\%), cross-traffic is mostly inelastic, resulting in \name picking its delay mode most of the time. Hence, its delays approach that of Vegas, while its throughput matches Cubic. 
%
%At high loads (70\%), \name chooses its competitive mode to retain throughput in the presence of (mostly elastic) cross-traffic. Hence, \possname throughput and delays both approach Cubic.
%
%Across all cross-traffic loads, \name with the larger pulse sizes (0.25$\times$ and 0.375$\times$) performs comparably to Cubic.
%
However, elasticity detection is less accurate with smaller pulse amplitude ($0.125\mu$), causing more errors in mode switching. Thus, with the smaller pulse, \name is less effective at medium load (50\%) when switching correctly matters more for good performance. 

% For lower loads (30\%), most of the time, cross traffic is inelastic. Hence, \name{} can be in delay mode longer and achieve much lower delays compared to Cubic. In such situations \name delay CDF approaches the delay CDF of Vegas. When the load is higher (70\%), the cross traffic is mostly elastic, \name{} has to be in competitive mode predominantly and thus won't be able to lower delays as well. In such situations \name delay CDF approaches the delay CDF of Cubic.

% We see that across all loads \name{} with pulse size 0.25 and 0.375 perform similar and are able to compete fairly, i.e. the CDF of their rate match that of Cubic. The CDF of delay also looks similar in all load settings. \name{} with pulse size 0.125, performs similar when switching is not required as often, i.e. when load is low(30\%) or high(70\%). For medium loads, pulse size of 0.125 performs worse, its rate CDF deviates from that of Cubic (showing it doesn't compete fairly) and delays are higher compared to \name with higher pulse sizes. This suggests that with low pulse size nimbus made errors in both detecting presence and absence of elastic cross traffic. By making error in detecting presence of elastic cross traffic, it lost throughput, by making errors in detecting absence of elastic cross traffic it lost an opportunity to lower queueing delays.



==> eval-switching.tex <==
%%% THIS FILE IS NOT IN USE ANYMORE. CONTENTS ARE DIRECTLY LINKED FROM eval.tex


% \vspace{-10pt}
% \subsection{Robustness of Switching}
% \vspace{-5pt}

% We first evaluate the robustness by emulating realistic WAN traffic. We then evaluate \name's performance under various network conditions by creating synthetic workloads. 



==> eval-versatility.tex <==
% \subsection{Versatility in choosing Loss and Competitive Mode Algorithms:}
%% \Para{How General is Mode Switching?}
\label{s:versatility}

\Para{Extending elasticity detection to other algorithms.}


A mode-switching transport can employ the elasticity-detection method while using a variety of congestion control algorithms for its \dcc and TCP-competitive modes.
We have implemented Cubic, Reno, and MulTCP~\cite{multcp} as competitive-mode algorithms, and \name-delay, Vegas, FAST~\cite{fasttcp}, and COPA~\cite{copa} as delay-mode algorithms. In \Fig{vs}, we illustrate two combinations of delay and competitive mode algorithms sharing a bottleneck link with synthetic elastic and inelastic cross-traffic active at different periods during the experiment. The fair-share rate over time is shown as a reference. 
Both Reno$+$Nimbus-delay-mode (\Fig{vs:reno}) and Cubic$+$COPA (\Fig{vs:COPA}) achieve
their fair-share rate while keeping the delays low in the absence of elastic cross-traffic. 

% \Fig{vs} repeats the experiment in ~\Fig{overview}. We try three new protocols/configurations 1) Reno Competitive with Nimbus Delay\footnote{elastic cross traffic in this case was 1 Reno flow}, 2) Cubic Competitive with Vegas Delay and 3) Cubic Competitive with COPA Delay. In all the configurations \name was able to switch correctly, and achieve fairshare of rate, while maintaining low delays in absence of elastic cross traffic.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-reno-delay-sigcomm19.pdf}
        \vspace{-6mm}
        \caption{\small{Reno + Nimbus delay}}
        \label{fig:vs:reno}
    \end{subfigure}
%%    \begin{subfigure}[b]{0.3\textwidth}
%%        \includegraphics[width=\textwidth]{images/overview-nimbus-cubic-vegas.pdf}
%%        \caption{Cubic Competitive - Vegas DS}
%%        \label{fig:vs:vegas}
%%    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-cubic-COPA-sigcomm19.pdf}
        \vspace{-6mm}
        \caption{\small{Cubic + COPA}}
        \label{fig:vs:COPA}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf \name's versatility.}  Mode switching with different combinations of \dcc and \tcpcomp algorithms.}
    \label{fig:vs}
\end{figure}

==> eval-wan-distribution.tex <==
%% \subsection{Comparing \name with Other Transports}
%% \subsection{Does \name Achieve Low Delays\\and High Throughput?}
\subsection{Nimbus Benefits from Elasticity Detection}
%% \subsection{Does \name get low delay and high rates?}
\label{s:other-bundle-transports}
\label{s:rw-wl} % real-world workload

\if 0
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/rtt.pdf}
        \vspace{-6mm}
        %\caption{\small{RTT}}
        \label{fig:emp:rtt}
    \end{subfigure}
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{images_sigcomm20/boxplot.pdf}
        \vspace{-6mm}
        %\caption{\small{Deviation from fair-share}}
        \label{fig:emp:box}
    \end{subfigure}
    \vspace{-5mm}
    \caption{\small{{\bf WAN cross-traffic.} The left figure shows average RTT, the right figure shows the deviation in throughput from the fair-share rate (over 5 s intervals). \name reduces delay relative to Cubic, BBR and PCC-Vivace. \name and Cubic achieve the best fairness. Vegas and Copa also reduce delay, but deviate from fair-share at lower percentiles and lose throughput.}}
    \label{fig:emp}
    \vspace{-4mm}
\end{figure}

\fi

\begin{figure}[t]
    \centering
\begin{subfigure}[t]{\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{images_sigcomm20/rtt2.pdf}
    \vspace{-5mm}
    \caption{\name reduces delay relative to Cubic, BBR and PCC-Vivace. It has higher delays than Copa and Vegas, but those two schemes have much lower throughput than the fair share (see \an{Figure~\ref{fig:emp:box}}).}
    \label{fig:emp:rtt}
%    \vspace{-3mm}
\end{subfigure}

\begin{subfigure}[t]{\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{images_sigcomm20/boxplot2.pdf}
    \vspace{-5mm}
    \caption{\small{Deviation in throughput from fair-share. \name and Cubic achieve highest fairness. Vegas and Copa deviate from fair-share at lower percentiles and lose throughput; BBR and PCC-Vivace are significantly higher than fair share. Midline is the median, the box edges are the 25\%ile and 75\%ile, the whisker notches are 10\%ile and 90\%ile.}}
    \label{fig:emp:box}
\end{subfigure}

\begin{subfigure}[t]{\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{images/emp-ts.pdf}
    \vspace{-5mm}
    \caption{\small{Copa incorrectly switches to its delay mode even when competing with Cubic, unlike \name{}.}}
    \label{fig:emp:ts}
    \vspace{-3mm}
\end{subfigure}
\caption{\an{Performance of NimbusCC}}
\end{figure}

\if 0
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/emp-combined-sigcomm19_v6.pdf}
    \vspace{-8mm}
    \caption{\small{\name reduces delay relative to Cubic and BBR while achieving comparable throughput on a cross-traffic workload derived from a packet trace collected at a WAN router. Vegas and Copa also reduce delay but lose throughput.}}
    \label{fig:emp}
    \vspace{-4.5mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images/emp-agg-custom.pdf}
    \vspace{-5mm}
    \caption{\small{Aggregate bytes sent.}}
    \label{fig:agg}
    \vspace{-5mm}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/time_lag_raw.pdf}
        \vspace{-5mm}
        \caption{\small{Raw}}
        \label{fig:lag:raw}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/time_lag_cdf.pdf}
        \vspace{-6mm}
        \caption{\small{CDF}}
        \label{fig:lag:cdf}
    \end{subfigure}
    \vspace{-5mm}
    \caption{\small{{\bf Time Lag.} }}
    \label{fig:lag}
    \vspace{-4mm}
\end{figure}

\begin{table}
\small
\begin{center}
\begin{tabular}{c |c}
Scheme & Norm. Throughput\\ 
 \hline
 \hline
 Nimbus & 0.99 \\
 \hline
 Cubic &  1.0\\
 \hline 
 BBR & 1.01 \\
 \hline 
 Vegas &  0.77\\
  \hline 
 BasicDelay & 0.99 \\
  \hline 
 Copa &  0.96\\
 \hline 
 PCC-Vivace &  1.38\\

\end{tabular}
\end{center}
\vspace{-1mm}
\caption{\small{\bf Average throughput achieved}}
\label{tab:elasticity}
\vspace{-12mm}
\end{table}
\fi

%\noindent\textbf{Throughput and delay with WAN cross-traffic.} 
We evaluate the delay and throughput benefits of mode switching using trace-driven emulation. We generate cross traffic from an empirical distribution of flow sizes derived from a wide-area packet trace from CAIDA~\cite{caida-dataset}.
%
This packet trace was collected at an Internet backbone router on January 21, 2016 and contains over 30 million packets recorded over 60 seconds. 
%\cut{The maximum rate over any 100 ms period is 2.2 Gbit/s.}
%
We generate Cubic cross-flows with flow sizes drawn from this data, with flow arrival times generated by a Poisson process to offer a fixed average load to fill 50\% of the link (48 Mbit/s).
%
Since the flow size distribution is heavy-tailed, the traffic trace consists of periods with {\em a mix of elastic and inelastic cross-traffic,} along with periods with only inelastic cross-flows.

One backlogged flow running a fixed algorithm (\name, Cubic, Copa, Vegas, PCC-Vivace or BBR) and the WAN-like cross-flows share a 96 Mbit/s \mahimahi bottleneck link with a propagation RTT of 50 ms and a buffer size of 100 ms.
For BasicDelay we used $\alpha=0.8$, $\beta=0.5$ and $d_t=12.5$ ms.

\noindent\textbf{\name{} reduces delays when possible while achieving stable, fair throughput.} 
\Fig{emp:rtt} shows the distribution of per-packet RTT and \Fig{emp:box} shows the deviation from fair-share throughput (over 5-second intervals) for various schemes. 
%We show deviation at 10$^{\text{th}}$, 25$^{\text{th}}$, 50$^{\text{th}}$, 75$^{\text{th}}$, and 90$^{\text{th}}$ percentile.
%Negative deviation means the scheme is sending less than its fair-share.
High deviation\footnote{\pg{Unlike \Fig{big}, the total bytes sent by the cross-traffic is fixed in this experiment. Even purely \dcc schemes (\eg Copa, BasicDelay) achieve the same average throughput as a perfectly fair scheme. \cut{Indeed we find that Copa, \name{}, BasicDelay (only delay-based, not shown here) and Cubic achieve the same average throughput.}}}, 
\ie unfairness with cross traffic, can harm application performance. For example, for a video application, temporary throughput drops can cause stalls, hurting user experience. 
%
%\an{
%Due to mode switching, \name achieves a comparable deviation profile to Cubic (since from a throughput perspective, \name{} emulates Cubic), but with far lower RTTs. Its median RTT is only $10$ms higher than Vegas's and $>50$ms lower than Cubic's and BBR's.
%}

\name and Cubic achieve the best fairness (lowest\footnote{Both \name{} and Cubic deviate from the fair share since Cubic is not perfectly fair to itself over short time periods.} deviation) among all the schemes. \possname deviation profile is comparable to Cubic; \name correctly switches to competitive mode in the presence of elastic flows, and from a throughput perspective, \name{} behaves just like Cubic. 
\cut{\an{this is sort of covered again later} Additionally, by switching to delay-controlling mode in the absence of elastic flows, \name achieves lower RTTs, with a median delay only $10$ ms higher than Vegas and $>50$ ms lower than Cubic and BBR.}
%Vegas suffers from low throughput (high negative deviation at lower percentiles). 

%
%Simultaneously,
%
%\smallskip
%\noindent\textit{Comparison with Copa and PCC-Vivace.} 

\noindent\textbf{Cost of incorrect elasticity detection.} 
Copa has a slightly smaller median delay than \name, but at a high cost:
Copa's throughput deviates from the fair-share at lower percentiles (10$^{\text{th}}$ and 25$^{\text{th}}$). 
\Fig{emp:ts} demonstrates why this is the case, comparing throughput for \name and Copa during a 60-second interval.
%during periods where the cross traffic includes elastic flows. 
%\name and Copa both achieve low delays, and Copa enjoys a slightly smaller delay than \name at the median. 
%However, Copa's throughput deviates from the fair-share at lower percentiles (10$^{th}$ and 25$^{th}$). 
%Unlike \name, Copa makes incorrect mode switches during periods where the cross traffic includes large elastic flows, losing throughput. 
%
%\Fig{emp:ts} demonstrates this by comparing throughput for \name and Copa during a 60-second interval.
%

\an{This point is nuanced and easy to miss:}

Unlike \name, Copa often incorrectly operates in its delay mode against Cubic, with prolonged periods when Copa experiences poor throughput (\eg $130$--$140$ s).
%
In contrast, \name competes fairly against elastic cross-flows over the entire duration. 
%\an{moved above:} Unfairness with cross traffic can hurt application performance. For example, for a video application using Copa, when the throughput drops, the video can stall hurting user experience. 
%
It is important to note \an{cut: that unlike \Fig{big}}, the cross-flow sizes are fixed \an{cut: in size}, and a flow can last for different time durations depending on its \an{cut: own} throughput. 
\an{Because \name{} is fairer to the cross-flows, they last longer in the \name{} experiment than in the Copa experiment. }
%Fair co-existence of \name with elastic cross-flows increases the lifetimes of those flows relative to Copa.
%
This results in \name achieving lower (but fairer) throughput than Copa during periods (\eg 120--130 s) when an elastic flow has completed in Copa, but not in \name. 
Moreover, since elastic flows last longer in \name{}, the delay is higher than Copa at the tail.

%\cut{We find that }
\noindent\textbf{Impact on cross-flows.}
\name helps cross traffic: the $95^{\text{th}}$ percentile flow completion time (FCT) of cross-traffic flows reduces by 3-4$\times$ compared to BBR, and 1.3$\times$ compared to Cubic for short ($\leq$ 15 KB) flows (Appendix~\ref{app:cross-traffic-impact}).
In contrast, PCC-Vivace is very unfair to the background flows (positive deviation). It grabs significantly more bandwidth than all the other schemes and keeps the buffer near-full more than half the time. 
The result is that many background flows do not complete, and their completion times are over 100$\times$ worse than with other schemes.
Furthermore, PCC-Vivace achieves significantly higher delays that any other scheme; the median delay is $90$ ms higher than \name.

\cut{We also evaluated a mode-switching protocol that employs Copa's default mode as its delay-control algorithm (instead of BasicDelay).
We find that its throughput and delay are very similar to \name; henceforth, we only report results for \name (Cubic+BasicDelay). }
%
We repeated the above experiment with cross-traffic BBR flows instead of Cubic. 
Again, \name{} achieves a throughput profile similar to Cubic while reducing delays (Appendix~\ref{app:bbr-comparison}).

\smallskip
\label{s:elasticity-in-real-cross-traffic}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/emp-switch3}
    \vspace{-5.5mm}
    \caption{\small{The elasticity metric, and hence \possname mode, closely tracks the prevalence of elastic cross-traffic (ground truth measured independently using the volume of ACK-clocked flows). Green-shaded regions indicate inelastic periods.}}
    \label{fig:emp:switch}
    \vspace{-4mm}
\end{figure}

%\noindent\textit{Elasticity metric $\eta$ \vs the ``true'' elasticity of cross-traffic.}
\noindent\textbf{Elasticity detection is accurate compared to ground truth.}
%How well does the detector's decision correlate with the true proportion of elastic traffic?
%We illustrate the efficacy of elasticity detection for a single experiment over time using our WAN traffic trace (same setup as \Fig{emp}). 
%We evaluated the accuracy of the elasticity detector in this experiment. 
To define ground truth, we note that
short flows (< 10 packets) transmit all data at once, without any rate adjustments.
%We thus classify a cross-flow in the trace as elastic if it finishes later than a \RTT, \ie flows with sizes higher than the initial congestion window of 10 packets. 
We thus classify a cross-flow as elastic if it is larger than the initial congestion window of 10 packets, finishing in greater than a \RTT.
%
\cut{We classify a cross-flow in the trace as elastic if it is guaranteed to have ACK-clocked packet transmissions over its lifetime, \ie flows with sizes higher than the initial congestion window of 10 packets.}

The top chart in \Fig{emp:switch} shows the fraction of bytes belonging to elastic flows as a function of time. 
The bottom chart shows the output of the elasticity detector with the dashed threshold line at $\eta=2$. 
The shading corresponds to periods when \name is in delay-control mode. 
Shaded regions correlate well with the periods when the true fraction of elastic traffic is low (\eg $<0.3$), while white regions correlate well with periods when the elastic fraction is high. 
Unlike Copa, our elasticity detector observes fluctuations in cross traffic \emph{over a period of time}, and the accuracy is less susceptible to variations in the cross traffic rate. Despite the churn in cross-traffic flows, the overall accuracy of our elasticity detector is over 90\%.

==> eval.tex <==


%%\vspace{-5pt}
\newcommand{\evalsec}{Evaluation}
\section{\evalsec}
\label{s:eval}
%%\vspace{-5pt}
%%\input{eval-big-graph}

We evaluate our elasticity detection method\pg{, \name{},} and a specific protocol using \name{}CC: Cubic+BasicDelay, as in \Sec{mode_switching}. We use the Mahimahi emulator and measure the performance benefits (\Sec{rw-wl}), robustness (\Sec{copa-compare}), and fairness (\Sec{multiple-nimbus-fair-sharing}) of elasticity detection with realistic traffic workloads. We also evaluate the performance of \name{}CC on real Internet paths (\Sec{realworld}). All experiments use our Linux implementation (\Sec{implementation}). 
%In emulation, we use \mahimahi~\cite{mahimahi}, as described earlier in \Sec{big-experiment}.
%% a link emulator that enables the operating system's TCP and UDP stacks to send traffic through a virtual network interface with the desired bottleneck link rate, propagation delay, buffering, and AQM policies. 
%% Our Internet experiments are over paths between Amazon's EC2 machines around the world, well-connected university networks, and residential hosts. 

\input{eval-wan-distribution}
\input{eval-realistic-cross-traffic.tex}
\input{eval-empirical-elasticity.tex}
%\input{eval-versatility.tex}


%% \input{eval-switching}
%\input{eval-cross-traffic-impact.tex}

%\input{eval-switching-wan-traces.tex}
\subsection{Robustness of Elasticity Detection}
\input{eval-switching-synthetic.tex}
%\input{eval-copa-compare-cross-traffic-rtt.tex}
\input{eval-robustness-parameter-sweep.tex}
\input{eval-copa-compare.tex}
\input{eval-multiple-nimbus.tex}
\input{eval-real-world}



%\input{eval-bundle-benefits}
%% Real-world experiments
%\input{eval-real-world}
%% Nimbus deep-dive

%% \begin{enumerate}

%% \item How well does the \name{} delay-control rule perform?
%%   Specifically, with inelastic cross traffic, how quickly does the
%%   sender infer and use the available rate, and does it maintain the
%%   specified target delay? We compare \name{} with BBR~\cite{bbr},
%%   Cubic, and Vegas.

%% \item How well does the mode-switching algorithm work at identifying
%%   the presence and absence of competing elastic traffic? Specifically,
%%   how long does it take to detect such traffic and what is the success
%%   rate of the detector?

%% \item In the face of elastic long-running TCP traffic, how well does
%%   the TCP-competitive mode of \name{} perform as the number of
%%   cross-traffic flows and the number of \name{} flows vary? The
%%   comparisons here are with MulTCP, EBCC, and running $n$ independent
%%   TCPs rather than emulating $n$ AIMDs in \name{}.

%% \item How often is switching modes utilized in real-world scenarios?

%% \end{enumerate}

%% Except where mentioned otherwise, we use a 24 Mbit/s emulated mahimahi
%% link with 50 ms of propagation delay and one BDP of buffering.  We use
%% the Linux implementations of the various schemes we consider.

%% To generate elastic cross traffic, we use iperf~\cite{iperf} for TCP
%% traffic configured to use TCP NewReno.  For inelastic traffic, we use
%% a Poisson traffic generator which is a subset of the \name{} userspace
%% implementation.

%% \input{eval-overall-perf}
%% \input{eval-switching}
%% \input{eval-delay-control}
%% \input{eval-tcp-comp}
%% \input{eval-bw-estimate}

==> fct-table-newintro.tex <==
{
\centering
%%\resizebox{0.5\textwidth}{!}{%
%\begin{tabular}{lllll}
\begin{tabular}{ccccc}
\hline

{\textbf{Algorithm}} &
% {\textbf{15 KB FCTs}} &
% {\textbf{150 MB FCTs}} \\
\multicolumn{2}{c}{\textbf{15 KB FCTs}} &
\multicolumn{2}{c}{\textbf{150 MB FCTs}} \\

&
{\textbf{\bundle}} &
{\textbf{cross}} &
{\textbf{\bundle}} &
{\textbf{cross}} \\

\hline
\hline

% No \bundle &
% \multicolumn{2}{c}{91 ms} &
% \multicolumn{2}{c}{\ngs{XXX}} \\
% 90 ms&
% 92 ms&
% 23.6 s \\
% 17.9 s\\
% \hline

\name &
0.71$\times$&
0.77$\times$&
0.76$\times$&
0.66$\times$\\

BBR &
1.16$\times$&
1.23$\times$&
0.75$\times$&
1.12$\times$\\

Cubic &
0.97$\times$&
1.01$\times$&
0.74$\times$&
1.04$\times$\\

Vegas &
0.63$\times$&
0.66$\times$&
1.35$\times$&
0.69$\times$ \\

\hline
\end{tabular}
%%}
%% \caption{Median FCTs for short and long flows under different \bundle congestion control algorithms.}
\vspace{-0.06in}
\label{fig:fct-summary}
}

==> impl.tex <==
\vspace{-10pt}
\section{Implementation}
\label{s:impl}
\vspace{-5pt}
We implemented \name with two components: a Linux kernel module and associated user-space component which communicate using Linux netlink sockets.
\name's congestion control algorithm, including the switching logic, delay control, and TCP-competitive mode, are $687$ lines of Go in the user-space program.
Meanwhile, the kernel module integrates with Linux Pluggable TCP~\cite{linux-pluggable} API to enforce rates and collect measurements -- the sending and receiving rates and round-trip time -- to report to the user-space component.


Our implementation is compatible with existing applications through the socket API. We have achieved transfer rates up to 10 Gbit/s in our testbed and observed rates up to 2 Gbit/s on intercontinental links in the WAN. Unless otherwise specified, our implementation uses $f_S = 5$ and $n_b = 2$.

%%We discuss our preliminary experience evalutating our implementation on real paths in~\ref{s:realworld}.

Because our algorithm runs in user-space, it is possible to implement \name on DPDK by replacing the kernel module with a similar component which interfaces with DPDK. We plan to explore this in the future.



==> intro-feb2020.tex <==
\section{Introduction}
\label{s:intro}

%To date, congestion control methods have used a number of congestion signals (losses, delays, rate estimates, etc.), but have not explicitly estimated or responded to what the competing traffic is trying to do. 

Achieving high throughput and low delay has been a key goal of congestion control research for decades. To achieve these goals, researchers have proposed many {\em delay-controlling} algorithms. These schemes (e.g., Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, Copa~\cite{copa}) reduce their rates as delays increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}, unlike methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound2} that must fill buffers to elicit congestion signals (packet losses or ECN).

% Congestion control
% algorithms can be broadly classified as {\em buffer-filling} or {\em
% delay-based}. buffer-filling
% methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound, compound2} reduce their window
% only in response to packet loss or explicit congestion notification (ECN) signals, whereas delay-based algorithms like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat},
% Sprout~\cite{sprout}, and Copa~\cite{copa} reduce their rates as delays
% increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}.

\if 0
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-cubic-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Cubic: High delay}}
        \label{fig:overview:cubic}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-delay-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Delay-control: Throughput drops}}
        \label{fig:overview:vegas}
    \end{subfigure}
    \begin{subfigure}[b]{0.34\textwidth}
        \includegraphics[width=0.94\textwidth]{images/overview-nimbus-cubic-delay-sigcomm19.pdf}
        \vspace{-3mm}
        \caption{\small{\name: Lower delay and high throughput}}
        \label{fig:overview:nimbus}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small On a 48 Mbit/s link, a flow competes with one elastic long-running Cubic flow for 60 seconds (starting at $t=30$ sec.), followed by 60 seconds of inelastic traffic sending at 24 Mbit/s. We compare Cubic, a delay-controlling scheme (\S\ref{s:mode_switching}), and Nimbus, configured to switch between these two methods based on cross traffic elasticity.     Cubic has a large queuing delay throughout. The delay-controlling scheme achieves low delay when the cross traffic is inelastic but suffers significant throughput loss when it competes with Cubic. Using mode switching, Nimbus achieves the fair throughput against Cubic {\em and} lower queuing delays when the cross traffic is inelastic.}
    \label{fig:overview}
    \vspace{-4.5mm}
\end{figure*}

\fi

There is, however, a major obstacle to deploying delay-controlling
algorithms on the Internet: their throughput is dismal when competing
against buffer-filling senders at a shared bottleneck. The reason
is that buffer-filling senders increase their rates until they observe
losses, which causes queuing delays to increase; in response to
increasing delays, a competing delay-controlling flow will reduce its rate. The buffer-filling flow then grabs this
freed-up bandwidth. The throughput of the delay-controlling flow
plummets, but delays don't reduce. Because most traffic on the Internet today uses buffer-filling algorithms, it is hard
to justify deploying a delay-controlling scheme.

Is it possible to achieve the benefits of \dcc algorithms while ensuring that throughput does not degrade in the presence of buffer-filling schemes? This question has received some attention recently, with Copa proposing an algorithm with two modes---a ``default'' mode that controls delay but which competes poorly against schemes like Cubic, and a ``TCP-competitive'' mode that has no delay control but competes more aggressively. Copa, however, bases its decision using heuristics to determine if the cross traffic is Copa or not, rather than on a deeper understanding of what the cross traffic is attempting; we find that it makes erroneous decisions in many cases.

%\cut{Copa uses round-trip time (RTT) observations to determine if the RTT time-series is consistent with only other Copa flows sharing the bottleneck (e.g., Copa periodically empties network queues); if so, the sender uses the delay-controlling mode, but if not, the sender switches to a TCP-competitive mode. }

We propose here a new, robust approach based on rigorously characterizing cross traffic as {\em elastic} or {\em inelastic} using round-trip time (RTT) observations at a sender. We define a flow to be ``elastic'' if, and only if, it {\em increases its rate when it senses that more bandwidth is available, and decreases it otherwise}. All other traffic is defined as ``inelastic''. Examples of elastic traffic include backlogged congestion-controlled flows using either buffer-filling methods like Cubic and NewReno, or delay-based schemes like Vegas, Copa, and BBR~\cite{bbr}. Examples of inelastic traffic, by contrast, include constant bit-rate (CBR) flows, short TCP connections, application-limited flows, and traffic bottlenecked at a different link. 

We have developed an {\em elasticity detector} called {\em Nimbus}, which any sender can implement. When Nimbus deems cross traffic to be inelastic, a \dcc algorithm can be used to achieve low delay, but when cross traffic is elastic, an algorithm that competes fairly with the cross traffic without necessarily attempting to control delay is required. We note that Nimbus determines if cross traffic is elastic, and not whether it is governed by a delay-controlling or buffer-filling algorithm. 
%(e.g., a \dcc scheme like Vegas is also elastic).
%A \dcc method may be unable to achieve a fair share of the throughput when sharing a bottleneck with a delay-based elastic flow; 
%As explained previously, the throughput of a delay-controlling algorithm suffers in the presence of buffer-filling schemes, but even in the presence of delay-based elastic flows, a delay-controlling algorithm may be unable to obtain its fair share of throughput.
%e.g., Vegas may compete fairly with other Vegas flows, but it may get less than its fair share of throughput against Copa. 

\if 0
\pg{In this paper, we ask the question, when is it absolutely safe to run a \dcc algorithm? We characterize cross traffic scenarios where running a \dcc algorithm might achieve lower throughput compared to a buffer-filling scheme. In case the cross traffic contains flows that adjust their rates based on the available bandwidth (i.e. the rate of the competing flows), then, throughput of the \dcc algorithm is dependent on the congestion control algorithms used by the cross traffic; and it might not be safe to run a \dcc algorithm. We call such flows that adjust their rates based on the rate of the cross-traffic as elastic flows. Examples of elastic flows include long-running Cubic, NewReno, Copa, Vegas and BBR~\cite{bbr} flows. Note that running a \dcc algorithm like Vegas against other \dcc algorithms like Copa might result in unfairness. In contrast running Vegas in presence of other Vegas flows is safe. Therefore, to be sure that running a \dcc algorithm is safe against other \dcc algorithms, we need to detect the CC protocol of the cross traffic. Detecting the cross traffic's CC remains an open problem. In this work we present the absence of elastic flows as a sufficient but not necessary condition for running a \dcc algorithm safely. }

\pg{By contrast, inelastic senders do not attempt to grab all unused bandwidth, and their rates do not vary with bandwidth availability. Examples include short TCP flows (flows that transmit all data without receiving ACKs or adjust the rate) or, application-limited flows (e.g., video streaming flows rate limited by the quality of the video), constant bit-rate streams, and flows that are bottlenecked at a different link. When the cross traffic is inelastic, delay-controlling schemes can achieve \pg{similar throughput as their buffer-filling counterparts} while maintaining low delay. Using aggressive \pg{buffer-filling} algorithms provides little benefit against in \pg{absence of elastic flows}, since they don't reduce their rate in response to cross traffic.}

 \pg{The goal our our work is to allow a sender to achieve similar throughput as a given ``TCP-Competetive'' congestion control protocol (e.g., Cubic) while reducing delays when possible. To achieve this, we introduce a new, robust approach to determine whether the cross traffic any elastic flows. In case the cross-traffic contains elastic flows, running a \dcc algorithm might be unsafe. In such a scenario, the sender should use the given TCP-competitive algorithm. Otherwise the sender can use a \dcc algorithm to reduce delays without worrying about losing throughput.}

\fi 

\cut{Our method explicitly characterizes whether the competing cross traffic contains any \emph{elastic} flows. An elastic flow is one that fills up all available bandwidth; it increases its rate if it perceives unused bandwidth, and it slows down if the available bandwidth drops. Examples of elastic flows include long-running Cubic, NewReno, Copa, Vegas and BBR~\cite{bbr} flows. When the cross traffic is elastic, delay-controlling algorithms are susceptible to poor throughput. To be safe, it is important to detect this situation and switch to a mode that mimics the behavior of the prevailing cross traffic.\footnote{Even if the cross traffic uses a delay-controlling protocol like Vegas, it might not be fair to other delay-controlling schemes (e.g., Copa). Hence, against elastic (i.e., long-running) delay-controlling flows we advocate mimicking widely-deployed TCP protocols like Cubic.}}

\cut{By contrast, inelastic senders do not attempt to grab all unused bandwidth, and their rates do not vary with bandwidth availability. Examples include short TCP flows, application-limited flows, constant bit-rate streams, and flows that are bottlenecked at a different link. When the cross traffic is inelastic, delay-controlling schemes can achieve high throughput while maintaining low delay. Using aggressive TCP-competitive methods  provides little benefit against inelastic flows, since they don't reduce their rate in response to cross traffic. }

\smallskip
\noindent
{\bf Elasticity detection.} Nimbus uses only end-to-end observations to monitor the cross traffic to determine if the cross traffic contains \emph{any} elastic flows. The sender continuously modulates its rate with sinusoidal pulses to create small traffic fluctuations at the bottleneck at a specific frequency (e.g., 5 Hz). It concurrently estimates the rate of the cross traffic based on the its own send and receive rates, and monitors its frequency response (FFT) to determine if the cross traffic's rate oscillates at the same frequency. If it does, then the sender concludes that the cross traffic contains elastic flows; otherwise, it is inelastic. 

This technique relies on two assumptions. First, the sender must be able to create sufficient pulses %(e.g., burst at 20\% of the bottleneck capacity)
and observe the impact on cross traffic over a period of time. Hence our technique is best suited for large data transfers.
%to senders that control large data transfers, such as large file downloads, data backups to the cloud, video, etc. 
Fortunately, it is precisely for such transfers that delay-controlling schemes can provide the most benefit, because short flows are unlikely to cause significant queueing delay~\cite{bufferbloat}. 

Second, pulsing is most effective when the elastic flows in the cross traffic are sensitive to traffic fluctuations at the bottleneck on a short timescale, for example, a few RTTs. If an elastic flow is slow to react to bandwidth changes, it can go undetected with small traffic pulses. While it is possible in theory to use large pulses to detect such ``sluggish'' elastic flows, this could cause congestion. Most congestion-controlled elastic flows react to bandwidth variations on RTT timescales. In particular, the majority of TCP traffic on the Internet is ACK-clocked. For these flows, RTT-timescale changes in the receive rate get reflected in similar changes to the send rate via ACKs, thereby causing the senders to oscillate at the same frequency as the traffic fluctuations at the bottleneck. Our elasticity detector is targeted at detecting {\em ACK-clocked elastic flows}, but we have also found that it classifies fast-reacting rate-based flows as elastic.

%\ma{I don't know if we should say the last sentence. i think the only example of a rate-based scheme that we can detect as elastic is the nimbus delay algorithm. The point I am trying to make is that the fundamental requirement is not ACK clocking but fast reaction to changes in cross traffic, which is a desirable property for congestion control.}

%This technique works well because elastic and inelastic flows react differently to short-timescale traffic variations at the bottleneck. In particular, \pg{we make use of the observation} that most elastic TCP flows are ACK-clocked; therefore, fluctuations in the inter-packet arrival times at the receiver, reflected in ACKs, cause similar fluctuations in subsequent packet transmissions at the sender. This causes the rate of these flows to oscillate at the same frequency as the traffic fluctuations at the bottleneck. By contrast, the rate of an inelastic flow is not sensitive to traffic variations at the bottleneck. 

%\pg{We dicuss the practical robustness of our approach in \S\ref{s:elasticity:properties}}

\textbf{Take away for the elasticity detector:}\pg{
\begin{CompactEnumerate}
\item The result is a robust method for elasticity detector. Our elasticity detector is robust to a variety of cross traffic conditions, achieving at least 85\% accuracy when: (i) the cross traffic is a combination of varying number of elastic flows and highly-varying inelastic short flows; (ii) the cross traffic RTT is different from \name's RTT; (iii) the cross traffic is composed of multiple elastic flows with different RTTs. These results hold across a wide range of network characteristics:  buffer sizes, RTTs, bottleneck link rates, active queue management schemes, and shares of the bottleneck link rate controlled by Nimbus.
\item Compared to Copa, our elasticity detector classifies cross traffic more accurately and is more robust. 1) Copa makes frequent incorrect mode switches. 2) Copa’s classifier fails when the inelastic cross traffic rate exceeds 80\%. 3) The accuracy of detecting elastic flows degrades from 85\% to 15\% when the RTT ratio between the cross traffic and Copa increases from 1 to 4. By contrast our accuracy is close to 100\% on the same benchmarks. 
\end{CompactEnumerate}
}


\smallskip
\noindent {\bf NimbusCC.} We describe and evaluate NimbusCC, a congestion control system that uses our elasticity detector to switch between   TCP-competitive and delay-controlling modes. NimbusCC can support a variety of algorithms in each mode. We report results with Vegas, Copa's ``default mode'', and a simple new method that uses our cross traffic rate estimator, as examples of \dcc algorithms, and Cubic and Reno as examples of buffer-filling algorithms. 
The absence of elastic flows in the cross traffic is a \emph{sufficient} (but not necessary) condition for operating in a delay-controlling mode without loss of throughput. Our goal is to ensure throughput on par with a baseline buffer-filling scheme like Cubic, while exploiting opportunities with no elastic cross traffic to switch to a delay-controlling scheme. We leave the problem of how to use a delay-controlling mode in the presence of delay-based elastic cross traffic to future work. This requires methods beyond elasticity detection, such as detecting the type of congestion control algorithm used by elastic cross traffic.   

%\Fig{overview} shows an example result with \name. 
%\ma{Do we really show results with all these schemes?}

\smallskip
\noindent {\bf Key results:} We have implemented the elasticity detector and Nimbus in Linux using CCP~\cite{ccp-sigcomm18}. Our experimental results show that:
\begin{CompactEnumerate}
\item We kick ass.
\item Accepting this paper is a no-brainer
\end{CompactEnumerate}

\textbf{Benefits of using elasticity detection for CC:}\pg{
\begin{CompactEnumerate}
\item With a synthetic cross traffic that include intermersed periods of both elastic and inelastic traffic. \name achieves the fairshare rate. Against elastic cross traffic Nimbus achieves 65\% throughput than Copa. Moreover \name reduces delay when the traffic is inelastic.
\item With a WAN cross-traffic trace, \name achieves throughput comparable to  Cubic and BBR but with 50 ms lower median delay. Copa incurs unfairness.
\item For video cross traffic, on average \name achieves throughput comparable to Cubic and 10$\times$ higher than Copa. Cubic incurs 30\% higher mean queuing delay than \name. PCC-Vivace and BBR incur higher delay and achieve lower throughput than \name.
\item On real Internet paths, \name (switching between Cubic and a simple delay-controlling scheme) achieves throughput comparable to or better than Cubic on most of the 25 real-world paths we tested, with lower delays in 60\% of paths and similar delays in the other 40\% of paths. Compared to BBR, \name achieves 10\% lower mean throughput, but at 40--50 ms lower packet delay.
\end{CompactEnumerate}
}

The principal new contribution of this paper is the idea that the {\em nature of cross traffic}, quantified here in the form of elasticity, is a useful building block for congestion control. We envision it being used to solve other problems in the future. For example, as 
in tools like speedtest or iperf to inform users of not only what the rate is, but also whether the rate is lower than expected due to elastic cross traffic. This can shed further light on traffic behavior and may also help guide the deployment of active queue management (AQM) schemes.  Another example is as a sub-system for aggregate traffic management of a traffic bundle consisting of many flows to achieve controlled delays. 


==> intro-sep2019.tex <==
\section{Introduction}
\label{s:intro}

Achieving high throughput and low delay has been a primary motivation for congestion 
control research for decades. To achieve these goals, researchers have proposed many {\em delay-controlling} algorithms over the years. Unlike {\em loss-based} methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound2}, delay-controlling schemes like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, and Copa~\cite{copa} reduce their rates as delays increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}. 

% Congestion control
% algorithms can be broadly classified as {\em loss-based} or {\em
% delay-based}. Loss-based
% methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound, compound2} reduce their window
% only in response to packet loss or explicit congestion notification (ECN) signals, whereas delay-based algorithms like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat},
% Sprout~\cite{sprout}, and Copa~\cite{copa} reduce their rates as delays
% increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-cubic-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Cubic: High delay}}
        \label{fig:overview:cubic}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-delay-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Delay-control: Throughput drops}}
        \label{fig:overview:vegas}
    \end{subfigure}
    \begin{subfigure}[b]{0.34\textwidth}
        \includegraphics[width=0.94\textwidth]{images/overview-nimbus-cubic-delay-sigcomm19.pdf}
        \vspace{-3mm}
        \caption{\small{\name: Lower delay and high throughput}}
        \label{fig:overview:nimbus}
    \end{subfigure}
    \vspace{-3.5mm}
    \caption{\small On a 48 Mbit/s link, a flow competes with one elastic long-running Cubic flow for 60 seconds (starting at $t=30$ sec.), followed by 60 seconds of inelastic traffic sending at 24 Mbit/s. We compare Cubic, a delay-controlling scheme (\S\ref{s:mode_switching}), and Nimbus, configured to switch between these two methods based on cross traffic elasticity.     Cubic has a large queuing delay throughout. The delay-controlling scheme achieves low delay when the cross traffic is inelastic but suffers significant throughput loss when it competes with Cubic. Using mode switching, Nimbus achieves the fair throughout against Cubic {\em and} lower queuing delays when the cross traffic is inelastic.}
    \label{fig:overview}
    \vspace{-4.5mm}
\end{figure*}

There is, however, a major obstacle to deploying delay-controlling
algorithms on the Internet: their throughput is dismal when competing
against loss-based senders at a shared bottleneck. The reason
is that loss-based senders increase their rates until they observe
losses, which causes queuing delays to increase; in response to
increasing delays, a competing delay-controlling flow will reduce its rate. The loss-based flow then grabs this
freed-up bandwidth. The throughput of the delay-controlling flow
plummets, but delays don't reduce. Because most traffic on the Internet today uses loss-based algorithms, it is hard
to justify deploying a delay-controlling scheme.

Is it possible to achieve the benefits of \dcc algorithms while ensuring that throughput does not degrade in the presence of schemes like Cubic or NewReno? This question has received some attention recently, with Copa proposing an algorithm with two modes---a ``default'' mode that controls delay but which competes poorly against schemes like Cubic, and a ``TCP-competitive'' mode that has no delay control but competes more aggressively. \cut{Copa uses round-trip time (RTT) observations to determine if the RTT time-series is consistent with only other Copa flows sharing the bottleneck (e.g., Copa periodically empties network queues); if so, the sender uses the delay-controlling mode, but if not, the sender switches to a TCP-competitive mode. }

Motivated by this question, we ask whether we can characterize cross traffic as {\em elastic} or {\em inelastic} using only observations of packet delivery timings at a sender and receiver. By ``elastic'', we mean traffic that increases its rate when it senses that more bandwidth is available, and decreases it otherwise. Examples of elastic traffic include backlogged congestion-controlled flows using either loss-based methods like Cubic and NewReno, or delay-based ones like Vegas, Copa, and BBR~\cite{bbr}. Examples of inelastic traffic, by contrast, include constant bit-rate (CBR) flows,  short TCP connections, application-limited flows, and cross traffic bottlenecked at a different link. 

We show that setting the operating mode of a congestion control algorithm using the output of an {\em elasticity detector} produces robust congestion controllers. When cross traffic is inelastic, a \dcc algorithm can be used to achieve low delay, but when cross traffic is elastic, an algorithm that competes fairly with the cross traffic without necessarily attempting to control delay is required. We note that the relevant aspect of cross traffic is its elasticity, and not whether it is governed by a delay-controlling or loss-based algorithm. A \dcc method may be unable to achieve a fair share of the throughput when sharing a bottleneck with a delay-based elastic flow; 
%As explained previously, the throughput of a delay-controlling algorithm suffers in the presence of loss-based schemes, but even in the presence of delay-based elastic flows, a delay-controlling algorithm may be unable to obtain its fair share of throughput.
e.g., Vegas may compete fairly with other Vegas flows, but it may get less than its fair share of throughput against Copa. 

We therefore seek to detect the absence of elastic flows in the cross traffic, as a \emph{sufficient} (but not necessary) condition for operating in a delay-controlling mode without loss of throughput. Our goal is to ensure throughput on par with a baseline TCP-competitive scheme like Cubic, while exploiting opportunities with no elastic cross traffic to switch to a delay-controlling scheme. We leave the problem of how to use a delay-controlling mode in the presence of delay-based elastic cross traffic to future work. This requires methods beyond elasticity detection, such as detecting the type of congestion control algorithm used by elastic cross traffic.   

\if 0
\pg{In this paper, we ask the question, when is it absolutely safe to run a \dcc algorithm? We characterize cross traffic scenarios where running a \dcc algorithm might achieve lower throughput compared to a loss-based scheme. In case the cross traffic contains flows that adjust their rates based on the available bandwidth (i.e. the rate of the competing flows), then, throughput of the \dcc algorithm is dependent on the congestion control algorithms used by the cross traffic; and it might not be safe to run a \dcc algorithm. We call such flows that adjust their rates based on the rate of the cross-traffic as elastic flows. Examples of elastic flows include long-running Cubic, NewReno, Copa, Vegas and BBR~\cite{bbr} flows. Note that running a \dcc algorithm like Vegas against other \dcc algorithms like Copa might result in unfairness. In contrast running Vegas in presence of other Vegas flows is safe. Therefore, to be sure that running a \dcc algorithm is safe against other \dcc algorithms, we need to detect the CC protocol of the cross traffic. Detecting the cross traffic's CC remains an open problem. In this work we present the absence of elastic flows as a sufficient but not necessary condition for running a \dcc algorithm safely. }

\pg{By contrast, inelastic senders do not attempt to grab all unused bandwidth, and their rates do not vary with bandwidth availability. Examples include short TCP flows (flows that transmit all data without receiving ACKs or adjust the rate) or, application-limited flows (e.g., video streaming flows rate limited by the quality of the video), constant bit-rate streams, and flows that are bottlenecked at a different link. When the cross traffic is inelastic, delay-controlling schemes can achieve \pg{similar throughput as their loss-based counterparts} while maintaining low delay. Using aggressive \pg{loss-based} algorithms provides little benefit against in \pg{absence of elastic flows}, since they don't reduce their rate in response to cross traffic.}

 \pg{The goal our our work is to allow a sender to achieve similar throughput as a given ``TCP-Competetive'' congestion control protocol (e.g., Cubic) while reducing delays when possible. To achieve this, we introduce a new, robust approach to determine whether the cross traffic any elastic flows. In case the cross-traffic contains elastic flows, running a \dcc algorithm might be unsafe. In such a scenario, the sender should use the given TCP-competitive algorithm. Otherwise the sender can use a \dcc algorithm to reduce delays without worrying about losing throughput.}

\fi 

\cut{Our method explicitly characterizes whether the competing cross traffic contains any \emph{elastic} flows. An elastic flow is one that fills up all available bandwidth; it increases its rate if it perceives unused bandwidth, and it slows down if the available bandwidth drops. Examples of elastic flows include long-running Cubic, NewReno, Copa, Vegas and BBR~\cite{bbr} flows. When the cross traffic is elastic, delay-controlling algorithms are susceptible to poor throughput. To be safe, it is important to detect this situation and switch to a mode that mimics the behavior of the prevailing cross traffic.\footnote{Even if the cross traffic uses a delay-controlling protocol like Vegas, it might not be fair to other delay-controlling schemes (e.g., Copa). Hence, against elastic (i.e., long-running) delay-controlling flows we advocate mimicking widely-deployed TCP protocols like Cubic.}}

\cut{By contrast, inelastic senders do not attempt to grab all unused bandwidth, and their rates do not vary with bandwidth availability. Examples include short TCP flows, application-limited flows, constant bit-rate streams, and flows that are bottlenecked at a different link. When the cross traffic is inelastic, delay-controlling schemes can achieve high throughput while maintaining low delay. Using aggressive TCP-competitive methods  provides little benefit against inelastic flows, since they don't reduce their rate in response to cross traffic. }

\smallskip
\noindent
{\bf Elasticity detection.} We have developed an elasticity detector that uses only end-to-end observations to monitor the cross traffic to determine if the cross traffic contains \emph{any} elastic flows. The sender continuously modulates its rate with sinusoidal pulses to create small traffic fluctuations at the bottleneck at a specific frequency (e.g., 5 Hz). It concurrently estimates the rate of the cross traffic based on the its own send and receive rates, and monitors its frequency response (FFT) to determine if the cross traffic's rate oscillates at the same frequency. If it does, then the sender concludes that the cross traffic contains elastic flows; otherwise, it is inelastic. 

This technique relies on two assumptions. First, the sender must be able to create sufficient pulses %(e.g., burst at 20\% of the bottleneck capacity)
and observe the impact on cross traffic over a period of time. Hence our technique is best suited for large data transfers.
%to senders that control large data transfers, such as large file downloads, data backups to the cloud, video, etc. 
Fortunately, it is precisely for such transfers that delay-controlling schemes can provide the most benefit, because short flows are unlikely to cause significant queueing delay~\cite{bufferbloat}. 

Second, pulsing is most effective when the elastic flows in the cross traffic are sensitive to traffic fluctuations at the bottleneck on a short timescale, for example, a few RTTs. If an elastic flow is slow to react to bandwidth changes, it can go undetected with small traffic pulses. While it is possible in theory to use large pulses to detect such ``sluggish'' elastic flows, this could cause congestion. Most congestion-controlled elastic flows react to bandwidth variations on RTT timescales. In particular, the majority of TCP traffic on the Internet is ACK-clocked. For these flows, RTT-timescale changes in the receive rate get reflected in similar changes to the send rate via ACKs, thereby causing the senders to oscillate at the same frequency as the traffic fluctuations at the bottleneck. Our elasticity detector is targeted at detecting {\em ACK-clocked elastic flows}, but we have also found that it classifies fast-reacting rate-based flows as elastic.


\textbf{Take away for the elasticity detector:}\pg{
\begin{CompactEnumerate}
\item The result is a robust method for elasticity detector. Our elasticity detector is robust to a variety of cross traffic conditions, achieving at least 85\% accuracy when: (i) the cross traffic is a combination of varying number of elastic flows and highly-varying inelastic short flows; (ii) the cross traffic RTT is different from \name's RTT; (iii) the cross traffic is composed of multiple elastic flows with different RTTs. These results hold across a wide range of network characteristics:  buffer sizes, RTTs, bottleneck link rates, active queue management schemes, and shares of the bottleneck link rate controlled by Nimbus.
\item Compared to Copa, our elasticity detector classifies cross traffic more accurately and is more robust. 1) Copa makes frequent incorrect mode switches. 2) Copa’s classifier fails when the inelastic cross traffic rate exceeds 80\%. 3) The accuracy of detecting elastic flows degrades from 85\% to 15\% when the RTT ratio between the cross traffic and Copa increases from 1 to 4. By contrast our accuracy is close to 100\% on the same benchmarks. 
\end{CompactEnumerate}
}

%\ma{I don't know if we should say the last sentence. i think the only example of a rate-based scheme that we can detect as elastic is the nimbus delay algorithm. The point I am trying to make is that the fundamental requirement is not ACK clocking but fast reaction to changes in cross traffic, which is a desirable property for congestion control.}

%This technique works well because elastic and inelastic flows react differently to short-timescale traffic variations at the bottleneck. In particular, \pg{we make use of the observation} that most elastic TCP flows are ACK-clocked; therefore, fluctuations in the inter-packet arrival times at the receiver, reflected in ACKs, cause similar fluctuations in subsequent packet transmissions at the sender. This causes the rate of these flows to oscillate at the same frequency as the traffic fluctuations at the bottleneck. By contrast, the rate of an inelastic flow is not sensitive to traffic variations at the bottleneck. 

%\pg{We dicuss the practical robustness of our approach in \S\ref{s:elasticity:properties}}

\smallskip
\noindent {\bf \name.}
We present the design and evaluation of \name, a congestion control system that uses our elasticity detector to switch between   TCP-competitive and delay-controlling modes. \name can support a variety of algorithms in each mode. We report results with Vegas, Copa's ``default mode'', and a simple new method that uses our cross traffic rate estimator, as examples of \dcc algorithms, and Cubic and Reno as examples of TCP-competitive algorithms. 
\Fig{overview} shows an example result with \name. 
%\ma{Do we really show results with all these schemes?}

Our elasticity detector is a building block not only for Nimbus, but we envision it being used to solve other problems. 
%One example is as a sub-system for  aggregate traffic management of a traffic bundle consisting of many flows to achieve controlled delays~\cite{bundler}. 
An example is a measurement and diagnostic tool to detect the nature of cross traffic, which might shed light on traffic behavior and guide the deployment of active queue management (AQM) schemes.


We have implemented the elasticity detector and Nimbus in Linux using CCP~\cite{ccp-sigcomm18}. Our experimental results show that:

\textbf{Benefits of using elasticity detection for CC:}\pg{
\begin{CompactEnumerate}
\item On 
\item On an emulated bottleneck link (96 Mbit/s, 50 ms delay, 100 ms buffering) with a WAN cross-traffic trace, \name achieves throughput comparable to  Cubic and BBR but with 50 ms lower median delay. 
\item
\end{CompactEnumerate}
}


\begin{CompactEnumerate}
\item On an emulated bottleneck link (96 Mbit/s, 50 ms delay, 100 ms buffering) with a WAN cross-traffic trace, \name achieves throughput comparable to  Cubic and BBR but with 50 ms lower median delay. 
%\pg{Copa achieves a 5 ms smaller median delay than \name, but at the expense of much lower throughput against elastic traffic.}
\cut{\item \possname reduction in overall delays benefits the cross-traffic significantly: tail flow completion times for cross-traffic sharing the link with \name are 3--4$\times$ smaller than with BBR both for short ($<$ 15 KB) and long ($>$ 150 MB) flows, and 1.25$\times$ smaller than Cubic for short flows.}
\item For video cross traffic, on average \name achieves throughput comparable to Cubic and 10$\times$ higher than Copa. Cubic incurs 30\% higher mean queuing delay than \name. PCC-Vivace and BBR incur higher delay and achieve lower throughput than \name.

\item Our elasticity detector is robust to a variety of cross traffic conditions, achieving at least 85\% accuracy when: (i) the cross traffic is a combination of varying number of elastic flows and highly-varying inelastic short flows; (ii) the cross traffic RTT is different from \name's RTT; (iii) the cross traffic is composed of multiple elastic flows with different RTTs.

\item Compared to Copa, our elasticity detector classifies cross traffic more accurately and is more robust. 
% inelastic cross traffic whereas Copa's accuracy is lower than 80\%. 
For instance, Copa's classifier fails when the inelastic cross traffic rate exceeds 80\%, and its accuracy of detecting elastic flows degrades from 85\% to 15\% when the RTT ratio between the cross traffic and Copa increases from 1 to 4. By contrast our accuracy is close to 100\%, dropping less then 10\% when the RTT ratio is 4:1.
%\item \pg{Verify} By varying the modulation frequency, \name can detect and synchronize with other \name flows (\S\ref{s:multinimbus}).
These results hold across a wide range of network characteristics: \cut{such as different} buffer sizes, RTTs, bottleneck link rates, active queue management schemes, and shares of the bottleneck link rate controlled by \name.

\item On real Internet paths, \name (switching between Cubic and a simple delay-controlling scheme) achieves throughput comparable to or better than Cubic on most of the 25 real-world paths we tested, with lower delays in 60\% of paths and similar delays in the other 40\% of paths. Compared to BBR, \name achieves 10\% lower mean throughput, but at 40--50 ms lower packet delay.
%
%% TODO: add a sentence about BBR if required
\end{CompactEnumerate}



==> intro.tex <==
\newcommand{\introsec}{Introduction}
\section{\introsec}
\label{s:intro}

Achieving high throughput and low delay has been a primary motivation for congestion control research for decades. To achieve these goals, researchers have proposed many {\em delay-controlling} algorithms over the years. Unlike {\em loss-based} methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound2}, delay-controlling schemes like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, and Copa~\cite{copa} reduce their rates as delays increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}. 

% Congestion control
% algorithms can be broadly classified as {\em loss-based} or {\em
% delay-based}. Loss-based
% methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound, compound2} reduce their window
% only in response to packet loss or explicit congestion notification (ECN) signals, whereas delay-based algorithms like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat},
% Sprout~\cite{sprout}, and Copa~\cite{copa} reduce their rates as delays
% increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-cubic-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Cubic: High delay}}
        \label{fig:overview:cubic}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-delay-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Delay-control (\S\ref{s:mode_switching}): Throughput drops}}
        \label{fig:overview:vegas}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-cubic-delay-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{\name: Lower delay}}
        \label{fig:overview:nimbus}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small On a 48 Mbit/s link, a flow competes with one elastic long-running Cubic flow for 60 seconds (starting at $t=30$ sec.), followed by 60 seconds of inelastic traffic sending at 24 Mbit/s. We compare Cubic, a delay-controlling scheme (\S\ref{s:mode_switching}), and Nimbus, configured to switch between these two methods based on cross traffic elasticity.     Cubic has a large queuing delay throughout. The delay-controlling scheme achieves low delay when the cross traffic is inelastic but suffers significant throughput loss when it competes with Cubic. Using mode switching, Nimbus achieves the fair throughput against Cubic {\em and} low queuing delay when the cross traffic is inelastic.}
    \label{fig:overview}
    \vspace{-4mm}
\end{figure*}

There is, however, a major obstacle to deploying delay-controlling
algorithms on the Internet: their throughput is dismal when competing
against loss-based senders at a shared bottleneck. The reason
is that loss-based senders increase their rates until they observe
losses, which causes queuing delays to increase; in response to
increasing delays, a competing delay-controlling flow will reduce its rate. The loss-based flow then grabs this
freed-up bandwidth. The throughput of the delay-controlling flow
plummets, but delays don't reduce. Because most traffic on the Internet today uses loss-based algorithms, it is hard
to justify deploying a delay-controlling scheme.

Can we achieve the benefits of \dcc algorithms whenever possible, while ensuring that throughput does not degrade in the presence of schemes like Cubic or NewReno? This question has received some attention recently, with Copa~\cite{copa} proposing an algorithm with two modes---a ``default'' mode that controls delay but which competes poorly against schemes like Cubic, and a ``TCP-competitive'' mode that has no delay control but competes more aggressively. Copa uses round-trip time (RTT) observations to determine if the RTT time-series is consistent with only other Copa flows sharing the bottleneck (e.g., Copa periodically empties network queues); if so, the sender uses the delay-controlling mode, but if not, the sender switches to a TCP-competitive mode. 

We introduce a new, more robust approach to determining the best operating mode. Our method explicitly characterizes whether the competing cross traffic contains any \emph{elastic} flows. An elastic flow is one that fills up all available bandwidth; it increases its rate if it perceives unused bandwidth, and it slows down if the available bandwidth drops. Examples of elastic flows include long-running Cubic, NewReno, Copa, Vegas and BBR~\cite{bbr} flows. When the cross traffic is elastic, delay-controlling algorithms are susceptible to poor throughput. To be safe, it is important to detect this situation and switch to a mode that mimics the behavior of the prevailing cross traffic.\footnote{Even if the cross traffic uses a delay-controlling protocol like Vegas, it might not be fair to other delay-controlling schemes (e.g., Copa). Hence, against elastic (i.e., long-running) delay-controlling flows we advocate mimicking widely-deployed TCP protocols like Cubic.}

By contrast, inelastic senders do not attempt to grab all unused bandwidth, and their rates do not vary with bandwidth availability. Examples include short TCP flows, application-limited flows, constant bit-rate streams, and flows that are bottlenecked at a different link. When the cross traffic is inelastic, delay-controlling schemes can achieve high throughput while maintaining low delay. Using aggressive TCP-competitive methods  provides little benefit against inelastic flows, since they don't reduce their rate in response to cross traffic. 

%(e.g., a video stream playing at its highest quality with rate of data generated being lesser than sending rate supported by underlying congestion control)

\if 0
Our experiments on more than 25 Internet paths show that scenarios where cross traffic is predominantly inelastic are common. Figure~\ref{fig:dsmotivation} shows results from one of these paths. The plot shows the average throughput and average delay for Cubic and a \dcc scheme (described in \S\ref{s:nimbus-protocol}) for 100 experiments with each protocol over a three-day period. Each experiment ran for 60 seconds. The \dcc scheme generally achieves much lower delays than Cubic, with similar throughput. This shows that there is an opportunity to significantly improve delays using \dcc algorithms, provided we can detect buffer-filling TCPs and compete with them fairly when needed. 

\begin{figure}
    \includegraphics[width=\columnwidth]{images/dsmotivation2.pdf}
    \caption{\small Buffer-filling vs. delay-control congestion control.  The plot shows the average throughput and delay for 100 experiments with Cubic and the Nimbus delay-control algorithm (\S\ref{s:nimbus-protocol}). The experiments were run between a residential client (location redacted for anonymity) and an EC2 server in California. Each experiment lasted one minute.}
    \label{fig:dsmotivation}
    \vspace*{-3pt}
\end{figure}

\fi

\smallskip
\noindent
{\bf Elasticity detection.} We have developed an elasticity detector that uses only end-to-end observations to monitor the cross traffic. The sender continuously modulates its rate with sinusoidal pulses to create small traffic fluctuations at the bottleneck at a specific frequency (e.g., 5 Hz). It concurrently estimates the rate of the cross traffic based on the RTT and its own send and receive rates, and determines if the cross traffic oscillates at the same frequency. If it does, then the sender concludes that it is elastic; otherwise, it is inelastic. 

This technique works well because elastic and inelastic flows react differently to short-timescale traffic variations at the bottleneck. In particular, most elastic TCP flows are ACK-clocked; therefore, fluctuations in the inter-packet arrival times at the receiver, reflected in ACKs, cause similar fluctuations in subsequent packet transmissions at the sender. This causes the rate of these flows to oscillate at the same frequency as the traffic fluctuations at the bottleneck. By contrast, the rate of an inelastic flow is not sensitive to traffic variations at the bottleneck. 

%\pg{We dicuss the practical robustness of our approach in \S\ref{s:elasticity:properties}}

\smallskip
\noindent {\bf \name.}
We present the design and evaluation of \name, a congestion control system that uses our elasticity detector to switch between   TCP-competitive and delay-controlling modes. \name can support a variety of algorithms in each mode. We report results with Vegas, Copa's ``default mode'', and a simple new method that uses our cross traffic rate estimator, as \dcc algorithms. And we consider Cubic, and Reno as examples of TCP-competitive algorithms. 
\Fig{overview} shows an example result with \name. 
%\ma{Do we really show results with all these schemes?}

We have implemented the elasticity detector and Nimbus in Linux using CCP~\cite{ccp-sigcomm18}. Our experimental results show that:

\begin{CompactEnumerate}
\item On an emulated bottleneck link (96 Mbit/s, 50 ms delay, 100 ms buffering) with a WAN cross-traffic trace, \name achieves throughput comparable to BBR and Cubic but with 50 ms lower median delay. 
%\pg{Copa achieves a 5 ms smaller median delay than \name, but at the expense of much lower throughput against elastic traffic.}
\cut{\item \possname reduction in overall delays benefits the cross-traffic significantly: tail flow completion times for cross-traffic sharing the link with \name are 3--4$\times$ smaller than with BBR both for short ($<$ 15 KB) and long ($>$ 150 MB) flows, and 1.25$\times$ smaller than Cubic for short flows.}
\item For video cross traffic, on average \name achieves throughput comparable to Cubic and 37\% higher than Copa. Cubic incurs 38\% higher mean delay than \name. PCC-Vivace and BBR incur higher delay and achieve lower throughput than \name.

\item Compared to Copa, \name classifies cross traffic more accurately and is more robust. 
% inelastic cross traffic whereas Copa's accuracy is lower than 80\%. 
For instance, Copa's classifier fails when the inelastic cross traffic rate exceeds 80\%, and its accuracy of detecting elastic flows degrades from 85\% to 15\% when the RTT ratio between the cross traffic and Copa increases from 1 to 4. By contrast Nimbus's accuracy is close to 100\%, dropping less then 10\% when the RTT ratio is 4:1.

\item Our elasticity detector is robust to a variety of cross traffic conditions, achieving at least 85\% accuracy when: (i) the cross traffic is a combination of varying number of elastic flows and highly-varying inelastic short flows; (ii) the cross traffic RTT is different from \name's RTT; (iii) the cross traffic is composed of multiple elastic flows with different RTTs.
%\item \pg{Verify} By varying the modulation frequency, \name can detect and synchronize with other \name flows (\S\ref{s:multinimbus}).
These results hold across a wide range of network characteristics such as different buffer sizes, RTTs, bottleneck link rates, active queue management schemes, and shares of the bottleneck link rate controlled by \name.


\item On Internet paths, \name (switching between Cubic and a simple delay-controlling scheme) achieves throughput comparable to or better than Cubic on most of the 25 real-world paths we tested, with lower delays in 60\% of paths and similar delays in the other 40\% of paths. Compared to BBR, \name achieves 10\% lower mean throughput, but at 40-50 ms lower packet delay.
%
%% TODO: add a sentence about BBR if required
\end{CompactEnumerate}

%The results presented in this paper demonstrate the utility and effectiveness of elasticity detection as a building block to achieve both high throughput and low delays. 

%% \pg{should we add a statement about copa here in the results?}

\if 0
\begin{itemize}
    \item We define elasticity and show that detecting elasticity requires observing how cross traffic changes across time; in particular, we show that simple approaches based on measurements of delays or rates at a single point in time cannot detect elasticity accurately (\S\ref{s:elasticity}).
    
    \item We present techniques for measuring both the volume of cross traffic and estimating its elasticity using only end-to-end observations of rates and round-trip delays (\S\ref{s:switching}).
    
    \item We develop \name, a full dual-mode congestion control protocol that uses our cross traffic estimation techniques to achieve low delay with inelastic cross traffic and compete fairly with elastic cross traffic. We show how multiple \name flows can coordinate to detect the nature cross traffic and select the right operating mode (\S\ref{s:impl}).
    
    \item We implement \name using the recent Congestion Control Plane (CCP)~\cite{ccp-hotnets} platform. Our implementation uses CCP to run on a Linux kernel datapath while performing \name's signal processing operations such as FFTs in a userspace program (\S\ref{s:impl}).
    
    \item We evaluate \name experimentally in a variety of emulated network conditions as well as real-world paths. Our results show...
    
\end{itemize}
\fi




 

\if 0
Transport protocols on the Internet may be characterized as either {\em elastic} or {\em inelastic}. An elastic sender uses feedback from the receiver to increase its rate if it perceives that the rate is lower than the available bandwidth, and slows down if it perceives an increase in cross traffic (e.g., by being ``ACK clocked'', by reacting to packet losses, etc.). Examples of elastic senders include congestion control algorithms such as Cubic~\cite{cubic}, NewReno~\cite{newreno}, Compound~\cite{compound}, and BBR~\cite{bbr}. By contrast, inelastic senders do not attempt to extract all available bandwidth,  and run in open-loop fashion independent of cross traffic; examples include short TCP flows, application-limited flows (e.g., a constant bit-rate video stream), and flows that are rate-limited.

This paper proposes a method for a transport protocol sender to detect whether the {\em competing} traffic sharing its bottleneck link is elastic or not, and shows that elasticity detection is a useful building block for end-to-end congestion control. The primary motivation is to deploy  congestion control methods that control packet delays. Examples of such {\em delay-based} algorithms include Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, and Copa~\cite{copa}; unlike {\em loss-based} methods like Cubic, NewReno, and Compound, which reduce their window only in response to packet loss or explicit congestion notification (ECN) signals, delay-based algorithms reduce their rates as delays increase, to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}.

\fi

%The research community has developed two broad categories of approaches to tackle bufferbloat: active queue management (AQM) and delay-based congestion control. AQM schemes~\cite{red, pi, avq, pie, codel} provide an early indication of congestion by dropping packets before buffers fill up at routers. In recent years, AQM schemes such as CoDel~\cite{codel} and PIE~\cite{pie} have shown promise, but their widespread deployment is challenging because they require changes to routers. An alternative approach is delay-based congestion control~\cite{ledbat, vegas, fasttcp, copa} algorithms; in these algorithms, endpoints sense increases in delay and react to it to keep low delays while achieving high throughput. Recent examples of delay-based congestion control algorithms include Copa~\cite{copa} and TIMELY~\cite{timely} (for datacenters).

\if 0
Researchers have developed two categories of approaches to tackle bufferbloat: active queue management (AQM) and delay-sensitive congestion control (\dcc) algorithms. AQM approaches~\cite{red, pi, avq, pie, codel} drop or mark packets before buffers fill up at routers; by providing earlier feedback of congestion to senders, buffer-filling senders can slow down before buffers fill. Because AQM schemes require changes to routers, however, they have faced deployment hurdles. By contrast, \dcc algorithms like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, and Copa~\cite{copa} require no router changes, using end-to-end delay and rate measurements to control queuing delay. 
%\dcc schemes operate at endpoints and do not require changes to routers.
%avoid unnecessary packet drops. 
%Recent examples of \dcc algorithms include Sprout~\cite{sprout}, Verus~\cite{verus}, Copa~\cite{copa}, and TIMELY~\cite{timely} (for datacenters).
\fi

\if 0
In practice, algorithms like Compound~\cite{compound} and BBR~\cite{bbr} that have been deployed use delay measurements (instead of, or in addition to, losses and ECN), but do not control delays.  For example, Compound combines delay and loss measurements to grab bandwidth quickly, but it fills up buffers at its bottleneck and does not achieve low delay.

While \dcc algorithms suffer low throughput when cross traffic is elastic, they exhibit the desired behavior when cross traffic is inelastic: they achieve low delays while fully utilizing the bottleneck link. Therefore, if we can detect the presence of elastic TCPs, we can use a {\em TCP-competitive} algorithm (e.g., Cubic) to compete fairly with elastic flows when they appear, but switch to a \dcc algorithm when the cross traffic is inelastic. We call this approach {\em explicit mode switching}.
\fi


==> intro_new.tex <==
%\newcommand{\introsec}{Introduction}
\section{Introduction}\label{s:intro}

Achieving high throughput and low delay has been a primary motivation for congestion control research for decades. To achieve these goals, researchers have proposed many {\em delay-controlling} algorithms over the years. Unlike {\em loss-based} methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound2}, delay-controlling schemes like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, and Copa~\cite{copa} reduce their rates as delays increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}. 

% Congestion control
% algorithms can be broadly classified as {\em loss-based} or {\em
% delay-based}. Loss-based
% methods like Cubic~\cite{cubic}, NewReno~\cite{newreno}, and Compound~\cite{compound, compound2} reduce their window
% only in response to packet loss or explicit congestion notification (ECN) signals, whereas delay-based algorithms like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat},
% Sprout~\cite{sprout}, and Copa~\cite{copa} reduce their rates as delays
% increase to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-cubic-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Cubic: High delay}}
        \label{fig:overview:cubic}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-delay-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{Delay-control: Throughput drops}}
        \label{fig:overview:vegas}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/overview-nimbus-cubic-delay-sigcomm19.pdf}
        \vspace{-7mm}
        \caption{\small{\name: Lower delay with high throughput}}
        \label{fig:overview:nimbus}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small On a 48 Mbit/s link, a flow competes with one elastic long-running Cubic flow for 60 seconds (starting at $t=30$ sec.), followed by 60 seconds of inelastic traffic sending at 24 Mbit/s. We compare Cubic, a delay-controlling scheme (\S\ref{s:mode_switching}), and Nimbus, configured to switch between these two methods based on cross traffic elasticity.     Cubic has a large queuing delay throughout. The delay-controlling scheme achieves low delay when the cross traffic is inelastic but suffers significant throughput loss when it competes with Cubic. Using mode switching, Nimbus achieves the fair throughout against Cubic {\em and} lower queuing delays when the cross traffic is inelastic.}
    \label{fig:overview}
    \vspace{-6mm}
\end{figure*}

There is, however, a major obstacle to deploying delay-controlling
algorithms on the Internet: their throughput is dismal when competing
against loss-based senders at a shared bottleneck. The reason
is that loss-based senders increase their rates until they observe
losses, which causes queuing delays to increase; in response to
increasing delays, a competing delay-controlling flow will reduce its rate. The loss-based flow then grabs this
freed-up bandwidth. The throughput of the delay-controlling flow
plummets, but delays don't reduce. Because most traffic on the Internet today uses loss-based algorithms, it is hard
to justify deploying a delay-controlling scheme.

Can we achieve the benefits of \dcc algorithms while ensuring that throughput does not degrade in the presence of schemes like Cubic or NewReno? This question has received some attention recently, with Copa~\cite{copa} proposing an algorithm with two modes---a ``default'' mode that controls delay but which competes poorly against schemes like Cubic, and a ``TCP-competitive'' mode that has no delay control but competes more aggressively. Copa uses round-trip time (RTT) observations to determine if the RTT time-series is consistent with only other Copa flows sharing the bottleneck (e.g., Copa periodically empties network queues); if so, the sender uses the delay-controlling mode, but if not, the sender switches to a TCP-competitive mode. 

In this paper, we introduce a new, more robust approach to set the best operating mode. Our method is based on a simple observation: it is safe and desirable to use a \dcc algorithm whenever the cross traffic is {\em inelastic}. An inelastic flow (or sender) is one that does not change its rate based on available bandwidth or the rate of other competing traffic. Examples include constant bit-rate (CBR) flows,  short TCP connections, application-limited flows, and flows that are bottlenecked at a different link. When cross traffic consists of only inelastic flows,  a delay-controlling scheme can maintain low queueing delay without worrying about losing throughput to competing flows. It can also achieve similar throughput as a loss-based scheme provided it maintains a high utilization of the bottleneck link. In fact, using more aggressive schemes against inelastic flows provides little throughput benefit and merely increases delay, since inelastic flows do not reduce their rate in response to competing traffic. 


On the other hand, delay-controlling algorithms are susceptible to poor throughput in the presence of {\em elastic} flows. Elastic flows increase their rate as bandwidth opens up, and slow down when they perceive an increase in cross traffic. Examples include backlogged flows using both loss-based schemes like Cubic and NewReno, and delay-based schemes like Vegas, Copa, and BBR~\cite{bbr}. Delay-controlling algorithms suffer throughput loss not only against loss-based schemes, but even against delay-based elastic flows, they may be unable to achieve a fair share of the throughput. 
%As explained previously, the throughput of a delay-controlling algorithm suffers in the presence of loss-based schemes, but even in the presence of delay-based elastic flows, a delay-controlling algorithm may be unable to obtain its fair share of throughput.
For example, a scheme like Vegas would compete fairly against other Vegas flows, but it may get less than its fair share of throughput against Copa. 

We therefore seek to detect the absence of elastic flows in the cross traffic, as a \emph{sufficient (but not necessary)} condition for operating in a delay-controlling mode without loss of throughput. Our goal is to ensure throughput on par with a baseline TCP-competitive scheme like Cubic, while exploiting opportunities with no elastic cross traffic to switch to a delay-controlling scheme. We leave the problem of how to use a delay-controlling mode in the presence of delay-based elastic cross traffic to future work. This requires methods beyond elasticity detection, such as detecting the type of congestion control algorithm used by cross traffic.   

\if 0
\pg{In this paper, we ask the question, when is it absolutely safe to run a \dcc algorithm? We characterize cross traffic scenarios where running a \dcc algorithm might achieve lower throughput compared to a loss-based scheme. In case the cross traffic contains flows that adjust their rates based on the available bandwidth (i.e. the rate of the competing flows), then, throughput of the \dcc algorithm is dependent on the congestion control algorithms used by the cross traffic; and it might not be safe to run a \dcc algorithm. We call such flows that adjust their rates based on the rate of the cross-traffic as elastic flows. Examples of elastic flows include long-running Cubic, NewReno, Copa, Vegas and BBR~\cite{bbr} flows. Note that running a \dcc algorithm like Vegas against other \dcc algorithms like Copa might result in unfairness. In contrast running Vegas in presence of other Vegas flows is safe. Therefore, to be sure that running a \dcc algorithm is safe against other \dcc algorithms, we need to detect the CC protocol of the cross traffic. Detecting the cross traffic's CC remains an open problem. In this work we present the absence of elastic flows as a sufficient but not necessary condition for running a \dcc algorithm safely. }

\pg{By contrast, inelastic senders do not attempt to grab all unused bandwidth, and their rates do not vary with bandwidth availability. Examples include short TCP flows (flows that transmit all data without receiving ACKs or adjust the rate) or, application-limited flows (e.g., video streaming flows rate limited by the quality of the video), constant bit-rate streams, and flows that are bottlenecked at a different link. When the cross traffic is inelastic, delay-controlling schemes can achieve \pg{similar throughput as their loss-based counterparts} while maintaining low delay. Using aggressive \pg{loss-based} algorithms provides little benefit against in \pg{absence of elastic flows}, since they don't reduce their rate in response to cross traffic.}

 \pg{The goal our our work is to allow a sender to achieve similar throughput as a given ``TCP-Competetive'' congestion control protocol (e.g., Cubic) while reducing delays when possible. To achieve this, we introduce a new, robust approach to determine whether the cross traffic any elastic flows. In case the cross-traffic contains elastic flows, running a \dcc algorithm might be unsafe. In such a scenario, the sender should use the given TCP-competitive algorithm. Otherwise the sender can use a \dcc algorithm to reduce delays without worrying about losing throughput.}

\fi 

\cut{Our method explicitly characterizes whether the competing cross traffic contains any \emph{elastic} flows. An elastic flow is one that fills up all available bandwidth; it increases its rate if it perceives unused bandwidth, and it slows down if the available bandwidth drops. Examples of elastic flows include long-running Cubic, NewReno, Copa, Vegas and BBR~\cite{bbr} flows. When the cross traffic is elastic, delay-controlling algorithms are susceptible to poor throughput. To be safe, it is important to detect this situation and switch to a mode that mimics the behavior of the prevailing cross traffic.\footnote{Even if the cross traffic uses a delay-controlling protocol like Vegas, it might not be fair to other delay-controlling schemes (e.g., Copa). Hence, against elastic (i.e., long-running) delay-controlling flows we advocate mimicking widely-deployed TCP protocols like Cubic.}}

\cut{By contrast, inelastic senders do not attempt to grab all unused bandwidth, and their rates do not vary with bandwidth availability. Examples include short TCP flows, application-limited flows, constant bit-rate streams, and flows that are bottlenecked at a different link. When the cross traffic is inelastic, delay-controlling schemes can achieve high throughput while maintaining low delay. Using aggressive TCP-competitive methods  provides little benefit against inelastic flows, since they don't reduce their rate in response to cross traffic. }

\smallskip
\noindent
{\bf Elasticity detection.} We have developed an elasticity detector that uses only end-to-end observations to monitor the cross traffic. The sender continuously modulates its rate with sinusoidal pulses to create small traffic fluctuations at the bottleneck at a specific frequency (e.g., 5 Hz). It concurrently estimates the rate of the cross traffic based on the RTT and its own send and receive rates, and monitors its frequency response (FFT) to determine if the cross traffic's rate oscillates at the same frequency. If it does, then the sender concludes that the cross traffic contains elastic flows; otherwise, it is inelastic. 

This technique relies on two assumptions. First, the sender must be able to create sufficient pulses %(e.g., burst at 20\% of the bottleneck capacity)
and observe the impact on cross traffic over a period of time. Hence our technique is best suited to senders that control large data transfers, such as large file downloads, data backups to the cloud, video, etc. Fortunately, it is precisely for such transfers that delay-controlling schemes can provide the most benefit, since short flows are unlikely to cause significant queueing delay~\cite{bufferbloat}. 

Second, pulsing is most effective when the elastic flows in the cross traffic are sensitive to traffic fluctuations at the bottleneck on a short timescale, for example, a few RTTs. If an elastic flow is slow to react to bandwidth changes, it can go undetected with small traffic pulses. While it is possible in theory to use large pulses to detect such ``sluggish'' elastic flows, this could cause congestion. Most congestion-controlled elastic flows react to bandwidth variations on RTT timescales. In particular, the majority of TCP traffic on the Internet is ACK-clocked. For these flows, RTT-timescale changes in the receive rate get reflected in similar changes to the send rate via ACKs, thereby causing the senders to oscillate at the same frequency as the traffic fluctuations at the bottleneck. Our elasticity detector is targeted at detecting ACK-clocked flows, but we have also found that it classifies fast-reacting rate-based flows as elastic.

%\ma{I don't know if we should say the last sentence. i think the only example of a rate-based scheme that we can detect as elastic is the nimbus delay algorithm. The point I am trying to make is that the fundamental requirement is not ACK clocking but fast reaction to changes in cross traffic, which is a desirable property for congestion control.}

%This technique works well because elastic and inelastic flows react differently to short-timescale traffic variations at the bottleneck. In particular, \pg{we make use of the observation} that most elastic TCP flows are ACK-clocked; therefore, fluctuations in the inter-packet arrival times at the receiver, reflected in ACKs, cause similar fluctuations in subsequent packet transmissions at the sender. This causes the rate of these flows to oscillate at the same frequency as the traffic fluctuations at the bottleneck. By contrast, the rate of an inelastic flow is not sensitive to traffic variations at the bottleneck. 


 Elasticity detection is a \emph{building block} for other congestion control schemes, rather than a standalone protocol. As such, while we evaluate it in the context of a single connection, we envision additional uses, such as: 
(1) a safeguard sub-system for delay-controlling aggregate traffic management. 
%For example, recent work~\cite{bundler} describes a use of elasticity detection in an edge-based traffic scheduling system for bundles of traffic consisting of many flows between two sites.
(2) a measurement tool to detect the nature of cross traffic. For example, running an elasticity detector could lend insight into a network's traffic behavior and guide the deployment of AQM schemes.



%\pg{We dicuss the practical robustness of our approach in \S\ref{s:elasticity:properties}}

%\smallskip
\noindent {\bf \name.}
We present the design and evaluation of \name, a congestion control system that uses our elasticity detector to switch between   TCP-competitive and delay-controlling modes. \name can support a variety of algorithms in each mode. We report results with Vegas, Copa's ``default mode'', and a simple new method that uses our cross traffic rate estimator, as examples of \dcc algorithms, and Cubic and Reno as examples of TCP-competitive algorithms. 
\Fig{overview} shows an example result with \name. 
%\ma{Do we really show results with all these schemes?}



We have implemented the elasticity detector and Nimbus in Linux using CCP~\cite{ccp-sigcomm18}. Our experimental results show that:

\begin{CompactEnumerate}
\item On an emulated bottleneck link (96 Mbit/s, 50 ms delay, 100 ms buffering) with a WAN cross-traffic trace, \name achieves throughput comparable to  Cubic and BBR but with 50 ms lower median delay. 
%\pg{Copa achieves a 5 ms smaller median delay than \name, but at the expense of much lower throughput against elastic traffic.}
\cut{\item \possname reduction in overall delays benefits the cross-traffic significantly: tail flow completion times for cross-traffic sharing the link with \name are 3--4$\times$ smaller than with BBR both for short ($<$ 15 KB) and long ($>$ 150 MB) flows, and 1.25$\times$ smaller than Cubic for short flows.}
\item For video cross traffic, on average \name achieves throughput comparable to Cubic and 37\% higher than Copa. Cubic incurs 38\% higher mean delay than \name. PCC-Vivace and BBR incur higher delay and achieve lower throughput than \name.

\item Compared to Copa, \name classifies cross traffic more accurately and is more robust. 
% inelastic cross traffic whereas Copa's accuracy is lower than 80\%. 
For instance, Copa's classifier fails when the inelastic cross traffic rate exceeds 80\%, and its accuracy of detecting elastic flows degrades from 85\% to 15\% when the RTT ratio between the cross traffic and Copa increases from 1 to 4. By contrast Nimbus's accuracy is close to 100\%, dropping less then 10\% when the RTT ratio is 4:1.

\item Our elasticity detector is robust to a variety of cross traffic conditions, achieving at least 85\% accuracy when: (i) the cross traffic is a combination of varying number of elastic flows and highly-varying inelastic short flows; (ii) the cross traffic RTT is different from \name's RTT; (iii) the cross traffic is composed of multiple elastic flows with different RTTs.
%\item \pg{Verify} By varying the modulation frequency, \name can detect and synchronize with other \name flows (\S\ref{s:multinimbus}).
These results hold across a wide range of network characteristics: \cut{such as different} buffer sizes, RTTs, bottleneck link rates, active queue management schemes, and shares of the bottleneck link rate controlled by \name.

\item On real Internet paths, \name (switching between Cubic and a simple delay-controlling scheme) achieves throughput comparable to or better than Cubic on most of the 25 real-world paths we tested, with lower delays in 60\% of paths and similar delays in the other 40\% of paths. Compared to BBR, \name achieves 10\% lower mean throughput, but at 40-50 ms lower packet delay.
%
%% TODO: add a sentence about BBR if required
\end{CompactEnumerate}







\cut{\pg{\textbf{Limitations:} Table ~\ref{tab:elasticity} summarizes elasticity classification by our detector for a variety of traffic classes. The elasticity detector classifies all ACK-clocked schemes (prevalent traffic) s as elastic. BBR is classified as elastic when it's window limited (on big buffers). Our evaluation shows that \name achieves similar throughput as Cubic while competing against BBR.} \ma{I think you can just move the table to the limitations sections. The new intro is explicit about our assumption of ACK clocking, so I don't think we need this early anymore.}}












%The results presented in this paper demonstrate the utility and effectiveness of elasticity detection as a building block to achieve both high throughput and low delays. 

%% \pg{should we add a statement about copa here in the results?}

\if 0
\begin{itemize}
    \item We define elasticity and show that detecting elasticity requires observing how cross traffic changes across time; in particular, we show that simple approaches based on measurements of delays or rates at a single point in time cannot detect elasticity accurately (\S\ref{s:elasticity}).
    
    \item We present techniques for measuring both the volume of cross traffic and estimating its elasticity using only end-to-end observations of rates and round-trip delays (\S\ref{s:switching}).
    
    \item We develop \name, a full dual-mode congestion control protocol that uses our cross traffic estimation techniques to achieve low delay with inelastic cross traffic and compete fairly with elastic cross traffic. We show how multiple \name flows can coordinate to detect the nature cross traffic and select the right operating mode (\S\ref{s:impl}).
    
    \item We implement \name using the recent Congestion Control Plane (CCP)~\cite{ccp-hotnets} platform. Our implementation uses CCP to run on a Linux kernel datapath while performing \name's signal processing operations such as FFTs in a userspace program (\S\ref{s:impl}).
    
    \item We evaluate \name experimentally in a variety of emulated network conditions as well as real-world paths. Our results show...
    
\end{itemize}
\fi




 

\if 0
Transport protocols on the Internet may be characterized as either {\em elastic} or {\em inelastic}. An elastic sender uses feedback from the receiver to increase its rate if it perceives that the rate is lower than the available bandwidth, and slows down if it perceives an increase in cross traffic (e.g., by being ``ACK clocked'', by reacting to packet losses, etc.). Examples of elastic senders include congestion control algorithms such as Cubic~\cite{cubic}, NewReno~\cite{newreno}, Compound~\cite{compound}, and BBR~\cite{bbr}. By contrast, inelastic senders do not attempt to extract all available bandwidth,  and run in open-loop fashion independent of cross traffic; examples include short TCP flows, application-limited flows (e.g., a constant bit-rate video stream), and flows that are rate-limited.

This paper proposes a method for a transport protocol sender to detect whether the {\em competing} traffic sharing its bottleneck link is elastic or not, and shows that elasticity detection is a useful building block for end-to-end congestion control. The primary motivation is to deploy  congestion control methods that control packet delays. Examples of such {\em delay-based} algorithms include Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, and Copa~\cite{copa}; unlike {\em loss-based} methods like Cubic, NewReno, and Compound, which reduce their window only in response to packet loss or explicit congestion notification (ECN) signals, delay-based algorithms reduce their rates as delays increase, to control packet delays and avoid ``bufferbloat''~\cite{bufferbloat}.

\fi

%The research community has developed two broad categories of approaches to tackle bufferbloat: active queue management (AQM) and delay-based congestion control. AQM schemes~\cite{red, pi, avq, pie, codel} provide an early indication of congestion by dropping packets before buffers fill up at routers. In recent years, AQM schemes such as CoDel~\cite{codel} and PIE~\cite{pie} have shown promise, but their widespread deployment is challenging because they require changes to routers. An alternative approach is delay-based congestion control~\cite{ledbat, vegas, fasttcp, copa} algorithms; in these algorithms, endpoints sense increases in delay and react to it to keep low delays while achieving high throughput. Recent examples of delay-based congestion control algorithms include Copa~\cite{copa} and TIMELY~\cite{timely} (for datacenters).

\if 0
Researchers have developed two categories of approaches to tackle bufferbloat: active queue management (AQM) and delay-sensitive congestion control (\dcc) algorithms. AQM approaches~\cite{red, pi, avq, pie, codel} drop or mark packets before buffers fill up at routers; by providing earlier feedback of congestion to senders, buffer-filling senders can slow down before buffers fill. Because AQM schemes require changes to routers, however, they have faced deployment hurdles. By contrast, \dcc algorithms like Vegas~\cite{vegas}, FAST~\cite{fasttcp}, LEDBAT~\cite{ledbat}, Sprout~\cite{sprout}, and Copa~\cite{copa} require no router changes, using end-to-end delay and rate measurements to control queuing delay. 
%\dcc schemes operate at endpoints and do not require changes to routers.
%avoid unnecessary packet drops. 
%Recent examples of \dcc algorithms include Sprout~\cite{sprout}, Verus~\cite{verus}, Copa~\cite{copa}, and TIMELY~\cite{timely} (for datacenters).
\fi

\if 0
In practice, algorithms like Compound~\cite{compound} and BBR~\cite{bbr} that have been deployed use delay measurements (instead of, or in addition to, losses and ECN), but do not control delays.  For example, Compound combines delay and loss measurements to grab bandwidth quickly, but it fills up buffers at its bottleneck and does not achieve low delay.

While \dcc algorithms suffer low throughput when cross traffic is elastic, they exhibit the desired behavior when cross traffic is inelastic: they achieve low delays while fully utilizing the bottleneck link. Therefore, if we can detect the presence of elastic TCPs, we can use a {\em TCP-competitive} algorithm (e.g., Cubic) to compete fairly with elastic flows when they appear, but switch to a \dcc algorithm when the cross traffic is inelastic. We call this approach {\em explicit mode switching}.
\fi


==> limitations.tex <==
\newcommand{\limitsec}{Limitations}
\section{\limitsec}
\label{s:limit}
\begin{table}
\small
\begin{center}
\begin{tabular}{cccc}
 Cross Traffic & Elastic & ACK-Clocked & Classification\\ 
 \hline
 \hline
 Cubic & Yes & Yes & Elastic \\
  \hline
 Reno & Yes & Yes & Elastic \\
  \hline
 Copa & Yes & Yes & Elastic \\
  \hline
 Vegas & Yes & Yes & Elastic \\
  \hline
 BBR & Yes & If CWND-limited & Elastic*\\
  \hline
 %BasicDelay & Yes & No & Elastic\\
 %  \hline
 PCC-Vivace & Yes & No & Inelastic* \\
  \hline
 Fixed window & Yes & Yes & Elastic \\
  \hline
 App. limited & No & No & Inelastic \\
  \hline
 Const. stream & No & No & Inelastic \\
\end{tabular}
\end{center}
\caption{\small{\bf Classification by the elasticity detector}}
\label{tab:elasticity}
\vspace{-11mm}
\end{table}



Table ~\ref{tab:elasticity} summarizes elasticity classification by our detector for a variety of traffic classes. 
Our method relies on the cross traffic responding to variations induced by pulses on an RTT timescale. 
This is true of all ACK-clocked protocols. 
For example, the detector does not always classify BBR cross traffic as elastic. When the buffer is large, BBR becomes ACK-clocked and is elastic. 
However, when the buffer is small, BBR responds on time-scales longer than an RTT; here, \name classifies it as inelastic and uses its delay-control mode. Nonetheless, we find that Nimbus (with Cubic as the TCP-competitive protocol) achieves similar throughput to Cubic when competing against BBR (which is known to be unfair), regardless of buffer size (Appendix $\S$\ref{app:bbr-comparison}). 
%For small buffers, BBR is known to be unfair; thus, both Cubic and \name achieve less throughput than BBR, which occupies 90\% of the link. With larger buffers, \name's throughput is similar to that of BBR. 

Rate-based protocols (\eg PCC-Vivace) may not react on RTT timescales.
For example, the detector classifies PCC-Vivace as inelastic because it does not react quickly enough to the elasticity detector's pulses.  
For such flows, on increasing the pulse duration, the elasticity detector correctly classifies them as elastic (see Appendix~\ref{app:slow-react}). 
Increasing the pulse duration might of course also increase queuing delays. Since most elastic traffic today is ACK-clocked, we use a small pulse duration by default. In the future, if rate-based  protocols become widely deployed, the pulse duration could be adjusted accordingly. 

%elasticity detector could be configured accordingly by  adjusting the pulse duration accordingly.

%\ma{this is good. keep it here and include the table. consider adding a row for BasicDelay, as an example of a rate-based scheme that can be detected as elastic, since it reacts to bandwidth changes quickly}
%The detector does not reliably characterize BBR as elastic because BBR responds on time scales longer than an RTT; here, Nimbus uses delay-based control more often than desired with BBR cross traffic. However, we find that Nimbus achieves similar throughput to Cubic in practice: with more than 1 BDP of router buffering, BBR becomes window-limited and is detected as elastic, but with shallow buffers, BBR obtains a disproportionate share of the link compared to both Cubic and Nimbus (Appendix $\S$\ref{app:bbr-comparison}).

The detector also assumes that the flow has a single bottleneck. Multiple bottlenecks can add noise to \name's rate measurements, preventing accurate cross-traffic estimation. The challenge is that the spacing of packets at one bottleneck is not preserved when traversing the second bottleneck.
%Fortunately, the single-bottleneck case is common, e.g., the bottleneck in home networks is often at the last hop. 
%Our method will also not work well for RTTs over 300 ms because the background traffic itself may starts to vary significantly over that time-scale. 

While the elasticity detector can detect presence of elastic flows, it cannot detect the specific congestion protocol used by competing flows. If the TCP-competitive protocol \name uses is different from that of the cross traffic, there could be unfairness. 
Conversely, if elastic cross traffic is using a \dcc scheme like Vegas, then running a buffer-filling TCP-competitive algorithm can cause unfairness and grow delays unnecessarily. Detecting the congestion control protocols used by competing elastic flows remains an open question.

%While the elasticity detector can detect presence of elastic flows, it cannot detect the congestion protocol used by competing flows. If the TCP-competitive protocol used by \name is different from that of the cross traffic, there could be  unfairness. Moreover, if the elastic cross traffic is using a \dcc scheme like Vegas, then running a buffer-filling TCP-competitive algorithm can cause delays to grow when high throughput could have been achieved with lower delays. Detecting the congestion control protocols used by competing elastic flows remains an open question.
%\footnote{Cross traffic can consist of multiple elastic flows using different congestion control protocol making this problem even more challenging.}

%The detector correctly characterizes \dcc schemes like Vegas as elastic, but in response runs TCP competitive algorithm (e.g., Cubic), which cause delays to grow when high throughput could have been achieved with lower delays. Determining if elastic cross traffic is also delay-controlled and \pg{using an appropriate delay control for \name, compatible with cross traffic's delay-control protocol are open questions}. 

%\noindent {\bf Detecting rate-based elastic flows.}

\if 0 
Our method detects only ACK-clocked flows as elastic, not rate-based ones.\pg{We need to change this a bit based on HB's intro. Please note that I have added an experiment with BBR in the appendix.} Almost all traffic today uses ACK-clocking, but a notable exception is BBR~\cite{bbr}, which uses both a rate and a congestion window. \name detects BBR only when they are window-limited.  
\fi

%\smallskip
%\noindent
%{\bf Multiple bottlenecks.}



%Making nimbus compete fairly with other delay-based protocols is an open problem (including competition with other nimbus flows). 

%% \begin{figure*}
%%     \centering
%%         \begin{subfigure}[t]{0.3\textwidth}
%% 			\centering
%% 			\includegraphics[width=\textwidth]{images/t-comparePulses-50}
%% 			\subcaption{50ms}
%% 			\label{fig:limits:50}
%% 		\end{subfigure}
%%         \begin{subfigure}[t]{0.3\textwidth}
%% 			\centering
%% 			\includegraphics[width=\textwidth]{images/t-comparePulses-100}
%% 			\subcaption{100ms}
%% 			\label{fig:limits:100}
%% 		\end{subfigure}
%%         \begin{subfigure}[t]{0.3\textwidth}
%% 			\centering
%% 			\includegraphics[width=\textwidth]{images/t-comparePulses-200}
%% 			\subcaption{200ms}
%%             \label{fig:limits:200}
%% 		\end{subfigure}
%%     \caption{
%%         Elasticity over a five-second window for varying pulse sizes and RTTs against a single TCP flow. At 200ms, \name's rate is too low to make elasticity measurements.
%%     }
%%     \label{fig:limits}
%% \end{figure*}

%% \name has two significant limitations. 
%% First, while the elasticity metric can reliably detect elastic traffic when the sending rate is high, it is unable to make large enough perturbations in the queue size to affect cross traffic when the rate is low. 
%% Furthermore, the convergence of the elasticity metric to a safe threshold depends on the RTT. 
%% Therefore, if \name is in delay-control mode and elastic traffic joins the queue, it will lose rate until it switches to TCP-Competitive mode. 

%% In practice, as Figure~\ref{fig:limits} shows, this means that in high-RTT networks, \name will not react to elastic traffic. In this experiment, we ran the \name against a single TCP NewReno flow on a 24Mbps link and varied the link RTT from $50$ms to $200$ms and varied the size of the pulses we sent to try to measure elasticity. 
%% In Figure~\ref{fig:limits:50}, the elasticity increases rapidly after the competing TCP flow begins, but when the RTT increases as in
%% Figure~\ref{fig:limits:200}, the flow rate becomes low, and even large pulses (80\% of the flow rate) cannot measure elasticity.

%% To mitigate this effect, it is possible to use \emph{additive} rather than multiplicative pulses, so that the pulse size is not scaled to the flow rate. 
%% This allows \name to measure elasticity, but causes changes in the queue disproportionate with the flow rate. 
%% Resolving this issue is an avenue for future work.

==> motivation.tex <==
\newcommand{\motivationsec}{Motivation}
\section{\motivationsec}
\label{s:motivation}

%\subsection{The Case for Aggregate Traffic Control (ATC)}

\textbf{Ideal goal:} The ideal goal for a congestion control protocol is to achieve its fair share of throughput while minimizing delays. \cut{One way of achieving ideal fairness is via deploying fair queuing at the bottleneck router. Fair queuing provides isolation for flows, i.e., a flow can achieve both its fair share rate and low queuing delays even if the competing flows are filling up the buffer (e.g., long running Cubic flows).} Achieving these goals is extremely challenging. Fair share of throughput for a flow depends on the congestion control protocol used by competing \textit{elastic} flows. Determining congestion control protocol used by competing flows in an end to end manner is hard. Moreover, this task is complicated by the fact that cross traffic might contain multiple flows, each using a different congestion control protocol. Further, achieving low delays is only possible if the cross traffic does not contain any buffer filling elastic flows.

To get around the problem of fairness, senders typically use a TCP-competitive buffer filling protocol (e.g., Cubic or BBR). The problem with such an approach is that even when the cross traffic does not contain any elastic flows, such scheme might still build up buffers. This extra buffer build up does not provide any additional throughput to the flow.

\noindent\textbf{\name's goal:} The goal of \name is to allow a flow to achieve similar throughput as a TCP-competitive buffer filling scheme, while minimizing delays when possible. \name uses the elasticity detector to determine if the cross traffic contains any elastic flows, if it does, then \name mimics the behaviour of a buffer filling scheme. Note that even if the competing elastic flows are running delay-controlling algorithms, running in \dcc mode might lead to a \name flow achieving lesser throughput than the TCP-competitive algorithm. Therefore, to achieve similar throughput as a TCP-competitive algorithm, in presence of any competing elastic flows, \name runs in the TCP-competitive mode. If the cross traffic does not contain any elastic flows, then \name runs in the \dcc mode to reduce delays without worrying about losing throughput. This reduction in delays benefits both \name and cross traffic flows.

\noindent\textbf{Understanding nuances of elasticity:} Formally, we define an elastic flow as one that adjusts its rate on perceived available bandwidth. An elastic flow increase it's rate if it senses unused available bandwidth, and slows down if the available bandwidth drops. If a flows throughput is limited by the congestion control protocol its using, then the flow is classified as elastic. Examples include congestion control limited (CCL) Cubic, BBR, Copa, Vegas, PCC-Vivace, etc. A flow sending at a fixed window (e.g., receiver limited window) is also considered an elastic flow. The throughput of such flow depends on the RTT, hence it depends on available bandwidth.

If a flow is application limited, i.e. the application is producing data at a rate lesser than the rate dictated by the congestion control protocol, then the flow doesn't change its rate based on perceived bandwidth and the flow is classified as inelastic. Examples of application limited flows include short-TCP flows (flows that transmit all data before receiving an ACK), video streaming flows that are buffering at the highest quality and are not limited by congestion control. Other examples of inelastic flows include constant-bit streams or flows that are bottlenecked at a different link (throughput of such flow is not governed by the available bandwidth on the bottleneck link for the \name flow). Table ~\ref{tab:elasticity} shows different categories of flows and whether they are elastic or not.

\begin{table}
\begin{center}
\begin{tabular}{ |c| c| c| }
\hline
 Traffic Class & Elastic & Classified as Elastic\\ 
 \hline
 CCL Cubic & \ding{51} & \ding{51} \\
  \hline
   CCL Reno & \ding{51} & \ding{51} \\
  \hline
   CCL Copa & \ding{51} & \ding{51} \\
  \hline
  CCL Vegas & \ding{51} & \ding{51} \\
  \hline
  CCL BBR & \ding{51} & \ding{51}*\\
  \hline
  CCL PCC-Vivace & \ding{51} & \ding{55} \\
  \hline
  Fixed window & \ding{51} & \ding{51} \\
  \hline
  Application limited & \ding{55} & \ding{55} \\
  \hline
   Constant bit stream & \ding{55} & \ding{55} \\
  \hline
\end{tabular}
\end{center}
\caption{\small{\bf Classification of traffic classes by the elasticity detector}}
\label{tab:elasticity}
\end{table}


\noindent\textbf{Elasticity detection:} A strawman approach for detecting elastic flows is for a \name flow to run in both TCP-competitive and \dcc mode for some interval and observe the throughput of the cross traffic in each mode. If the throughput of cross traffic is more in the \dcc mode, then the cross traffic contains elastic flows. The problem with such an approach is that a \name flow might loose significant throughput in the \dcc mode in the presence of elastic flows. Alternatively, against inelastic cross traffic running in the TCP-competitive mode can increase delays unnecessarily.

Our technique for the elasticity detector doesn't need to switch modes to detect elastic flows, instead it follows directly from our definition of elasticity. To detect presence of elastic flows (flows that adjust their rates on available capacity), the elasticity detector creates small fluctuations in its sending rate to create variations is the perceived available bandwidth. If the cross traffic contains any elastic flows, then the throughput of the elastic portion of the cross traffic (hence the throughput of cross traffic) will respond to such variations, and the elasticity detector will classify cross traffic as elastic (i.e., it contains elastic flows). For robustness, the elasticity detector creates multiple such variations (by pulsing its rate at a frequency) in an interval, each such variation is on an RTT timescale. The elasticity detector looks at the response of cross traffic's rate in this interval. 

\noindent\textbf{Limitations of elasticity detection:} Our elasticity detection method relies on the cross traffic responding to variations induced by pulses on an RTT timescale. This property is satisfied by all ACK-clocked protocols, but not for some rate-based protocols. For example, the detector does not always classify BBR cross traffic as elastic. When the buffer is large BBR becomes ACK-clocked and is classified as elastic. However, when the buffer is small, BBR responds on time-scales longer than an RTT; here, \name classifies it as inelastic and uses its delay-control mode. Nonetheless, we find that Nimbus (with Cubic as the TCP-competitive protocol) still achieves its goal of similar throughput to Cubic when competing against BBR, regardless of buffer size (Appendix $\S$\ref{app:bbr-comparison}). For small buffers, both \name and Cubic achieve much less throughput than BBR, since BBR is very  aggressive in these situations, occupying 90\% of the link. With large buffers, \name's throughput is similar to that of BBR. The detector also classifies PCC-Vivace as inelastic because it is rate-based. In this case, \name uses a \dcc algorithm compromising fairness but maintaining low delays. Table \ref{tab:elasticity} summarizes elasticity classification by our detector for a variety of traffic classes.


\noindent\textbf{Use cases:} \pg{do we need this?}

% \smallskip
% \noindent{\bf Opportunities for ATC.}


% Benefits of ATC.

% Implications of ATC: persistent traffic. In congestion control, traffic is power.

% \subsection{Challenges}

% Three desirable properties:
% 1. High throughput
% 2. Low delay
% 3. Firm but fair competition with other traffic

% In many ways, these are perennial challenges for congestion control on the Internet. Brief paragraph on the history of loss and delay-based congestion control.

% ATC presents an opportunity to rethink how to tackle these goals. 

% \subsection{Nimbus's Key Insights}




==> multiple_nimbus.tex <==
\newcommand{\multinimbussec}{Multiple Nimbus Flows}
\section{\multinimbussec}
\label{s:multinimbus}

%\an{why is this after the big experiment? Should change title to ``independent elasticity detectors and move to eariler (after cross traffic estimation section)}

What happens when a bottleneck is shared by multiple \name flows? Ideally, we want all the \name flows to remain in delay-control mode when there is no elastic cross traffic, and compete well with elastic cross traffic otherwise. 

%However, pulses may create adverse interactions that confuse the different \name instances. 

%We consider three approaches: (1) all \name{} flows pulse at the same frequency, (2) \name{} flows use different pulsing frequencies for pulsing, (3) only 1 \name flow pulses and the remaining flows watch the response of cross traffic to the pulses.

One approach is for the \name flows to all pulse at the same frequency. However, in this case, they will all detect a peak in the FFT at the oscillation frequency. They will all then stay in TCP-competitive mode and won't be able to maintain low delays, even when there is no elastic cross traffic. A second approach is for different \name flows to pulse at different frequencies. But this approach cannot scale to more than a few flows, because the set of distinguishable frequencies is limited (recall that the pulse period $T$ cannot be too small). 

%\smallskip
\noindent{\bf The pulser and the watchers.}
We propose a third approach. One of the \name{} flows assumes the role of the {\em pulser}, while the others are {\em watchers}. The coordination between them involves no explicit communication; in fact, each \name flow is unaware of the identities, or even existence, of the others.

The \pulser sends data by modulating its rate with asymmetric sinusoids. The \pulser uses two different frequencies, $f_{pc}$ in TCP-competitive mode, and $f_{pd}$ in delay-control mode. The values of these frequencies are fixed and agreed upon beforehand; we use $f_{pc}=5$ Hz and $f_{pd}=6$ Hz in our experiments.\footnote{These values are in accordance with bounds on $T$ and $f$ described in \S\ref{s:nimbus-protocol}} 

A \watcher infers whether the \pulser is pulsing at frequency $f_{pc}$ or frequency $f_{pd}$ by computing the FFT of its receive rate, $R$, at these two frequencies. It then picks the mode corresponding to the larger peak to match the pulser's mode. Note that since a watcher is not pulsing, it can detect the pulser's pulses in its own receive rate, $R$; i.e., it does not even need to estimate $z$. The pulser, on the other hand, cannot look at its own $R$ to detect pulses in the cross traffic, since it will end up detecting its own pulses.  


%The variation in the queuing due to pulsing will cause a \watcher flow's receive rate to pulse at the same frequency. 


%; it need not even be a persistent flow.

For multiple \name{} flows to maintain low delays during times when there is no elastic cross traffic on the link, the \pulser must classify \watcher traffic as inelastic. Note that from the \pulser's perspective, the \watchers flows are part of the cross traffic; thus, to avoid confusing the \pulser, the rate of \watchers must not react to the pulses of the \pulser. To achieve this goal, a watcher applies an exponentially weighted moving average (EWMA) filter to its transmission rate before sending data. The EWMA filter cuts off all frequencies in the sending rate that exceed $\min(f_{pc},f_{pd})$.

\smallskip
\noindent
{\bf Pulser election.}
A decentralized and randomized election process decides which flow is the \pulser and which are \watchers. If a \name flow determines that there is no \pulser (by seeing that there is no peak in the FFT at the two potential pulsing frequencies), then it decides to become a pulser with a probability proportional to its transmission rate:
%\vspace{-3mm}
\begin{equation}
   p_{i} = \frac{\kappa\tau}{\textnormal{FFT Duration}} \times \frac{R_{i}}{\mu}.
   \label{eq:pi}
 %  \vspace{-3mm}
\end{equation}
Each flow makes decisions periodically, \eg every $\tau = 10$ ms, $\kappa$ is a constant, and $R_i$ is the receive rate of the $i^{th}$ flow. This rule ensures that the expected number of flows that become pulsers over the FFT duration is at most $\kappa$. To see why, note that the expected number of pulsers is equal to the sum of the probabilities in Eq.~\eqref{eq:pi} over all the decisions made by all flows in the FFT duration. Since $\sum_i R_i \leq \mu$ and each flow makes ($\textnormal{FFT Duration} / \tau$) decisions, these probabilities sum up to at most $\kappa$.

%Since the FFT duration is 5 seconds, each $p_i$ is small (note that $\sum_i R_i \leq \mu$), but since flows make decisions every $\tau$ seconds, eventually one will become a pulser. 

%We show that the probability that more than one flow becomes a pulser within one FFT duration is small; thus, after one flow becomes a pulser, the probability that a second flow will also decide to become a pulser before it can detect the pulses of the first pulser in its FFT measurements is small. 



%The mean time for the first pulser to start after the first FFT duration is 
%$$X_{1} = \frac{\tau}{1 - \prod_{i} (1-p_{i}) } \approx \frac{\tau}{\sum_i p_i}.$$
%Here, we have assumed for simplicity that the probabilities $p_i$ do not change with time. Now if the estimates $\hat{\mu}_{i}$ are accurate and equal to true bottleneck rate $\mu^{*}$, a first-order approximation for $p_i \ll 1$ yields
%$$X_{1} = \frac{\mu^{*}}{\sum_{j=0}^{n}R_{j}} \times \textnormal{Duration of FFT} = \textnormal{Duration of FFT}.$$

It is also not difficult to show that the number of pulsers within an FFT duration has  approximately a Poisson distribution with a mean of $\kappa$~\cite{probabilitybook}. Thus the probability that after one flow becomes a pulser, a second flow also becomes a pulser before it can detect the pulses of the first flow in its FFT measurements is $1 - e^{-\kappa}$. Therefore, $\kappa$ involves a tradeoff: a smaller $\kappa$ will lead to fewer conflicts but will take longer to elect a pulser.


For any value of $\kappa$, there is a non-zero probability of more than one concurrent pulser. If there are multiple pulsers, then each pulser will observe that the cross traffic has more variation than the variations it creates with its pulses. This can be detected by comparing the magnitude of the FFT of the cross traffic $z(t)$ at $f_p$ with the FFT of the pulser's receive rate $R(t)$ at $f_p$.  If the cross traffic's FFT has a larger magnitude at $f_p$, \name concludes that there must be multiple pulsers and switches to a watcher with a fixed probability.

\if 0
\smallskip
\noindent{\bf Remark.}
This scheme for coordinating pulsers is similar to receiver-driven layered multicast (RLM) congestion control~\cite{rlm}. In RLM, a sender announces to the multicast group that it is conducting a probe experiment at a higher rate, so any losses incurred during the experiment should not be heeded by the other senders. In contrast, in \name, there is no explicit coordination channel, and the pulsers and watchers coordinate via their independent observations of cross traffic patterns.
\fi

%a single pulser flow it will observe that $\mid FFT_{z_{\mbox{out}}}(f_p)\mid < |FFT_{z}(f_p)\mid$, but not when there are multiple pulsers. When this condition is seen, a pulser switches to becoming a watcher with some probability.


%The variations in cross traffic are quantified by $\mid FFT_{z}(f_p)\mid$. 

%effect of the variation introduced by the pulsers in aggregate can be quantified by $\mid FFT_{z_{\mbox{out}}}(f_p)\mid$, where $z_{\mbox{out}} = \mu - R(t)$. When there is a single pulser flow it will observe that $\mid FFT_{z_{\mbox{out}}}(f_p)\mid < |FFT_{z}(f_p)\mid$, but not when there are multiple pulsers. When this condition is seen, a pulser switches to becoming a watcher with some probability.

\if 0

Using a similar argument and assuming $\tau$ to be small, it will take another
$$X_{2} = \sum_{i=0}^{n}\frac{p_{i}}{\sum_{j=0}^{n}p_{j}}(\frac{\mu^{*}}{\sum_{j=0,j\ne i}^{n}R_{j}}) * \textnormal{Duration of FFT}$$ 
for a second Pulser to be elected. Since $X_{2}$ is greater than Duration of FFT, this rule ensures that in expectation atmost 1 pulser will be elected. Not only that this rule gives higher preference to bigger watcher flows over smaller ones.

But, what if multiple flows become Pulser at the same time? 


\pg{Talk about cases where pulser and watcher election is not required. Say that FFT used by watcher is smaller to increase switching speed}

\fi


==> nimbus-protocol.tex <==
\newcommand{\nimbusprotcol}{Nimbus}
\section{Nimbus}
\label{s:nimbus-protocol}

%This section describes a protocol that uses mode switching. It has a TCP-competitive mode in which the sender transmits using Cubic's congestion avoidance phase, and a delay-control mode that uses a method, described below. The sender switches between the two modes using the elasticity detector described in the previous section, transmitting data at the time-varying rate dictated by the congestion control, and modulating its transmissions on the asymmetric sinusoid of \Fig{semi-sine}. 

\name is a congestion control system that uses mode switching. It has a TCP-competitive mode in which the sender transmits using a TCP-competitive congestion control algorithm (e.g., Cubic), and a delay-control mode that uses a \dcc algorithm (e.g., Copa). \name switches between the two modes using the elasticity detector described in the previous section. 


\if 0
\subsection{Delay-Control Rule}
\label{s:delay-control}



\Para{Competitive mode:} \name{} emulates TCP Cubic for TCP-competitive mode. The choice of Cubic is guided by the fact that Cubic  is the default congestion control algorithm on linux. This suggests that most of elastic cross traffic is composed of Cubic flows and in order to compete with the elastic flows fairly, \name{} must emulate Cubic. \name calculates the congestion window using Cubic's congestion window update rule and sets the pre-pulsing rate to (congestion window)/$RTT$. All the Cubic congestion control parameters were chosen to match the default linux implementation.



Nimbus uses a delay-control control rule inspired by ideas in XCP~\cite{xcp}, TIMELY~\cite{timely}, and PIE~\cite{pie}. It seeks to achieve high throughput while maintaining a specified threshold queuing delay, $d_t >0$. A positive $d_t$ ensures that the link is rarely under-utilized, and allows us to estimate $z(t)$. The protocol seeks to deliver an ideal rate of $\mu-z(t)$. The reason we designed our own method rather than use an existing one like Vegas~\cite{vegas} is because our ability to estimate $z$ yields tighter controls on delay than prior protocols.

The control rule has two terms. The first seeks to achieve the ideal rate, $\mu - z$. The second seeks to maintain a specified threshold queuing delay, $d_t$, to prevent the queue from both emptying and growing too large. 

Denote the minimum RTT by $x_{\min}$ and the current RTT by $x_t$. The \name delay-control rule is 
\begin{equation}
S(t+\delta) = 
    (1-\alpha) S(t) 
    + \alpha (\mu - z(t)) 
    + \beta\frac{\mu}{x_t}
        (x_{\min} + d_t  - x_t).
\label{eq:delayrule}
\end{equation}
Prior work (XCP~\cite{xcp} and RCP~\cite{rcpstable}) has established stability bounds on $\alpha$ and $\beta$ for nearly identical control laws. Our implementation uses $\alpha=0.8$, and $\beta=0.5$.

\fi
\subsection{Mode Switching}
\label{s:mode_switching}
At any given time, \name transmits data at the time-varying rate dictated by the congestion control algorithm running at that time. It modulates this rate with asymmetric sinusoidal pulses (\Fig{semi-sine}). \name uses the pulsing parameters described in $\S$\ref{s:elasticity:parameter_tuning}, calculating $S$ and $R$ over one window's worth of packets. It computes the FFT for the $z$ measurements reported in the last 5 seconds to calculate elasticity ($\eta$) using Eq. \eqref{eq:elasticity}, and it picks the mode by comparing $\eta$ to $\eta_{thresh} = 2$ (\S\ref{s:elasticity:parameter_tuning}).

%We found earlier that a good threshold for $\eta$ is 2 (\Fig{elasticity:cdf} and discussion in \S\ref{s:elasticity:parameter_tuning}). To prevent frequent mode switches, \name applies a hysteresis to this threshold before switching modes. When in delay-control mode, $\eta$ must exceed 2.25 to switch to TCP-competitive mode, and when in TCP-competitive mode, $\eta$ must be lower than 2 to switch to delay-control mode.

We support Cubic and NewReno for the TCP-competitive mode and Copa's default mode and Vegas for the delay-control mode. We also implemented a basic delay-controlling algorithm, BasicDelay, using our cross traffic rate estimator. 
%\an{ We support Cubic and NewReno for the TCP-competitive mode and Copa's default mode, Vegas, and BasicDelay --- a delay-controller which uses our cross traffic estimator --- for the delay-control mode.  }
%\an{We support Cubic and NewReno in TCP-competitive mode. In delay-control mode, we support Copa's default mode, Vegas, and a basic delay-controller (BasicDelay) which uses our cross traffic estimator.}

Let $S$ be the sending rate and $\hat z$ be the estimated cross-traffic rate, both measured over the last window of packets. Also, let $x$ be the current RTT, and $x_{min}$ be the minimum observed RTT. Upon receiving an ACK, BasicDelay sets its current rate to:
\vspace{-1mm}
\begin{equation}
 \text{Rate} \leftarrow
    S 
    + \alpha (\mu - S - \hat z) 
    + \beta\frac{\mu}{x}
        (x_{\min} + d_t  - x),
\label{eq:delayrule}
\end{equation}
%\vspace{-1mm}
where $\alpha$ and $\beta$ are constants smaller than 1, and $d_t$ is a target queuing delay. The term $(\mu - S - z)$ is the sender's estimate of the spare capacity in the last RTT. By adding an $\alpha$-fraction of the spare capacity to $S(t)$, BasicDelay tries to get closer to the ideal rate. The second term in the above rule seeks to maintain a specified queuing delay, $d_t$, to prevent the queue from both growing too large or going empty. Recall that our cross traffic estimator, Eq.~\eqref{eq:zfromR}, requires a non-empty queue to estimate $z$.

% inspired by ideas in XCP~\cite{xcp}, TIMELY~\cite{timely}, and PIE~\cite{pie}. This control law uses our estimate of the cross traffic ($z$) to have a tighter law on delays compared to previous \dcc schemes.

% \an{move to appendix?}
% \pg{We denote the minimum RTT by $x_{\min}$ and the current RTT by $x_t$. The proposed delay-control rule is 
% %\abovedisplayskip
% \begin{equation}
% S(t+\delta) = 
%     (1-\alpha) S(t) 
%     + \alpha (\mu - z(t)) 
%     + \beta\frac{\mu}{x_t}
%         (x_{\min} + d_t  - x_t).
% \label{eq:delayrule}
% \end{equation}
% %\belowdisplayskip
% The control rule has two terms. The first seeks to achieve the ideal rate, $\mu - z$. The second seeks to maintain a specified threshold queuing delay, $d_t$, to prevent the queue from both emptying (\name requires a non-empty queue for estimating $z$) and growing too large.}
%Unless specified we use Cubic for TCP-competetive mode and the above control law for delay-control mode.}

%The rate must be initialized carefully when switching to TCP-competitive mode. 
\name takes special care in initializing the rate when switching to TCP-competitive mode.
\name sets the rate (and equivalent window) to the rate that was used 5 seconds ago because the elasticity detector takes 5 seconds (FFT Duration) to detect elastic cross traffic. 
During this time, the elastic traffic could cause a reduction in the delay-control mode's rate. 
Hence, \name resets its rate to the rate at the beginning of the 5-second detection period. 

%We set the new congestion window to the inflection point of the Cubic function, so the rate over the next few RTTs will rise faster in each successive RTT, and we reset \texttt{ssthresh} to this congestion window to avoid entering slow start.

%While switching to delay mode, \name resets the delay threshold to the current value of $x_t - x_{\min}$, rather than to the desired threshold $d_t$, and linearly decreases the threshold used in the control rule to the desired $d_t$ over several RTTs. The reason is that $x_t - x_{\min}$ is likely to have grown much larger than $d_t$ in TCP-competitive mode, and using $d_t$ would only cause the sender to reduce its rate and go down in throughput. The approach we use ensures instead that the delay mode will drain the queues gradually and won't lose throughput instantly, and also provides a safeguard against incorrect switches to delay mode.

\if 0
There are some special cases to handle. First, if there is no observable peak in FFT of $z$, the sender has no good estimate of the elasticity, so \name defaults to competitive mode. Second, when the current rate is less than 10\% of the bottleneck link, \name switches to TCP-competitive mode as it has too little of the bottleneck for delay mode to be effective. Third, when the current rate is greater than 90\% of bottleneck rate switch to delay mode, because \name is the dominant contributor to that network path.
    
\fi



%\input{multiple_nimbus.tex}


    
\subsection{Implementation}
\label{s:implementation}

We implemented \name using CCP~\cite{ccp-sigcomm18}, which provides a convenient way to express the signal processing operations in user-space code.
%while achieving sending rates of up to 10 Gbit/s.
It uses estimates of $S$, $R$, the RTT, and packet losses from the Linux kernel every 10 ms. 

\cut{
On every measurement report, \name (1) updates the congestion control variables of the current mode and calculates a pre-pulsing sending rate, (2) superimposes the asymmetric pulse in \Fig{semi-sine} to obtain the actual sending rate, and (3) generates the FFT of $z$ and makes a decision to switch modes using a 5-second measurement period for the FFT.
}

%\an{move this para to cross traffic estimator section?}
Calculating $\hat z$ requires an estimate of the bottleneck link rate ($\mu$). There has been much prior work~\cite{packettrain, dovrolis2001packet, downey1999using, lai2000measuring, jacobson1997pathchar, lai2001nettimer, mar2000pchar} in estimating $\mu$, which \name{} could use.
We use the maximum received rate as the estimate, taking care to avoid incorrect estimates due to ACK compression. We evaluate the impact of errors in estimating $\mu$ on elasticity detection in \Sec{robustness-synthetic}.
%% and dilation. \ngs{What's ack dilation?}

==> outline.tex <==
\section{Outline}

Sec I. Intro

* Context
- holy grail goal for all apps: high throughput and low delay.
    -- Delay based protocols can work with low delays (new protocols are trying to get low delays COPA/BBR)
        --- good when the cross traffic is not competitive(UDP or application limited) bad when it isn't (cross traffic will kill)
    -- Loss based protocols are not able to get low delays even when possible
    -- Nimbus build an estimator for estimating competitiveness(elasticity) of cross traffic , use it to for a dual mode congestion control protocol that combines a delay and loss based scheme
    -- Show Figure 2 of NSDI as an Illustration

- use cases
    -- home networks
    -- data centers
    -- aggregation between organizations 
    -- Internet traffic Analysis?

* Contributions:
- Concept of elasticity and formal definition of elastic traffic.
- Estimating Cross Traffic elasticity
- Pulsing to detect cross traffic elasticity
- Multiple Nimbus
- Build Nimbus as a TCP, practical scheme
    
* Assumptions
- Single Bottleneck link. Widely accepted for home settings. Justify this for aggregates as well
- Nimbus Pulser controls a reasonable fraction of the link capacity and can pulse



Sec II. System

-Cross traffic estimation logic
    -- How are send rate (Rin) and receive rate (Rout) calculated
    -- Include Figure 3 from NSDI paper

- Elasticity overview
    -- Define what it means to be elastic (ACK clocked)
    -- Show that elastic cross traffic reacts to pulses and inelastic doesn't (Figure 4 NSDI)
    -- Introduce FFTs and how we calculate elasticity (Figure 5 NSDI)
        --- Explain why just looking queuing delays is not enough
        --- Explain advantages of FFTs, cross traffic can have different/variable base RTTs, can pulses continuously
    --Assymetric pulse
    -- Introduce Elasticity metric for switching
        --- Show figure 6 of NSDI paper as a proof of concept
        --- Show how and when are measurements taken and used for switching
    -- bottleneck bandwidth estimation use old techniques such as packet train or 
    

- Multiple Nimbuses
    -- Introduce pulser and watcher. Pulser makes decisions for watchers/followers.
        -- Pulser uses frequency 1 for competitive and frequency 2 for delay based
        -- Watchers don't react to pulses by the pulser, watchers use EWMA to smoothen reactions to pulses of the pulser
        -- Emphasize watcher doesn't need to estimate Z for deciding mode
    -- Election process for pulser watcher switching
        --Show an illustration figure???

- Show that we can use any competetive scheme (cubic, mulTCP, reno) and any delay based scheme(vegas, fast, our own delay based scheme)
    - Figure????
    - Introduce or delay based scheme as well


Sec VI. Evaluations

(1) Big Experiment
    - Figure 11 of NSDI paper
    - Redo with just cubic instead of MulTCP


(2) Empirical Traffic Generator (figure 12 and 13 of NSDI)
    - Nimbus gets same throughput but way lower delays
    - Show switching works under complicated scenarios

(3) Real World Experiment (fig 16 of NSDI)
    - 5 Servers in 5 different countries
    - 5 client in 2 different countries
    - We do good on paths with buffering
    - Show policed paths
    
(4) Nimbus can be used for aggregation (Fig 14 NSDI) - under debate
    - Maybe show default scheduling instead of complicated scheduling

Robustness

(5) Heat Map of percentage of times switched correctly

(6) Elasticity works for cross traffic RTT and buffer scenarious (Show CDF of elasticity)

(7) Multiple Nimbus
    - demonstrate pulser/watcher switchins
        -- Experiment with multiple flows coming and leaving
    - Show switching works with multiple nimbuses
        --Overview experiment 


Limitations
- Model doesn't take into account aggress traffic which is not Ack clocked (for example BBR)
- Systems issues involved
    - Bad Rin and Rout measurements under specific conditions (for example WIFI)




==> overview.tex <==
\newcommand{\modelsec}{System Model and Goals}
\section{\modelsec}
\label{s:model}
\label{s:overview}

A persistent traffic source, unlike one that comes and goes, can learn the congestion state of
the network all the time to more accurately estimate and react to cross traffic. %% Each \name instance controls traffic belonging to a {\em bundle}, which we define as the subset of flows in an aggregate that shares the same bottleneck queues in the network and whose offered load is persistent.

\begin{figure}[t]
    \includegraphics[width=0.9\columnwidth]{images/sys-model2}
    \caption{\small {\bf \name system model---}An aggregate sender sends packets to an aggregate receiver. The network has cross traffic from flows outside of the aggregate running a variety of protocols. The time-varying total rate of this cross traffic is $z(t)$, of which $z_i(t)$ is ``inelastic''; the rest is transmitted by $n_x(t)$ long-running TCP flows.  The bottleneck link rate is $\mu$. The control algorithm's goal is to compute a time-varying transmission rate, $R(t)$ for the aggregate, such that it behaves like $n_b$ long-running TCP flows. We denote the rate of traffic received by the \name{} receiver by $\Rout$.}
    \label{fig:sysmod}
\end{figure}

\Fig{sysmod} shows the system model for \name's design and introduces some notation. The \name sender transmits packets aggregated from many flows at a time-varying total rate, $R(t)$. The sender chooses which packet to transmit according to a scheduling policy across aggregated flows, such as round-robin, shortest-flow-first (SRPT), etc. Although we focus on determining the aggregate rate, we also evaluate the impact of a few bundle scheduling policies in $\S$\ref{s:scheduling}.

\smallskip
\noindent{\bf What is the correct rate, $R(t)$ for the aggregate?} One answer could be to estimate the difference between the bottleneck link capacity and the bandwidth used by the cross traffic: $\mu - z(t)$. This is wrong because when cross traffic is elastic, this quantity will be close to 0, because elastic flows will tend to grab all available bandwidth. In the presence of elastic flows, \name must compete for its fair share of the bottleneck bandwidth, not just settle for the left-over bandwidth. 

We define the desired value for $R(t)$ as the average rate that $n_b$ long-running TCPs would achieve under the same cross traffic conditions. The choice of $n_b$ is a local policy decision and affects how aggressively the bundle behaves; one setting could be the number of TCP flows longer than some length in the bundle. 

If the inelastic portion of the cross traffic is $z_i(t)$, and the cross traffic also contains $n_x$ long-running elastic flows, then we define the desired rate for the bundle to be
\vspace{5pt}
\begin{equation}
R(t) = (\mu - z_i(t))\frac{n_b}{n_b + n_x}.
\label{eqn:nimbusgoal}
\end{equation}
\vspace{5pt}
The intuition for this equation is that inelastic traffic does not adapt its rate to congestion; hence, elastic flows in the cross traffic and in \name should divide the remaining capacity, $\mu - z_i(t)$, in the ratio $n_x$ to $n_b$.\footnote{\name may also include inelastic flows, but we can account for these by setting $n_b$ higher to ensure that \name does not put itself at a disadvantage relative to cross traffic.}

% When we use the term
%``available bandwidth'' in this paper, we mean the ``right'' bandwidth
%as defined above; the context (elastic or not) matters.

Of course, \name does not know the value of $z(t)$, nor whether the cross traffic includes elastic flows. Nonetheless, achieving the rate in Eq.~(\ref{eqn:nimbusgoal}) by itself is not difficult. Any scheme that emulates TCP's congestion control rules for $n_x$ flows will achieve this rate on average. However, as explained in $\S$\ref{s:intro}, \name also aims to minimize self-inflicted delay. Whenever cross traffic is inelastic, we can potentially achieve the same rate with much lower delay than traditional loss-based control algorithms (especially in networks with deep buffers). This makes the problem much more challenging and requires new techniques to infer the elasticity of cross traffic using observations by the \name sender and receiver.



% The key idea in \name{} is to explicitly identify an operating mode and
% switch between them. The reason is that if the cross traffic is
% inelastic, a delay-based controller is potentially superior to
% traditional loss-based control because it may be possible to satisfy
% property A from \Sec{intro}: high utilization with lower delay
% especially in networks with deep buffers compared to the
% bandwidth-delay product (BDP). \name{} develops a new delay-control
% rule for this purpose.

% Conversely, when cross traffic is elastic, delays are much higher and
% delay-based control is overwhelmed by legacy loss-based
% controllers. The right reaction here is to emulate $x$ long-running
% TCPs (the choice of $x$ is a local policy decision; one setting could
% be the number of TCPs longer than some length seen in the bundle).

% Developing a method to identify when to switch modes is difficult
% because it requires the sender of the aggregate to be able to infer
% cross traffic that it does not directly observe. We propose a new
% technical contribution to solve this problem called an {\em elasticity
%   estimator}. The estimator relies on an estimator for the overall
% volume of cross traffic, and on the sender modulating its packet
% transmissions atop a square-shaped pulse. By observing the changes in
% the rate at which it receives packets and the change in delays of
% those packets, the estimator determines whether the cross traffic is
% elastic or not.

% Figure~\ref{fig:sysmod} shows the system model and introduces some
% notation.




==> packages.tex <==
\if 0
\setlength\paperheight{11in}
\setlength\paperwidth{8.5in}
\setlength{\textwidth}{7in}
\setlength{\textheight}{9.25in}
\setlength{\oddsidemargin}{-.25in}
\setlength{\evensidemargin}{-.25in}

\fi

%
\usepackage{xspace}
\usepackage{multirow}
\usepackage{comment}
\usepackage{fancybox, fancyvrb, calc}
\usepackage{subcaption}
\usepackage[inline]{enumitem}
\usepackage{amsmath, amssymb}
\usepackage{cite,url}
\usepackage{pbox}
\usepackage{balance}
\usepackage{wrapfig}
%
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{mathptmx}
\usepackage{enumitem}
\setlist{nolistsep}
\usepackage{hhline}
%
\captionsetup[table]{skip=-1pt,font={footnotesize}}
\captionsetup[subfigure]{skip=-1pt,font={footnotesize}}
\captionsetup[figure]{font={footnotesize}}
\Urlmuskip=0mu plus 1mu
\hypersetup{%
  colorlinks=true,      % false: boxed links; true: colored links
  linkcolor=blue,       % color of internal links
  citecolor=magenta,    % color of links to bibliography
  filecolor=cyan,       % color of file links
  urlcolor=blue          % color of external links
}
%
\usepackage{leading}
\leading{12pt}
%
\usepackage{minted}
%
\usepackage[subtle]{savetrees}
\usepackage[small,compact]{titlesec}
\usepackage{outlines}
%
\newcommand{\cut}[1]{}
%
\newcommand{\paragraphnone}[1]{\vspace{0.075in}\noindent{\bf #1}}
\newcommand{\paragrapha}[1]{\vspace{0.075in}\noindent{\bf #1.}}
\newcommand{\paragraphq}[1]{\vspace{0.075in}\noindent{\bf #1}}
%
\newcommand{\eg}{e.g., }
\newcommand{\etc}{{etc.}\xspace}
\newcommand{\ie}{i.e., }
\newcommand{\ccp}{CCP\xspace}
%
\newcommand{\an}[1]{{\color{green}\bf AN: {#1}}}
\newcommand{\sn}[1]{{\color{purple}\bf NG: {#1}}}
\newcommand{\hb}[1]{{\color{brown}\bf HB: {#1}}}
\newcommand{\ma}[1]{{\color{red}\bf MA: {#1}}}
\newcommand{\pg}[1]{{\color{blue}\bf PG: {#1}}}
\newcommand{\fc}[1]{{\color{blue}\bf FC: {#1}}}
\newcommand{\dr}[1]{{\color{magenta}\bf DR: {#1}}}
%
\newcommand{\datapath}{datapath\xspace}
\newcommand{\datapaths}{datapaths\xspace}
\newcommand{\Datapaths}{Datapaths\xspace}
\newcommand{\Datapath}{Datapath\xspace}
%
\frenchspacing
%
\newcommand{\handlers}{callbacks\xspace}
\newcommand{\userspace}{user-space\xspace}
\newcommand{\kernelspace}{kernel-space\xspace}
%
\newcommand{\controller}{agent\xspace}

==> rate-delay-table-newintro.tex <==
{\centering
%%\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{ccc}
\hline

{\textbf{Algorithm}} &
{\textbf{Median RTT}} &
{\textbf{Average rate}} \\

&
{\textbf{(ms)}} &
{\textbf{(Mbit/s)}} \\

\hline
\hline

\name &
\ \ 64&
51.4
\\

BBR &
118&
52.0\\

Cubic &
112&
52.4
\\

Vegas &
\ \ 53 &
45.0\\

\hline
\end{tabular}
%%}
%\vspace{...}
\label{fig:tput-delay-summary}
}

==> related.tex <==
\newcommand{\relworksec}{Related Work}
\section{\relworksec}
\label{s:related}

\if 0
Vegas aims to maintain between $\alpha$ and $\beta$ packets in the bottleneck queue using AIAD on its window. Similar to Vegas, FAST~\cite{fasttcp} exploits delay information to set its congestion window to maintain a fixed number of packets in the bottleneck queue. TCP Nice~\cite{tcp-nice} and LEDBAT~\cite{rfc6817} are delay-based algorithms to utilize spare bandwidth without hurting ``foreground'' transfers like web traffic. Timely~\cite{timely} is a delay-based algorithm designed to work in data centers over RDMA. These schemes don't perform well when competing with buffer-filling algorithms.
\fi 

\if 0
TCP Nice maintains two estimates of RTTs, a min RTT and a max RTT, through which it
tracks an estimate of the maximum queueing delay possible. Along with Vegas-like
increase/decrease rules, Nice multiplicatively decreases its congestion window
whenever a fraction $f$ of its packets experience queueing delay more than a
fraction $t$ of the maximum queueing delay possible. LEDBAT~\cite{rfc6817} is
another delay-based algorithm with a set target delay. It increases its
congestion window proportional to the difference between the target and the
current delay, \ie target - current.
\fi

\if 0
FAST, Nice and LEDBAT can achieve high throughput and low delays when there is a
low volume of cross-traffic. But they are not designed to be
throughput-competitive with loss-based algorithms that probe aggressively for
bandwidth. \name detects the presence of aggressive cross-traffic, and competes
fairly by switching to its TCP-competitive mode.
\fi

\if 0
Compound TCP~\cite{compound} maintains both a loss-based window and
a delay-based window, and transmits data based on the sum of the two
windows. Compound achieves high throughput as soon as the link utilization drops because of its delay window, but does not control self-inflicted delays because of its loss window. 
\fi



%%mPERT~\cite{mpert} \ngs{Should complete this.}
%%% Prateesh on mPERT:
%%% http://www.hamilton.ie/lukasz/downloads/papers/IWQoS-draft-08.pdf They have
%%% designed an algorithm where drop_probability is virtually set as a function
%%% of current queuing delay, For a particular Throughput (or drop probability)
%%% there are two points(or
%%% queuing delays), one with low queuing delay and one with high queuing delay,
%%% In absence of elastic background traffic the equilibrium happens at low
%%% queuing delay, in presence of elastic queueing traffic the equilibrium is at
%%% higher queuing delay

\if 0

Equation-based congestion control
(EBCC~\cite{ebcc}) sends traffic at a rate computed to match TCP under similar
RTT and drop probabilities in the network.  EBCC maintains a rate of `loss
events,' where a loss event may include multiple packets lost within an RTT. The
loss event rate and the RTT are used to compute the desired transmission rate
using the TCP throughput equation. EBCC uses packet loss as a signal for
congestion control, and hence cannot achieve a low queuing delay. In contrast,
\name controls delays directly.

MulTCP~\cite{multcp} emulates the behavior of an aggregate of $N$ TCP loss-based
algorithms. It evolves its congestion window as follows. It increases its
congestion window by $N/cwnd$ for each ACK, and decreases it to $cwnd *
(N-0.5)/N$ after each drop. However, as our experiments show (\S\ref{s:eval}),
MulTCP sending rates are very bursty and variable, and MulTCP competes unfairly
with other loss-based TCPs. \name's TCP-competitive mode is smoother and fairer
to other elastic traffic than MulTCP.

\fi

BBR~\cite{bbr} maintains estimates of the bottleneck bandwidth ($b$) and minimum propagation delay ($d$). It  paces traffic at a rate $b$ while keeping $b\times d$ packets in flight. The presence of other loss-based algorithms sharing the bottleneck buffer inflates BBR's delay estimate, $d$. Depending on the bottleneck buffer size, either the BBR-induced losses limit the throughput of the other TCP flows, or BBR's delay probing reduces its in-flight data, resulting in lower throughput for BBR itself~\cite{bbr-reno-graph}.

% The bandwidth estimate tracks the maximum packet delivery rate to the receiver, while the delay estimate tracks the minimum delay achieved. BBR paces traffic at a rate $b$ while keeping $b\times d$ packets in flight. Unfortunately, the presence of other loss-based algorithms sharing the bottleneck buffer inflates BBR's delay estimate $d$. Depending on the bottleneck buffer size, either the BBR-induced losses limit the throughput of the other TCP flows, or BBR's delay probing reduces its in-flight data, resulting in lower throughput for BBR itself~\cite{bbr-reno-graph}.

Vegas~\cite{vegas}, FAST~\cite{fasttcp}, and Copa~\cite{copa} all aim to maintain a bounded number of packets in the bottleneck queue using different control rules. TCP Nice~\cite{tcp-nice} and LEDBAT~\cite{rfc6817} are delay-based algorithms to use spare bandwidth without hurting ``foreground'' transfers. Timely~\cite{timely} is a designed for RDMA in datacenters. Other than Copa, these schemes perform poorly when competing with buffer-filling algorithms. Copa has a mechanism to switch into a TCP-competitive mode, but it relies on low-level properties of the dynamics of Copa and does not generalize.

\if 0
PCC~\cite{pcc} adapts the sending rate based on ``micro-experiments'' that evaluate how changing the sending rate (multiplicatively) impacts performance according to a specified utility function. PCC defines two utility functions: one targeting high throughput and low loss, and the other targeting low delay. PCC's behavior depends on the utility function; unlike \name, it does not achieve both low delay and compete with elastic loss-based TCPs. 
\fi

\if 0
Prior work on estimating cross-traffic rate~\cite{strauss2003measurement,jain2002pathload,hu2003evaluation} use probe packets, and are slow in estimating cross traffic. For example pathload~\cite{jain2002pathload} takes 10-30 s to generate a single cross traffic estimate. In contrast, our method is in-band and it relies on the property that the sender is backlogged.
\fi

The multiple-\name scheme for coordinating pulsers bears resemblance to receiver-driven layered multicast (RLM) congestion control~\cite{rlm}. In RLM, a sender announces to the multicast group that it is conducting a probe experiment at a higher rate, so any losses incurred during the experiment should not be heeded by the other senders. By contrast, in \name, there is no explicit coordination channel, and the pulsers and watchers coordinate via their independent observations of cross traffic patterns.

\if 0
The idea of sharing congestion information among connections was explored in Congestion Manager~\cite{CM} for traffic between a single pair of hosts. \name can provide this benefit for larger traffic aggregates, such as all traffic between two organizations.

\fi


==> related_v2.tex <==
\newcommand{\relworksec}{Related Work}
\section{\relworksec}
\label{s:related}

The works most closely related to our elasticity detector are congestion control schemes Copa~\cite{copa} and BBR~\cite{bbr}. 

%\smallskip
\noindent{\bf Copa.} Copa aims to maintain a bounded number of packets in the bottleneck queue. Copa induces a periodic pattern of sending rate that nearly empties the queue once every 5 RTTs. This helps Copa flows obtain an accurate estimate of the minimum RTT and the queuing delay. In addition, Copa uses this pattern to detect the presence of  non-Copa flows: Copa expects the queue to be nearly empty at least once every 5 RTTs, provided only Copa flows with similar RTTs share the bottleneck link.
%\footnote{Copa estimates if a queue is ``nearly empty'' using the observed short-term RTT variation (see $\S$2.2 of~\cite{copa}).} 
If the estimated queuing delay does not drop below a threshold in 5 RTTs, Copa switches to a TCP-competitive mode.

% short-term RTT variation is smaller than a threshold, 

%\looseness=-1
Unlike Copa, our elasticity detector does not look for a pattern in the RTTs caused by its transmission pattern. Instead, it estimates the rate of the cross traffic and observes how the cross traffic reacts to the rate fluctuations it induces over a period of time. This enables our elasticity detector to directly estimate the elasticity of cross traffic. 
Although elasticity detection takes a few seconds, our experiments show that is significantly more robust than Copa's method. 1) Copa switches mode incorrectly frequently and loses throughput against elastic cross-traffic (\S\ref{s:big-experiment} and \S\ref{s:rw-wl}). Copa uses instantaneous measurements for mode-switching and is vulnerable to variation in the cross traffic. 2) Copa misclassifies cross traffic when the inelastic traffic rate is high, or when elastic flows have high RTTs ($\S$\ref{s:copa-compare}). 
Moreover, since \name's cross traffic estimation technique does not rely on properties of any specific rate control algorithm (e.g., emptying queues every 5 RTTs), it can be applied to any combination of TCP-competitive and delay-controlling schemes. 
%\looseness=-1

\smallskip
\noindent{\bf BBR.}
BBR estimates the bottleneck bandwidth ($b$) and minimum RTT ($d$). 
It paces traffic at a rate $b$ while capping the number of in-flight packets to $2\times b\times d$.
To estimate the bottleneck, BBR periodically increases its rate over $b$ for about one RTT and then reduces it for the following RTT. 
BBR uses this sending-rate pattern to obtain estimates of $b$; specifically, it tests if the bottleneck rate exceeds the current estimate $b$ in the rate-increase phase. However, BBR doesn't use these pulses to infer the nature of cross traffic.

\cut{ and subsequently drains the extra queuing this causes in the rate-decrease phase}

\cut{BBR does not compete fairly with other TCP flows (e.g., Cubic). \cut{In particular, }BBR's method to set rate can be overly aggressive in the presence of other TCP flows. Depending on the bottleneck buffer size, either the BBR-induced losses limit the throughput of the other TCP flows (with shallow buffers), or BBR's hard cap on its in-flight data based on $d$ causes it to get lower throughput than its fair share (with deep buffers)~\cite{bbr-evaluation}. }
% \smallskip
% \pg{\noindent{\bf PCC-Vivace}
% PCC-Vivace~\cite{vivace} uses an online learning algorithm to adapt its sending rate to maximize a utility function and achieve high performance. Its utility function incorporates achieved rate, delay gradient and loss information for latency minimization and TCP friendliness. 
% Our experiments ($\S$\ref{s:big-experiment}, $\S$\ref{s:rw-wl}) show that Vivace fails to achieve low delay and TCP friendliness simultaneously.}

% \pg{Against inelastic traffic, Vivace fails to maintain low delays when cross traffic occupies a substantial fraction of the link (50\%). Because of variations in cross traffic, Vivace's sending rate can become greater than its fairshare, filling up the buffer. If subsequent rates picked by Vivace's algorithm are above its fair share, then, the buffer will stay full. Delay gradient will become zero and Vivace's utility will depend only on loss and rate. Without the delay gradient term, Vivace will incur high losses and delay\footnote{In presence of inelastic cross traffic, increasing Vivace's sending rate increases both rate achieved and losses incurred. Based on coefficients of loss and delay term, Vivace's sending rate will converge to a rate greater than its fairshare.}. Against elastic traffic, Vivace fails to achieve  throughput similar to TCP(Cubic). Vivace's utility function depends on delay gradient and is different from standard TCP's utility function, leading to unfairness.}


%PCC~\cite{pcc} adapts the sending rate based on ``micro-experiments'' that evaluate how changing the sending rate (multiplicatively) impacts performance according to a specified utility function. PCC defines two utility functions: one targeting high throughput and low loss, and the other targeting low delay. Recently, PCC-Vivace~\cite{vivace} improved on PCC with a utility function framework and a rate control algorithm based on regret minimization. The behavior of these schemes depends on the utility function; unlike \name, they do not achieve both low delay and compete well with elastic loss-based TCPs simultaneously.

\smallskip
\noindent{\bf Other related schemes.}  
Vegas~\cite{vegas} and FAST~\cite{fasttcp} are delay-based algorithms that aim to maintain small queues at the bottleneck using different control rules. Other delay-based algorithms include TCP Nice~\cite{tcp-nice}, LEDBAT~\cite{rfc6817}, and Timely~\cite{timely} (which is designed for datacenters). These schemes generally perform poorly when competing with buffer-filling algorithms.  
PCC-Vivace~\cite{vivace} uses an online learning algorithm to adapt its sending rate to maximize a utility function that incorporates the achieved rate, delay, and loss rate. Our experiments ($\S$\ref{s:big-experiment}, $\S$\ref{s:rw-wl}) show that Vivace cannot achieve both low delay with inelastic cross traffic and compete fairly with elastic TCP flows.  Compound TCP~\cite{compound} maintains both a loss-based window and a delay-based window, and transmits data based on the sum of the two windows. Compound does not attempt to switch between two modes, and therefore it incurs high queuing delays due to its loss-based window.
 %queues  not achieves high throughput as soon as the link utilization drops because of its delay window, but does not control self-inflicted delays because of its loss window.  


%\ma{we should add back the two paragraphs on PCC and prior work on estimating rate of cross traffic if at all possible} \pg{can we put them in the appendix?}


\if 0
PCC~\cite{pcc} adapts the sending rate based on ``micro-experiments'' that evaluate how changing the sending rate (multiplicatively) impacts performance according to a specified utility function. PCC defines two utility functions: one targeting high throughput and low loss, and the other targeting low delay. PCC's behavior depends on the utility function; unlike \name, it does not achieve both low delay and compete with elastic loss-based TCPs. 
\fi

\if 0
Prior work on estimating cross-traffic rate~\cite{strauss2003measurement,jain2002pathload,hu2003evaluation} use probe packets, and are slow in estimating cross traffic. For example pathload~\cite{jain2002pathload} takes 10-30 s to generate a single cross traffic estimate. In contrast, our method is in-band and it relies on the property that the sender is backlogged.
\fi

\if 0
The multiple-\name scheme for coordinating pulsers bears resemblance to receiver-driven layered multicast (RLM) congestion control~\cite{rlm}. In RLM, a sender announces to the multicast group that it is conducting a probe experiment at a higher rate, so any losses incurred during the experiment should not be heeded by the other senders. By contrast, in \name, there is no explicit coordination channel, and the pulsers and watchers coordinate via their independent observations of cross traffic patterns.
\fi

\cut{
\an{I have rewritten this section to focus on elasticity detection instead of CC}
%
The works most closely related to our elasticity detector are congestion control schemes Copa~\cite{copa} and BBR~\cite{bbr}. 
These schemes also periodically modulate their sending rates.%, but they do not infer the elasticity of cross traffic.

\noindent\textbf{Pulsing.} BBR and Copa use periodic sending patterns, or pulses, in their designs. 
BBR estimates the bottleneck bandwidth ($b$) and minimum RTT ($d$). 
To estimate the bottleneck, BBR periodically increases its rate over $b$ for about one RTT and then reduces it for the following RTT. 
BBR uses this sending-rate pattern to obtain estimates of $b$; specifically, it tests if the bottleneck rate exceeds the current estimate $b$ in the rate-increase phase.
Meanwhile, Copa induces a periodic pattern of sending rate that nearly empties the queue once every 5 RTTs. 
This helps Copa flows obtain an accurate estimate of the minimum RTT and the queuing delay.

\noindent\textbf{Pulsing to determine cross traffic.} While BBR does not attempt to determine the cross traffic's nature, Copa uses a heuristic to determine whether cross traffic consists of other Copa flows: Copa expects the queue to be nearly empty at least once every 5 RTTs, provided only Copa flows with similar RTTs share the bottleneck link.
If the estimated queuing delay does not drop below a threshold in 5 RTTs, Copa switches to a TCP-competitive mode.

%Nimbus was inspired by the idea of pulsing to determine cross traffic, but takes the additional step of analyzing the cross traffic's response to the pulses in the frequency domain.
In contrast, Nimbus explicitly models the cross traffic's volume and nature
This has several advantages: 
%for example, differences in flow RTTs (evaluated in \S\ref{s:robustness-synthetic}) are represented in phase, not amplitude, so are simpler to account for.
Although elasticity detection takes a few seconds, our experiments show that is significantly more robust than Copa's method. 1) Copa switches mode frequently and loses throughput against elastic cross-traffic (\S\ref{s:big-experiment} and \S\ref{s:rw-wl}). Copa uses instantaneous measurements for mode-switching and is vulnerable to variation in the cross traffic. 2) Copa misclassifies cross traffic when the inelastic traffic rate is high, or when elastic flows have high RTTs ($\S$\ref{s:copa-compare}). 
Moreover, since \name's cross traffic estimation technique does not rely on properties of any specific rate control algorithm (e.g., emptying queues every 5 RTTs), it can be applied to any combination of TCP-competitive and delay-controlling schemes.


\noindent\textbf{Learning-based approaches.} The PCC family of algorithms~\cite{pcc, vivace} argue that black-box experimentation is sufficient to achieve the benefits of elasticity detection for congestion control.
However, a learning-based approach does not provide diagnostic or measurement information, since it does not justify its actions. A PCC user wishing to learn about the nature of cross traffic on a link would have to infer this information indirectly from the algorithm's decisions.
Furthermore, from a congestion control perspective, our experiments ($\S$\ref{s:big-experiment}, $\S$\ref{s:rw-wl}) show that Vivace, the latest iteration, cannot achieve both low delay with inelastic cross traffic and compete fairly with elastic TCP flows.

\noindent\textbf{Measuring congestion.} Prior work~\cite{inferring-interdomain} has measured congestion at Internet scale using carefully placed ICMP probes to measure queueing, finding persistent congestion at some inter-domain links.
}

==> related_v3.tex <==
\newcommand{\relworksec}{Related Work}
\section{\relworksec}
\label{s:related}

%
The works most closely related to our elasticity detector are congestion control schemes Copa~\cite{copa} and BBR~\cite{bbr}. 
These schemes also periodically modulate their sending rates.

\noindent\textbf{Learning-based approaches.} The PCC family of algorithms~\cite{pcc, vivace} argue that black-box experimentation is sufficient to achieve the benefits of elasticity detection for congestion control.
However, a learning-based approach does not provide diagnostic or measurement information, since it does not justify its actions. A PCC user wishing to learn about the nature of cross traffic on a link would have to infer this information indirectly from the algorithm's decisions.
Furthermore, from a congestion control perspective, our experiments ($\S$\ref{s:big-experiment}, $\S$\ref{s:rw-wl}) show that Vivace, the latest iteration, cannot achieve both low delay with inelastic cross traffic and compete fairly with elastic TCP flows.

\noindent\textbf{Measuring congestion.} Prior work~\cite{inferring-interdomain} has measured congestion at Internet scale using carefully placed ICMP probes to measure queueing, finding persistent congestion at some inter-domain links.


\smallskip
\noindent{\bf Copa.} Copa~\cite{copa} aims to maintain a bounded number of packets in the bottleneck queue. Copa induces a periodic pattern of sending rate to obtain an accurate estimate of the minimum RTT and the queuing delay. In addition, Copa uses this pattern to detect the presence of  non-Copa flows.
% short-term RTT variation is smaller than a threshold, 

%\looseness=-1
Unlike Copa, \name does not look for a pattern in the RTTs caused by its transmission pattern. Instead, it estimates the rate of the cross traffic and observes how the cross traffic reacts to the rate fluctuations it induces over a period of time. This enables \name to directly estimate the elasticity of cross traffic. 
Although elasticity detection takes a few seconds, our experiments show that is significantly more robust than Copa's method. 1) Copa switches mode frequently and loses throughput against elastic cross-traffic (\S\ref{s:big-experiment} and \S\ref{s:rw-wl}). Copa uses instantaneous measurements for mode-switching and is vulnerable to variation in the cross traffic. 2) Copa misclassifies cross traffic when the inelastic traffic rate is high, or when elastic flows have high RTTs ($\S$\ref{s:copa-compare}). 
Moreover, since \name's cross traffic estimation technique does not rely on properties of any specific rate control algorithm (e.g., emptying queues every 5 RTTs), it can be applied to any combination of TCP-competitive and delay-controlling schemes. 
%\looseness=-1

\smallskip
\noindent{\bf BBR.}
BBR~\cite{bbr} estimates the bottleneck bandwidth ($b$) and minimum RTT ($d$). 
It paces traffic at a rate $b$ while capping the number of in-flight packets to $2\times b\times d$.
To estimate the bottleneck, BBR periodically increases its rate over $b$ for about one RTT and then reduces it for the following RTT. 
BBR uses this sending-rate pattern to obtain estimates of $b$; specifically, it tests if the bottleneck rate exceeds the current estimate $b$ in the rate-increase phase. However, BBR doesn't use these pulses to infer the nature of cross traffic.

\smallskip
\noindent{\bf Other related schemes.}  
Vegas~\cite{vegas} and FAST~\cite{fasttcp} are delay-based algorithms that aim to maintain small queues at the bottleneck using different control rules. Other delay-based algorithms include TCP Nice~\cite{tcp-nice}, LEDBAT~\cite{rfc6817}, and Timely~\cite{timely} (which is designed for datacenters). These schemes generally perform poorly when competing with loss-based  algorithms.  PCC-Vivace~\cite{vivace} uses an online learning algorithm to adapt its sending rate to maximize a utility function that incorporates the achieved rate, delay, and loss rate. Our experiments ($\S$\ref{s:big-experiment}, $\S$\ref{s:rw-wl}) show that Vivace cannot achieve both low delay with inelastic cross traffic and compete fairly with elastic TCP flows.  Compound TCP~\cite{compound} maintains both a loss-based window and a delay-based window, and transmits data based on the sum of the two windows. Compound does not attempt to switch between two modes, and therefore it incurs high queuing delays due to its loss-based window.

\if 0
PCC~\cite{pcc} adapts the sending rate based on ``micro-experiments'' that evaluate how changing the sending rate (multiplicatively) impacts performance according to a specified utility function. PCC defines two utility functions: one targeting high throughput and low loss, and the other targeting low delay. PCC's behavior depends on the utility function; unlike \name, it does not achieve both low delay and compete with elastic loss-based TCPs. 
\fi

\if 0
Prior work on estimating cross-traffic rate~\cite{strauss2003measurement,jain2002pathload,hu2003evaluation} use probe packets, and are slow in estimating cross traffic. For example pathload~\cite{jain2002pathload} takes 10-30 s to generate a single cross traffic estimate. In contrast, our method is in-band and it relies on the property that the sender is backlogged.
\fi

\if 0
The multiple-\name scheme for coordinating pulsers bears resemblance to receiver-driven layered multicast (RLM) congestion control~\cite{rlm}. In RLM, a sender announces to the multicast group that it is conducting a probe experiment at a higher rate, so any losses incurred during the experiment should not be heeded by the other senders. By contrast, in \name, there is no explicit coordination channel, and the pulsers and watchers coordinate via their independent observations of cross traffic patterns.
\fi

==> simulation-confidence.tex <==
\section{Bundle FCT Simulator Correctness}
\label{app:simulator-correct}

\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{images/emp-sim-em-20-60-fgrnd.pdf}
    \caption{{\bf Validation of bundle FCT simulator---}FCT from simulation and emulation match for the FIFO scheduling discipline.}
    \label{fig:bundle:verify}
\end{figure}

We validate the fidelity of our simulator by comparing the FCT from the simulated FIFO \bundle to our emulation setup (which implements FIFO). 
%
\Fig{bundle:verify} compares the FCT of flows of varying size ranges, normalized by the median FCT obtained from emulation for each flow size.
%
The box shows 
the $25^{\text{th}}$, $50^{\text{th}}$, and $75^{\text{th}}$ percentiles, 
while the whiskers show the $10^{\text{th}}$ and $90^{\text{th}}$ percentiles.
%
There is a close match between the simulated and emulated results in all the flow size ranges, providing confidence in the results of our simulation.

==> title.tex <==


\begin{center}

\textbf{\LARGE Elasticity Detection: A Building Block for  Delay-Sensitive Congestion Control}

\vspace{5mm}

{\large by}

\vspace{5mm}

{\LARGE Prateesh Goyal}

\vspace{5mm}
{\large B.Tech. Computer Science, IIT Bombay (2016)}
\vspace{3mm}

{\large Submitted to the Department of Electrical }

\vspace{1mm}
{\large Engineering and Computer Science}

\vspace{1mm}
{\large in partial fulfillment of the requirements for the degree of}

\vspace{1mm}
{\large Master of Science in Computer Science and Engineering}

\vspace{4mm}
{\large at the}

\vspace{4mm}
{\large MASSACHUSETTS INSTITUTE OF TECHNOLOGY}

\vspace{1mm}
\large{May, 2018}

{\textcopyright 2018 Massachusetts Institute of Technology. All rights reserved.}

\end{center}
\vspace{2mm}
\begin{flushright}
Author $\rule{13.2cm}{0.15mm}$\\
Department of Electrical Engineering and Computer Science\\
\today
\end{flushright}
\begin{flushright}
Certified by $\rule{12.5cm}{0.15mm}$\\
Hari Balakrishnan, Fujitsu Chair Prof. of EECS\\
\end{flushright}
\begin{flushright}
Certified by $\rule{12.5cm}{0.15mm}$\\
Mohammad Alizadeh, Assistant Prof. of EECS 
\end{flushright}
\begin{flushright}
Accepted by $\rule{12.3cm}{0.15mm}$\\
Leslie A. Kolodziejski\\
Chair, Department Committee on Graduate Thesis
\end{flushright}
